Interpreting a concurrent $\lambda$-calculus in differential proof nets (extended version)

In this paper, we show how to interpret a language featuring concurrency, references and replication into proof nets, which correspond to a fragment of differential linear logic. We prove a simulation and adequacy theorem. A key element in our translation are routing areas, a family of nets used to implement communication primitives which we define and study in detail.

==> paper-csl-long arxiv/parts/conclusion.tex <==
\section{Conclusion}
\label{section:conclusion}

In this paper, we presented a translation of a $\lambda$-calculus with higher
order references and concurrency inside a fragment of differential proof nets.
While several translations of effectful languages have been proposed in the
literature, none supports this combination of features to our knowledge. We
introduced a generalization of communication areas, routing areas, which turned
out to be a useful device to encode references. More generally, we think that
routing areas can be used to express various kind of non-deterministic,
concurrent communications. 

%

Modeling concurrency comes at a price, as terms such as $(\lambda x.
\set{r}{x})\ \get{r} \parallel (\lambda x. \set{r}{x})\ \get{r})$ translates to
a net that do not respect the differential proofs nets correctness
criterion~\cite{ehrhard:hal-00150274}. Inside each thread, the $\set{r}{x}$
depends on the $\get{r}$ whose value will replace the $x$ variable. But of these
$\get{r}$ may also depend from the $\set{r}{x}$ of the other thread, creating a
seemingly circular dependence which breaks the acyclicity required for
correctness. This ambiguity is avoided at execution, as the first $\get{r}$ to
reduce will be forced to chose an available {\setw}: these set-get dependencies
are in fact mutually exclusive. But proof nets seems unable to express this
subtlety. Differential {\LL} seems to suffer from more fundamental limitations
as a model of concurrency as pointed out by Mazza~\cite{Mazza:TrueConcMSCS}. It is
yet to be clarified how these results apply to the fragment presented here.
While seriously limiting what can be modeled in proof nets, this might not be an
obstacle when aiming for practical parallel or distributed implementations.

%

The enrichment of the source language, such as switching to a more realistic
erase-on-write semantic for stores, or the addition of new effects and features
(synchronization operations, sum types, divergence either by fixpoint or
references, \emph{etc .}) is the main focus of future work.


==> paper-csl-long arxiv/parts/intro.tex <==
\section{Introduction}
\label{sec:intro}

\newcommand{\LL}{\textsf{LL}}
\newcommand{\torework}[1]{{\color{red}{#1}}}

% Plan :
% \begin{itemize}
%   \item Linear Logic : what ? (Logic of resource, decompose, fine grained)
%  \item Translations into Linear logic : generic information, interesting, semantics,
%  etc.
%  \item But also from a concrete perspective : parallelization, GoI, complexity,
%  compilation, linear types
%  \item We go a step further to encode concurrency and references into proof nets,
%  constructing on [erhardlaurent] and [tranquilli]. Amadio calculus (examples ?)
%  \item Doing so, we introduct a generalization of communication areas, routing areas
%  little blahblah and a language with references explicit substitutions, modeling
%  the message-passing dynamic of proof nets.
% \end{itemize}
The distinctive feature of Linear Logic~\cite{GIRARD19871} (\LL) is to be a
resource-aware logic, which explains its success as a tool to study
computational processes. The native language for {\LL} proofs - or rather,
\emph{programs} - are proof nets, a graph representation endowed with a local
and asynchronous cut-elimination procedure.  The fine-grained computations and
the explicit management of resources in {\LL} make it an expressive target to
translate various computational primitives. Girard provided two translations in
its original paper, later clarified as respectively a call-by-value and
call-by-name translation of the $\lambda$-calculus~\cite{MARAIST1995370}.
PCF~\cite{Mackie:1995:GIM:199448.199483} has also been considered. Other
works have tackled the intricate question of modeling side-effects. State has been considered in a $\lambda$-calculus with
references~\cite{tranquilli:hal-00465793}. Another direction which has been explored is
concurrency and non-determinism. The extension of {\LL} with dual structural
rules, Differential Linear Logic~\cite{ehrhard:hal-00150274}, happens to be
powerful enough to accommodate non-determinism as demonstrated by the encoding
of a $\pi$-calculus without replication~\cite{EHRHARD2010606}.

These translations allow to relate and compare different computational
frameworks.  They benefit from the consequent work on the semantic and the
dynamic of {\LL} which has been carried for thirty years.  They are also of
practical interest : the proof net representation naturally leads to parallel
implementations~\cite{mackie94,Pedicini:2007,Pinto:2001} and forms the basis for
concrete operational semantics in the form of token-based
automata~\cite{DANOS199640,Lago:2015:PSI:2876514.2876564}. In this regard, one
may consider {\LL} as a ``functional assembly language'' with a diverse collection of
semantics and abstract machines.

While $\lambda$-calculus is a fundamental tool in the study and design of
functional programming languages, mainstream programming languages are pervaded
with features that enable productive development such as support for parallelism
and concurrency, communication primitives, imperative references, \emph{etc }.
Most of them imply side-effects, which are challenging to model, to compose, and
to reason about. While some have been investigated individually through the lens
of {\LL}, our goal is to go one step further by modeling a language featuring at
the same time concurrency, references and replication. The constructs involved in the
translation are inspired by the approach in~\cite{EHRHARD2010606} for
concurrency and non-determinism coupled with a monadic translation~\cite{tranquilli:hal-00465793} for
references.  Our goal is to exploit the ability of proof nets to enable
independent computations to be done in parallel without breaking the original operational
semantic. The translation we propose can be seen as a compilation
from a {\em global shared memory} model to a {\em local message passing} one, in
line with proof nets philosophy.

\paragraph*{Routing areas}

In a concurrent imperative language, references are a means to exchange
information between threads. In order to implement communication primitives in
proof nets, we use and extend the concept of \emph{communication areas}
introduced in \cite{EHRHARD2010606}. A \emph{communication area} is a particular
proof net whose external interface, composed of wires, is split between an equal
number of inputs and outputs. Inputs and outputs are grouped by pairs
representing a plug on which other nets can be connected. They are simple yet
elegant devices, whose role is similar to the one of a network switch which
connects several agents.  Connecting two \emph{communication areas} yields a
\emph{communication area} again: this key feature enables their use as modular
blocks that can be combined into complex assemblies. In this paper, we introduce
\emph{routing areas}, which allows a finer control on the wiring diagram. They
are parametrized by a relation which specifies which inputs and outputs are
connected.  Extending our network analogy, \emph{communication areas} are rather
hubs: they simply broadcast every incoming message to any connected agent. On
the other hand, \emph{routing areas} are more like switches: they are able to
choose selectively the recipients of messages depending on their origin.
\emph{Routing areas} are subject to atomic operations that decompose the
operation of connecting \emph{communication areas}. These operations also
have counterparts on relations.

We show that \emph{routing areas} are sufficient to actually describe all the normal
forms of the fragment of proof nets composed solely of structural
rules.  The algebraic description of \emph{routing areas} then provides a
semantic for this fragment.

%%%%%%%%%%%%%%%%%%% EXPL SUBST FOR REFS - OLD - BEGIN %%%%%%%%%%%%%%%%%%%

% \paragraph*{Explicit substitutions.}
% The $\beta$-reduction of $\lambda$-calculus is a meta-rule where substitution is
% defined inductively and performed at once on the whole term. But its
% implementation is a whole different story : to avoid the size explosion in
% presence of duplication (as in $(\lambda x . x\ x\ x\ x)\ N$) of the naive
% implementation, mechanisms such as sharing must be deployed. Abstract machines
% implement various specific strategies that may either be representable in pure
% $\lambda$-calculus (call-by-value or call-by-name) or for which the
% syntax needs to be augmented
% with new objects (e.g. call-by-need or linear head reduction). The
% mismatch between $\beta$-reduction, that is rather a specification, and actual
% implementations can make the proof of correction for an evaluator or a compiler
% a highly nontrivial task. The heart of the theory of explicit substitutions,
% introduced in ~\cite{Abadi:1989:ES:96709.96712}, is to give substitutions a
% first class status as objects of the syntax to better understand the dynamic and
% implementation of $\beta$-reduction. The approach is similar to the proof-nets
% philosophy on the calculus side, decomposing the substitutions into explicit
% atomic steps. The main ingredient is to modify the $\beta$ rule so
% that $M\ N$ reduces to $M[N/x]$ and where $M[N/x]$ is now part of the
% syntax. Additional reduction
% rules are then provided to propagate the substitutions $[N/x]$ to atoms.
%
% Calculi with such a structure have been extensively studied
% in~\cite{Accattoli2010,DBLP:journals/corr/abs-0905-2539,Abadi:1989:ES:96709.96712}
% as well as their close relation to proof
% nets~\cite{Accattoli:2015:PNC:2852784.2853038,Accattoli:2014:NST:2535838.2535886}.
% They are sensitive to the definition of reduction rules, for if one is too
% liberal in how substitutions can be composed then a strongly normalizing
% $\lambda$-term may diverge in the calculus with explicit
% substitions~\cite{Mellies1995}. If one is too restrictive, confluence on
% metaterms is lost~\cite{Curien:1996:CPW:226643.226675}. The challenge is to
% carefully design the language to implement desirable features without losing
% fundamental properties. Many solutions have been proposed to fix these defects,
% such as~\cite{DBLP:journals/corr/abs-0905-2539,Accattoli2010}.
%
% \paragraph*{References and termination.}
% While a simple type system for usual $\lambda$-calculus ensures
% termination, the situation is quite different in a language with
% higher-order references. The so called Landin's trick allows to encode
% a fixpoint in the simply typed version of a calculus with references
% as follows.
% \begin{tabred}
%   \get{r}\ \ast \parallel \store{r}{(\lambda x . \get{r}\ \ast)}
%   & \to & (\lambda x . \get{r}\ \ast)\ \ast \parallel \store{r}{(\lambda x .
%     \get{r}\ \ast)} \\
%     & \to & \get{r}\ \ast \parallel \store{r}{(\lambda x . \get{r}\ \ast)} \\
%   & \to & \ldots
% \end{tabred}
%
% The problem lies in the fact that one can store in a reference $r$ values that
% can themselve read from the very same reference, leading to a circularity.
% Here, $\vdash \lambda x . \get{r}\ \ast : \text{Unit} \to \text{Unit}$ and $r$
% is a reference that stores $\text{Unit} \to \text{Unit}$ values.
% More generally, we can define a fixpoint combinator
% $$\mu_r f. \lambda x. M = \set{r}{\lambda x . M \{ \lambda y . \get{r}\ y / f \} };
% \get{r}\ \ast.$$
%
% In order to address this issue, type and effects systems have been
% introduced to track the potential effects produced by a term during
% its evaluation.  Together with stratification, a discipline on
% references proposed by Boudol~\cite{BOUDOL2010716}, one can recast termination
% in such an imperative context.  Intuitively, stratification imposes an
% order between references such that a reference can only store terms
% that access smaller ones and our previous fixpoint becomes
% ill-typed. Formally, this allows to apply the usual reducibility
% argument to a calculus with references : stratification ensures that
% the inductive definition of reducibility sets on types with effects is
% well-founded.
%

%%%%%%%%%%%%%%%%%%% EXPL SUBST FOR REFS - OLD - END %%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%% EXPL SUBST FOR REFS - BEGIN %%%%%%%%%%%%%%%%%%%

% We introduce a language with explicit substitutions as intermediate
% representation between \lamadio and proof nets, \lthis, which has a term syntax
% like the source language but a dynamic close to the proof nets one. 
% $\lambda$-calculi with explicit substiutions are known to have a
% % Calculi with such a structure have been extensively studied
% % in~\cite{Accattoli2010,DBLP:journals/corr/abs-0905-2539,Abadi:1989:ES:96709.96712}
% close relation to proof
% nets~\cite{Accattoli:2015:PNC:2852784.2853038,Accattoli:2014:NST:2535838.2535886}.
% Looking at terms as trees, we can see the usual variable substitutions
% emitted by a $\beta$-reduction as a message dispatched from an
% application node downward through the term until it reaches the leafs.  Consider for example the reduction
% of the term $(\lambda x . x\ y\ z)\ (\lambda x . x)$:
%
% \begin{center}
% \scalebox{.8}{%
% \begin{tabular}{ccccc}
%   \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$(\lambda x . x\ y\ z)\ (\lambda x.x)$};
%     \node[draw=none] (M) at (-1,-1)
%       {$\lambda x. x\ y\ z$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (X) at (-1,-3)
%       {$x$};
%     \node[draw=none] (N) at (1,-1)
%       {$(\lambda x. x)$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (M) at (0,0)
%     {$\vars{x}{(\lambda x. x)}{x\ y\ z}$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$x$};
%
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (M) at (0,0)
%       {$x\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\vars{x}{(\lambda x. x)}{\ldots}$};
%     \node[draw=none] (X) at (0,-2)
%       {$x$};
%
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (M) at (0,0)
%       {$x\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$\vars{x}{(\lambda x. x)}{x}$};
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (M) at (0,0)
%       {$(\lambda x. x)\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$\lambda x. x$};
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (X);
%   \end{tikzpicture}
% \end{tabular}%
% } % END SCALEBOX
% \end{center}
%
% A reference assignation is more involved. Indeed, an {\setw} occurs at
% a leaf and must be able to reach a {\getw} located in a different part
% of the tree. To do so, we introduce two types of reference 
% substitutions : one that goes upward (indicated by $\uparrow$) from a
% $\set{r}{V}$, climbing up the whole tree to the root, and one that
% goes downward (indicated by $\downarrow$), similar to variable
% substitutions. Each time an upward substitution go through a multi-ary
% constructor -- as an application or a $\parallel$ -- it propagates
% downard substitutions in all the children of this constructor, except
% the one it comes from, and continues its ascension. Eventually, all
% the leafs will be reached by a corresponding downward
% substitution. Consider a term $M\ N$ where $M$ contains a $\get{r}$
% somewhere and $N$ a $\set{r}{V}$, the explicit substitution reduction
% now goes as
%
%
% \begin{center}
% \scalebox{.8}{%
% \begin{tabular}{cccc}
%   \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$M$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\set{r}{V}$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (G);
%     \draw[->,>=latex] (N) -- (N2);
%     \draw[->,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$M$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast [r \Leftarrow V]\uparrow$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (G);
%     \draw[->,>=latex] (N) -- (N2);
%     \draw[->,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots [r \Leftarrow V]\uparrow $};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (G);
%     \draw[->,>=latex] (N) -- (N2);
%     \draw[->,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N [r \Leftarrow V]\uparrow$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (G);
%     \draw[->,>=latex] (N) -- (N2);
%     \draw[->,>=latex] (N2) -- (S);
%   \end{tikzpicture} \\
%
%   \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$(M\ N)[r \Leftarrow V]\uparrow$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M [r \Leftarrow V]\downarrow$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (G);
%     \draw[->,>=latex] (N) -- (N2);
%     \draw[->,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$(M\ N)[r \Leftarrow V]\uparrow$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots [r \Leftarrow V]\downarrow$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (G);
%     \draw[->,>=latex] (N) -- (N2);
%     \draw[->,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$(M\ N)[r \Leftarrow 1]\uparrow$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r) [r \Leftarrow V]\downarrow$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (G);
%     \draw[->,>=latex] (N) -- (N2);
%     \draw[->,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}
%     \node[draw=none] (MN) at (0,0)
%       {$(M\ N)[r \Leftarrow V]\uparrow$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$V$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[->,>=latex] (MN) -- (M);
%     \draw[->,>=latex] (MN) -- (N);
%     \draw[->,>=latex] (M) -- (M2);
%     \draw[->,>=latex] (M2) -- (G);
%     \draw[->,>=latex] (N) -- (N2);
%     \draw[->,>=latex] (N2) -- (S);
%   \end{tikzpicture}
% \end{tabular}%
% } % END SCALEBOX
% \end{center}
%
% Hence communication through references is represented by bidirectionnal
% substitutions. Introduced for the sake of the translation, our language with
% explicit substitution makes the execution model of the proof net side clearer:
% This is a shift from a global shared memory model to a message passing one.
%

%%%%%%%%%%%%%%%%%%% EXPL SUBST FOR REFS - END %%%%%%%%%%%%%%%%%%%

\paragraph*{A Concurrent $\lambda$-calculus}
We consider a paradigmatic concurrent lambda-calculus with higher-order
references -- {\lamadio} below -- which has been introduced by Amadio
in~\cite{Amadio2009}. It is a call-by-value $\lambda$-calculus extended with:
%
\begin{itemize}
\item a notion of threads and an operator $\parallel$ for parallel
  composition of threads,
\item two terms $\set{r}{V}$ and $\get{r}$, to respectively
  assign a value to and read from a reference,
\item special threads $\store{r}{V}$, called stores, accounting for
  assignments.
\end{itemize}
%
% When $\set{r}{V}$ is reduced, it turns to the unit value $\ast$ and produces a
% store $\store{r}{V}$ making the value available to all the other threads. A
% corresponding construct $\get{r}$ is reduced by choosing non deterministically a
% value among all the available stores. For example, assuming some support for
% basic arithmetics consider the program
% $
% (\lambda x. x + 1)\ \get{r} \parallel
%   \set{r}{0} \parallel \set{r}{1}.
% $
% It consists of 3 threads: two concurrent assignments $\set{r}{0}$
% and $\set{r}{1}$, and an application $(\lambda x. x + 1)\,\get{r}$.
% This programs admits two normal forms depending on which
% assignment ``wins'':  the term $1 \parallel
% \ast \parallel \ast \parallel r \Leftarrow 0 \parallel
% \store{r}{1}$ and the term $2 \parallel
% \ast \parallel \ast \parallel r \Leftarrow 0 \parallel
% \store{r}{1}$.
%
In this language, the stores are global and cumulative: their scope is the whole
program, and each {\setw} adds a new binding that does not erase the previous
ones. Reading from a store is a non deterministic process that chooses a value
among the available ones. References are able to handle an unlimited number of
values and are understood as a typed abstraction of possibly several concrete
memory cells. This feature allows {\lamadio} to simulate various other calculi
with references such as variants with dynamic references or
communication~\cite{madet:tel-00794977}.  The language is endowed with an
appropriate type and effects system ensuring termination. The translation is
presented on an explicit substitutions version of {\lamadio}, introduced to
serve as an intermediate representation. This intermediate language is presented
and studied in details in \cite{HamdaouiValiron2018}.

% While a simple type system for usual $\lambda$-calculus ensures
% termination, the situation is quite different in a language with
% higher-order references. The so called Landin's trick allows to encode
% a fixpoint in the simply typed version of a calculus with references.
% The problem lies in the fact that one can store in a reference $r$
% values that can themselves read from the reference~$r$, leading
% to a circularity. For example, the term $\get{r}\ \ast \parallel r
% \Leftarrow (\lambda x. \get{r}\ \ast)$ loops while involving only simple types
% $\mbox{Unit}$ and $\mbox{Unit} \to \mbox{Unit}$.
%
% In order to address this issue, type and effects systems have been
% introduced to track the potential effects produced by a term during
% its evaluation. Together with stratification on
% references~\cite{BOUDOL2010716}, one can recast termination in such an
% imperative context. Intuitively, stratification imposes an order
% between references: a reference can only store terms that
% access smaller ones, ruling out Landin's fixpoint. Formally, this
% allows to apply the usual reducibility argument to a calculus with
% references: stratification ensures that the inductive definition of
% reducibility sets on types with effects is well-founded.
%
% However, an unconstrained scheduling such as the one
% in~\cite{Amadio2009} can cause additional difficulties. There, the proof of
% termination resorts to what amounts to infinite
% terms with the notion of saturated stores.
%
% $\lambda$-calculus is a fundamental tool in the study and design of functionnal
% programming languages. however nobody would consider it for a day-to-day
% programming task, as it lacks a whole set of modern features that enable
% productive development such as parallelism and concurrency, communication
% primitives, imperative references, \emph{etc }. One such effectful language -- referred as
% \lamadio below -- considers concurrency and references. It was introduced by
% Amadio in~\cite{Amadio2009} as an extension of the call-by-value
% $\lambda$-calculus with: \begin{itemize} \item an operator $\parallel$ for
%     parallel composition of threads, \item two constructors $\set{r}{V}$ and
%     $\get{r}$, to respectively assign a value to and read from a reference, \item
%       special threads $\store{r}{V}$, called stores accounting for assignations.
%   \end{itemize} When a $\set{r}{V}$ is reduced, it turns to the unit value
%   $\ast$ and produces a store $\store{r}{V}$ making the value available to all
%   the other threads. A corresponding construct $\get{r}$ is reduced by choosing
%   non deterministically a value among all the available stores. Here is a simple
%   example of reduction where we assume some support for basic arithmetic to make
%   it more readable: 
% %
% \[
% \begin{array}{l}
% (\lambda x. x + 1)\ \get{r} \parallel
%   \set{r}{0} \parallel \set{r}{1} \\
% \qquad\qquad\begin{array}{lll}
%   & \to^\ast & (\lambda x. x + 1)\ \get{r}
%                \parallel \ast \parallel \ast \parallel r \Leftarrow 0 \parallel
%                \store{r}{1} \\ 
%   & \to & (\lambda x. x + 1)\ 0 \parallel \ast \parallel \ast
%           \parallel r \Leftarrow 0 \parallel \store{r}{1} \\ 
%   & \to^\ast & 1 \parallel
%     \ast \parallel \ast \parallel r \Leftarrow 0 \parallel
%                \store{r}{1}
% \end{array}
% \end{array}
% \]
% % 
% There is another possible normal form, which is $2 \parallel \ast
%   \parallel \ast \parallel \store{r}{0} \parallel \store{r}{1}$.  We notice that
%   the stores are global and cumulative : their scope is the whole program, and
%   each {\setw} adds a new binding that does not erase the previous one. This is
%   the cause of the non deterministic reduction. References are able to handle an
%   unlimited number of values and must be understood as a typed abstraction of
%   possibly several actual memory cells. This feature allows \lamadio to simulate
%   various other references calculi, such as variants with dynamic references or
%   communication channel as discussed in the introduction of Madet's Ph.D.
%   thesis~\cite{madet:tel-00794977}. The termination of \lamadio
%   implies the termination of the others.
%

% While a simple type system for usual $\lambda$-calculus ensures
% termination, the situation is quite different in a language with
% higher-order references. The so called Landin's trick allows to encode
% a fixpoint in the simply typed version of a calculus with references.
% The problem lies in the fact that one can store in a reference $r$
% values that can themselves read from the reference~$r$, leading
% to a circularity. For example, the term $\get{r}\ \ast \parallel r
% \Leftarrow (\lambda x. \get{r}\ \ast)$ loops while involving only simple types
% $\mbox{Unit}$ and $\mbox{Unit} \to \mbox{Unit}$.
%
% In order to address this issue, type and effects systems have been
% introduced to track the potential effects produced by a term during
% its evaluation. Together with stratification on
% references~\cite{BOUDOL2010716}, one can recast termination in such an
% imperative context. Intuitively, stratification imposes an order
% between references: a reference can only store terms that
% access smaller ones, ruling out Landin's fixpoint. Formally, this
% allows to apply the usual reducibility argument to a calculus with
% references: stratification ensures that the inductive definition of
% reducibility sets on types with effects is well-founded.

% \paragraph*{Difficulties}
% Modeling concurrency comes at a price: as discussed further in
% \ref{section:cycles}, the translation of terminating terms may generate objects
% that are not the representation of any proof, as they contain causal cycles
% that seems hard to eliminate statically. For proof nets, this means that neither
% termination nor confluence may be taken for granted: one has to tune reduction
% rules to get a well-behaved system. However, we think that cyclic
% structures make sense as computational entities. 
%
\paragraph*{Contributions.}
The contributions of this paper are:
\begin{itemize}
  \item We introduce and study \emph{routing areas} which are flexible devices
    for implementing communication in proof nets. From routing areas we derive a
    semantic for a fragment of proof nets.
  \item We illustrate the use of routing areas by translating a concurrent
    $\lambda$-calculus to proof nets. Routing areas are the building block of
    this translation.
  \item We prove a \emph{simulation} and \emph{adequacy} theorem for this
    translation.
\end{itemize}

\paragraph*{Plan of the paper.}
\begin{itemize}
  \item In Section~\ref{section:nets}, we detail our proof nets setting and state its 
    properties
  \item We go on to define routing areas and study them more in detail
    in Section~\ref{section:areas}.
  \item In Section~\ref{section:lamadio}, we introduce the source language of our
    translation, the concurrent $\lambda$-calculus \lamadio.
  \item Section~\ref{section:translation} is devoted to the translation. We explain its underlying
    principles and give some representative cases.
  \item Section~\ref{section:properties} gives the simulation, termination and
    adequacy theorems together with their proof.
\end{itemize}


==> paper-csl-long arxiv/parts/language-amadio.tex <==
\section{The Concurrent $\lambda$-calculus \lamadio}
\label{section:lamadio}

We present the 
{\lamadio}~\cite{Amadio2009} calculus, 
following the presentation in Madet's Ph.D
thesis~\cite{madet:tel-00794977}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The \lamadio\ calculus is a call-by-value $\lambda$-calculus, equipped with {\em
references} that abstract the notion of global memory cells. The calculus is
enriched with a parallel composition operator $\parallel$ for modeling
concurrency.

\subsection{Syntax}
Variables are
denoted with $x,y,\ldots$ while references are
denoted with $r,s,\ldots$. The language consists of {\em values}, {\em
  terms}, {\em stores} and {\em programs}. A {\em store} is a
top-value set of associations between references and values, while a
program is a store together with a set of terms. The terms in a
program can be regarded as threads running in parallel, while the
stores represent the state of the global memory. Programs are the
objects of interest in \lamadio.
%
\begin{center}
\begin{tabular}{llll}
  -values & $V$ & $::=$ & $x \mid \ast \mid \lambda x.M $ \\
  -terms & $M$ & $::=$ & $V \mid M\ M \mid \get{r} \mid
  \set{r}{V} \mid M \parallel M$ \\
  -stores & $S$ & $::=$ & $r \Leftarrow V \mid (S \parallel S)$ \\
  -programs & $P$ & $::=$ & $M \mid S \mid (P \parallel P)$ \\
\end{tabular}
\end{center}
%
The constant value $\ast$ stands for the return value of a reference
assignation: it carries no particular information.
%
The primitives $\set{r}{V}$ and $\get{r}$ respectively
writes a value $V$ to and reads from a given reference $r$.
%
While {\setw}s can be only performed on values, a more general
$\set{r}{M}$ can be encoded as $(\lambda x . \set{r}{x})\,M$ for an
arbitrary term $M$. 
%
Once reduced, a $\set{r}{V}$ produces the special kind of thread
$r \Leftarrow V$ at top level in a store, adding $V$ as the
possible values available for the reference $r$.
%
Parallelism is accounted for using the operator~$\parallel$. Terms,
programs and stores can be placed in parallel. For stores, this simply
means that all the corresponding associations reference/value are
available for substitution of reference in the threads.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Reduction}

The calculus is endowed with the usual structural rules for the
parallel operator, namely associativity and commutativity
(Table~\ref{fig:lam-struct-rules}). 
%
The rewrite rules for the language are found in
Table~\ref{fig:lam-red-rules}. Together with the $\beta_v$ rule are
two new reductions, one that turns an assignment to a store and one
that turns a get to a value. 
%
The rules use the evaluation contexts defined in
Table~\ref{fig:lam-eval-context} to handle congruence. The context $E$ denotes a
weak call-by-value weak reduction which is neither right-to-left or
left-to-right. The context $C$ allows reduction to occurs in any thread of a
program.

The substitution of a reference is a non-deterministic
operation. Reference must be seen as an abstraction for a set of typed memory
cells that can hold many values. Let $\mbox{proj}_1 = \lambda x y . x$ and
$\mbox{proj}_2 = \lambda x y . y$ be the Church projections, and consider the
term $$P = (\lambda x . x\ V_1\ V_2)\ \get{r} \parallel (\lambda y .\set{r}{y})\
\get{s} \parallel \set{s}{\mbox{proj}_1} \parallel \set{s}{\mbox{proj}_2}$$ 
The two \setw\ can be reduced to stores :
$$P \to^\ast (\lambda x . x\ V_1\ V_2)\ \get{r} \parallel (\lambda y . \set{r}{y})\
\get{s} \parallel \ast \parallel \ast \parallel \store{s}{\mbox{proj}_1}
\parallel \store{s}{\mbox{proj}_2}$$ for some distinct values $V_1$ and $V_2$.
Here, $\get{s}$ have essentially two incompatible ways to reduce : either it
is replaced by $\mbox{proj}_1$ or by $\mbox{proj}_2$. In the first case,
\begin{tabred}
  P & \to^\ast & (\lambda x. x\ V_1\ V_2)\ \get{r} \parallel \set{r}{\mbox{proj}_1}
  \parallel P' \\
  & \to^\ast & (\lambda x . x\ V_1\ V_2)\ \get{r} \parallel \ast \parallel
  \store{r}{\mbox{proj}_1} \parallel P' \\
  & \to^\ast & (\lambda x . x\ V_1\ V_2)\ \mbox{proj}_1 \parallel \ast \parallel
  \store{r}{\mbox{proj}_1} \parallel P' \\
  & \to^\ast & V_1 \parallel \ast \parallel
  \store{r}{\mbox{proj}_1} \parallel P' \\
\end{tabred}
  where $P' = \ast \parallel \ast \parallel \store{s}{\mbox{proj}_1} \parallel
  \store{s}{\mbox{proj}_2}$. However if $\get{s}$ is replaced by
  $\mbox{proj}_2$, we get that $P \to^\ast V_2 \parallel \ast \parallel
  \store{r}{\mbox{proj}_2} \parallel P'$ : $P$ has two distinct normal forms.

%

Despite the $\parallel$ operator being a static constructor, it can be embedded
in abstractions and thus dynamically liberated or duplicated. For example, the
term $(\lambda f. f\ \ast \parallel f\ \ast)$ act like a \emph{fork} operation:
if applied to $M$, it generates two copy of its argument in two parallel threads
$M\ \ast \parallel M\ \ast$.
The next section is devoted to detailing how terms of {\lamadio} are translated
to proof nets described in \ref{section:nets}, thanks to the areas introduced in
\ref{section:areas}.
%%% ---------------------------------------------------------------------
\begin{table}[t]
\centering
\begin{minipage}{.4\linewidth}
\centering
\begin{tabular}{rcl}
$P \parallel P'$ & = & $P \parallel P'$ \\
$(P \parallel P') \parallel P''$ & = & $P \parallel (P' \parallel
P'')$\mynl
\end{tabular}
\caption{Structural Rules}\label{fig:lam-struct-rules}
\end{minipage}
\begin{minipage}{.4\linewidth}
\centering
\begin{tabular}{lcl}
$E$ & $::=$ & $[.] \mid E\ M \mid M\ E$ \\
$C$ & $::=$ & $[.] \mid (C \parallel P) \mid (P \parallel C)$\mynl
\end{tabular}
\caption{Evaluation Contexts}\label{fig:lam-eval-context}
\end{minipage}
\mynl
\begin{tabular}{lrcl}
$(\beta_v)$ & $C[E[(\lambda{x}.M)\ V]$ &
  $\rightarrow$ & $ C[E[M[V/x]]]$ \\
$(\texttt{\text{get}})$ & $C[E[\get{r}]] \parallel r \Leftarrow V$ &
  $\rightarrow$ & $ C[E[V]] \parallel r \Leftarrow V$ \\
$(\texttt{\text{set}})$ & $C[E[\set{r}{V}]]$ &
  $\rightarrow$ & $ C[E[\ast]] \parallel r \Leftarrow V $\mynl
\end{tabular}
\caption{Reduction Rules}\label{fig:lam-red-rules}
\end{table}
%%%-------------------------------------------------------------------

%
% \subsection{Terms}
%
% \begin{tabular}{llll}
%   -variables & \multicolumn{3}{l}{$x,y,\ldots$} \\
%   -regions & \multicolumn{3}{l}{$r,s,\ldots$} \\
%   -values & $V$ & $::=$ & $x \mid \ast \mid \lambda x.M $ \\
%   -terms & $M$ & $::=$ & $V \mid M\ M \mid \get{r} \mid
%   \text{set}(r,V) \mid M \parallel M$ \\
%   -stores & $S$ & $::=$ & $r \Leftarrow V \mid (S \parallel S)$ \\
%   -programs & $P$ & $::=$ & $M \mid S \mid (P \parallel P)$ \\
% \end{tabular}
%
% \subsection{Reduction}
%
% \begin{center}
% \begin{tabular}{rcl}
% \hline
% \multicolumn{3}{|c|}{Structural rules} \\
% \hline
% $P \parallel P'$ & = & $P \parallel P'$ \\
% $(P \parallel P') \parallel P''$ & = & $P \parallel (P' \parallel P'')$ \\
% \end{tabular}
% \end{center}
%
% \paragraph{}
% \begin{center}
% \begin{tabular}{lcl}
% \hline
% \multicolumn{3}{|c|}{Evaluation contexts} \\
% \hline
% $E$ & $::=$ & $[.] \mid E\ M \mid V\ E$ \\
% $C$ & $::=$ & $[.] \mid (C \parallel P) \mid (P \parallel C)$ \\
% \end{tabular}
% \end{center}
%
% \paragraph{}
% \begin{center}
% \begin{tabular}{lrcl}
% \hline
% \multicolumn{4}{|c|}{Reduction rules} \\
% \hline
% $(\beta_v)$ & $C[E[(\lambda{x}.M)\ V]$ &
%   $\rightarrow$ & $ C[E[M[V/x]]]$ \\
% $(\texttt{\text{get}})$ & $C[E[\get{r}]] \parallel r \Leftarrow V$ &
%   $\rightarrow$ & $ C[E[V]] \parallel r \Leftarrow V$ \\
% $(\texttt{\text{set}})$ & $C[E[\text{set}(r,V)]]$ &
%   $\rightarrow$ & $ C[E[\ast]] \parallel r \Leftarrow V $ \\
%
% \end{tabular}
% \end{center}


==> paper-csl-long arxiv/parts/language-ces.tex <==
\subsection{A language with explicit substitutions: \lthis}

\lthis\ is a $\lambda$-calculus with explicit substitutions for both variables
and references, non deterministic sum and parallel composition. It serves as an
intermediate language between \lamadio\ and nets, easing the proofs of simulation
and termination.

%

The language {\lthis} has two kinds of variables: term variables (simply named
{\em variables}) represented with $x,y,\ldots$, and {\em references},
represented with $r,r',\ldots$.  Substitutions are represented by partial
functions with finite support. Variable substitutions, denoted with Greek
letters $\sigma,\tau,\ldots$, map variables to values. Reference substitutions,
denoted with calligraphic uppercase letters $\multv{V},\multv{U},\ldots$,
map references to {\em finite multisets} of values. Multisets reflect the
non-determinism, as multiple writes may have been performed on the same
reference. They are represented with the symbol $\mathcal{E}$.
%
The language consists
of values, terms and sums of terms, representing non-determinism.
\begin{center}
\begin{tabular}{llll}
  -values & $V$ & $::=$ & $x \mid \ast \mid \lambda x.M$ \\
  -terms & $M$ & $::=$ & $V \mid \varss{\sigma}{M} \mid
                         \refssl{r}{V}{(M\,M)} \mid \get{r}
\mid \refssd{r}{V}{M} \mid \refssu{r}{V}{M} \mid M \parallel M$ \\
  -sums & $\mathbf{M}$ & $::=$ & $\mathbf{0} \mid M \mid \mathbf{M} +
  \mathbf{M}$ \\
\end{tabular}
\end{center}
The construct $\varss{\sigma}{M}$ stands for the explicit substitutions
of variables in $M$ under the substitution $\sigma$. There are three
constructs for explicit substitutions for references:
$\refssd{r}{V}{M}$ and $\refssu{r}{V}{M}$ are respectively the
downward and upward references substitutions, while
$\refssl{r}{V}{(M\,M)}$ is the $\lambda$-substitution. The reason for
which the language needs three distinct notations is explained in the
next section while presenting the reduction rules.

Terms are considered modulo the same kind of equivalence relation as \lamadio.
The sum is idempotent, associative and commutative, while the parallel
composition is associative and commutative.


\begin{remark}
  The three constructs $\refssd{r}{V}{}$, $\refssu{r}{V}{}$ and
  $\refssl{r}{V}{}$ encapsulate the assignments in terms and in stores
  presented in Section~\ref{sec:intro}: there is no need anymore for
  ${\rm set}(r,V)$ and $r\Leftarrow V$. See
  Section~\ref{sec:discussion} for a discussion of this aspect.
\end{remark}

\begin{notation}
  Reference substitutions will be sometimes written
  with the notation $[\store r V]$ to mean $[\multv{V}]$ with $\multv{V} : r
  \mapsto [V]$.
\end{notation}

We will not describe \lthis\ more in detail. A complete formulation of the
reduction together with a type system and a proof of termination may be found in
\cite{paper-esop}. The reduction and typing rules are included in
Appendix~\ref{appendix:lces}.

%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Reduction of \lthis}
%
% We adopt a weak call-by-value reduction where the reduction order of
% an application is not specified. It is weak in the sense that no
% reduction occurs under abstractions.
%
% Although in a general setting non-determinism and call-by-value taken together
% may break confluence even when collecting all possible
% outcomes~\cite{deLiguoroP95},
% this phenomenon doesn't happen here. Indeed, we can't reduce under
% abstractions, and the only non-deterministic construct $\get{r}$ must be reduced
% before being duplicated, avoiding problematic interactions between
% $\beta$-reduction and non-deterministic choice.
%
% The language {{\lthis}} is equipped with the reduction defined
% in Table~\ref{fig:lth-red-rules}. The rules make use of several notations
% that we lay out below.
% Rules devoted to dispatching substitutions are referred as
% \emph{structural rules}. The \emph{variable} (resp. \emph{downward},
% \emph{upward}) \emph{structural rules} consist in \rrulet{subst}{}
% (resp.  \rrulet{subst-r}{}, \rrulet{subst-r'}{}) rules excluding
% \rrulet{subst}{var} (resp.  \rrulet{subst-r}{get},
% \rrule{subst-r}{\top}). An in-depth discussion about these rules follows.
%
%
%
% %%% -------------------------------------------------------------------
% \begin{table}[tb]
% \centering
% \begin{minipage}{.49\linewidth}
% \centering
% \begin{tabular}{rcl}
% $M \parallel M'$ & = & $M' \parallel M$ \\
% $(M \parallel M') \parallel M''$ & = & $M \parallel (M' \parallel M'')$ \\
% $\mathbf{M} + \mathbf{M}'$ & = & $\mathbf{M}' + \mathbf{M}$ \\
% $(\mathbf{M} + \mathbf{M}') + \mathbf{M}''$ & = & $\mathbf{M} + (\mathbf{M}' +
% \mathbf{M}'')$ \\
% $\mathbf{M} + \mathbf{M}$ = $\mathbf{M} + \mathbf{0}$ & = & $\mathbf{M}$
% \mynl
% \end{tabular}
% \caption{Structural Rules}\label{fig:lth-struct-rules}
% \end{minipage}
% \begin{minipage}{.49\linewidth}
% \centering
% \begin{tabular}{lcl}
% ~\\
% $E$ & $::=$ & $[.] \mid \refssl{r}{V}{E\ M} \mid
%   \refssl{r}{V}{M\ E}\mid{} $ \\
% & & $\refssd{r}{V}{E}
%   \mid \refssu{r}{V}{E}$ \\
% $C$ & $::=$ & $[.] \mid (C \parallel M) \mid (M \parallel C)$ \\
% $\mathbf{S}$ & $::=$ & $[.] \mid \mathbf{S} + \mathbf{M} \mid \mathbf{M} +
% \mathbf{S}$ \mynl
% \end{tabular}
% \caption{Evaluation Contexts}\label{fig:lth-eval-context}
% \end{minipage}
% \end{table}
% %%%-------------------------------------------------------------------
%
%
%
% %%%-------------------------------------------------------------------
% \begin{table}[!p]
% \begin{center}
% \begin{tabular}{lrcl}
% \hline
% \multicolumn{4}{|c|}{{\bf (a)}~$\beta$-reduction} \\
% \hline
% $(\beta_v)$ & $\refssl{r}{U}{((\lambda x.M)\,V)}$ & $\rightarrow$ &
% $\refssd{r}{U}{(\varss{\sigma}{M})}$ \\
% \\
% \multicolumn{4}{l}{If $M \rightarrow M'$ with rule $(\beta_v)$, then
%   $\mathbf{S}[C[E[M]]] \rightarrow \mathbf{S}[C[E[M']]]$}\\
% \\
% \hline
% \multicolumn{4}{|c|}{{\bf (b)}~Variable Substitutions} \\
% \hline
% \rrulet{subst}{var} & $\varss{\sigma}{x}$
% & $\to$ & $\sigma(x)$ if defined, or $x$ otherwise\\
% \rrulet{subst}{unit} & $\varss{\sigma}{\ast}$
% & $\to$ & $\ast$ \\
% \rrulet{subst}{app} & $\varss{\sigma}{\refssl{}{V}{(M\,N)}}$ & $\to$
% & $\refrawsl{}{\varss{\sigma}{\multv{V}}}{((\varss{\sigma}{M})\,(\varss{\sigma}{N}))}$ \\
% \rrule{subst}{\lambda} & $\varss{\sigma}{(\lambda y.M)}$ & $\to$
%   & $\lambda y.(\varss{\sigma}{M})$ \\
% \rrulet{subst}{get} & $\varss{\sigma}{\get{r}}$ & $\to$
%  & $\get{r}$ \\
% \rrule{subst}{\parallel} & $\varss{\sigma}{(M \parallel M')}$ & $\to$
% & $(\varss{\sigma}{M}) \parallel (\varss{\sigma}{M'})$ \\
% \rrulet{subst}{subst-r} &
% $\varss{\sigma}{( \refssd{r}{V}{M} )}$ & $\to$
% & $\refsrawsd{}{\metas{\sigma}{\multv{V}}}{\varss{\sigma}{M}}$ \\
% \rrulet{subst}{subst-r'} &
% $\varss{\sigma}{( \refssu{r}{V}{M} )}$ & $\to$
% & $\refsrawsu{}{\metas{\sigma}{\multv{V}}}{\varss{\sigma}{M}}$ \\
% \rrulet{subst}{merge} & $\varss{\tau}{\varss{\sigma}{M}}$ & $\to$ &
% $\varss{\sigma,\tau}{M}$
% % & & & \\[-2ex]
% %  & \multicolumn{3}{c}{
% %   where $W_i =
% %   \begin{cases*}
% %     V_i & \text{if $i \in \mathcal{I}$} \\
% %     \varmetas{(x_k)_{k \in \mathcal{I}}}{(V_k)_{k \in \mathcal{I}}}{U_i} & \text{if $i \in \mathcal{J}$} \\
% %   \end{cases*}$} \\
% \mynl
% \multicolumn{4}{l}{Congruence case: }\\
% \multicolumn{4}{l}{If $M \rightarrow M'$ by any of the previous rules, then
%   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% \\
% \hline
%   \multicolumn{4}{|c|}{{\bf (c)}~Downward Reference Substitutions} \\
% \hline
% \rrulet{subst-r}{val} & $\refssd{}{V}{V}$
% & $\to$ & $V$ \\
% \rrule{subst-r}{\parallel} & $\refssd{}{V}{(M
% \parallel M')}$ & $\to$
% & $(\refssd{}{V}{M}) \parallel (\refssd{}{V}{M'})$ \\
% \rrulet{subst-r}{subst-r'} &
% $\refssd{r}{V}{\refssu{s}{U}{M}}$ & $\to$
% & $\refssu{s}{U}{\refssd{r}{V}{M}}$ \\
%  & & & \\
% \rrulet{subst-r}{merge} &
% $\refssd{}{V}{\refssd{}{U}{M}}$ & $\to$
% & $\refsrawsd{}{\multv{U},\multv{V}}{M}$ \\
% \rrulet{subst-r}{app} &
% $\refssd{}{V}{\refssl{}{U}{(M\,N)}}$ & $\to$
% & $\refsrawsl{}{\multv{U},\multv{V}}{(\refssd{}{V}{M})\ (\refssd{}{V}{N})}$ \mynl
% \multicolumn{4}{l}{Congruence cases:}\\
% \multicolumn{4}{l}{If $M \rightarrow M'$ by any of the previous rules, then
%   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \mynl
% \multicolumn{4}{l}{Finally:}\\
% \rrulet{subst-r}{get} &
% $\mathbf{S}[C[E[\refssd{}{V}{\get{r}}]]]$ & $\to$
% & $\mathbf{S}[C[E[\get{r}]]] + \sum_{V \in \multv{V}(r)}
% C[E[V]]$ \\
% \\
% \hline
% \multicolumn{4}{|c|}{{\bf (d)}~Upward Reference Substitutions} \\
% \hline
% \rrule{subst-r'}{\parallel} & $(\refssu{r}{V}{M}) \parallel N$
% & $\to$ & $\refssu{r}{V}{(M \parallel (\refssd{r}{V}{N}))}$ \\
%  & & & \\
% \rrulet{subst-r'}{lapp} &
% $\refssl{}{U}{((\refssu{}{V}{M})\,N)}$ & $\to$ &
% $\refssu{}{V}{\refsrawsl{}{\multv{U},\multv{V}}{(M\,(\refssd{}{V}{N}))}}$ \\
% \rrulet{subst-r'}{rapp} &
% $\refssl{}{U}{(M\,(\refssu{}{V}{N}))}$ & $\to$ &
% $\refssu{}{V}{\refsrawsl{}{\multv{U},\multv{V}}{((\refssd{}{V}{M})\,N)}}$ \mynl
% \multicolumn{4}{l}{Congruence case:}\\
% \multicolumn{4}{l}{If $M \rightarrow M'$ by any of the previous rules, then
%   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \mynl
% \multicolumn{4}{l}{Finally:}\\
% \rrule{subst-r'}{\top} & $\mathbf{S}[\refssu{r}{V}{M}]$
% & $\to$ & $\mathbf{S}[M]$
% \end{tabular}
% \end{center}
% \caption{Reduction Rules}\label{fig:lth-red-rules}
% \end{table}
% %%%-------------------------------------------------------------------
%
%
% \begin{notation}\label{not:context}\rm
%   the contexts $E$, $C$ and $\mathbf{S}$ are defined in
%   Table~\ref{fig:lth-eval-context}. The context $E$ stands for a usual
%   call-by-value applicative context, $C$ picks a thread, while
%   $\mathbf{S}$ picks a term in a non-deterministic sum. Note how
%   $E$ does not enforce any reduction order on an application.
% \end{notation}
% %
% \begin{notation}\label{not:subst}\rm
%   Given a variable substitution $\sigma$ and a value $V$, we define
%   the value $\metas{\sigma}V$ as follows:
%   $\metas{\sigma}{(\lambda x . M)} = \lambda x .
%   (\varss{\sigma}{M})$,
%   $\metas{\sigma}{(x)} = \sigma(x)$ if $\sigma$ is defined at $x$ or
%   $\metas{\sigma}{(x)} = x$ if not, and
%   $\metas{\sigma}{(\ast)} = \ast$.
% \end{notation}
% %
% \begin{notation}\label{not:subst2}\rm
%   We use the
%    notation $\multv{X} = \multv{V},\multv{W}$ for the juxtaposition of
%    references substitutions. It is defined by
%    %
%    $\multv{X}(r) =
%    \multv{V}(r) + \multv{W}(r)$ if both are defined and where $+$ is the union of multisets,
%    $\multv{V}(r)$ if only $\multv{V}$ is defined, and
%    $\multv{W}(r)$ if only $\multv{W}$ is defined.
%    %
%    We use the same notation for the
%    composition of variable substitutions, defined by
%    %
%    $(\sigma,\tau)(x) =
%      \metas{\tau}{\sigma(x)}$ if both are defined,
%      $\sigma(x)$ if only $\sigma$ is defined
%      $\tau(x)$  if only $\tau$ is defined.
%    %
%    Finally, we define
%    $\metas{\sigma}{\multv{V}} : r \mapsto [ \metas{\sigma}{V_i} \mid V_i \in
%    \multv{V}(r) ]$.
% \end{notation}
%
% We now give some explanations on the rules of Table~\ref{fig:lth-red-rules}.
%
% \paragraph*{(a) $\beta$-reduction}
% %
% If one forgets the $\lambda$-substitution explained below in
% Subsection (d), this set of rules encapsulates the call-by-value
% behavior of the language: only values can be substituted in the body
% of abstractions, and this happens within a thread in a call-by-value
% applicative context.
%
% \paragraph*{(b) Variable Substitutions}
%
% A variable
% substitution can be seen as a message emitted by a $\beta$-redex and
% dispatched through the term seen as a tree. The substitution flows
% from the redex downward the term-tree until it reaches the occurrence
% of a variable. The occurrence is then replaced, or not, depending on
% the variable to be substituted. The rules in
% Table~\ref{fig:lth-red-rules}(a) are an operational formalization of
% this step-by-step procedure.
% %
% Consider for example the reduction of the term
% $(\lambda x . x\ y\ z)\ (\lambda x . x)$. The redex triggers with
% $(\beta_v)$ the substitution of all occurrences of $x$ in what was the
% body of the lambda-abstraction. The substitution goes down the
% corresponding sub-term and performs the substitution when it reaches an
% occurrence of $x$.
% %
% \begin{center}
% \scalebox{.8}{%
% \begin{tabular}{ccccc}
%   \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$(\lambda x . x\ y\ z)\ (\lambda x.x)$};
%     \node[draw=none] (M) at (-1,-1)
%       {$\lambda x. x\ y\ z$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (X) at (-1,-3)
%       {$x$};
%     \node[draw=none] (N) at (1,-1)
%       {$(\lambda x. x)$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (M) at (0,0)
%     {$\varss{x \mapsto (\lambda x. x)}{x\ y\ z}$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$x$};
%
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (M) at (0,0)
%       {$x\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%     {$\varss{x \mapsto (\lambda x. x)}{\ldots}$};
%     \node[draw=none] (X) at (0,-2)
%       {$x$};
%
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (M) at (0,0)
%       {$x\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$\varss{x \mapsto (\lambda x. x)}{x}$};
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (M) at (0,0)
%       {$(\lambda x. x)\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$\lambda x. x$};
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
% \end{tabular}%
% } % END SCALEBOX
% \end{center}
%
% % \begin{remark}
% \paragraph{Remark}
% On rules \rrulet{subst}{subst-r} and \rrulet{subst}{subst-r'}.
% %
% When composing or swapping substitutions, non-values may appear in
% unfortunate places: take for example
% $\varss{\sigma}{(\refssu{}{V}{\ast})}$, its reduction should be
% $\refrawsu{}{\multv{V'}}{(\varss{\sigma}{\ast})}$ where
% $\multv{V}'(r) = [ \varss{\sigma}{V} \mid V \in \multv{V}(r) ]$ when
% $\multv{V}(r)$ is defined. But $\varss{\sigma}{V}$ are not necessarily
% values and should then be able to be reduced inside
% substitutions. However, note that that $\varss{\sigma}{V}$ always
% reduces in one step to the value $\metas{\sigma}{V}$. To avoid
% additional complexity, we perform this reduction at the same time,
% whence the use of $\metas{\sigma}{V}$ instead of $\varss{\sigma}{V}$
% in the actual rules.
% % \end{remark}
%
%
% \paragraph*{(c) Downward Reference Substitutions}
%
% An {\setw} can occur anywhere within a term and it must be able to reach a
% {\getw} located in an arbitrary position. In a language such
% as~\cite{Amadio2009}, as discussed in Section~\ref{sec:amadio}
% the solution is to keep all assignments in a global
% store. When a {\getw} gets evaluated, the value for the reference is
% taken from the store.  This approach is very global in nature: the
% store is ``visible'' by every subterm.
%
% The language {{\lthis}} features a step-by-step decomposition of
% reference assignments akin to term variable substitutions: an
% assignment follows the branches of the term-tree, actively seeking a
% {\getw}.
% %
% We therefore introduce two sorts of reference substitutions: one that
% goes downward (indicated by $\downarrow$), similar to variable
% substitutions, and one that goes upward (indicated by $\uparrow$). Starting from
% an \setw, the latter climbs up the tree up to the root. The rules in
% Table~\ref{fig:lth-red-rules}(c) describes the former while the rules in
% Table~\ref{fig:lth-red-rules}(d) describes the latter.
%
% % \begin{remark}
% \paragraph{Remark}
%   In Table~\ref{fig:lth-red-rules}, the rule \rrulet{subst-r}{get} is
%   the central case of the reduction of reference substitutions. It
%   says that whenever a downward substitution reaches a $\get{r}$, then
%   it generates a non deterministic sum of all the available values for
%   the reference $r$ (if $\multv{V}$ is undefined at $r$, then this sum
%   is understood as a neutral element $\mathbf{0}$) plus a term where
%   the substitution was discarded but the $\get{r}$ is left
%   unreduced. To see why this ``remainder'' is necessary, consider the
%   term $\refsrawsd{}{\store r V_2}{\refsrawsd{}{\store r V_1}{\get{r}}}$.  If we
%   omit the remainder, the term could reduce to
%   $\refrawsd{}{\store r V_2}{V_1}$ and finally to $V_1$. But another
%   reduction is possible: one can first reduce the term to
%   $\refsrawsd{}{\store{r}{V_1},\store{r}{V_2}}{\get{r}}$ and then to $V_1 + V_2$.  The
%   $\get{r}$ must not be greedy: when it meets a substitution, it has
%   to consider the possibility that other substitutions will be
%   available later. This aspect will be crucial when considering the
%   proof of strong normalization of the language in
%   Section~\ref{sec:term}.
% % \end{remark}
%
% \paragraph*{(d) Upward Reference Substitutions}
%
% Each time an upward reference substitution goes through a multi-ary constructor --
% as an application or a parallel composition -- it propagates downward
% substitutions in all the children of the constructor except the one
% it comes from, while continuing its ascension. Eventually, all the
% leafs are reached by a corresponding downward substitution. To
% illustrate the idea, consider a term $M\ N$ where $M$ contains a
% $\get{r}$ somewhere and $N$ an {\setw} $\refrawsu{}{\store r V}{\ast}$. The reduction of explicit
% substitutions would go as follows.
%
% \begin{center}
% \scalebox{.8}{%
% \begin{tabular}{cccc}
%   % \begin{tikzpicture}[yscale=\mytikshrink]
%   %   \node[draw=none] (MN) at (0,0)
%   %     {$M\ N$};
%   %   \node[draw=none] (M) at (-1,-1)
%   %     {$M$};
%   %   \node[draw=none] (M2) at (-1,-2)
%   %     {$\ldots$};
%   %   \node[draw=none] (G) at (-1,-3)
%   %     {$\text{get}(r)$};
%   %   \node[draw=none] (N) at (1,-1)
%   %     {$M$};
%   %   \node[draw=none] (N2) at (1,-2)
%   %     {$\ldots$};
%   %   \node[draw=none] (S) at (1,-3)
%   %     {$\set{r}{V}$};
%   %
%   %   \draw[-,>=latex] (MN) -- (M);
%   %   \draw[-,>=latex] (MN) -- (N);
%   %   \draw[-,>=latex] (M) -- (M2);
%   %   \draw[-,>=latex] (M2) -- (G);
%   %   \draw[-,>=latex] (N) -- (N2);
%   %   \draw[-,>=latex] (N2) -- (S);
%   % \end{tikzpicture}
%   %
%   \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\refrawsu{}{\store r V}{\ast}$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\refrawsu{}{\store r V}{\ldots}$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$\refrawsu{}{\store r V}{N}$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture} \\
%
%   \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$\refrawsu{}{\store r V}{(M\ N)}$};
%     \node[draw=none] (M) at (-1,-1)
%       {$\refrawsd{}{\store r V}{M}$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$\refrawsu{}{\store r V}{(M\ N)}$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\refrawsd{}{\store r V}{\ldots}$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$\refrawsu{}{\store r V}{(M\ N)}$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\refrawsd{}{\store r V}{\get r}$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$\refrawsu{}{\store r V}{(M\ N)}$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$V$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
% \end{tabular}%
% } % END SCALEBOX
% \end{center}
%
%
%
% One last subtlety in the movement of reference substitutions concerns
% $\lambda$-abstractions. As made explicit in
% Table~\ref{fig:lth-red-rules}(a), the language is call-by-value:
% reduction does not happen under $\lambda$-abstractions. In particular, a
% read within the body of a $\lambda$-abstraction should only be accessible
% by an assignment when the $\lambda$-abstraction is opened: we have a
% natural notion of pure and impure terms. Pure terms are terms that
% won't produce any effect when reduced, and in particular, all values
% are expected to be pure terms since they can't reduce further. This is
% highlighted by rule \rrulet{subst-r}{val}: when encountering a pure
% term, a reference substitution vanishes. But the case of abstraction
% is more subtle: computational effects frozen in its body are freed
% when the abstraction is applied. If one implements naively the
% reduction rules of reference substitutions, then the following example
% doesn't behave as expected:
% $\refssd{}{V}{((\lambda x. \get{r})\ \ast)} \to
% (\refssd{}{V}{(\lambda x .  \get{r})})\ (\refssd{}{V}{\ast}) \to
% (\lambda x .  \get{r})\ \ast \to \get{r}$.
% We end up with an orphan $\get{r}$ despite the fact that a substitution was
% available at the beginning.
% The problem is that the substitution diffuses through the application,
% then encounters two pure terms and vanishes.
%
% In an application, the left term eventually exposes the body of an
% abstraction, and this body should be able to use any substitution that
% was in its scope. The $\lambda$-substitution $[-]_\lambda$ is a
% special stationary reference substitution attached to an
% application. Its goal is precisely to record all the substitutions
% that went down through it with Rules \rrulet{subst-r'}{lapp} and
% \rrulet{subst-r'}{rapp}. When the application is finally reduced with
% a $\beta_v$-rule, this substitution will turn to a downward one and
% feed the $\get{r}$'s that were hidden in the abstraction's
% body.
%
% % \begin{remark}
% \paragraph{Remark}
%   An alternative approach to $\lambda$-substitution would be to make
%   downward substitutions not vanish (i.e. getting rid of Rule
%   \rrulet{subst-r}{val}). In this situation, values would be handled
%   with their whole context of references assignment. Apart from the
%   heavy syntactical cost of carrying around a lot of similar and
%   possibly useless substitutions, the idea that hidden effects are
%   released at application appears more natural regarding type and
%   effect systems, as the one we introduce in Section~\ref{sec:type}.
% % \end{remark}
%
% % \begin{remark}
% \paragraph{Remark}
%   Rule \rrule{subst-r'}{\top} acts as a garbage
%   collection to eliminating top-level upward substitutions. While not
%   necessary, this will greatly ease the statement and proof of lemmas
%   and theorems (such as Lemma~\ref{lemma-progress}).
% % \end{remark}
%
% %
% % \paragraph{Terms}
% %
% % We define $\finsup{A}{B}$ as the set of partial functions $f : A \rightharpoonup
% % B$ with finite
% % support. Substitutions will be represented by such functions, mapping a finite
% % set of variable (resp. locations) to a value (resp. a multiset of values).
% % We write $\fmset{A}$ for the finite multisets of elements of $A$, or in other
% % word, $\finsup{A}{\mathbb{N}}$.
% %
% % \vspace{0.5cm}
% %
% % \begin{tabular}{llll}
% %   -variables & \multicolumn{3}{l}{$x,y,\ldots$} \\
% %   -regions & \multicolumn{3}{l}{$r,r',\ldots$} \\
% %   -values & $V$ & $::=$ & $x \mid \ast \mid \lambda x.M$ \\
% %   % csubst values & $V^s$ & $::=$ & $V \mid \varss{x}{V}{V^s}$ \\
% %   -rsubsts & $\mathcal{V}$ & : & $\finsup{\text{regions}}{\text{values}}$ \\
% %   -vsubsts & $\sigma$ & : & $\finsup{\text{variables}}{\fmset{\text{values}}}$ \\
% %   -terms & $M$ & $::=$ & $V \mid \varss{\sigma}{M} \mid \refssl{r}{V}{M\ M} \mid
% %   \get{r} \mid \text{set}(r,V)$ \\
% %   & & & $\mid \refssd{r}{V}{M} \mid \refssu{r}{V}{M} \mid M \parallel M$ \\
% %   -sums & $\mathbf{M}$ & $::=$ & $\mathbf{0} \mid M \mid \mathbf{M} +
% %   \mathbf{M}$ \\
% % \end{tabular}
% %
% % \paragraph{}
% % We will use the synctatic sugar $\varss{\sigma}{\multv{V}} = \multv{V}'$ where
% % $\multv{V}'(r) = \{ \varss{\sigma}{V_i} \mid V_i \in \multv{V}(r) \}$.
% %
% % \paragraph{}
% % For a value $V$, we define a meta substitution $\varmetas{(x_k)}{(U_k)}{V}$ by
% % the normal form of $\vars{(x_k)}{(U_k)}{V}$ which is :
% % \begin{itemize}
% %   \item $\varmetas{(x_k)}{(U_k)}{y} = U_k$ if $\exists k, y = x_k$, or $y$
% %     otherwise
% %   \item $\varmetas{(x_k)}{(U_k)}{\ast} = \ast$
% %   \item $\varmetas{(x_k)}{(U_k)}{(\lambda y . M)} = \lambda y .
% %     (\vars{(x_k)}{(U_k)}{M})$
% % \end{itemize}
% %
% % \subsection{Reduction}
% % We adopt a weak CBV reduction, where the reduction order of an application is not
% % specified (nor left-to-right neither right-to-left). The sum is idempotent,
% % associative and commutative, with $\mathbf{0}$ as neutral element. The parallel
% % composition is associative and commutative.
% % \begin{center}
% % \begin{tabular}{rcl}
% % \hline
% % \multicolumn{3}{|c|}{Structural rules} \\
% % \hline
% % $M \parallel M'$ & = & $M' \parallel M$ \\
% % $\mathbf{M} + \mathbf{M}'$ & = & $\mathbf{M}' + \mathbf{M}$ \\
% % $(\mathbf{M} + \mathbf{M}') + \mathbf{M}''$ & = & $\mathbf{M} + (\mathbf{M}' +
% % \mathbf{M}'')$ \\
% % $(M \parallel M') \parallel M''$ & = & $M \parallel (M' \parallel M'')$ \\
% % $\mathbf{M} + \mathbf{0}$ & = & $\mathbf{M}$ \\
% % \end{tabular}
% % \end{center}
% %
% % \paragraph{}
% % \begin{center}
% % \begin{tabular}{lcl}
% % \hline
% % \multicolumn{3}{|c|}{Evaluation contexts} \\
% % \hline
% % % $E$ & $::=$ & $[.] \mid \refssl{r}{V}{E\ M} \mid
% % %   \refssl{r}{V}{M\ E}$ \\
% % $E$ & $::=$ & $[.] \mid \refssl{r}{V}{E\ M} \mid
% %   \refssl{r}{V}{M\ E} $ \\
% % & & $\refssd{r}{V}{E}
% %   \mid \refssu{r}{V}{E}$ \\
% % % $G$ & $::=$ & $[.] \mid \refssl{r}{V}{G\ M} \mid
% % %   \refssl{r}{V}{M\ G} \mid \varss{\sigma}{G}$ \\
% % $C$ & $::=$ & $[.] \mid (C \parallel M) \mid (M \parallel C)$ \\
% % $\mathbf{S}$ & $::=$ & $[.] \mid \mathbf{S} + \mathbf{M} \mid \mathbf{M} +
% % \mathbf{S}$ \\
% % \end{tabular}
% % \end{center}
% %
% % \paragraph{}
% % \begin{center}
% % \begin{tabular}{lrcl}
% % \hline
% % \multicolumn{4}{|c|}{Reduction rules (main)} \\
% % \hline
% %
% % $(\beta_v)$ & $\refssl{r}{U}{(\lambda x.M)\ V}$ & $\rightarrow$ &
% % $\refssd{r}{U}{\varss{\sigma}{M}}$ \\
% %
% % % $(\texttt{\text{set}})$ & $\text{set}(r,V)$ & $\rightarrow$ & $
% % % \substup{(r)}{([V])}{\ast}$ \\
% % \\
% %
% % \hline
% % \multicolumn{4}{c}{If $M \rightarrow M'$ by any of the previous rules, then
% %   $\mathbf{S}[C[E[M]]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% %
% % \end{tabular}
% % \paragraph{}
% % \begin{tabular}{lrcl}
% %
% % \hline
% % \multicolumn{4}{|c|}{Reduction rules (variables substitutions)} \\
% % \hline
% % \rrulet{subst}{var} & $\varss{\sigma}{x}$
% % & $\to$ & $\sigma(x)$ if defined, or $x$ otherwise\\
% %
% % \rrulet{subst}{unit} & $\varss{\sigma}{\ast}$
% % & $\to$ & $\ast$ \\
% %
% % \rrulet{subst}{app} & $\varss{\sigma}{\refssl{}{V}{M\
% % N}}$ & $\to$
% % & $\refrawsl{}{(\varss{\sigma}{\multv{V}})}{(\varss{\sigma}{M})\
% % (\varss{\sigma}{N})}$ \\
% %
% % \rrule{subst}{\lambda} & $\varss{\sigma}{\lambda y.M}$ & $\to$
% %   & $\lambda y.(\varss{\sigma}{M})$ \\
% %
% % \rrulet{subst}{get} & $\varss{\sigma}{\get{r}}$ & $\to$
% %  & $\get{r}$ \\
% %
% % % $(\texttt{subst}_\texttt{set})$ & $\varss{\sigma}{\text{set}(r,U)}$ & $\to$
% % %  & $\text{set}(r,\varss{\sigma}{U})$ \\
% %
% % \rrule{subst}{\parallel} & $\varss{\sigma}{M \parallel M'}$ & $\to$
% % & $(\varss{\sigma}{M}) \parallel (\varss{\sigma}{M'})$ \\
% %
% % \rrulet{subst}{subst-r} &
% % $\varss{\sigma}{( \refssd{r}{V}{M} )}$ & $\to$
% % & $\refsrawsd{}{\varss{\sigma}{\multv{V}}}{\varss{\sigma}{M}}$ \\
% %
% % \rrulet{subst}{subst-r'} &
% % $\varss{\sigma}{( \refssu{r}{V}{M} )}$ & $\to$
% % & $\refsrawsu{}{\varss{\sigma}{\multv{V}}}{\varss{\sigma}{M}}$ \\
% %
% % \rrulet{subst}{merge} & $\vars{(x_i)_{i \in \mathcal{I}}}{(V_i)_{i \in
% % I}}{\vars{(y_i)_{i \in \mathcal{J}}}{(U_i)_{i \in \mathcal{J}}}{M}}$ & $\to$
% % & $\vars{(z_i)_{i \in \mathcal{I} \cup \mathcal{J}}}{(W_i)_{i \in \mathcal{I} \cup \mathcal{J}}}{M}$ \\
% % & & & \\
% %  & \multicolumn{3}{c}{
% %   $\mathcal{W}_i =
% %   \begin{cases*}
% %     V_i & \text{if $i \in \mathcal{I}$} \\
% %     \varmetas{(x_k)_{k \in \mathcal{I}}}{(V_k)_{k \in \mathcal{I}}}{U_i} & \text{if $i \in \mathcal{J}$} \\
% %   \end{cases*}$} \\
% % \\
% %
% % \\
% % \hline
% % \multicolumn{4}{c}{If $M \rightarrow M'$ by any of the previous rules, then
% %   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% %
% % \end{tabular}
% % \paragraph{}
% % \begin{tabular}{lrcl}
% %
% % \hline
% % \multicolumn{4}{|c|}{Reduction rules (downward references substitutions)} \\
% % \hline
% %
% % \rrulet{subst-r}{val} & $\refssd{}{V}{V}$
% % & $\to$ & $V$ \\
% %
% % % $(\texttt{subst-r}_\texttt{set})$ &
% % % $\refssd{r}{V}{\text{set}(s,V)}$ & $\to$ &
% % % $\text{set}(s,V)$ \\
% %
% % \rrule{subst-r}{\parallel} & $\refssd{}{V}{M
% % \parallel M'}$ & $\to$
% % & $(\refssd{}{V}{M}) \parallel (\refssd{}{V}{M'})$ \\
% %
% % \rrulet{subst-r}{subst-r'} &
% % $\refssd{r}{V}{\refssu{s}{U}{M}}$ & $\to$
% % & $\refssu{s}{U}{\refssd{r}{V}{M}}$ \\
% %
% %  & & & \\
% %
% % \rrulet{subst-r}{merge} &
% % $\refssd{}{V}{\refssd{}{U}{M}}$ & $\to$
% % & $\refsrawsd{}{\multv{U},\multv{V}}{M}$ \\
% % % \rrulet{subst-r}{merge} & \multicolumn{3}{l}{
% % %  $\substdown{(r_i)_{i \in \mathcal{I}}} {(\mathcal{U}_i)_{i \in \mathcal{I}}} {(
% % %     \substdown{(r_j)_{j \in \mathcal{J}}} {(\mathcal{V}_j)_{j \in \mathcal{J}}} {M}
% % %   )}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\to$
% % %     $\substdown{(r_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {(\mathcal{W}_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {M}$} \\
% % % \\
% %
% % \rrulet{subst-r}{app} &
% % $\refssd{}{V}{\refssl{}{U}{M\ N}}$ & $\to$
% % & $\refsrawsl{}{\multv{V},\multv{U}}{(\refssd{}{V}{M})\ (\refssd{}{V}{N})}$ \\
% % % \rrulet{subst-r}{app} & \multicolumn{3}{l}{
% % %  $\substdown{(r_i)_{i \in \mathcal{I}}} {(\mathcal{U}_i)_{i \in \mathcal{I}}} {(
% % %     \substl{(r_j)_{j \in \mathcal{J}}} {(\mathcal{V}_j)_{j \in \mathcal{J}}}{M\ N}
% % %   )}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\to \text{subst}^\lambda \ {(r_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %     ={(\mathcal{W}_i)_{i \in \mathcal{I}\cup\mathcal{J}}} \text{ in }$} \\
% % %     & \multicolumn{3}{l}{
% % %       $\phantom{\to C[G[}(\substdown{(r_i)_{i \in \mathcal{I}}}{(\mathcal{U}_i)_{i
% % %         \in \mathcal{I}}}{M})
% % %       \ (\substdown{(r_i)_{i \in \mathcal{I}}}{(\mathcal{U}_i)_{i
% % %         \in \mathcal{I}}}{N})$} \\
% % %  & & & \\
% % %  & \multicolumn{3}{c}{
% % %   $\mathcal{W}_i =
% % %   \begin{cases*}
% % %     \mathcal{U}_i & \text{if $i \in \mathcal{I} \setminus (\mathcal{I} \cap \mathcal{J})$} \\
% % %     \mathcal{V}_i & \text{if $i \in \mathcal{J} \setminus (\mathcal{I} \cap \mathcal{J})$} \\
% % %     \mathcal{U}_i + \mathcal{V}_i & \text{if $i \in \mathcal{I} \cap \mathcal{J}$}
% % %   \end{cases*}$} \\
% % % \\
% % % \hline
% %
% % \multicolumn{4}{c}{If $M \rightarrow M'$ by any of the previous rules, then
% %   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% %
% % \\
% % \rrulet{subst-r}{get} &
% % $\mathbf{S}[C[E[\refssd{}{V}{\get{r}}]]]$ & $\to$
% % & $\mathbf{S}[C[E[\get{r}]]] + \sum_{V \in \multv{V}(r)}
% % C[E[V]]$ \\
% %
% % \end{tabular}
% % \paragraph{}
% % \begin{tabular}{lrcl}
% %
% % \hline
% % \multicolumn{4}{|c|}{Reduction rules (upward references substitutions)} \\
% % \hline
% %
% %
% % % $(\texttt{subst-r'}_\texttt{$\parallel$})$ & $M \parallel (\refssu{r}{V}{N})$
% % % & $\to$ & $\refssu{r}{V}{(\refssd{r}{V}{M}) \parallel N}$ \\
% %
% % \rrule{subst-r'}{\parallel} & $(\refssu{r}{V}{M}) \parallel N$
% % & $\to$ & $\refssu{r}{V}{M \parallel (\refssd{r}{V}{N})}$ \\
% %  & & & \\
% %
% % \rrulet{subst-r'}{lapp} &
% % $\refssl{}{U}{(\refssu{}{V}{M})\ N}$ & $\to$ &
% % $\refssu{}{V}{\refsrawsl{}{\multv{V},\multv{U}}{M\ (\refssd{}{V}{N})}}$ \\
% %
% % % \rrulet{subst-r'}{lapp} & \multicolumn{3}{l}{
% % %  $\substl{(r_i)_{i \in \mathcal{I}}} {(\mathcal{U}_i)_{i \in \mathcal{I}}} {
% % %     (\substup{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in \mathcal{J}}}
% % %     {M})\ N}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\to\ \substup{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in
% % %       \mathcal{J}}}{}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\phantom{\to\ }
% % %       \substl{(r_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {(\mathcal{W}_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {M\ (\substdown{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in
% % %         \mathcal{J}}}{N})}$} \\
% % %  & & & \\
% %
% % \rrulet{subst-r'}{rapp} &
% % $\refssl{}{U}{M\ (\refssu{}{V}{N})}$ & $\to$ &
% % $\refssu{}{V}{\refsrawsl{}{\multv{V},\multv{U}}{(\refssd{}{V}{M})\ N}}$ \\
% %
% % % \rrulet{subst-r'}{rapp} & \multicolumn{3}{l}{
% % %  $\substl{(r_i)_{i \in \mathcal{I}}} {(\mathcal{U}_i)_{i \in \mathcal{I}}} {
% % %     M\ (\substup{(r_j)_{j \in \mathcal{J}}} {(\mathcal{V}_j)_{j \in \mathcal{J}}}
% % %     {N}
% % %   )}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\to\ \substup{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in
% % %       \mathcal{J}}}{}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\phantom{\to\ C[E[}
% % %       \substl{(r_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {(\mathcal{W}_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {(\substdown{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in
% % %         \mathcal{J}}}{M})\ N}$} \\
% % %  & & & \\
% %
% % % ****** EST-CE QU'IL FAUDRAIT UN MERGE POUR SUBST UP ÉGALEMENT ??? ****** %
% % \\
% %
% % \hline
% % \multicolumn{4}{c}{If $M \rightarrow M'$ by any of the previous rules, then
% %   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% % \\
% % \rrule{subst-r'}{\top} & $\mathbf{S}[\refssu{r}{V}{M}]$
% % & $\to$ & $\mathbf{S}[M]$ \\
% %
% % \end{tabular}
% %
% % \end{center}
% %
% % \subsection{ }
% %
% % In [US], we define a type system for \lthis and gives proof for the following
% % statements:
% %
% % \begin{theorem}{Type soundness}\\
% %   Typing is preserved by reduction.
% % \end{theorem}
% %
% % \begin{theorem}{Confluence}\\
% %   \lthis\ is confluent on well-typed terms.
% % \end{theorem}
% %
% % \begin{theorem}{Termination}\\
% %   Well typed terms are strongly normalizing.
% % \end{theorem}
% %
% % \subsection{Simulation}
% %
% % \newcommand{\vstore}{\multv{V}_S}
% % \newcommand{\strans}{$\overline{\phantom{M}}^S$}
% % \newcommand{\sleq}{\rightsquigarrow_s}
% %
% % The intermediate language \lthis\ is capable of simulating \lamadio. Moreover, a
% % result of adequacy is proven, in the sense that it does not produce more values
% % than the original \lamadio\ term.
% %
% % \begin{definition}{Translation of \lamadio in \lthis}\\
% %     Let $M$ be a term and $S$ be a store of \lamadio.
% %     S can be written as
% %     \[
% %       S = r_1 \Leftarrow V^1_1 \parallel \ldots \parallel r_1
% %       \Leftarrow V^1_{k_1} \parallel \ldots \parallel r_n \Leftarrow
% %       V^n_1 \parallel \ldots \parallel r_n \Leftarrow
% %       V^n_{k_n}
% %     \]
% %     Let $\multv{V}_S : r_i \mapsto [V^i_1, \ldots, V^i_{k_i}]$.
% %   We define the translation of $M$ under $S$ by
% %     \begin{itemize}
% %       \item If $M = V$ or $M = \text{set}(s,V)$ then $\overline{M}^S = M$
% %       \item If $M = N\ N'$ then $\overline{M}^S = \refsrawsl{r}{\vstore}(\overline{N}^S)\
% %         (\overline{N'}^S)$
% %       \item If $M = \get{s}$ then $\overline{M}^S =
% %         \refsrawsd{r}{\vstore}{\get{s}}$
% %       \item If $M = N \parallel N'$ then $\overline{M}^S = \overline{N}^S
% %         \parallel \overline{N'}^S$
% %     \end{itemize}
% %
% %     In fact, one can see that $\overline{M}^S$ is the normal form of
% %     $\refsrawsd{r}{\vstore}{M}$ for the reduction defined by all
% %     \rrulet{subst-r}{} rules except \rrulet{subst-r}{get}.
% %
% %     We extend it to contexts $E,F$ and $G$ by adding the rule $\overline{[.]}^S = [.]$.
% %     \\
% %     Finally, for any program $P = M \parallel S$, we define $\overline{P} =
% %     \overline{M}^S$.
% %     If $P = M$ then $\overline{P} = \overline{M} = M$.
% %   \end{definition}
% %
% %   % Originally put restrictions like $M$ and $N$ must not be parallel,
% %   % or that some reduction on parallel must not be used, but now I don't
% %   % see why this would be the case, so just removing
% %   % \begin{lemma}{Context reduction}\label{lemma-ctxt-red}\\
% %   %   Let $M,N$ be terms of \lthis such that $M \to^\ast N$ without using
% %   %   \rrule{subst-r}{\top}, then for any
% %   %   context $C$ and $E$, $C[E[M]] \to^\ast C[E[N]]$ using the same reduction
% %   %   rules.
% %   % \end{lemma}
% %   %
% %   % \begin{lemma}{Context decomposition}\label{lemma-ctxt-decomp}\\
% %   %   Let $P$ be a program of \lamadio,
% %   %   \begin{itemize}
% %   %     \item $P = C[E[M]] \text{ with } C = [.] \text{ or } C = [.] \parallel N \implies
% %   %       \overline{P} = P$
% %   %     \item $P = C[E[M]] \text{ with } C = [.] \parallel N \parallel S \implies
% %   %       \overline{P} = \overline{E}^S[\overline{M}^S] \parallel \overline{N}^S$
% %   %   \end{itemize}
% %   % \end{lemma}
% %   %
% %   % \begin{proof}
% %   %   This is an easy induction following the definition of \strans.
% %   % \end{proof}
% %   %
% %   % \begin{lemma}{Substitution for \strans}\label{lemma-subst}\\
% %   %   Let $M,M'$ be terms, $V$ a value and $S$ a
% %   %   store of \lamadio. Then
% %   %   \[
% %   %     \overline{M[x/V]}^S = \overline{M}^S[x/V]
% %   %   \]
% %   % \end{lemma}
% %   % \begin{proof}
% %   %   By induction
% %   % \end{proof}
% %   %
% %   % \begin{lemma}{Absorption}\label{lemma-absorption}\\
% %   %   Let $M$ be a term and $S = S' \parallel r \Leftarrow V$ be a store of
% %   %   \lamadio, $C$ and $E$ be context of \lthis, and $\multv{V}
% %   %   : r \mapsto [V]$. Then
% %   %   $$C[E[\refssd{}{V}{\overline{M}^{S'}}]] \to_\texttt{aux}^\ast
% %   %   C[E[\overline{M}^{S}]]$$
% %   % \end{lemma}
% %   %
% %   % \begin{proof} By induction on $M$, using the definition of
% %   %   \strans and the \texttt{subst-r} reductions.
% %   % \end{proof}
% %   %
% %   % \begin{lemma}{Diffusion}\label{lemma-diffusion}\\
% %   %   Let $N$ be a term, $E$ a context, $S = S' \parallel r \Leftarrow V$ a store of
% %   %   \lamadio and $\multv{V} : r \mapsto [V]$. Let $M$ be a term of \lthis. Then
% %   %   \begin{equation}\label{lemma-diff-eq1}
% %   %     \overline{E}^{S'}[\refssu{}{V}{M}]
% %   %     \to_\texttt{aux}^\ast \refssu{}{V}{\overline{E}^S[M]}
% %   %   \end{equation}
% %   %   \begin{equation}\label{lemma-diff-eq2}
% %   %     \refssu{}{V}{M} \parallel \overline{N}^{S'}
% %   %     \to_\texttt{aux}^\ast \refssu{}{V}{(M \parallel
% %   %     \overline{N}^S)}
% %   %   \end{equation}
% %   %   \begin{equation}\label{lemma-diff-eq3}
% %   %     \overline{E}^{S'}[\refssu{}{V}{M}] \parallel \overline{N}^{S'}
% %   %     \to_\texttt{aux}^\ast \refssu{}{V}{\overline{E}^S[M] \parallel
% %   %     \overline{N}^S}
% %   %   \end{equation}
% %   %   using only rules \rrulet{subst-r}{} or \rrulet{subst-r'}{}.
% %   % \end{lemma}
% %   %
% %   % \begin{proof}
% %   %   \begin{itemize}
% %   %
% %   %     \item For (\ref{lemma-diff-eq1}), we work by induction on $E$. As we
% %   %       will need \ref{lemma-ctxt-red}, we add the induction hypothesis
% %   %       that the rule $(\texttt{subst-r'}_\top)$ is not used.
% %   %       \begin{itemize}
% %   %         \item $\overline{E}^{S'} = [.]$ nothing to do
% %   %         \item $\overline{E}^{S'} = \refssl{s}{U}{\overline{E'}^{S'}\
% %   %         \overline{M'}^{S'}}$\\
% %   %           By IH, $\overline{E'}^{S'}[\refssu{}{V}{M}] \to^\ast
% %   %           \refssu{}{V}{\overline{E'}^{S}[M]}$ using no
% %   %           \rrule{subst-r'}{\top} rules.
% %   %           We use \ref{lemma-ctxt-red} and get
% %   %           $$\overline{E}^{S'}[\refssu{}{V}{M}] \to^\ast
% %   %           \refssl{s}{U}{(\refssu{}{V}{\overline{E'}^{S}[M]})
% %   %           \ \overline{M'}^{S'}}$$
% %   %           We then apply \rrulet{subst-r'}{lapp} to get
% %   %           $$\overline{E}^{S'}[\refssu{}{V}{M}] \to^\ast \refssu{}{V}{\refssl{t}{W}{(\overline{E'}^{S}[M])
% %   %           \ (\refssd{}{V}{\overline{M'}^{S'}})}}$$
% %   %           Using \ref{lemma-absorption}, we get that the right part of the
% %   %           application reduces to $\overline{M'}^S$. Finally, by definition of
% %   %           \strans, the right hand side is $\refssu{}{V}{\overline{E}^S[M]}$.
% %   %         \item Other cases are treated alike
% %   %        \end{itemize}
% %   %   \item To prove (\ref{lemma-diff-eq2}), we apply
% %   %     \rrule{subst-r'}{\parallel}. We then use
% %   %     \ref{lemma-absorption} on $\refssd{}{V}{\overline{N}^{S'}}$ to get
% %   %     $\overline{N}^S$ and \ref{lemma-ctxt-red} with $C = M \parallel [.]$
% %   %     to get the desired result.
% %   %   \item Finally, we prove (\ref{lemma-diff-eq3}) by combining the two results. We
% %   %     first use the strenghtened version of $(\ref{lemma-diff-eq1})$, so we can
% %   %     apply \ref{lemma-ctxt-red} and get
% %   %     $$\overline{E}^{S'}[\refssu{}{V}{M}] \parallel \overline{N}^{S'}
% %   %     \to^\ast \refssu{}{V}{M}{\overline{E}^S[M]} \parallel \overline{N}^{S'}$$.
% %   %     We use (\ref{lemma-diff-eq2}) with $M' = E[M]$ to get the result.
% %   %   \end{itemize}
% %   % \end{proof}
% %
% %   Our reduction have the drawback of not reducing under abstractions, such that
% %   some of the variable substitution propagation will be delayed until the
% %   corresponding lambda will be applied (or forever). To cope with this subtelty,
% %   we introduce a relation on terms of \lthis\ that morally states that a
% %   term $M$ is related to $N$ if $M$ is the same as $N$ up to some pending
% %   substitutions hidden under lambdas, such that if we could reduce these
% %   subtitution under abstraction $M$ would actually reduce to $N$.
% %
% %   \begin{definition}{Substitution order}\label{definition-substitution-equivalence}\\
% %     We define $\sleq$ as :
% %     \begin{itemize}
% %       \item $x \sleq x$, $\get r \sleq \get r$, $\set r V \sleq \set r V$
% %       \item $\refssl{}{V}{M\ N} \sleq \refssl{}{V}{M'\ N'}$
% %         or $M \parallel N \sleq M' \parallel N'$ iff $M \sleq M'$ and $N \sleq N'$
% %       \item $\lambda x.M \sleq \lambda x.M'$ if $M =
% %         \varss{\sigma_1}{\varss{\ldots}{\varss{\sigma_n}{N}}}$ such that
% %         $N\{\sigma_1,\ldots,\sigma_n\} = N$.
% %       \item $\refssd{}{V}{M} \sleq \refssd{}{V}{M'}$ or $\refssu{}{V}{M}
% %         \sleq \refssu{}{V}{M'}$ iff $M \sleq M'$
% %     \end{itemize}
% %   \end{definition}
% %
% %   \begin{lemma}{Properties of the substitution
% %     order}\label{lemma-substitution-equivalence-prop}\\
% %     $\sleq$ is a simulation order, meaning that if $M \sleq N$ and $M \to
% %     M'$, then $N \to^\ast N'$ with $M' \sleq N'$
% %   \end{lemma}
% %
% %   We can now state the following result modulo this equivalence
% %
% %   \begin{lemma}{Explicit substitution}\label{lemma-expl-subst}\\
% %     Let $P = C[E[\varss{\sigma}{M}]]$ with $M$ containing no explicit
% %     substitutions nor upward reference substitution.
% %     Then $$P \to_\texttt{aux}^\ast P' \sleq C[E[\varmetas{x}{V}{M}]]$$
% %   \end{lemma}
% %
% %   % \begin{proof}
% %   %   By induction on $M$.
% %   %   \begin{itemize}
% %   %     \item Neutral \\
% %   %       If $M=\ast$, $M=\get{r}$ or $M=y$ with $y \neq x$, then
% %   %       $\varmetas{x}{V}{M}=M$. If we apply \rrulet{subst}{unit} (resp.
% %   %       \rrulet{subst}{get},\rrulet{subst}{var}) we also get
% %   %       that $$C[E[\varss{\sigma}{M}]] \to_\text{aux} C[E[M]]$$
% %   %     \item $M=x$ \\
% %   %       $\varmetas{x}{V}{M}=V$. By \rrulet{subst}{var},
% %   %       $$C[E[\varss{\sigma}{x}]] \to_\text{aux} C[E[V]]$$
% %   %     \item $M=\lambda y. M'$ \\
% %   %       $\varmetas{x}{V}{M}=\lambda y.(\varmetas{x}{V}{M'})$. By
% %   %       \rrule{subst}{\lambda},
% %   %       $$C[E[\varss{\sigma}{\lambda y. M'}]] \to_\text{aux}
% %   %       C[E[\lambda y. (\varss{\sigma}{M'})]]
% %   %       \sleq C[E[\lambda y.(M'\{\sigma\})]]$$
% %   %     \item \ldots \\
% %   %       The remaining cases are treated similarly, the reduction rules being
% %   %       designed to make this lemma work.
% %   %       TODO : explain why we don't care about reference substitution, that
% %   %       cannot have free variables in the translation
% %   %       % There is a little subtelty, depending on how the substitution
% %   %       % $\varmetas{M}{x}{V}$ is defined with respect to references substitutions, ie when $M =
% %   %       % \refssd{r}{\mathcal{V}}{M'}$ for example. Actually, the
% %   %       % variables appearing in $\mathcal{V}$ should not be bound by any lambda because these
% %   %       % values have been emitted by sets, and sets can't be reduced under
% %   %       % lambdas. Thus all substitutions of bound variables in $\mathcal{V}$
% %   %       % already occured, and only globally free variables can remain. We define $M[x/V]$ to be
% %   %       % $\substvg{r}{\mathcal{V}}{(M'[x/V])}$, which matches the reduction rule
% %   %       % $\texttt{subst}_{\texttt{subst}_\texttt{r}}$, and this case is treated
% %   %       % as others.
% %   %   \end{itemize}
% %   % \end{proof}
% %   %
% % \subsection{One-step simulation}
% %   We prove now the technical result that will give the main theorem, which is
% %   contained in this lemma :
% %
% %   \begin{theorem}{One-step simulation}\label{theorem-simulation}\\
% %     Let $P,Q$ be \lamadio programs such that $P
% %     \rightarrow_\texttt{orig} Q$. Then
% %     $$\overline{P} \rightarrow_\texttt{aux}^\ast M \sleq \overline{Q}$$
% %   \end{theorem}
% %
% %   From which, thanks to \ref{lemma-substitution-equivalence-prop}, we easily deduce
% %
% %   \begin{theorem}{Simulation}\label{theorem-simulation}\\
% %     Let $P,Q$ be \lamadio programs such that $P
% %     \rightarrow_\texttt{orig}^\ast Q$. Then
% %     $$\overline{P} \rightarrow_\texttt{aux}^\ast M \sleq \overline{Q}$$
% %   \end{theorem} 
% %
% %   % \begin{proof}\ref{theorem-simulation}\\
% %   %   By case analysis on the reduction rule applied :
% %   %   \begin{description}
% %   %     \item[$\beta_v$] We have $P = E[(\lambda x. M)\ V] \parallel N \parallel
% %   %       S$ and $Q = E[\varmetas{x}{V}M] \parallel N \parallel S$. Let
% %   %       By ~\ref{lemma-ctxt-decomp}, $\overline{P} =
% %   %       \overline{E}^S[\refrawsl{r}{\vstore}{\lambda x. M
% %   %       \ V}] \parallel \overline{N}^S$ and $\overline{Q} =
% %   %         \overline{E}^S[\overline{\varmetas{x}{V}{M}}^S] \parallel \overline{N}^S$. Then, by
% %   %       one application of $\beta_v$ in \lthis, we have $\overline{P}
% %   %       \rightarrow_\texttt{aux} Q_0 =
% %   %       \overline{E}^S[\varss{\sigma}{\refrawsd{}{\vstore}{M}}] \parallel
% %   %       \overline{N}^S$.
% %   %       We apply \ref{lemma-absorption} with to deduce
% %   %       $Q_0 \to^\ast Q_1 = \overline{E}^S[\varss{\sigma}{\overline{M}^S}]
% %   %       \parallel \overline{N}^S$. Using \ref{lemma-expl-subst} and
% %   %       \ref{lemma-subst}, we get $Q_1
% %   %       \to^\ast Q_2 \sleq \overline{E}^S[\overline{\varmetas{x}{V}{M}}^S] \parallel
% %   %       \overline{N}^S=\overline{Q}$.
% %   %     \item[get] We have $P = E[\get{r}] \parallel N \parallel S$ with
% %   %       $S=S' \parallel
% %   %       r \Leftarrow V$, and $Q = E[V] \parallel N \parallel S$.
% %   %       By \ref{lemma-ctxt-decomp},
% %   %       $\overline{P} = \overline{E}^S[\refssd{}{V}{\get{r}}]
% %   %       \parallel \overline{N}^S$ and $\overline{Q} = \overline{E}^S[V]
% %   %       \parallel \overline{N}^S$.
% %   %       The rule \rrulet{subst-r}{get} gives $\overline{P} \to_\text{aux}
% %   %       \overline{E}^S[V] \parallel \overline{N}^S = \overline{Q}$.
% %   %     \item[set] We have $P = E[\set r V] \parallel N \parallel S'$ and $Q = E[\ast]
% %   %       \parallel N \parallel S$ with $S = S' \parallel r \Leftarrow V$. By
% %   %       \ref{lemma-ctxt-decomp}, $\overline{P} =
% %   %       \overline{E}^{S'}[\refssu{}{V}{\ast}]
% %   %       \parallel \overline{N}^{S'}$ and $\overline{Q} = \overline{E}^S[\ast]
% %   %       \parallel \overline{N}^S = \overline{E[\ast] \parallel N}^S$.
% %   %       We apply \ref{lemma-diffusion} to get
% %   %       $P \to^\ast \refssu{}{V}{(\overline{E}^S[\ast] \parallel
% %   %       \overline{N}^S)}$ and then use the rule \rrule{subst-r}{\top} to get
% %   %       rid of the toplevel reference substitution.
% %   %   \end{description}
% %   % \end{proof}


==> paper-csl-long arxiv/parts/language-properties.tex <==
\section{Properties of $\lamlang{aux}$}

\input{parts/properties-type}
\input{parts/properties-termination}


==> paper-csl-long arxiv/parts/nets-results.tex <==
\section{Properties of the translation}
\label{section:properties}

\subsection{Simulation}
The first result is the simulation theorem. The formulation precises
that a deterministic step in {\lamadio} is mapped to a deterministic reduction in nets, and
only the reduction of $\get{r}$ produces a non-deterministic sum.

\begin{theorem}{Simulation}\label{theorem-nets-simulation}\\ Let $\vdash M :
  (\alpha,e)$ be a closed well-typed term of \lamadio. Then
  \begin{itemize}
    \item If $M \to N$  by $(\beta_v)$ or $(\texttt{set})$ then
      $M^\bullet \to^\ast N^\bullet$
    \item If $M \to N_i$ by $(\texttt{get})$ then
      $M^\bullet \to^\ast \net R + \sum_i {N_i}^\bullet$
  \end{itemize}
\end{theorem}

The presence of the additional term $\net R$ is linked to the
local nature of non-determinism in proof nets. When facing a get
reduction, the proof net can either select one of the available {\setw}, or drop
them all and wait for an hypothetical future one, which corresponds to this
$\net R$ net. This is better understood when stating the simulation theorem on
{\lthis}:

\begin{theorem}{Simulation for {\lthis}}\label{theorem-nets-simulation-lthis}\\
  Let $\vdash M : (\alpha,e)$ be a closed well-typed term of \lthis
  . If $M \to^\ast N$, then $M^\bullet \to^\ast N^\bullet$.
\end{theorem}

Here, the term $\net R$ is totally internalized in {\lthis} and we get a clean
simulation theorem.  To derive this result, we start by defining a notion of
typed context and a translation of contexts to nets.

\begin{definition}{Hole typing rule}\label{definition-nets-simulation-typehole}\\
\[
  \infer[(hole)]
  {R,[.] : (\alpha,e) \vdash [.] : (\alpha,e)}
  {R \vdash (\alpha,e)}
\]
\end{definition}

\begin{center}
  \begin{tabular}{|c|c|}

  \end{tabular}
\end{center}

$[.]$ can be seen just as a special kind of variable in the typing derivation
that can be substituted by something else than a value. We use the usual typing
rules to build derivations of typed contexts. A context can then be translated
to a net, with an interface determined by $\alpha$ and $e$, labelling
free ports.  This is what we call net contexts. The substitution of nets
consists in plugging the translation of a term with a matching type in this interface.

\begin{definition}{Hole translation}\label{definition-nets-simulation-holetrans}\\
  We define the translation of a typed hole $R \vdash [.] : (\alpha,e)$
as

\begin{center}
  \begin{tabular}{DD}
  \[
    \infer[(hole)]
    {R,[.] : (\alpha,e) \vdash [.] : (\alpha,e)}
    {R \vdash (\alpha,e)}
  \]
   &
    \includegraphics{figures/translation/pdfs/translation-hole.pdf} \\
  \end{tabular}
\end{center}

We can then carry on and use the usual term translation to build the
translation of a context $(C[E])^\bullet$, which is a net of the form

\begin{center}
  \includegraphics{figures/translation/pdfs/translation-context.pdf}
\end{center}

The substitution of $M^\bullet$, or of any net with a compatible interface for
that matter, in $(C[E])^\bullet$ is defined by just connecting the free wires of
the substituted net to the corresponding free wire of the context hole :

\begin{center}
  \includegraphics{figures/translation/pdfs/translation-context-subst.pdf}
\end{center}

\end{definition}

The fundamental property of net contexts and net substitutions is that the
substitution commutes with the translation, in the following sense :

\begin{property}{Nets substitution}\label{property-nets-substitution}\\
  Let $ \vdash [.] : (\alpha,e)$ be a typed hole, $[.] : (\alpha,e) \vdash C[E]
  : (\beta,e')$ a typed context, and $ \vdash M : (\alpha,e)$ a term. Then :
\[
  (C[E[M]])^\bullet = (C[E])^\bullet[M^\bullet]
\]
\end{property}

% The proof is an easy induction: the base case when $C[E] = [.]$ is immediate,
% and by definition of the context translation, so is the inductive case.
%
The very definition of net reduction immediately entails that if $M^\bullet
\to^\ast N^\bullet$ then $(C[E])^\bullet[M^\bullet] \to^\ast
(C[E])^\bullet[N^\bullet]$. Together with
Property~\ref{property-nets-substitution}, this ensures that we can focus on the case
where $C = E = [.]$, as the general case follows seamlessly.

From here, we check that each reduction rule of \lthis\ can be simulated on the
net side, relying on the definition of the reduction and the behavior of routing areas.

% \paragraph{Reference substitutions}
%
% We state and prove a few lemma about the reduction of the translation of reference
% substitutions.
%
% [TODO]

\paragraph{Variable substitutions reductions}

Let us show the simulation for \rrulet{subst}{} rules, involving mainly
duplication. Thanks to the previous theorem, we can assume that contexts are
empty without loss of generality. We consider only closed terms. Indeed, since
reduction contexts $S,C,E$ do not bind variables, all the terms appearing in the
premise of a rule are thus closed terms, and we can
omit their context. For each rule, we write the translation of the premise
followed by its reduction in nets, which matches the conclusion.

The fundamental rule is the variable one.

\begin{center}
  \begin{longtable}{lDED}
    \rrulet{subst}{var} ($\sigma(x)$ undefined)
    & \includegraphics{figures/simulation/pdfs/subst-var-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/subst-var-reduct.pdf} \\

    \rrulet{subst}{var} ($\sigma(x)$ defined)
    & \includegraphics{figures/simulation/pdfs/subst-var-2-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/subst-var-2-reduct.pdf} \\
  \end{longtable}
\end{center}

\vspace{0.5cm}
When reaching a $\get{r}$ or a $\ast$, the substitution simply vanishes.
\begin{center}
 \begin{longtable}{lDED}
    \rrulet{subst}{unit}
    & \includegraphics{figures/simulation/pdfs/subst-unit-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/subst-unit-reduct.pdf} \\
  \end{longtable}
\end{center}

\vspace{0.5cm}
The \rrulet{subst}{app}, \rrulet{subst}{subst-r} and \rrulet{subst}{subst-r'}
perform a duplication and propagate the substitution inside reference
substitutions.

\begin{center}
  \begin{longtable}{lDED}
    \rrulet{subst}{app}
    & \multicolumn{3}{D}{
      \includegraphics{figures/simulation/pdfs/subst-app-redex.pdf}
    } \\

    $\to^\ast$
    & \multicolumn{3}{D}{
      \includegraphics{figures/simulation/pdfs/subst-app-reduct.pdf}
    } \\

    \rrulet{subst}{subst-r}
    & \includegraphics{figures/simulation/pdfs/subst-substr-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/subst-substr-reduct.pdf} \\

    \rrulet{subst}{subst-r'}
    & \includegraphics{figures/simulation/pdfs/subst-substrp-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/subst-substrp-reduct.pdf} \\
  \end{longtable}
\end{center}

\vspace{1cm}
The \rrule{subst}{\parallel} just duplicate the variable substitution to the two
threads
\begin{center}
  \begin{longtable}{lDED}
    \rrule{subst}{\parallel}
    & \includegraphics{figures/simulation/pdfs/subst-par-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/subst-par-reduct.pdf} \\
  \end{longtable}
\end{center}

\vspace{0.5cm}
Finally, the \rrulet{subst}{merge} distributes the outter substitution to both
the term and the inner substitution.
\begin{center}
  \begin{longtable}{lDED}
    \rrulet{subst}{merge}
    & \includegraphics{figures/simulation/pdfs/subst-merge-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/subst-merge-reduct.pdf} \\
  \end{longtable}
\end{center}

\paragraph{Downward reference substitutions reductions}

The propagation of references substitutions relies on the behavior of routing
area, and especially Property~\ref{property-translation-transit}. The
fundamental case is the non deterministic reduction happening when reducing a
$\get{r}$ whose redex is
\begin{center}
  \begin{longtable}{lD}
    \rrulet{subst-r}{get}
    & \includegraphics{figures/simulation/pdfs/substr-get-redex.pdf} \\
  \end{longtable}
\end{center}

Then for each $V$ in the image of $\multv{V}$, there will be exactly one summand
of the following form

\begin{center}
  \begin{longtable}{DED}
    \includegraphics{figures/simulation/pdfs/substr-get-reduct-1-1.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/substr-get-reduct-1-2.pdf} \\
  \end{longtable}
\end{center}

The remaining term does indeed reduce to the translation of $\get{r}$:
\begin{center}
  \begin{longtable}{DED}
    \includegraphics{figures/simulation/pdfs/substr-get-reduct-2-1.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/substr-get-reduct-2-2.pdf} \\
  \end{longtable}
\end{center}

\vspace{0.5cm}
\rrulet{subst-r}{val}, \rrule{subst-r}{\parallel} and \rrulet{subst-r}{app} are
just direct application of the Property~\ref{property-translation-transit}.

\begin{center}
  \begin{longtable}{lDED}
    \rrulet{subst-r}{val}
    & \includegraphics{figures/simulation/pdfs/substr-val-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/substr-val-reduct.pdf} \\

    \rrule{subst-r}{\parallel}
    & \includegraphics{figures/simulation/pdfs/substr-par-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/substr-par-reduct.pdf} \\

    \rrulet{subst-r}{app}
    & \multicolumn{3}{D}{
      \includegraphics{figures/simulation/pdfs/substr-app-redex.pdf}
    } \\
    $\to^\ast$
    & \multicolumn{3}{D}{
      \includegraphics{figures/simulation/pdfs/substr-app-reduct.pdf}
    } \\
  \end{longtable}
\end{center}

\vspace{0.5cm}
\rrulet{subst-r}{merge} and \rrulet{subst-r}{subst-r'} amount to nothing in nets, as the translation
already identifies the redex and the reduct of these rules.

\begin{center}
  \begin{longtable}{lDlD}
    \rrulet{subst-r}{subst-r'}
    & \includegraphics{figures/simulation/pdfs/substr-substrp-both.pdf}
    & \rrulet{subst-r}{merge}
    & \includegraphics{figures/simulation/pdfs/substr-merge-both.pdf} \\
  \end{longtable}
\end{center}

\paragraph{Upward reference substitutions reduction}
As for downward substitutions, the main ingredient is the Transit lemma applies
to our specific routing area $\delta$ and $\gamma$.

\begin{center}
  \begin{longtable}{lDED}
    \rrule{subst-r'}{\parallel}
    & \includegraphics{figures/simulation/pdfs/substrp-par-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/substrp-par-reduct.pdf} \\

    \rrulet{subst-r'}{lapp}
    & \includegraphics{figures/simulation/pdfs/substrp-lapp-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/substrp-lapp-reduct.pdf} \\

    \rrulet{subst-r'}{rapp}
    & \includegraphics{figures/simulation/pdfs/substrp-rapp-redex.pdf}
    & $\to^\ast$
    & \includegraphics{figures/simulation/pdfs/substrp-rapp-reduct.pdf} \\
  \end{longtable}
\end{center}
\newcommand{\labelsubst}[2]{|{#1}|_{#2}}
\newcommand{\lthisplus}{$\lamlang{cES+}$}

\subsection{Termination}
The second result states that the translation of a term is strongly
normalizing:

\begin{theorem}{Termination}\label{theorem-termination}\\
  The translation of a well typed term of {\lamadio} terminates.
\end{theorem}

The theorem that we will actually prove is rather the following:
\begin{theorem}{Termination of \lthis}\label{theorem-termination-lthis}\\
  The translation of the normal form of a well-typed term of {\lthis} terminates.
\end{theorem}

While {\lthis} is closer to nets that {\lamadio}, unfortunately a normal form of
{\lthis} is not translated to a normal form in proof nets. The corresponding net
can still perform some reductions. But we will see that these are unessential
and limited: in a few steps, a normal form is reached in nets.

We proceed in two stages: first, we extend {\lthis} to a language {\lthis +}
that is able to do just a little more reductions than {\lthis}. The extension of
the translation and the simulation theorem for {\lthis +} are straightforward.
Then, we show that {\lthis +} also terminates, give an explicit grammar for its
normal forms, and show that the translation of these normal forms are
strongly normalizing proof nets.

\paragraph{\lthis +}

We add a labelled reference substitution variable substitution to {\lthis}
: $\refssdbar{}{V}{M} \mid \varsbar{x}{N}{M}$. The first one,
$\refssdbar{}{V}{M}$, correspond to a downward reference substitution where
$\multv{V}$ has no free variables. The second one corresponds to a variable
substitution of a term that is not a value. Both can appear during the reduction
in proof nets but are not accounted for in {\lthis}. $\varsbar{x}{N}{M}$ can't
be reduced, either in $N$ or by \rrulet{subst}{} rules (whether $N$ is a value or
not). The labelled reference forbids any reduction under it, except for the
labelled reference substitutions.  We extend the reduction rules
\rrulet{subst-r}{} to the labelled substitution $\refssdbar{}{V}{}$. They can be
performed anywhere (included under a variable substitution) except under
abstraction, in a context defined by the following grammar: $J ::= [.] \mid J\ M
\mid M\ J \mid \refssd{}{V}{J} \mid \varss{\sigma}{J} \mid \varsbar{x}{N}{J}$.

We also add a $\beta$-rule to fire such labelled substitution :
\[
  (\beta_{V}') \refssl{}{V}{(\lambda x . M)\ N} \to
  \varsbar{x}{N}{\refssdbar{}{V}{M}}
\]

This corresponds to the additional reduction nets can do. Indeed a $\beta$ redex
can always be fired in nets even if the argument is not a value. But then, the
corresponding term do need to be reduced before any duplication, erasure or
substitution. Let us now show termination and describe the normal forms of {\lthis+}:

\begin{mdef}{$F$-normal forms}\label{lemma-progress-auxplus}\\
  Let $M$ be a normal form of the form of {\lthis}. It belongs to the grammar
  $M_\text{norm}$ (cf~\cite{HamdaouiValiron2018}). Then $M$ reduces to a sum
  of terms in {\lthis +} that belongs to the
 following grammar of $F$-normal forms :
\begin{tabred}
  F_\text{norm} & ::= & \get{r} \mid \refssl{}{V}{F_\text{norm}\ V} \mid
  \refssl{}{V}{F_\text{norm}\ F_\text{norm}} \mid \varsbar{x}{F_\text{norm}}{M} \\
\end{tabred}
where the $M$ is in \lthis (contains no labelled substitution).
\end{mdef}

\begin{proof}
  By induction on the structure of $M$, with the additional hypothesis that only
  the additional rules are performed (no upward substitution) :
  \begin{itemize}
    \item $M = \get{r}$ : ok 
    \item $M = \refssl{}{V}{M_\text{norm}\ V}$ : by induction, $M_\text{norm}$
      reduces to a sum of $F_\text{norm}$. Take one such summand $N$, then $M \to^\ast
      \refssl{}{V}{N_\text{norm}\ V}$ (because no rule \rrule{subst-r'}{\top} was
      used)
    \item $M = \refssl{}{V}{M_\text{norm}\ M'_\text{norm}}$ : we proceed as the
      previous case
    \item $M = \refssl{}{V}{V\ M_\text{norm}}$ : by induction, $M_\text{norm}$
      reduces to some $N$ in $F_\text{norm}$ grammar, so $M \to^\ast
      \refssl{}{V}{V\ N}$. Then, by inversion of typing rules, $V$ is of the
      form $\lambda x . P$ and we can apply the new $\beta$-reduction to get
      $\varsbar{x}{N}{\refssdbar{}{V}{P}}$. By pushing down $\refssdbar{}{V}{}$ in
      $P$, we can reduce it to a sum of $P_i$s where each $P_i$ do not contain
      labelled substitutions. Then $M \to^\ast \sum_i \vars{x}{N}{P_i}$
  \end{itemize}
\end{proof}

\begin{lemma}
$F$-normal forms are normal.
\end{lemma}

\begin{proof}
  By induction :
  \begin{itemize}
    \item $M = \get{r}$ : ok
    \item $M = \refssl{}{V}{F_\text{norm}\ V}$ : by induction, $F_\text{norm}$
      is normal, and values are not $F$-normal form, so the application can't create any
      $\beta$-redex.
    \item $M = \refssl{}{V}{M_\text{norm}\ M'_\text{norm}}$ : same as the
      previous case
    \item $M = \varsbar{x}{F_\text{normal}}{M}$ : the explicit substitution
      prevents any reduction except \rrulet{subst-r}{} ones for labelled
      reference substitution, but by definition, $M$ does not contain any.
  \end{itemize}
\end{proof}

\paragraph{$F$-normal forms and proof nets}
We will see in the following that the translation of a $F$-normal form has not
many possible reductions left.  However, a few steps may remain to eventually
reach a normal form. The first step is to collect and merge all the routing
areas that are created and connected during the translation. Doing so, we
separate the net between a part that closely follows the translated term
structure, and a big routing area which connects various subterms to enable
communication through references between them. Once this is done, a few starving
{\getw s} may interact with the routing area, but nothing more. The following
definition give the shape obtained after the merging of routing:

\begin{definition}{Separability}\label{definition-nets-termination-separability}\\
  Let $\mathcal{R}$ be the translation of a {\lthis +}
  term, then $\mathcal{R}$ is say to be \emph{separable} if
  it can be reduced to the following form :

  \begin{center}
    \includegraphics{figures/termination/pdfs/termination-separability-def.pdf}
  \end{center}

  % \begin{center}
  %   \tikzvcenter{
  %     \begin{proofnet}
  %       % Communication box
  %       \node[net={40pt}{40pt}] (box) {\mathbf{R}};
  %       % Remaining part of the net
  %       \init[grow=left]([xshift=15ex]box.east){
  %         \nary[shape=rectangle,cell={net={40pt}{30pt}},name=sigma]{\mathcal{S}}{
  %           \point(sigmai1),
  %           \point(sigmao1),
  %           \point(sigmain),
  %           \point(sigmaon)
  %         }
  %       }
  %       % Box coordinates
  %       \coordinate (i1) at ([yshift=-13pt]box.east);
  %       \coordinate (o1) at ([yshift=-8pt]box.east);
  %       \coordinate (in) at ([yshift=8pt]box.east);
  %       \coordinate (on) at ([yshift=13pt]box.east);
  %       \coordinate (i0) at ([yshift=-3pt]box.west);
  %       \coordinate (o0) at ([yshift=2pt]box.west);
  %       % Sigma coordinates
  %       \coordinate (sigmai1) at ([yshift=-13pt]sigma.north);
  %       \coordinate (sigmao1) at ([yshift=-8pt]sigma.north);
  %       \coordinate (sigmain) at ([yshift=8pt]sigma.north);
  %       \coordinate (sigmaon) at ([yshift=13pt]sigma.north);
  %       % Connect box and sigma
  %       \init[grow=up]{
  %         \wirefromto{sigmai1}{sigmai1}{i1}{i1}
  %         \wirefromto{sigmain}{sigmain}{in}{in}
  %         \wirefromto{sigmao1}{sigmao1}{o1}{o1}
  %         \wirefromto{sigmaon}{sigmaon}{on}{on}
  %         \wirefromto{[xshift=-10pt]i0}{[xshift=-10pt]i0}{i0}{i0}
  %         \wirefromto{[xshift=-10pt]o0}{[xshift=-10pt]o0}{o0}{o0}
  %       }
  %       %
  %       \pdots[2pt]([xshift=10pt]o1)([xshift=10pt]in)
  %     \end{proofnet}
  %   }
  % \end{center}
  where $\mathbf{R}$ is a routing area and $\mathcal{S}$ a net with free wires labelled by
  $i_1,\ldots,i_n,o_1,\ldots,o_m,O$, satisfying :
  \begin{description}
    \item[(a)] There is no redex in $\mathcal{S}$
    \item[(b)] $i_1,\ldots,i_n$ are either connected to the auxiliary port of a
      $\otimes$ cell, to the auxiliary port of a cocontraction or to the principal port of a dereliction
    \item[(c)] $o_1,\ldots,o_m,O$ are either connected to a
      $\parr$ cell, or to the principal door of an open box
  \end{description}
\end{definition}

The translation of term with at least one free variable is separable.  The
reason is that constructors such as application, substitution, parallel
composition, etc. preserve separability. Moreover, the translation of values
with free variables are obviously separable. The weakenings, which correspond to
free variables, materialize as auxiliary doors of exponential boxes, thus
blocking further reduction.

\begin{lemma}{Open terms separability}\label{lemma-nets-termination-otsep}\\
  Let $\Gamma,x:A \vdash M : (\alpha,e)$ a {\lthis} well-typed term, then its
  translation $M^\bullet$ is separable.
\end{lemma}

\begin{proof}\ref{lemma-nets-termination-otsep}\\
  We proceed by induction on terms.
\begin{description}
  \item[Values] As stated above, we can first observe that the translation of $\ast$, of a
    variable $x$ and an abstraction all satisfy the separability conditions.
    Indeed, they are composed of a box with at least one auxiliary door, and the
    inside of the box is a normal form (by induction for abstraction and
    trivially for others). As they are pure terms, $m = n = 0$.
  \item[Get] It is almost the same as values, except that the output $o$
    corresponding to the reference of $\get{r}$ is connected to a dereliction, which is
    allowed in \textbf{(b)}.
  \item[Application] By induction, $M^\bullet$ and $N^\bullet$ are
    separable, thus can be decomposed in the following way :

    \begin{center}
      \includegraphics{figures/termination/pdfs/termination-separability-app.pdf}
    \end{center}

    We can merge the 3 routing areas $\routarea{R}, \routarea{R}_1$ and
    $\delta$. All the inputs or outputs previously connected to one of the small
    areas immediately satisfy the conditions \textbf{(b,c)} by IH. The two
    remaining wires $i$ and $o$ are respectively connected to the auxiliary port
    of a par and the auxiliary port of a cocontraction, thus satisfy
    \textbf{(b,c)}.  $\mathcal{S}$ and $\mathcal{S}_1$ are normal by IH, and the
    translation of $\multv{V}$ is easily seen as normal. $O$ is the conclusion of
    a par, hence satisfies \textbf{(b,c)}. It only remains to see that the whole
    net excepted the routing areas is normal, but the only redex that could appear
    is the connection of a dereliction to $M^\bullet$. By \textbf{(c)},
    the output of $M^\bullet$ is either the conclusion of an open box or a par which do not form a
    redex.  The condition \textbf{(a)} is verified.
  \item[Parallel] Similar to application
  \item[Variable substitution] As for application, we apply the IH on
    $M^\bullet$ and $V^\bullet$, merge the routing areas, and just check that the
    connection of $V^\bullet$ to $M^\bullet$ can not create new redexes using
    \textbf{(b)} on the output wire of $V^\bullet$.
  \item[Reference substitutions] Again, the same technique is applied.
\end{description}

\end{proof}

Finally, the main result we rely on as explained above is the following one :

\begin{lemma}{Normal form separability}\label{lemma-nets-termination-nfsep}\\
  The translation of a $F$-normal form is separable
\end{lemma}

It is proved as Lemma~\ref{lemma-nets-termination-otsep}, by induction on the
syntax of $F$-normal forms. We can eventually prove from this last lemma:

\begin{lemma}{Termination of {\lthis +}}\label{lemma-termination-lthisp}\\
  The translation of a $F$-normal form is strongly normalizing.
\end{lemma}

From which we deduce:

\begin{corollary}{Strong normalization}\label{corollary-termination-sn}\\
  \begin{enumerate}
    \item The translation of a closed well-typed term of {\lthis +} is strongly normalizing.
    \item The translation of a closed well-typed term of {\lthis} is strongly
      normalizing (Theorem~\ref{theorem-termination-lthis}).
  \end{enumerate}
\end{corollary}

\begin{proof}{Lemma~\ref{lemma-termination-lthisp}}\\
  We apply \ref{lemma-nets-termination-nfsep} to reduce the translation of a
  $F$-normal form $F$ to a routing area $\routarea R$ connected to $\mathcal{S}$
  satisfying separability conditions. $\mathcal{S}$ and $\routarea R$ are
  normal. The potential redexes must involve a wire at the interface of
  $\routarea{R}$ and $\mathcal{S}$. The inputs of $\routarea{R}$ are connected
  to $\mathcal{S}$, either to a par or to the conclusion of an open box and thus
  can't form any redex with (co)weakenings and (co)contractions of $\routarea
  R$.

  The outputs of $\routarea R$ are either connected to the auxiliary port of a
  tensor, the auxiliary port of a cocontraciton or to a dereliction. Only the
  latter may form a new redex. If the output of $\mathbf{R}$ is a coweakening,
  then everything reduces to $\mathbf{0}$. If it is just a wire, then the
  dereliction is connected through this wire to an input of $\routarea R$ which
  again can't be part of any redex. The only remaining case is when the output
  of $\routarea R$ is a cocontraction tree.  Then we can perform the
  non-deterministic $\red{ba}$ reductions, and we go back to exactly the two
  previous cases as the dereliction is finally connected to a leaf of the tree
  of an input.

  Hence, after we performed finitely many $\red{ba}$ reductions,
  we finally get a normal form, which is either $\mathbf{0}$, or a sum of the
  previous net $\mathbf{S}$ connected to simpler routing area $\routarea{R}_i$.
\end{proof}

Simulation and termination ensure that if a term $M$ reduces to $T = V_1 \parallel
\ldots \parallel V_n$, then:
\begin{itemize}
  \item By simulation, the translation $M^\bullet$ can be reduced to a non
    deterministic sum in which one summand will be $T^\bullet$
  \item By termination, this does not depend on the path of reduction we chose:
    any reduction will converge to a normal form whose summands contain the
    net $T^\bullet$.
\end{itemize}

The normal form of $M^\bullet$ must contain the summand $T$. However, this does
not tell us anything about what are the other summands of $M^\bullet$. Let us
pretend the support for integers in \lamadio. Assume that a term $M$ have $2$ as
only normal form. Because of this additional term $\net R$ appearing in the
simulation theorem, our results do not prevent $M^\bullet$ to reduce to
$1^\bullet + 2^\bullet + 3^\bullet$. In such a case, one may argue that the
proof nets do not reflect faithfully the language as they may have a lot more
possible outcomes.

\subsection{Adequacy}

The adequacy theorem states that the summands of the normal form of
$M^\bullet$ are either the translation of a normal form $T = V_1 \parallel
\ldots \parallel V_n$ that is a reduct of the original $M$, or garbage, that is
a non correct net that corresponds to execution paths which deadlocked. We can
recognize this garbage, thus eliminate it: with this additional operation, the
summands of the normal form of $M^\bullet$ coincide with the values that are
reachable by $M$.

% \newcommand{\values}[1]{\text{Val}({#1})}
\begin{theorem}{Adequacy}\label{theorem-adequacy}\\
  Let $M$ be well-typed term of \lamadio. We write $\values{M} := \{
  T = \ \parallel_i V_i \mid M \to^\ast T \}$. Similarly, for a net $\net R$
  with normal form $\net N$, we define $\values{\net R} = \{ \net S \mid \net N =
  \net S + \net S',\ \net S \text{ is a value net } \}$. Then
  $$\values{M} = \values{M^\bullet}$$
\end{theorem}

We first need to prove adequacy between {\lamadio} and {\lthis}:

\begin{theorem}{Adequacy for {\lthis}}\label{theorem-adequacy-lthis}\\
  Let $P$ be a term of {\lamadio} and $M = \widetilde{P}$ its translation in
  \lthis, if $M \to^\ast \sum_i M_i$ a normal form, then $\forall
  i, P \to^\ast P_i$ such that $M_i \rincl \widetilde{P_i}$. In other words, any
  term appearing in the normal form of the translation of $P$ is bounded by the
  translation of a reduct of $P$.
\end{theorem}

In particular, applied to values, this gives the sought property for {\lthis}:

\begin{corollary}\label{corollary-adequacy-simulation-orig}
  Let $P$ be a term of {\lamadio}, $M = \widetilde{P}$ its translation in
  {\lthis} such that $M \to^\ast M' + \mathbf{M''}$ where $M'$ is a normal
  form.
  \begin{itemize}
    \item If $M' = V \parallel N$, then $P \to^\ast U \parallel Q$ with $V =
      \widetilde{U}$.
    \item In particular, if $M' = \parallel_i V_i$, then $P \to^\ast \parallel_i
      U_i$ with $V_i = \widetilde{U}_i$
  \end{itemize}
\end{corollary}

The only problematic case is the non deterministic reduction
\rrulet{subst-r}{get} which creates new summands. The proof consist in showing
that these summands are actually limited in what they can do. Formally, they are
bounded by the initial term that is being reduced, in the sense of the preorder
$\rincl$ defined in~\cite{HamdaouiValiron2018}. The following lemma state that
indeed the case of deterministic reduction is trivial:

\begin{lemma}{Values preservation}\label{lemma-preservation-values}\\
  Let $M$ be a term of {\lamadio}, and $M \to^\ast M'$ without using
  \rrulet{subst-r}{get}. We define $\text{NF}(M) = \{ T \mid T \text{ normal}
  \text{ and } M \to^\ast T \}$. Then $\text{NF}(M) = \text{NF}(M')$
\end{lemma}

\begin{proof}
  If we do not use \rrulet{subst-r}{get}, the two reduction (full and
  non-deterministic) coincide and we use the confluence in {\lamadio}.
\end{proof}

\begin{lemma}{}\label{lemma-onestep-adequacy} Let $M = \widetilde{P}$ be the
  translation of a {\lamadio} term, such that $M \to M'$. Then there exists
  $M'',N'$, such that $M' \to^\ast M'' \rincl \widetilde{N'}$ and $N
  \to^{\{0,1\}} N'$, with all reductions from $M'$ to $M''$ not being
\rrulet{subst-r}{get}.  \end{lemma}

\begin{proof}
  The only redexes in $M$ are either premises of \rrulet{subst-r'}{},
  $(\beta_v)$ or \rrulet{subst-r}{get}.
  In the first case, it corresponds to a reducible set whose reduction can be
  carried on in $M'$ by pushing the upward substitution to the top and pushing
  down the corresponding generated downward substitutions, to obtain the translation of
  $N'$ (which is $N$ where we the set is reduced). We can proceed the same way
  with $(\beta_v)$ : this corresponds to a $\beta$-redex in $N$, where $N'$ is
  the result of reducing it, and $M''$ is obtained by pushing down the generated
  substitutions (variable and refenreces).

  Finally, if the reduction rule is \rrulet{subst-r}{get}, then either it
  choosed one of the available values and it corresponds exactly to a get
  reduction $N \to N'$, or it threw away available values, in which case $N =
  N'$, $M' = M''$ and clearly $M'' \rincl \widetilde{N'}$.
\end{proof}

\begin{proof}{Theorem~\ref{theorem-adequacy-lthis}}\\
  We proceed by induction on $\eta (M)$, the length of the longest reduction
  starting from $M$. If $\eta (M) = 0$, ie $M$ is a normal form, this is
  trivially true.
  \\
  To prove the induction step, consider a reduct $M'$ of $M$. We use
  \ref{lemma-onestep-adequacy} to get $M' \to^\ast M'' \rincl \widetilde{P'}$ for some reduct
  $P'$ of $P$, such that the reduction to $M''$ doesn't use
  \rrulet{subst-r}{get}. Thus, by \ref{lemma-preservation-values},
  $\text{NF}(M'') = \text{NF}(M')$. By induction on $M''$, $\forall T \in
  \text{NF}(M''), \exists Q, P \to^\ast Q \text{ and } T \rincl \widetilde{Q}$.
  But this is true for any reduct $M'$, and we have $\text{NF}(M) = \bigcup_{M \to
  M'} \text{NF}(M')$, hence this is true for $M$.
\end{proof}

From there, we get the result combining Theorem~\ref{theorem-adequacy-lthis} and
Theorem~\ref{theorem-nets-simulation-lthis}. One can extract from the proof of
Lemma~\ref{lemma-nets-termination-nfsep} that the translation of a summand that
is not a parallel of values either reduces to $\mathbf{0}$, or to a net which is not a
translation of a value.


==> paper-csl-long arxiv/parts/nets-routing.tex <==
% \newcommand{\conn}[1]{\textbf{co}({#1})}

\section{Routing Areas}
\label{section:areas}

Let us now define and study a special kind of nets: the
\emph{routing areas}. It is a generalization of the construction of
communication areas introduced in \cite{EHRHARD2010606}. The approach is
similar: we aim at constructing nets to be used as building blocks to implement
communication primitives. We shall see that this seemingly restricted class of nets is
actually the set of normal forms of a fragment of proof nets
(Theorem~\ref{theorem-mrarea-charact}). Routing areas are composed only of structural
rules: contraction, weakening, cocontraction and coweakening. These basic
components act as resource dispatchers (a resource designates a closed exponential box in
the following):

\begin{itemize}
  \item
    $\tikzvcenter{\begin{proofnet}\init[grow=left]{\wire{}}\end{proofnet}}$\\ A
    free wire acts as the identity. It passively forwards a resource
    that is connected on the \emph{input} (the left port) to the \emph{output}
    (the right port).
  \item 
    $\tikzvcenter{\begin{proofnet}
    \init[grow=right]{\binary{\wn}{\wire{}}{\wire{}}} \end{proofnet}}$ \\ A
    contraction is a broadcaster with one input and two outputs. A resource
    connected on the left will be copied to both outputs on the right. A
    weakening is a degenerate case of a broadcaster with zero outputs as
    broadcasting something to no one is the same as erasing it.
    % Stacking up contractions, a contraction tree with $n$ leafs is a
    % broadcaster that copies anything coming from its one input to all of the
    % $n$ outputs.
  \item 
    $\tikzvcenter{\begin{proofnet}
      \init[grow=left]{\binary{\oc}{\wire{}}{\wire{}}}
    \end{proofnet}}$ \\
    Dually, a cocontraction is a packer with two inputs and one output. A packer
    aggregates its two inputs non deterministically. When a dereliction is
    connected to the output to consume two packed resources, a non-deterministic
    sum of the two possible choices for the one to be provided is produced.
    Similarly, coweakening is seen as a degenerate packer with no inputs.
\end{itemize}

% A question which naturally arises is does this intuitive interpretation as a
% wiring between inputs and outputs scale to an arbitrary combination of these
% cells, that is a routing net ? Theorem~\ref{theorem-mrarea-charact} gives a
% positive answer, with reasonable requirements in the definition of a routing net
% (Definition~\ref{definition-mrarea-rnets}).
%
A routing area can be seen as a router, or a circuit, between inputs and
outputs.  Inputs are connected to contractions which broadcast resources they
receive to cocontractions. Cocontractions may gather resources from
multiple such sources.  The conclusion of these cocontractions form the outputs.
A routing area is then described by a slight generalization of a relation
between sets, a
\emph{multirelation}.  Its role is to define the \emph{wiring diagram} which
specifies which inputs and outputs are connected. Let us first introduce
multirelations:

% \newcommand{\labin}{\mathcal{L}_i}
% \newcommand{\labout}{\mathcal{L}_o}
% \newcommand{\cardn}[1]{| {#1} |}
% \newcommand{\routarea}[1]{\mathbf{#1}}

% Our device  then determined by the data of which input is connected to which output,
% with multiplicity, as an input could feed several copies to the same
% output. We encode this information through a relation with multiplicity, that we
% call a \emph{multirelation} :

\begin{description}
  \item[Multirelation] Let $A$ and $B$ be two sets, a \emph{multirelation} $R$
    between $A$ and $B$ is a multiset of elements of $A \times B$, or concretely
    a map $R : A \times B \to \mathbb{N}$.  For $k \in \mathbb{N}$, we write $x
    \mathrel{R_k} y$ if $R(x,y) = k$.
  \item[Relations and multirelations] 
    A relation $R$ between $A$ and $B$ can be seen as a multirelation by taking
    its characteristic function $\mathbbm{1}_{R}$.Conversely, we can forget the
    multiplicity of a multirelation $S$ and recover a relation by taking the
    subset of $A \times B$ defined by $\{ (x,y) \in A \times B \mid S(x,y) \geq
    1 \}$.
  \item[Composition]
    Multirelations enjoy a composition operation that computes all the ways
    to go from an element to another with multiplicities. For multirelations $R,S$
    respectively between $A$ and $B$, and $B$ and $C$,
    \[
      (S \circ R)(x,z) = \sum_{y \in B} R(x,y)S(y,z)
    \]
    This composition is associative, coincides with the usual one for relations,
    and has the identity relation (seen as a multirelation) for neutral. This is
    in fact the matrix multiplication, seeing a multirelation between $A$ and
    $B$ as a $\cardn{B} \times \cardn{A}$ matrix with integer coefficients
    $R(i,j)$ (identifying finite sets with their cardinal).
  \item[The \textbf{FMRel} Category] Finite sets and multirelations between them
    form a category \cat{FMRel}, with the category \cat{FRel} of finite sets and
    relations as a subcategory.  \cat{FMRel} has finite coproducts, extending
    the one of \cat{FRel}, and corresponding to the direct sum of matrices.
\end{description}

% We pictured here the two multirelations $R$ between $\{1,2,3\}$ and $\{1,2\}$, $S$
% between $\{1,2\}$ and $\{1,2,3\}$. We represents them as weighted graphs, with
% the domain on the left the codomain on the right. We connect a vertice $x$ of
% the domain to a vertice $y$ of the codomain with an edge weighted by $k =
% R(x,y)$ when $k > 0$.
%
% [SCHEMA]
%
% The composition is obtained by gluing the codomain of $R$ with the domain of
% $S$, and computing the sum $s = \sum_{p \in \text{Path}(x,y)} w(p)$ of the weights of paths between a vertice $x$ in the
% domain of $R$ and $y$ in the codomain of $S$ where the weight of a path is
% defined to be the product of the weights of the edges composing it.
% We add an edge between $x$ and $y$ weighted by $s$ if $s > 0$.

% \begin{proof}\ref{property-mrarea-coprod}\\
%   From $R : A \to C$ and $S : B \to C$, we can
%   form a multirelation $T : A + B \to C$
%   \[
%     T(x,c) =
%     \begin{cases}
%       R(a,c) & \text{ if } x = \textbf{inl}(a) \\
%       S(b,c) & \text{ if } x = \textbf{inr}(b)
%     \end{cases}
%   \]
%   One can easily check that this forms a coproduct in \cat{FMRel}, noted $T = R + S$.
% \end{proof}
%

A routing area is described by a multirelation between its inputs and its
outputs. Its value at the pair $(i,o)$ indicates how many times the input $i$ is
connected to the output $o$.  We are now ready to construct the \emph{routing
area} defined by a multirelation.


\begin{definition}{Routing area}\label{definition-routingarea}\\
  Let $\labin, \labout$ be two finite sets called the input labels and the
  output labels, and a multirelation $R$ between $\labin$ and $\labout$. A  
  routing area $\routarea R$ associated to the triplet $(\labin,\labout,R)$
  is a net constructed as follows:
  \begin{itemize}
    \item It has $\cardn{\labin} + \cardn{\labout}$ free wires partitioned into
      $\cardn{\labin}$ \emph{inputs} and $\cardn{\labout}$ \emph{outputs}. Each input is
      labelled by a distinct element of $\labin$, while outputs are labelled by
      distinct elements of $\labout$.
  % \begin{center}
  %   \tikzvcenter{
  %     \begin{proofnet}
  %       \node[net={40pt}{40pt}] (box) {\routarea R};
  %       \coordinate (i1) at ([yshift=-10pt]box.west);
  %       \coordinate (im) at ([yshift=10pt]box.west);
  %       \coordinate (o1) at ([yshift=-10pt]box.east);
  %       \coordinate (on) at ([yshift=10pt]box.east);
  %       \init{ 
  %         \wirefromto{[xshift=-10pt]i1}{[xshift=-10pt]i1}{i1}{i1}
  %         \wirefromto{[xshift=-10pt]im}{[xshift=-10pt]im}{im}{im}
  %         \wirefromto{[xshift=10pt]o1}{[xshift=10pt]o1}{o1}{o1}
  %         \wirefromto{[xshift=10pt]on}{[xshift=10pt]on}{on}{on}
  %       }
  %       \pdots[2pt]([xshift=-5pt]i1)([xshift=-5pt]im)
  %       \pdots[2pt]([xshift=5pt]o1)([xshift=5pt]on)
  %     \end{proofnet}
  %   }
  % \end{center}
    \item Each input (resp. output) is connected to the main port of a
      contraction (resp. cocontraction) tree. Then, for every $(i,o) \in \labin
      \times \labout$, we connect the tree of the input $i$ to the tree of
      output $o$ with exactly $R(i,o)$ wires.
  \end{itemize}
\end{definition}
\begin{center}
  \tikzvcenter{
    \begin{proofnet}
      % Tree of i1
      \init[grow=right]{
        \nary[name=i1]{\wn}{
          \wire{\point(i11)},
          \point(i12),
          \wire{\point(i13)}
        }
      }
      % Tree of im
      \init[grow=right]([yshift=7.5ex,xshift=-5pt]i1.pal){
        \nary[name=im]{\wn}{
          \wire{\point(im1)},
          \point(im2),
          \wire{\point(im3)}
        }
      }
      % Tree of o1
      \init[grow=left]([xshift=15ex]i1.pal){
        \nary[name=o1]{\oc}{
          \wire{\point(o11)},
          \point(o12),
          \wire{\point(o13)}
        }
      }
      % Tree of on
      \init[grow=left]([yshift=7.5ex,xshift=5pt]o1.pal){
        \nary[name=on]{\oc}{
          \wire{\point(on1)},
          \point(on2),
          \wire{\point(on3)}
        }
      }
      \pdots[2pt](i11)(i13)
      \pdots[2pt](im1)(im3)
      \pdots[5pt](i1.pal)(im.pal)
      \pdots[2pt](o11)(o13)
      \pdots[2pt](on1)(on3)
      \pdots[5pt](o1.pal)(on.pal)
    \end{proofnet}  
  }
\end{center}
We represent them as rectangular boxes, with the inputs appearing on the left and
outputs on the right.

%%%%%%%%%%%%%%%%%%%% --- EXTENDED --- %%%%%%%%%%%%%%%%%%%
\begin{definition}{Arity}\label{definition-routing-arity}\\
Let $(\labin, \labout, R)$ be a routing area. For an input $i \in \labin$, we
define its \emph{arity} as the number of leafs of the associated contraction
tree given by $\arity{i} = \sum_{o \in \labout} R(i,o)$. Similarly, the arity of
an output $o \in \labout$ is defined by $\arity{o} = \sum_{i \in \labin}
R(i,o)$. The set of outputs (resp. inputs) connected to an input $i$ (resp.
output $o$) is defined as $\conn{i} = \{ o \in \labout \mid R(i,o) \geq 1 \}$
(resp. $\conn{o} = \{ i \in \labin \mid R(i,o) \geq 1 \}$). In general, for an
input or an output $x$, $\arity{x} \leq \cardn{\conn{x}}$.  This is an equality
for all $x$ if and only if $R$ is a relation.
\end{definition}
%%%%%%%%%%%%%%%%%% --- END EXTENDED --- %%%%%%%%%%%%%%%%%

% Routing areas are defined up to relabelling : if $\routarea R$ is defined
% by $(\labin,\labout,R)$ then for any pair of permutation $\sigma : \labin' \to
% \labin$ and $\tau : \labout' \to \labout$, the conjugate relation
% $(\labin',\labout',\sigma R \tau^{-1})$ defines the same routing area,
% where $\sigma R \tau^{-1}$ is the composition of multirelations. Conversely, two
% descriptions $(\labin,\labout,R)$ and $(\labin',\labout',S)$ defining the same
% area must be conjugates: for each input wire, $\sigma$ sends the label
% attributed in $\labin'$ by the first one to the label attributed in $\labin$ by
% the second one. $\tau$ does the same for each output wire, and by definition of
% routing areas $\sigma S \tau^{-1}$ is totally determined and must be equal to
% $R$.

Routing areas may be combined in two ways such that the
resulting proof net reduces to a new routing area. The multirelation
describing the result can be computed directly from the initial multirelations of routing
areas involved, giving a way of building complex circuits from small components.

\paragraph*{Operations}

The first operation, juxtaposition, amounts to put side by side two routing areas.
The result is immediately seen as a routing area itself, described by the
coproduct of the two multirelations:

\begin{definition}{Juxtaposition}\label{definition-mrarea-juxt}\\
  Let $\routarea R = (\labin,\labout,R)$ and $\routarea S =
  (\labin',\labout',S)$, we define the juxtaposition $\routarea R + \routarea S$
  by $(\labin + \labin', \labout + \labout', R + S)$. The corresponding net is
  obtained by juxtaposing the nets of $\routarea R$ and $\routarea S$:

  \begin{center}
    \tikzvcenter{
      \begin{proofnet}
        \node[net={30pt}{30pt}] (R) {R};
        \coordinate (Ri1) at ([yshift=-10pt]R.west);
        \coordinate (Rim) at ([yshift=10pt]R.west);
        \coordinate (Ro1) at ([yshift=-10pt]R.east);
        \coordinate (Ron) at ([yshift=10pt]R.east);
        \init{
          \wirefromto{[xshift=-10pt]Ri1}{[xshift=-10pt]Ri1}{Ri1}{Ri1}
          \wirefromto{[xshift=-10pt]Rim}{[xshift=-10pt]Rim}{Rim}{Rim}
          \wirefromto{[xshift=10pt]Ro1}{[xshift=10pt]Ro1}{Ro1}{Ro1}
          \wirefromto{[xshift=10pt]Ron}{[xshift=10pt]Ron}{Ron}{Ron}
        }
        \pdots[2pt]([xshift=-5pt]Ri1)([xshift=-5pt]Rim)
        \pdots[2pt]([xshift=5pt]Ro1)([xshift=5pt]Ron)
        %
        \node[net={30pt}{30pt},below=10pt of R] (S) {S};
        \coordinate (Si1) at ([yshift=-10pt]S.west);
        \coordinate (Sim) at ([yshift=10pt]S.west);
        \coordinate (So1) at ([yshift=-10pt]S.east);
        \coordinate (Son) at ([yshift=10pt]S.east);
        \init{
          \wirefromto{[xshift=-10pt]Si1}{[xshift=-10pt]Si1}{Si1}{Si1}
          \wirefromto{[xshift=-10pt]Sim}{[xshift=-10pt]Sim}{Sim}{Sim}
          \wirefromto{[xshift=10pt]So1}{[xshift=10pt]So1}{So1}{So1}
          \wirefromto{[xshift=10pt]Son}{[xshift=10pt]Son}{Son}{Son}
        }
        \pdots[2pt]([xshift=-5pt]Si1)([xshift=-5pt]Sim)
        \pdots[2pt]([xshift=5pt]So1)([xshift=5pt]Son)
        %
      \end{proofnet}
      $=$
      \begin{proofnet}
        \node[net={30pt}{70pt}] (box) {\routarea{R} + \routarea{S}};
        \coordinate (i1) at ([yshift=-20pt]box.west);
        \coordinate (im) at ([yshift=20pt]box.west);
        \coordinate (o1) at ([yshift=-20pt]box.east);
        \coordinate (on) at ([yshift=20pt]box.east);
        \init{
          \wirefromto{[xshift=-10pt]i1}{[xshift=-10pt]i1}{i1}{i1}
          \wirefromto{[xshift=-10pt]im}{[xshift=-10pt]im}{im}{im}
          \wirefromto{[xshift=10pt]o1}{[xshift=10pt]o1}{o1}{o1}
          \wirefromto{[xshift=10pt]on}{[xshift=10pt]on}{on}{on}
        }
        \pdots[2pt]([xshift=-5pt]i1)([xshift=-5pt]im)
        \pdots[2pt]([xshift=5pt]o1)([xshift=5pt]on)
      \end{proofnet}
    }
  \end{center}
\end{definition}

% \begin{lemma}{Juxtaposition}\label{lemma-mrarea-juxt}\\
%   Let $\mathbf{R} = (\labin,\labout,R)$ and $\mathbf{S} = (\labin',\labout',S)$
%   be two routing area. Then their juxtaposition is also a routing area
%   $\routarea{R} + \routarea{S}$ defined by $(\labin + \labin',\labout +
%   \labout',R + S)$
%   
%   \end{lemma}

The second one is more involved: the trace operation consists in connecting
an input to an output given that they are not related to begin with, to avoid
the creation of a cycle. Doing so, we remove this output and input from the
external interface, and create new internal paths between remaining inputs and
outputs. If we reduce the resulting net to a normal form, we obtain a new area,
whose multirelation can be computed from the initial one. 

\begin{definition}{Trace}\label{definition-mrarea-trace}\\
  Let $\mathbf{R} = (\labin,\labout,R)$ be a routing area, and $(i,o) \in \labin
  \times \labout$. The \emph{trace} at $(i,o)$ of $\routarea
  R$ is obtained by connecting the input $i$ with the output $o$ of $\routarea
  R$ and reducing this net to its normal form.
\end{definition}

\begin{property}{Trace is a routing area}\label{property-mrarea-trace}\\
  Let $\mathbf{R} = (\labin,\labout,R)$ be a routing area, and $(i,o) \in \labin
  \times \labout$ such that $i \mathrel{R_0} o$. Then the trace at $(i,o)$ of
  $\routarea R$ is a routing area $\routarea T$ :
  \begin{center}
    \tikzvcenter{
      \begin{proofnet}
        \node[net={30pt}{30pt}] (R) {R};
        \coordinate (Ri1) at ([yshift=-10pt]R.west);
        \coordinate (Rim) at ([yshift=10pt]R.west);
        \coordinate (Ro1) at ([yshift=-10pt]R.east);
        \coordinate (Ron) at ([yshift=10pt]R.east);
        \init{
          \wirefromto{[xshift=-10pt]Ri1}{[xshift=-10pt]Ri1}{Ri1}{Ri1}
          \wirefromto{[xshift=-10pt]Rim}{[xshift=-10pt]Rim}{Rim}{Rim}
          \wirefromto{[xshift=10pt]Ro1}{[xshift=10pt]Ro1}{Ro1}{Ro1}
          \wirefromto{[xshift=10pt]Ron}{[xshift=10pt]Ron}{Ron}{Ron}
        }
        \pdots[2pt]([xshift=-5pt]Ri1)([xshift=-5pt]Rim)
        \pdots[2pt]([xshift=5pt]Ro1)([xshift=5pt]Ron)
        \draw[rounded corners=3pt]
          ([xshift=-10pt]Ri1) -- ++(0,-10pt) -| ([xshift=10pt]Ro1);
      \end{proofnet}
      $\to^\ast$
      \begin{proofnet}
        \node[net={30pt}{30pt}] (box) {T};
        \coordinate (i1) at ([yshift=-10pt]box.west);
        \coordinate (im) at ([yshift=10pt]box.west);
        \coordinate (o1) at ([yshift=-10pt]box.east);
        \coordinate (on) at ([yshift=10pt]box.east);
        \init{
          \wirefromto{[xshift=-10pt]i1}{[xshift=-10pt]i1}{i1}{i1}
          \wirefromto{[xshift=-10pt]im}{[xshift=-10pt]im}{im}{im}
          \wirefromto{[xshift=10pt]o1}{[xshift=10pt]o1}{o1}{o1}
          \wirefromto{[xshift=10pt]on}{[xshift=10pt]on}{on}{on}
        }
        \pdots[2pt]([xshift=-5pt]i1)([xshift=-5pt]im)
        \pdots[2pt]([xshift=5pt]o1)([xshift=5pt]on)
      \end{proofnet}
    }
  \end{center}
  Where $\routarea T = (\labin - \{i\},\labout - \{o\},T)$ is defined by the
  multirelation :
  \begin{equation}\label{routing-eq-trace}
    T(x,y) = R(x,y) + R(x,o)R(i,y)
  \end{equation}
\end{property}

The formula~\ref{routing-eq-trace} expresses that in the resulting routing area
$\routarea T$, the total number of ways to go from an input $x$ to an output $y$
is the number of direct paths $R(x,y)$ from $x$ to $y$ that were originally in $R$, plus
all the ways of going from $x$ to $o$ times the ways of going from $i$ to $y$.
Indeed, any pair of such paths yields a new distinct path in the trace once
$i$ and $o$ have been connected.



% \begin{proof}\ref{property-mrarea-trace}
%
%   If $\arity{i} = \arity{o} = 0$, then we connected a coweakening to a weakening
%   and we can erase them to recover the desired area where $T$ is just the
%   restriction of $R$ to $(\labin - \{i\}) \times (\labout - \{o\})$, which
%   agrees with the formula of \ref{property-mrarea-trace} as the product
%   $R(x,o)R(i,y)$ is always zero.
%
%   Now, assume that $\arity{o} = 0 < \arity{i}$. We can reduce the introduced
%   redex as follow :
% \begin{center}
%   \tikzvcenter{
%     \begin{proofnet}
%       % Tree of i1
%       \init[grow=left]{
%         \zeroary[normal,name=i1]{\oc}
%       }
%       % Tree of im
%       \init[grow=right]{
%         \nary[name=im]{\wn}{
%           \wire{\point(im1)},
%           \point(im2),
%           \wire{\point(im3)}
%         }
%       }
%       \pdots[2pt](i11)(i13)
%       \pdots[2pt](im1)(im3)
%       % \pdots[5pt](i1.pal)(im.pal)
%       % \pdots[2pt](o11)(o13)
%       % \pdots[2pt](on1)(on3)
%       % \pdots[5pt](o1.pal)(on.pal)
%     \end{proofnet}  
%     $\to^\ast$
%     \begin{proofnet}
%       % Tree of o1
%       \init[grow=left]{
%         \zeroary[normal,name=o1]{\oc}
%       }
%       % Tree of on
%       \init[grow=left]([yshift=7.5ex,xshift=5pt]o1.pal){
%         \zeroary[normal,name=on]{\oc}
%       }
%       \pdots[5pt](o1.pal)(on.pal)
%     \end{proofnet} 
%   }
% \end{center}
%
%
% These coweakening are connected to the trees of the outputs $\conn{i}$.
% These are either connected to a wire, or a
% cocontraction tree and we can eliminate superfluous coweakening using the equivalence
% relation. Once again, we didn't create new paths and recover an area whose
% relation is the restriction of $R$, still agreeing with the formula as
% $\arity{i} = 0$ implies $R(x,o)R(i,y)$ being zero again. The dual case $\arity{i} = 0 <
% \arity{o}$ is treated the same.
%  
% The general case relies on the commutation of contractions and cocontractions
% trees that can be derived by iterating the corresponding reduction rule. We can apply the
% following reduction on the trees of $i$ and $o$ that have been connected :
%
% \begin{center}
%   \includegraphics{figures/routing-areas/pdfs/area-trace-bigstepred.pdf}
% \end{center}
%
% where wires $i_1,\ldots,i_p$ are connected to the trees of the inputs in
% $\conn{o}$ and $o_1,\ldots,o_q$ to the trees of the outputs of $\conn{i}$. The
% reduced net now have the form of a routing area. As before, the direct
% paths between $x$ and $y$ when $x \neq i$ and $y \neq o$ are left unchanged. But
% any couple of paths in $R$ between $x$ and $o$ arriving at some $i_k$ and
% between $i$ and $y$ arriving at $o_l$ yields exactly one new path between $x$
% and $y$ in the new area (see \ref{property-mrarea-path-preservation} below). By
% definition, there are $R(x,o)$ paths connecting $x$ to $o$ and $R(i,y)$
% connecting $i$ to $y$ : hence there are $R(x,o)R(i,y)$ such couples.
% \end{proof}
%


%%%%%%%%%%%%%%%%%%%% --- EXTENDED --- %%%%%%%%%%%%%%%%%%%
\begin{proof}Property~\ref{property-mrarea-trace}\\
  If $\arity{i} = \arity{o} = 0$, then we connected a coweakening to a weakening
  and we can erase them to recover the desired area where $T$ is just the
  restriction of $R$ to $(\labin - \{i\}) \times (\labout - \{o\})$, which
  agrees with the formula of \ref{property-mrarea-trace} as the product
  $R(x,o)R(i,y)$ is always zero.

  Now, assume that $\arity{o} = 0 < \arity{i}$. We can reduce the introduced
  redex as follow :
\begin{center}
  \tikzvcenter{
    \begin{proofnet}
      % Tree of i1
      \init[grow=left]{
        \zeroary[normal,name=i1]{\oc}
      }
      % Tree of im
      \init[grow=right]{
        \nary[name=im]{\wn}{
          \wire{\point(im1)},
          \point(im2),
          \wire{\point(im3)}
        }
      }
      \pdots[2pt](i11)(i13)
      \pdots[2pt](im1)(im3)
      % \pdots[5pt](i1.pal)(im.pal)
      % \pdots[2pt](o11)(o13)
      % \pdots[2pt](on1)(on3)
      % \pdots[5pt](o1.pal)(on.pal)
    \end{proofnet}  
    $\to^\ast$
    \begin{proofnet}
      % Tree of o1
      \init[grow=left]{
        \zeroary[normal,name=o1]{\oc}
      }
      % Tree of on
      \init[grow=left]([yshift=7.5ex,xshift=5pt]o1.pal){
        \zeroary[normal,name=on]{\oc}
      }
      \pdots[5pt](o1.pal)(on.pal)
    \end{proofnet} 
  }
\end{center}

These coweakening are connected to the trees of the outputs $\conn{i}$.
These are either connected to a wire, or a
cocontraction tree and we can eliminate superfluous coweakening using the equivalence
relation. Once again, we didn't create new paths and recover an area whose
relation is the restriction of $R$, still agreeing with the formula as
$\arity{i} = 0$ implies $R(x,o)R(i,y)$ being zero again. The dual case $\arity{i} = 0 <
\arity{o}$ is treated the same way.
 
The general case relies on the commutation of contractions and cocontractions
trees that can be derived by iterating the $\red{ba}$ rule. We can apply the
following reduction on the trees of $i$ and $o$ that have been connected :

\begin{center}
  \includegraphics{figures/routing-areas/pdfs/area-trace-bigstepred.pdf}
\end{center}

where wires $i_1,\ldots,i_p$ are connected to the trees of the inputs in
$\conn{o}$ and $o_1,\ldots,o_q$ to the trees of the outputs of $\conn{i}$. The
reduced net now has the shape of a routing area. As before, the direct
paths between $x$ and $y$ when $x \neq i$ and $y \neq o$ are left unchanged. But
any couple of paths in $R$ between $x$ and $o$ arriving at some $i_k$ and
between $i$ and $y$ arriving at some $o_l$ yields exactly one new path between $x$
and $y$ in the new area (see \ref{property-mrarea-path-preservation} below). By
definition, there are $R(x,o)$ paths connecting $x$ to $o$ and $R(i,y)$
connecting $i$ to $y$ : hence there are $R(x,o)R(i,y)$ such couples.
\end{proof}
%%%%%%%%%%%%%%%%%% --- END EXTENDED --- %%%%%%%%%%%%%%%%%

These two operations are sufficient to implement composition which is the
connection of an output of an area to an input of another area. Composition is a
fundamental feature of routing areas. This is what makes them modular, allowing
to build routing areas by composing simple blocks. To connect an output $o$ of
$\routarea R$ to an input $i$ of $\routarea S$, we first perform the
juxtaposition followed by a trace at $(i,o)$.  This is similar both in form and
in spirit, to the composition of Game Semantic or Geometry of Interaction whose
motto is ``composition = parallel composition plus hiding''. 

\begin{corollary}{Composition}\label{corollary-mrarea-composition}\\
  Let $\routarea{R} = (\labin,\labout,R)$ and $\routarea{S} = (\labin',\labout',S)$ be
  two routing areas, $o \in \labout$ and $i \in \labin'$. Then the net resulting
  from connecting the output $o$ to the input $i$ can be reduced to a new
  routing area $\routarea{T} = (\labin + \labin' - \{i\}, \labout + \labout' -
  \{o\}, T)$
  
  \begin{center}
    \tikzvcenter{
      \begin{proofnet}
        \node[net={30pt}{30pt}] (R) {R};
        \coordinate (Ri1) at ([yshift=-10pt]R.west);
        \coordinate (Rim) at ([yshift=10pt]R.west);
        \coordinate (Ro1) at ([yshift=-10pt]R.east);
        \coordinate (Rok) at (R.east);
        \coordinate (Ron) at ([yshift=10pt]R.east);
        \init{
          \wirefromto{[xshift=-10pt]Ri1}{[xshift=-10pt]Ri1}{Ri1}{Ri1}
          \wirefromto{[xshift=-10pt]Rim}{[xshift=-10pt]Rim}{Rim}{Rim}
          \wirefromto{[xshift=10pt]Ro1}{[xshift=10pt]Ro1}{Ro1}{Ro1}
          \wirefromto{[xshift=10pt]Ron}{[xshift=10pt]Ron}{Ron}{Ron}
        }
        \pdots[2pt]([xshift=-5pt]Ri1)([xshift=-5pt]Rim)
        \pdots[2pt]([xshift=5pt]Ro1)([xshift=5pt]Rok)
        \pdots[2pt]([xshift=5pt]Rok)([xshift=5pt]Ron)
        %
        \node[net={30pt}{30pt},right=10ex of R] (S) {S};
        \coordinate (Si1) at ([yshift=-10pt]S.west);
        \coordinate (Sil) at (S.west);
        \coordinate (Sim) at ([yshift=10pt]S.west);
        \coordinate (So1) at ([yshift=-10pt]S.east);
        \coordinate (Son) at ([yshift=10pt]S.east);
        \init{
          \wirefromto{[xshift=-10pt]Si1}{[xshift=-10pt]Si1}{Si1}{Si1}
          \wirefromto{[xshift=-10pt]Sim}{[xshift=-10pt]Sim}{Sim}{Sim}
          \wirefromto{[xshift=10pt]So1}{[xshift=10pt]So1}{So1}{So1}
          \wirefromto{[xshift=10pt]Son}{[xshift=10pt]Son}{Son}{Son}
          \wirefromto{Rok}{Rok}{Sil}{Sil}
        }
        \pdots[2pt]([xshift=-5pt]Si1)([xshift=-5pt]Sil)
        \pdots[2pt]([xshift=-5pt]Sil)([xshift=-5pt]Sim)
        \pdots[2pt]([xshift=5pt]So1)([xshift=5pt]Son)
        %
      \end{proofnet}
      $\to^\ast$
      \begin{proofnet}
        \node[net={30pt}{30pt}] (box) {T};
        \coordinate (i1) at ([yshift=-10pt]box.west);
        \coordinate (im) at ([yshift=10pt]box.west);
        \coordinate (o1) at ([yshift=-10pt]box.east);
        \coordinate (on) at ([yshift=10pt]box.east);
        \init{
          \wirefromto{[xshift=-10pt]i1}{[xshift=-10pt]i1}{i1}{i1}
          \wirefromto{[xshift=-10pt]im}{[xshift=-10pt]im}{im}{im}
          \wirefromto{[xshift=10pt]o1}{[xshift=10pt]o1}{o1}{o1}
          \wirefromto{[xshift=10pt]on}{[xshift=10pt]on}{on}{on}
        }
        \pdots[2pt]([xshift=-5pt]i1)([xshift=-5pt]im)
        \pdots[2pt]([xshift=5pt]o1)([xshift=5pt]on)
      \end{proofnet}
    }
  \end{center}
\end{corollary}

\begin{remark}
This operation can be generalized to the connection of $n$ outputs of $R$ to
$n$ inputs of $S$. When $n = \cardn{\labout} = \cardn{\labin'}$, the 
multirelation $T$ describing the resulting routing area is the
composed $S \circ R$.
\end{remark}

The following property gives the high level operational behavior of a routing
area. It supports our interpretation of routing areas as dispatchers of
exponential boxes. Given a closed exponential box, we connect it to the
auxiliary port of a cocontraction to obtain a module which can then be connected
to an input $i$ of an area.  Through reduction, the box will traverse the area
and be duplicated $R(i,o)$ times to each output $o$. The role of the additional
cocontraction is to preserve the area and allow future connections to the same
input. We would get a similar transit property connecting directly the
exponential box to $i$, but the process is destructive as it erases
the input wire of $i$ and prevents any future use.

\begin{property}{Transit}\label{property-translation-transit}\\
  Let $\sigma$ be a closed exponential box, $\mathbf{R} = (\labin,\labout,R)$ a
  routing area, $i \in \labin$. Let $\{ o_1, \ldots, o_p \} = \conn{i}$ and for $1 \leq k \leq p,\ c_k = R(i,o_k)$. Then :
  \begin{center}
    \includegraphics{figures/routing-areas/pdfs/area-transit.pdf} 
  \end{center}
\end{property}

The property is straightforward application of reduction rules and the net
equivalence.

\subsection{The Routing Semantic}

Routing areas do not only fulfill practical needs. They are general enough to be
the language of normal forms of \emph{routing nets}. Let us first give a precise
definition. A correct net is a net satisfying the correctness criterion defined
in~\cite{ehrhard:hal-00150274}:

\begin{definition}{Routing nets}\label{definition-mrarea-rnets}\\
  A routing net $\net R$ is a correct net composed only of weakenings,
  coweakenings, contractions, cocontractions, and possibly floating wires.
  Moreover, we ask that all wires are labelled with the same formula $\oc A$,
  fixing de facto their orientation.
\end{definition}

%%%%%%%%%%%%%%%%%%%% --- EXTENDED --- %%%%%%%%%%%%%%%%%%%
Paths will also be of interest in the rest of this subsection. 

\begin{definition}{Paths}\label{definition-mrarea-paths}\\
  Let $\net R$ be a net. We recall that for a cell $c$ of $\net R$, we write
  $p_i(c)$ for its $i$-th auxiliary port (if it exists) and $p(c)$ for its main
  port. For a wire $w$, $s(w)$ designates the source port of $w$ while $e(w)$
  is its end port.
  Let $\net R$ be a net without exponential boxes, we construct the associated
  undirected graph $G(\net R)$ with ports as vertices and: 
  \begin{description}
    \item[Wire edges] For any wire $w$ of $\net R$, we add an edge between $s(w)$
      and $e(w)$.
    \item[Cell edges] For every auxiliary port $p_i(c)$ of a cell, we add an edge between $p_i(c)$ and $p(c)$.
  \end{description}
  A path $p$ in $\net R$ is a finite sequence
  $(p_1,e_1,p_2,e_2,\ldots,e_n,p_{n+1})$ such that $p_i$ is a port of $\net R$,
  $e_i$ an edge of $G(R)$ linking $p_i$ and $p_{i+1}$ and such that $e_i$ and
  $e_{i+1}$ are of distinct nature (cell/wire edge). We extend $s$ and $e$ to operate on path, defined by
  $s(p) = p_1$ and $e(p) = p_{n+1}$. Paths whose starting and ending edges are wire edges
  can also be described as a sequence of corresponding wires $(w_1,\ldots,w_m)$
  as internal ports and cell edges can be recovered.  We note $P(\net R)$ the
  set of paths in $\net R$ and $P_f(\net R)$ the paths starting and ending on
  free ports. 
\end{definition}

Albeit closed to \emph{switching paths} (the ones involved in the correctness
criterion), they do not match exactly. A path in a switching graph can arrive at
an auxiliary port of a cocontraction and bounce back in the other, while the
paths we have defined here must continue via the principal port. However, a
correct (routing) net do not contain cyclic paths, which means that switching acyclicity
implies acyclicity:

\begin{property}{Acyclicity of correct nets}\label{property-mrarea-path-switching}\\
  A routing net is acyclic, that is there is no path $p$ such that $s(p) = t(p)$.
\end{property}

\begin{proof}\ref{property-mrarea-path-switching}\\
  We prove that the existence of a cycle implies the existence of a cycle in a
  switching graph. Assume that a cycle exist and take a one of minimal
  length.  Assume that the two auxiliary ports of a cell (contraction or
  cocontraction) are both visited by the cycle. By the definition of paths, when
  the cycle visits one of these auxiliary port, it must continue in the
  principal port.  But then a smaller cycle would be derivable, by taking the
  sub path starting at the principal port of this cell and stopping as long as
  it comes back by any of the auxiliary ports. Thus a minimal cycle visits at most
  once of the auxiliary port of any cell, and is also a cycle in a switching
  graph.  
  %
\end{proof}

We now state a fundamental property relating reduction to paths:

\begin{property}{Path preservation}\label{property-mrarea-path-preservation}\\
  Let $\net R$ be a routing net, $p_1$ and $p_2$ be free ports. We write
  $P_f(\net R,p_1,p_2) = \{
  p \in P_f(\net R) \mid s(p) = p_1, e(p) = p_2 \}$. If $\net R \to
  \net{R}'$, then $P_f(\net R,p_1,p_2) = P_f(\net{R}',p_1,p_2)$. In particular,
  $P_f(\net R) = \sum P_f(\net R,p_i,p_{i'}) = P_f(\net{R}')$.
\end{property}

\begin{proof}\ref{property-mrarea-path-preservation}
  The proof is simple in the case of routing nets. As a path in $P_f(R,p_1,p_2)$
  must begin and end in a free port, it can't go through a weakening or a
  coweakening, and the corresponding reductions leave such paths unchanged. The
  only relevant reduction is the $\red{ba}$ rule:
  \begin{center}
    \includegraphics{figures/routing-areas/pdfs/area-path-preservation.pdf}
  \end{center}
  Let us define the application $\tau : P_f(R,p_1,p_2) \to P_f(R',p_2,p_2)$. For
  a path $p$ which does not cross the redex, $\tau(p) = p$. Otherwise, we
  replace any subsequence in the left column by the one in the right column:
  \begin{center}
    \begin{tabular}{c|c}
      Subsequence & Image by $\tau$ \\
      \hline
      $i_1,c,o_1$ & $i_1,c_1,o_1$ \\
      $i_1,c,o_2$ & $i_1,c_2,o_2$ \\
      $i_2,c,o_1$ & $i_2,c_3,o_1$ \\
      $i_2,c,o_2$ & $i_2,c_4,o_2$ \\
    \end{tabular}
  \end{center}
  We omitted the four other possibilities which can be deduced from this table
  by reversing both the subsequence and its image. It is easily seen that $\tau$
  is an bijection.
\end{proof}
%%%%%%%%%%%%%%%%%% --- END EXTENDED --- %%%%%%%%%%%%%%%%%

The following theorem establishes the link between routing
areas and normal forms of routing nets. We propose two different intuitive
explanations of why the theorem holds:

\begin{enumerate}
  \item The basic components of routing nets, (co)contractions, wires
    and (co)weakenings, are routing areas. Then, juxtaposition and trace
    operations are general enough to combine them into an arbitrary routing net that
    reduces to a routing area according to Property~\ref{property-mrarea-trace}.
  \item In a routing net, the $\red{ba}$ rule allows to commute all contractions
    and cocontractions. Then, by equivalence, we can erase weakenings and
    coweakenings that are not connected to a free wire. At the end of this
    process, the resulting net must have the shape of a routing area.
\end{enumerate}

\begin{theorem}{Routing area characterization}\label{theorem-mrarea-charact}\\
 The normal form of a routing net $\net S$ is a routing area $\routarea R =
 (\labin,\labout,R)$.
\end{theorem}

For a routing net $\net S$, we can define the application $\sem{.} : \net S
\mapsto R$ that maps $S$ to the multirelation $R$ describing its normal form. By
unicity of normal forms, this application is invariant by reduction and is thus a
semantic for routing nets. It has the following properties:
\begin{description}
  \item[Soundness] The multirelation only depends on the normal form.
  \item[Adequacy] Two routing nets with the same denotation have the same normal
    form because a multirelation defines a routing area uniquely.
  \item[Full completeness] Any multirelation between finite sets is realized by the 
    associated routing area.
  \item[Compositionnality] We can compute the semantic of a net in a
    compositional way from the semantic of its smaller parts through
    juxtaposition and trace.
\end{description}

%%%%%%%%%%%%%%%%%%%% --- EXTENDED --- %%%%%%%%%%%%%%%%%%%
\begin{proof}Theorem~\ref{theorem-mrarea-charact}\\
 We prove the result by induction on the number $n$ of cells of $\net R$.
 \begin{itemize}
   \item ($n=0$) $\net R$ is only composed of free wires. We take $\labin = \{
     s(w) \mid w \mbox{ wire }\}$, $\labout = \{ e(w) \mid w \mbox{ wire } \}$
     and $R$ is the relation defined by $i \mathrel R o \iff \exists w,\ i =
     s(w), o = e(w)$.
   \item (induction step) Let take any node $N$ of $\net R$. We call
     $\net{R}'$ the subnet obtained by removing $N$ and replacing its ports by
     free ports.

    \begin{center}
      \includegraphics{figures/routing-areas/pdfs/area-rnet-decomposition.pdf}
    \end{center}

    By induction, $\net{R}'$ can be reduced to a routing area
    $\routarea{R}'$.

     \begin{description}
       \item[(co)weakening] If $N$ is a weakening or coweakening, it is a
         routing area and can be composed with $\routarea{R}'$, and reduced to a
         new routing area $\routarea{R}$ according to
         \ref{corollary-mrarea-composition}. Thus we can
         reduce the whole net to $\routarea{R}$. 
       \item[(co)contraction] If $N$ is a contraction or a cocontraction, it can
         still be seen as a routing area and we juxtapose it to $\routarea{R}'$.
         What remains to do is to perform three traces operations to recover the
         original net and reduce the whole net to a routing area
         $\routarea{R}$. However, we must ensure that the input and the output
         we connect at each step are not already connected in the routing
         area. The first operation is always legal, as it is actually a merge
         operation of previously disjoint areas. The following traces are also
         valid, as reduction does not create cycles, as implied by
         \ref{property-mrarea-path-preservation}. 
     \end{description}
 \end{itemize}
\end{proof}
%%%%%%%%%%%%%%%%%% --- END EXTENDED --- %%%%%%%%%%%%%%%%%

For a routing net $\net S$, we can define the application $\sem{.} : \net S
\mapsto R$ that maps $S$ to the multirelation $R$ describing its normal form. By
unicity of normal forms, the application is invariant by reduction and is thus a
semantic for our routing nets, with the following remarkable properties:
\begin{description}
  \item[Sound] The multirelation only depends on the normal form, this is invariant by reduction.
  \item[Adequate] Two routing nets with the same denotation have the same normal
    form, as a multirelation define a routing area uniquely.
  \item[Fully complete] Any multirelation on finite sets is realised by the 
    associated routing area.
  \item[Compositionnal] We can compute the semantic of a net in a
    compositional way from the semantic of its smaller parts, through
    juxtaposition and trace.
\end{description}

%%%%%%%%%%%%%%%%%%%% --- EXTENDED --- %%%%%%%%%%%%%%%%%%%
This semantic can be defined without resorting reduction, by
counting paths.

\begin{theorem}{Path semantic}\label{theorem-mrarea-pathsemantic}\\
  Let $\net S$ be a routing net. Let $\labin$ be the set of free ports of
  $\net S$ which are the source point of a wire, and $\labout$ the ones
  that are the end point. Then $\sem{\net S}$
  is the multirelation between $\labin$ and $\labout$ given by
  \[
    \sem{\net S}(i,o) = \cardn{ P_f(\net S,i,o) }
  \]
\end{theorem}

\begin{proof}\ref{theorem-mrarea-pathsemantic}
  \begin{itemize}
    \item For normal forms, this follows from the very definition of a
      routing area associated to the multirelation $\sem{\net S}$ :
      $\sem{\net S}(i,o)$ counts precisely the number of paths starting
      at port $i$ and ending at port $o$.
    \item Otherwise, by path preservation (\ref{property-mrarea-path-preservation}), this
      quantity is invariant by reduction. We conclude by induction on the length
      of the longest reduction of $\net S$ to its normal form.
  \end{itemize}
\end{proof}
%%%%%%%%%%%%%%%%%% --- END EXTENDED --- %%%%%%%%%%%%%%%%%

% : the multirelation $\sem{\net S}$ corresponds in fact to a count of 
% maximal paths starting and ending on free wires, allowing to compute it
% directly on a routing net. 
%
%
% \begin{proof}\ref{theorem-mrarea-pathsemantic}
%   \begin{itemize}
%     \item For normal forms, this follows from the very definition of a
%       routing area associated to the multirelation $\sem{\net S}$ :
%       $\sem{\net S}(i,o)$ counts precisely the number of paths starting
%       at port $i$ and ending at port $o$.
%     \item Otherwise, by path preservation (\ref{property-mrarea-path-preservation}), this
%       quantity is invariant by reduction. We conclude by induction on the length
%       of the longest reduction of $\net S$ to its normal form.
%   \end{itemize}
% \end{proof}

% \quad\quad
% \begin{proofnet}[baseline=-.5ex]
%   \init[grow=right]{
%     \binary[very very small,bottom=15pt]{\wn}{\wire{\point(a)}}{\wire{}}
%   }
%   \draw[railed] (7.5pt,12.5pt) coordinate (x)-- ++(0,-17.5pt) coordinate (y);
%   \draw[densely dotted] (y) -- ++(0,-7.5pt);
%   \draw (x)-- ([xshift=-7.5pt]x-|a) coordinate (y);
%   \draw[densely dotted] (y) -- (y-|a);
% \end{proofnet}
%   \equiv
% \begin{proofnet}[baseline=-.5ex]
%   \init[grow=right]{
%     \binary[very very small]{\wn}{\wire[bottom=15pt]{\point(a)}}{\wireupto(a){\wire[wire=fake]{\point(a)}}}
%   }
%   \draw[railed] (22.5pt,12.5pt) coordinate (x)-- ++(0,-17.5pt) coordinate (y);
%   \draw[densely dotted] (y) -- ++(0,-7.5pt);
%   \draw (x)-- ([xshift=-7.5pt]x-|a) coordinate (y);
%   \draw[densely dotted] (y) -- (y-|a);
% \end{proofnet}

\begin{remark}{Communication Areas}\label{mrem-mrarea-communication-areas}\\
The communication areas defined in~\cite{EHRHARD2010606} are a special case of
routing areas: for $n \leq 1$, the $n$-communication area is the routing area
$(\{1,\ldots,n\},\{1,\ldots,n\},R)$ where $x \mathrel{R} y \iff x \neq y$.
\end{remark}

\begin{remark}{Canonicity of multirelations}\\
  The multirelation defining an area is actually not unique from a set-theoretic
  point of view: indeed, for $\routarea R = (\labin,\labout,R)$, then all
  multirelations in $\{ \tau^{-1} \circ R \circ \sigma : E \to F \mid \sigma : E
    \to \labin, \tau : F \to \labout, \sigma \text{ and } \tau \text{ bijective
  } \}$ describe the same area. Even though this object is a proper class,
  all these relations are considered isomorphic (for example, in the arrow
  category of \cat{FMRel}). After all, even finite deterministic automata suffer
  this kind of subtlety, which is not relevant in practice.
\end{remark}

We are now armed to encode communication primitives.  This is illustrated in
Section~\ref{section:translation} by the translation of the {\lamadio} calculus,
succinctly described in the following section.


==> paper-csl-long arxiv/parts/nets-simulation.tex <==
\section{Simulation}

We are now equipped to state the simulation result. The one step simulation
result, which bears all the technical content, states that a one step reduction
in \lthis can be simulated by a many step reduction in nets, up to some
administrative reductions.

\begin{lemma}{One step simulation}\label{lemma-nets-simulation-onestep}\\
  Let $\vdash M : (\alpha,e)$ be closed well-typed term of \lthis
  . If $M \to N$, then $M^\bullet \to^\ast N^\bullet$.
\end{lemma}

\begin{theorem}{Simulation}\label{theorem-nets-simulation}\\
  Let $\vdash M : (\alpha,e)$ be a closed well-typed term of \lthis.
  If $M \to^\ast N$, then $M^\bullet \to^\ast N^\bullet$. 
\end{theorem}

\subsection{Nets context}

In order to prove simulation, it will be handy to manipulate the translation of
not only terms, but contexts. We add a typing rule for the hole

\begin{definition}{Hole typing rule}\label{definition-nets-simulation-typehole}\\
\[
  \infer[(hole)]
  {R,[.] : (\alpha,e) \vdash [.] : (\alpha,e)}
  {R \vdash (\alpha,e)}
\]
\end{definition}

\begin{center}
  \begin{tabular}{|c|c|}
    
  \end{tabular}
\end{center}

$[.]$ can be seen just as a special distinguished variable in the typing
derivation. From this, we use the usual rule to build derivations of typed
contexts. A context can then be translated to a net, with a special interface
determined by $\alpha$ and $e$, labelling free ports. This is what we call net
contexts. The substitution of nets consists in plugging the translation of term
of this type in this interface. 

\begin{definition}{Hole translation}\label{definition-nets-simulation-holetrans}\\
  We define the translation of a typed hole $R \vdash [.] : (\alpha,e)$
as 

\begin{center}
  \begin{tabular}{DD}
  \[
    \infer[(hole)]
    {R,[.] : (\alpha,e) \vdash [.] : (\alpha,e)}
    {R \vdash (\alpha,e)}
  \]
   & 
    \includegraphics{figures/translation/pdfs/translation-hole.pdf} \\
  \end{tabular}
\end{center}


We can then carry on and use the usual term translation to build the
translation of a context $(C[E])^\bullet$, which is a net of the form

\begin{center}
  \includegraphics{figures/translation/pdfs/translation-context.pdf}
\end{center}


The substitution of $M^\bullet$, or of any net with a compatible interface for
that matter, in $(C[E])^\bullet$ is defined by just connecting the free wires of
the substituted net to the corresponding free wire of the context hole :

\begin{center}
  \includegraphics{figures/translation/pdfs/translation-context-subst.pdf}
\end{center}

\end{definition}

The fundamental property of net contexts and net substitutions is that the substitution commutes to the translation, in the
following sense :

\begin{theorem}{Nets substitution}\label{theorem-nets-simulation-commutation}\\
  Let $ \vdash [.] : (\alpha,e)$ be a typed hole, $[.] : (\alpha,e) \vdash C[E]
  : (\beta,e')$ a typed context, and $ \vdash M : (\alpha,e)$ a term. Then :
\[
  (C[E[M]])^\bullet = (C[E])^\bullet[M^\bullet]
\]
\end{theorem}

The proof is an easy induction: the base case when $C[E] = [.]$ is immediate,
and by definition of the context translation, so is the inductive case.

The very definition of net reduction immediately entails that if $M^\bullet
\to^\ast N^\bullet$ then $(C[E])^\bullet[M^\bullet] \to^\ast
(C[E])^\bullet[N^\bullet]$. Together with
\ref{theorem-nets-simulation-commutation}, this ensures that we can focus on the case
where $C = E = [.]$, as the general case follows seamlessly.

% \subsection{Reference substitutions}
%
% We state and prove a few lemma about the reduction of the translation of reference
% substitutions.
%
% TODO
%
% \subsection{Variable substitutions reductions}
%
% Let us show the simulation for \rrulet{subst}{} rules, involving mainly
% duplication. Thanks to the previous theorem, we can assume that contexts are
% empty without loss of generality. We consider only closed terms. Indeed, since 
% reduction contexts $S,C,E$ do not bind variables, all the terms appearing in the
% premise of a rule ($V$,$M$,$\multv{V}$,\ldots) are thus closed terms, and we can
% omit their context. For each rule, we write the translation of the premise
% followed by its reduction in nets, that match the conclusion.
%
% The fundamental rule is the variable one.
%
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrulet{subst}{var} ($\sigma(x)$ undefined)
%     & \includegraphics{figures/simulation/pdfs/subst-var-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-var-reduct.pdf} \\
%
%     \rrulet{subst}{var} ($\sigma(x)$ defined)
%     & \includegraphics{figures/simulation/pdfs/subst-var-2-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-var-2-reduct.pdf} \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% When reaching a $\get{r}$ or a $\ast$, the substitution simply vanishes.
% \begin{center}
%  \begin{longtable}{lDED}
%     \rrulet{subst}{unit}
%     & \includegraphics{figures/simulation/pdfs/subst-unit-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-unit-reduct.pdf} \\
%   \end{longtable} 
% \end{center}
%
% \paragraph{}
% The \rrulet{subst}{app}, \rrulet{subst}{subst-r} and \rrulet{subst}{subst-r'}
% perform a duplication and make use of \ref{REDUCTION-SUBST-SUBSTR} to propagate
% the substitution inside reference substitutions.
%
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrulet{subst}{app}
%     & \multicolumn{3}{D}{
%       \includegraphics{figures/simulation/pdfs/subst-app-redex.pdf}
%     } \\
%
%     $\to^\ast$
%     & \multicolumn{3}{D}{
%       \includegraphics{figures/simulation/pdfs/subst-app-reduct.pdf}
%     } \\
%
%     \rrulet{subst}{subst-r}
%     & \includegraphics{figures/simulation/pdfs/subst-substr-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-substr-reduct.pdf} \\
%
%     \rrulet{subst}{subst-r'}
%     & \includegraphics{figures/simulation/pdfs/subst-substrp-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-substrp-reduct.pdf} \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% The \rrule{subst}{\parallel} just duplicate the variable substitution to the two
% threads
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrule{subst}{\parallel}
%     & \includegraphics{figures/simulation/pdfs/subst-par-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-par-reduct.pdf} \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% Finally, the \rrulet{subst}{merge} distributes the outter substitution to both
% the term and the inner substitution.
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrulet{subst}{merge}
%     & \includegraphics{figures/simulation/pdfs/subst-merge-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-merge-reduct.pdf} \\
%   \end{longtable}
% \end{center}
%
% \subsection{Downward reference substitutions reductions}
%
% The propagation of references substitutions relies on the behavior of routing
% area, and especially the Transit lemma (\ref{lemma-route-transit}). The
% fundamental case is the non deterministic reduction happening when reducing a
% $\get{r}$ whose redex is 
% \begin{center}
%   \begin{longtable}{lD}
%     \rrulet{subst-r}{get}
%     & \includegraphics{figures/simulation/pdfs/substr-get-redex.pdf} \\
%   \end{longtable}
% \end{center}
%
% Then for each $V$ in the image of $\multv{V}$, there will be exactly one summand
% of the following form
%
% \begin{center}
%   \begin{longtable}{DED}
%     \includegraphics{figures/simulation/pdfs/substr-get-reduct-1-1.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substr-get-reduct-1-2.pdf} \\
%   \end{longtable}
% \end{center}
%
% The remaining term does indeed reduce to the translation of $\get{r}$:
% \begin{center}
%   \begin{longtable}{DED}
%     \includegraphics{figures/simulation/pdfs/substr-get-reduct-2-1.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substr-get-reduct-2-2.pdf} \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% \rrulet{subst-r}{val}, \rrule{subst-r}{\parallel} and \rrulet{subst-r}{app} are
% just direct application of the Transit lemma.
%
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrulet{subst-r}{val}
%     & \includegraphics{figures/simulation/pdfs/substr-val-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substr-val-reduct.pdf} \\
%
%     \rrule{subst-r}{\parallel}
%     & \includegraphics{figures/simulation/pdfs/substr-par-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substr-par-reduct.pdf} \\
%
%     \rrulet{subst-r}{app}
%     & \multicolumn{3}{D}{
%       \includegraphics{figures/simulation/pdfs/substr-app-redex.pdf}
%     } \\
%     $\to^\ast$
%     & \multicolumn{3}{D}{
%       \includegraphics{figures/simulation/pdfs/substr-app-reduct.pdf}
%     } \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% \rrulet{subst-r}{merge} and \rrulet{subst-r}{subst-r'} amount to nothing in nets, as the translation
% already identifies the redex and the reduct of these rules.
%
% \begin{center}
%   \begin{longtable}{lDlD}
%     \rrulet{subst-r}{subst-r'}
%     & \includegraphics{figures/simulation/pdfs/substr-substrp-both.pdf}
%     & \rrulet{subst-r}{merge}
%     & \includegraphics{figures/simulation/pdfs/substr-merge-both.pdf} \\
%   \end{longtable}
% \end{center}
%
% \subsection{Upward reference substitutions reduction}
% As for downward substitutions, the main ingredient is the Transit lemma applies
% to our specific routing area $\delta$ and $\gamma$.
%
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrule{subst-r'}{\parallel}
%     & \includegraphics{figures/simulation/pdfs/substrp-par-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substrp-par-reduct.pdf} \\
%
%     \rrulet{subst-r'}{lapp}
%     & \includegraphics{figures/simulation/pdfs/substrp-lapp-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substrp-lapp-reduct.pdf} \\
%
%     \rrulet{subst-r'}{rapp}
%     & \includegraphics{figures/simulation/pdfs/substrp-rapp-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substrp-rapp-reduct.pdf} \\
%   \end{longtable}
% \end{center}


==> paper-csl-long arxiv/parts/nets-termination.tex <==
\newcommand{\labelsubst}[2]{|{#1}|_{#2}}
\newcommand{\lthisplus}{$\lamlang{cES+}$}

\section{Termination}

We introduced an intermediate language \lthis and showed its termination.
However, a few steps may remain to eventually reach a normal form. The first
step is to collect and merge all the routing areas that are created and
connected during the translation. Doing so, we separate the net between a part
that closely follows the translated term structure, and a big routing area which
connects various substerms to enable communication through references between
them. Once this is done, the only remaining possible redexes are dereliction,
introduced by $\get r$, facing the cocontraction tree of a input of the routing
area. A non deterministic reduction can occur, but these gets will never be fed
anything after that : there is no available assignment in the original term.
Hence, after these two steps, the nets are constrained enough to ensure that no
more redex appear. This is the essence of the proof of
\ref{lemma-nets-termination-sn}.

We first define the list of constraints that the non-routing part of the net
will satisfy :

\begin{definition}{Separability}\label{definition-nets-termination-separability}\\
  Let $\mathcal{R}$ be the translation of a \lthis or \lthisplus
  term, then $\mathcal{R}$ is say te be \emph{separable} if 
  can be reduced to the following form :

  \begin{center}
    \tikzvcenter{
      \begin{proofnet}
        % Communication box
        \node[net={40pt}{40pt}] (box) {\mathbf{R}};
        % Remaining part of the net
        \init[grow=left]([xshift=15ex]box.east){
          \nary[shape=rectangle,cell={net={40pt}{30pt}},name=sigma]{\mathcal{S}}{
            \point(sigmai1),
            \point(sigmao1),
            \point(sigmain),
            \point(sigmaon)
          }
        }
        % Box coordinates
        \coordinate (i1) at ([yshift=-13pt]box.east);
        \coordinate (o1) at ([yshift=-8pt]box.east);
        \coordinate (in) at ([yshift=8pt]box.east);
        \coordinate (on) at ([yshift=13pt]box.east);
        \coordinate (i0) at ([yshift=-3pt]box.west);
        \coordinate (o0) at ([yshift=2pt]box.west);
        % Sigma coordinates
        \coordinate (sigmai1) at ([yshift=-13pt]sigma.north);
        \coordinate (sigmao1) at ([yshift=-8pt]sigma.north);
        \coordinate (sigmain) at ([yshift=8pt]sigma.north);
        \coordinate (sigmaon) at ([yshift=13pt]sigma.north);
        % Connect box and sigma
        \init[grow=up]{ 
          \wirefromto{sigmai1}{sigmai1}{i1}{i1}
          \wirefromto{sigmain}{sigmain}{in}{in}
          \wirefromto{sigmao1}{sigmao1}{o1}{o1}
          \wirefromto{sigmaon}{sigmaon}{on}{on}
          \wirefromto{[xshift=-10pt]i0}{[xshift=-10pt]i0}{i0}{i0}
          \wirefromto{[xshift=-10pt]o0}{[xshift=-10pt]o0}{o0}{o0}
        }
        %
        \pdots[2pt]([xshift=10pt]o1)([xshift=10pt]in)
      \end{proofnet}
    }
  \end{center}
  where $\mathbf{R}$ is a routing area and $\mathcal{S}$ a net with free wires labelled by
  $i_1,\ldots,i_n,o_1,\ldots,o_m,O$, satisfying :
  \begin{itemize}
    \item There is no redex in $\mathcal{S}$
    \item $i_1,\ldots,i_m$ are either connected to the auxiliary port of a
      $\otimes$ cell, or to the principal port of a dereliction
    \item $o_1,\ldots,o_n,O$ are either connected to a
      $\parr$ cell, or to the principal door of an open box
  \end{itemize}

\end{definition}

The following lemma states that the translation of any open term is separable.
The main reason is that constructors as application, substitution, parallel,
etc. preserve separability. But the translation of values with free variables
are obviously separable.  This comes from the fact that we pushed weakening deep
inside atoms' exponential boxes, so any pending variable that is not bound
forces an auxiliary door on all the boxes, blocking further reduction.

\begin{lemma}{Open terms separability}\label{lemma-nets-termination-otsep}\\
  Let $\Gamma,x:A \vdash M : (\alpha,e)$ a \lthis well-typed term, then its
  translation $M^\bullet$ is separable. 
\end{lemma}

% \begin{proof}\ref{lemma-nets-termination-ostep}\\
% \begin{description}
%   \item[Values] As stated above, we can first observe that the translation of $\ast$, of a
%     variable $x$ and an abstraction all statisfy the separability conditions.
%     Their general form is :
%
%     % \begin{center}
%     %   \includegraphics{}
%     % \end{center}
%
%     Which is normal, and the box $R$ is just a juxtaposition of $0$-communication
%     areas, corresponding to references introduced by subtyping in $e$. Thus $m = n
%     = 0$. The net is normal, and its output $O$ is the the principal door of an
%     open box.
%   \item[Get] It is almost the same as for values, except that the output $o$
%     corresponding to the get's reference is connected to a dereliction, which is
%     allowed in (blah).
%   \item[Application] By induction, $M^\bullet$, $N^\bullet$ and $\multv{V}$ are
%     separable, thus can be decomposed in the following way :
%
%     % \begin{center}
%     %   \includegraphics{}
%     % \end{center}
%
%     We can merge all the communcation boxes in the left circle together. All the 
%     inputs or outputs previously connected to one of the small area immediatly
%     satisfies the condition (blah) by IH. The two remaining
%     wires $i_0$ and $o_0$ are respectively connected to the auxiliary port of
%     a par and the auxiliary port of a cocontraction, thus satisfy (blah). We take
%     the right circle to be our second part $\mathcal{S}$.
%     $\mathcal{S}_N$, $\mathcal{S}_M$ and $\mathcal{S}_\multv{V}$ are normal by IH.
%     $O$ is the conclusion of par, hence satisfies (blah). It only remains to see
%     that the wole net contained in the circle is normal, but the only redex that
%     could appear is the connection of a dereliction to $M^\bullet$. But by (blah),
%     $O_M$ is either the conclusion of an open box or a par, and thus the whole net
%     is normal indeed, and (blah) is verified.
%   \item[Parallel] Similar to application
%   \item[Variable substitution] As for application, we apply the IH on
%     $M^\bullet$ and $V^\bullet$, merge the routing areas, and just check that the
%     connection of $V^\bullet$ to $M^\bullet$ can't create new redexes. Indeed, by
%     (blah), the outpout $O_V$ can't be part of any redex.
%   \item[Reference substitutions] Again the same technique is applied, and we see
%     that the resulting net and routing area satisfies the conditions.
% \end{description}
%
% \end{proof}

Finally, the main result we rely on as explained above is the following one :

\begin{lemma}{Normal form separability}\label{lemma-nets-termination-nfsep}\\
  The translation of a \lthisplus normal form is separable
\end{lemma}

% \begin{proof}{\ref{lemma-nets-termination-sn}}\\
%   We apply \ref{lemma-nets-termination-nfsep} to reduce the translation of $F$ to
%   a routing area connected to $\mathcal{S}$ satisfying $P$. $\mathcal{S}$ and
%   $\routarea R$ are normal. The potential ones must take place at the interface
%   of $\routarea{R}$ and $\mathcal{S}$. The inputs of $\routarea{R}$ are
%   connected to $\mathcal{S}$, being either connected to a par or the conclusion
%   of an open box, and thus can't form any redex with (co)weakenings and
%   (co)contractions of $\routarea R$.
%
%   The output of $\routarea R$ are connected to the auxiliary port of a tensor,
%   or to a dereliction. Only the latter may form a new redex. If the output of
%   $\mathbf{R}$ is a coweakening, then everything reduces to $\mathbf{0}$. If it
%   is just a wire, then the dereliction is connected through this wire to an
%   input of $\routarea R$ which again can't be part of any redex. The only
%   remaining case is when the output of $\routarea R$ is a cocontraction tree.
%   Then we can perform the non-deterministic reduction, and we go back to exactly
%   the two previous cases as the dereliction is finally connected to a leaf of
%   the tree of an input.
%
%   Hence, after we performed finitely many dereliction/cocontraction reductions,
%   we finally get a normal form, which either $\mathbf{0}$, or a sum of the
%   previous net $\mathbf{S}$ connected to simpler routing area $\routarea{R}_i$.
% \end{proof}

Which leads us to the main result :

\begin{theorem}{Termination for nets}\\
  The translation of a well typed term of \lthis\ terminates.
\end{theorem}


==> paper-csl-long arxiv/parts/nets-translation.tex <==
\section{Translation}
\label{section:translation}

To implement the translation, we make use of two specific routing areas that we
introduce below. In the following, $E_i = \{1,\ldots,i\}$ and $R_i$ is the binary relation defined on
$E_i$ by $k \mathrel{R_i} l \iff k \neq l$.

% We use pervasively routing areas as building blocks of our translation. While
% having described their structure and how to combine them, we haven't yet
% justified the "routing" part in their name by more than intuition. The role of
% the Transit property is to give a formal account of it. Given a closed
% exponential box, we connect it to the auxiliary port of a cocontraction to
% obtain a little module which can then be connected to an input $i$ of an area.
% Through reduction, it will traverse the area and be duplicated $R(i,o)$ times to
% each output $o$. The role of the additionnal cocontraction is to preserve the
% area and allow future connections to the same output: we would get a similar
% transit property connecting directly the exponential box to $i$, but the process
% would erases the input and prevents any future use.
%
% \begin{property}{Transit}\label{property-translation-transit}\\
%   Let $\sigma$ be a closed exponential box, $\mathbf{R} = (\labin,\labout,R)$ a
%   routing area, $i \in \labin$. Let $\{ o_1, \ldots, o_p \} = \conn{i}$ and for $1 \leq k \leq p,\ c_k = R(i,o_k)$. Then :
%   \begin{center}
%     \includegraphics{figures/routing-areas/pdfs/area-transit.pdf} 
%   \end{center}
% \end{property}
%
% \begin{proof}\ref{property-mrarea-transit}
%   Put the figure of the generalized reduction
% \end{proof}
%
% As opposed to the general setting of Differential Linear Logic where linear
% combination of terms may have their coefficients in an arbitrary semiring, we
% interpret in our work the differential sum as a non deterministic operator,
% which is idempotent. As such, two copies of the same box cocontracted together
% will be collapsed into just one outcome as soon as this cocontraction meets a
% dereliction and is reduced. Hence, we are interested in the special
% case of routing areas $(\labin,\labout,R)$ where $R$ is actually a relation, id
% est $\max{R(x,y)} \leq 1$.
%
% This property is preserved by merging: indeed, we can never create multiple
% paths by connecting two disjoints area, thus the merging of two such areas give
% again an area whose multirelation is a relation. On the opposite, the trace operation
% clearly does not preserve this property.
%
%   In this subsection, we define the two fundamental routing areas
% that will be used as building blocks for the translation. Note that they verify
% the above condition.
%
%
% This reformulation shows that communication areas are a special case of routing
% areas, which are themselves a subsets of routing areas.

The $\gamma$ area is defined by $(E_3,E_3,R_\gamma = R_3)$. $\gamma$ is actually
a communication area, composed of $3$ pairs of input and outputs grouped by
label. Each such pair represents a plug to which translated terms will be
connected. The definition of $R_\gamma$ expresses that the input and the output
of a plug are not connected, as a component should not receive the data it sent
himself: this would be the analog of a short-circuit. All others inputs and
output are connected.

%

The $\delta$ area is an analog structure with $4$ plugs: $(E_4,E_4,R_\delta)$.
It is designed to handle the application $M\ N$ which includes three potential sources of effects : 
\begin{enumerate}
  \item The effects $e_1$ produced by reducing $M$ to $\lambda x. M'$
  \item The effects $e_2$ produced by reducing $N$ to value $V_N$
  \item The effects $e_3$ produced by reducing $M'[V_N/x]$ to the final result
    $V$
\end{enumerate}
The reduction of {\lamadio} imposes that $e_1$ and $e_2$ happen before $e_3$,
while $e_1$ and $e_2$ may happen concurrently. For $1 \leq i \leq 3$, the plug
$(i,i)$ of $\delta$ corresponds to the effects $e_i$. The last one is the
external interface for future connections. We easily accommodate $\delta$ to
implements the sequentiality constraint by removing the couples $(3,1)$ and
$(3,2)$ from $R_4$ to form $R_\delta$. Indeed $e_1$ and $e_2$ happens before $e_3$ thus can not observe
any {\setw} made by the latter. Thus we just cut the corresponding wires.  We see
that the formalism of routing areas allows us to easily encode the order of effects.

\subsection{Translating types and effects}
Before translating terms, we need to translate the types from the type and
effects system for {\lamadio} to plain {\LL} formulas. We use the approach of
\cite{tranquilli:hal-00465793}, a monadic translation, explained in the following. Before
translating to {\LL}, let us first try to take a type with effects and translate
it to a pure simple type. Let $e = \{r_1,\ldots,r_n\}$ be an effect (a finite set of references), assume we can assign a simple type $R_i$ to each
reference $r_i$. We can type a store $S_e = R_1 \times \ldots \times R_n$
representing the current state of the memory. We transform a term $M$ of type $A$
producing effects to a pure term which takes the initial state of the store, and
returns the value it computes together with the new state of the store after
this computation. Using curryfication for the arrow type, we define the 
translation: 

\begin{center}
  \begin{tabular}{rcl}
    $T_e(\alpha)$ & $=$ & $S \to S \times \alpha$ \\
    $T_e(A \sur{\to}{e} \alpha)$ & $=$ & $A \to (S \to (S \times \alpha))
    \cong A \times S \to S \times \alpha$
  \end{tabular}
\end{center}

From there, we go to {\LL} types by implementing the pair type $A \times B$ as
$\oc A \otimes \oc B$, and the usual call-by-value translation for the arrow $(A
\to B)^\bullet = \oc(A^\bullet \multimap B^\bullet)$~\cite{MARAIST1995370}. We still
have to determine each $R_i$ first. Using the previous formula, we may
associate an {\LL} type variable $X_{r_i}$ to each reference and plug everything
together to obtain the following equations (where $A_i$ is the type given 
to $r_i$ by the reference context):
\begin{center}
  \begin{tabular}{rcl}
    $\text{Unit}^\bullet$ & $=$ & $\oc{1}$ \\
    $(A \sur{\to}{\{s_1, \ldots, s_m\}} \alpha)^\bullet$ & $=$ 
     & $\oc{((A^\bullet \otimes X_{s_1} \ldots \otimes X_{s_m}) \multimap (X_{s_1}
       \otimes \ldots \otimes X_{s_m} \otimes \alpha^\bullet))}$ \\
   $X_{r_i}$ & $=$ & ${A_i}^\bullet$
  \end{tabular}
\end{center}

This system is solvable precisely because the type system is
stratified~\cite{tranquilli:hal-00465793}, and we can thus translates all the
types of {\lamadio} to plain {\LL} types. The behavior type $\mathbf{B}$ will be
translated to types of the form $A_1 \parr \ldots \parr A_n$ as the translation
remembers the types of each threads.

\subsection{Translating terms}

The general form of the translation of a term $x_1:A_1,\ldots,x_n:A_n \vdash M :
(\alpha, \{r_1,\ldots,r_k\})$ is given by 
$$
\tikzvcenter{
  \begin{tikzpicture}
    \node[net={80pt}{40pt}] (delta) {M^\bullet};
    \draw [arrowed] (delta.east) -- node[above,m] {\alpha^\bullet} ++(15pt,0);
    \draw [arrowed] ([xshift=-15pt]delta.south east) coordinate (a) -- node[left,m] {\oc X_{r_k}} ++(0,-15pt) coordinate (b)  node [below,m,dist=1.5pt] (rk) {r_k};
    \draw [arrowed] ([xshift=-40pt]a) coordinate (b) -- node[left,m] {\oc X_{r_k}} ++(0,-15pt)  node [below,m,dist=1.5pt] (r1) {r_1};
    \proofdots(r1.mid east)(rk.mid west)
    \draw [reverse arrowed] (a|-delta.north) -- node[left,m] {\oc X_{r_k}} ++(0,15pt)  node [above,m,dist=1.5pt] (rk) {r_k};
    \draw [reverse arrowed] (b|-delta.north) coordinate (c) -- node[left,m] {\oc X_{r_1}} ++(0,15pt)  node [above,m,dist=1.5pt] (r1) {r_1};
    \proofdots(r1.mid east)(rk.mid west)
    \draw [reverse arrowed] ([yshift=-10pt]delta.north west) -- node[above,m] (lab1) {A_1^\bullet} ++(-15pt,0) node[left,m,dist=1pt] (x1) {x_1};
    \draw [reverse arrowed] ([yshift=10pt]delta.south west) -- node[below,m] (lab2) {A_n^\bullet} ++(-15pt,0) node[left,m,dist=1pt] (xn) {x_n};
    \proofdots(x1)(xn)
  \end{tikzpicture}
}
$$

We distinguish three different types of free wires:
\begin{description}
  \item[Output wire] The right wire, labelled by $\alpha^\bullet$, corresponds
    to the result of the whole term.
  \item[Variable wires] Each wire on the left corresponds to a variable of the
    context. The (explicit) substitution of a variable $x$ for a term
    $V^\bullet$ is obtained by connecting the output wire of $V^\bullet$ to the
    wire of $x$.
  \item[References wires] The wires positioned at the top are
    input wires corresponding to references and have a similar role as variable wires,
    while the wires at the bottom corresponds dually to the output. References
    wires will be connected by routing areas.
\end{description}
    
We present some representative cases of the translation: $\get{r}$ and
$\set{r}{V}$ for reference management, the abstraction to show how effects are
thunked in a function's body following the monadic translation, and the
application that shows the usage of routing areas to handle non-trivial effects
scheduling. We start with reference operations, which serve as switch from and
to reference wires:

% $$
% \tikzvcenter{
%   \tikztarget(mtrad){
%     \begin{proofnet}[baseline=-5.ex]
%       \init[grow=left]{
%         \boxpal{lambda}{
%           \binary{\parr}{
%             \binary{\otimes}{
%               \nary[name=mtrad,shape=rectangle,cell={net={40pt}{60pt}}]{M}{
%                 {\wire{}},
%                 {\point(xvar)}
%               }}
%               {\point(outeff)}}
%             {
%               \binary{\parr}{}{\point(ineff)}
%             }
%         }
%       }
%       \draw (outeff) -- (mtrad.east);
%       \drawbox{lambda}
%     \end{proofnet}
%   }
% }
% $$

\paragraph*{Set (Figure~\ref{figure:set})}
A $\set{r}{V}$ connects the output of the translation of $V$ to the output
reference wire corresponding to $r$. As other {\setw s} are not relevant a
weakening is connected on the input wire to ignore any incoming resource. In
{\lamadio}, a set reduces to $\ast$ as it does not compute anything valuable.
Consequently the output is the conclusion of a banged $1$ which is the
translation of $\ast$.

One important remark is that an additional exponential layer is added around the
translation of $V$. In a call-by-value language, the non determinism is strict
in the sense that non-deterministic term must be evaluated before any copy. For
example, the term $(\lambda fx .f\ x\ x)\ \get{r} \parallel \store{r}{V_1}
\parallel \store{r}{V_2}$ can reduce either to $f\ V_1\ V_1$ or $f\ V_2\ V_2$
but not to $f\ V_1\ V_2$. Differential {\LL} rather implements the latter
call-by-name semantic as hinted at by the $\red{ba}$ rule which 
expresses that duplication and non-determinism should commute. The mismatch is
due to two different usages we want to make of the $\oc$: 

\begin{itemize}
  \item The first one allows to discriminate what proof nets can be the target
    of structural rules, which implements substitution. In call-by-value, the
    only terms that can be substituted are values. The $\oc$ is introduced by
    the translations of values, using $\oc_p$, and eliminated at usage - when
    applied to another term - for each copy by a dereliction.
  \item The second usage relates to the differential part. The bang denotes
    resources that may be packed non deterministically by a cocontraction. The
    choice is made when a dereliction is met.
\end{itemize}

But as we noted, these two usages are in contradiction: a non-deterministic
packing should not be allowed to be substituted. Technically, the
dereliction corresponding to the place of usage and the dereliction corresponding
to the non-deterministic choice should not be the same. This is the reason
of the additional $\oc$ layer introduced by an exponential box around
$V^\bullet$. The corresponding dereliction is found in the translation of $\get{r}$.

\begin{figure}[tb]
\centering
\begin{minipage}{0.29\textwidth}
\centering
  $\infer[(set)]
  { R;\Gamma \vdash set(r,V) : (\text{Unit},\{ r \}) }
  { R;\Gamma \vdash r : \text{Reg}_r{A} \qquad R;\Gamma \vdash V : (A,\emptyset)
  }$
\end{minipage}
\begin{minipage}{0.69\textwidth}
\centering
  \includegraphics{figures/translation/pdfs/translation-set-sem.pdf}
\end{minipage}
\caption{Translation of $\set{r}{V}$}\label{figure:set}
\end{figure}

\paragraph*{Get (Figure~\ref{figure:get})}
The $\get{r}$, dual of the set, takes a resource from the corresponding input reference wire
and redirects it to the output wire. It outputs a coweakening on the reference wire
as it does not produce any {\setw}. As mentioned in the previous case, a
dereliction is added on the input wire to force the non-deterministic choice and
strip the exponential layer added by the set.

\begin{figure}[tb]
\centering
\begin{minipage}{0.29\textwidth}
\centering
  $\infer[(get)]
  { R;\Gamma \vdash \get{r} : (A,\{ r \}) }
  { R \vdash \Gamma }$
\end{minipage}
\begin{minipage}{0.69\textwidth}
\centering
 \includegraphics{figures/translation/pdfs/translation-get.pdf}
\end{minipage}
\caption{Translation of $\get{r}$}\label{figure:get}
\end{figure}

\paragraph*{Abstraction (Figure~\ref{figure:abs})}
The abstraction thunks the potential effects of the body $M$ in the pure term
$\lambda x. M$. Following the monadic translation, the input effects are
tensorized with the bound variable, and the output effects with the output of
$M$. Finally the whole term is put in an exponential box as it is a value.

\begin{figure}[tb]
\centering
\begin{minipage}{0.29\textwidth}
\centering
  $\infer[(lam)]
    { R;\Gamma \vdash \lambda{x}.M : (A \sur{\to}{e} \alpha, \emptyset) }
    { R;x:A,\Gamma \vdash M : (\alpha,e) }$
\end{minipage}
\begin{minipage}{0.69\textwidth}
\centering
  \includegraphics{figures/translation/pdfs/translation-lam.pdf}
\end{minipage}
\caption{Translation of $\lambda x. M$}\label{figure:abs}
\end{figure}

\paragraph*{Application (Figure~\ref{figure:app})}
Finally, the application put the routing area at use. Using the same terminology
as in the introduction of this section, we see the effects $e_1$ and $e_2$
coming respectively from the evaluation of $M$ and $N$, and $e_3$, liberated by
the body of the function being applied, plugged on the $\delta$ area.

\begin{figure}[tb]
\centering
$\infer[(app)]
  { R;\Gamma \vdash \refssl{}{\multv{V}}{M\ N} : (\alpha, e=e_1 \cup e_2 \cup e_3) }
  { R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha, e_2)
    \qquad R;\Gamma \vdash N : (A,e_3)
    \qquad R;\Gamma \vdash V \in \multv{E}_i : (R(r_i),\emptyset)}$
\centering
\includegraphics{figures/translation/pdfs/translation-app-sem.pdf}
\caption{Translation of $M\ N$}\label{figure:app}
\end{figure}

\subsection{Full translation of {\lthis} into proof nets}
We presented some interesting cases of the translation of {\lamadio} to proof
nets to provide the reader with some intuition. However the complete translation
is rather operating on the
intermediate language {\lthis}. A translation and a simulation theorem between
{\lamadio} and {\lthis} are given in~\cite{HamdaouiValiron2018}, completing the
picture.

\begin{center}
\begin{longtable}{|c|c|}
\hline
Typing derivation & Translation \\
\hline
$\infer[(var)]{\Gamma,x : A \vdash x : (A,\emptyset)}{}$
& \includegraphics{figures/translation/pdfs/translation-var.pdf} \\
\hline

$\infer[(unit)]{\Gamma \vdash \ast : (\texttt{Unit},\emptyset)}{}$
& \includegraphics{figures/translation/pdfs/translation-unit.pdf} \\
\hline

$\infer[(lam)]
{ \Gamma \vdash \lambda{x}.M : (A \sur{\to}{e} \alpha, \emptyset) }
{ x:A,\Gamma \vdash M : (\alpha,e) }$
& \includegraphics{figures/translation/pdfs/translation-lam.pdf} \\
\hline

$\infer[(app)]
{ \Gamma \vdash \refssl{}{\multv{V}}{M\ N} : (\alpha, e=e_1 \cup e_2 \cup e_3) }
{ \Gamma \vdash M : (A \sur{\to}{e_1} \alpha, e_2)
  \qquad \Gamma \vdash N : (A,e_3)
  \qquad \Gamma \vdash V \in \multv{E}_i : (B_i,\emptyset)}$
& \includegraphics{figures/translation/pdfs/translation-app.pdf} \\
\hline

$\infer[(get)]
{ \Gamma \vdash \get{r} : (A,\{ r \}) }
{ \vdash \Gamma }$
& \includegraphics{figures/translation/pdfs/translation-get.pdf} \\
\hline

% $\infer[(set)]
% { R;\Gamma \vdash set(r,V) : (\text{Unit},\{ r \}) }
% { R \vdash r:\text{Reg}_r\ A \qquad R;\Gamma \vdash V : (A,\emptyset) }$
% & \tikzvcenter{
%   \tikztarget(set){
%     \begin{proofnet}[baseline=-.5ex]
%       \init[grow=left]{
%         \boxpal[name=ppal]{p}{
%           \nary[wire=arrowed,shape=rectangle,cell={net={15pt}{20pt}},name=V,fix=both]{V^\bullet}{\wire[inbox={}]{\coord(vgamma)}}
%         }
%       }
%       \init[grow=down]([yshift=6ex,xshift=7.5ex]V.east){
%         \zeroary[name=myweak1]{\wn}
%       }
%       \init[grow=left]([xshift=15ex]V.south){
%         \boxpal{pone}{
%           \zeroary[name=one]{1}
%         }
%       }
%       % \init[grow=right]{
%       %   \flipped[small,name=myweak1]{\wn}{}{\point(pend1)}
%       % }
%       % \init[grow=left]([yshift=20pt,xshift=21pt]myweak1){
%       %   \boxpal{p}{
%       %     \unary[flip]{\wn}{
%       %       \wire[inbox={}]{\wire[inbox={}]{\point(pend)}}
%       %     }
%       %   }
%       % }
%       % \addtobox{p}{myweak1}
%       % \draw let \p1=(pend), \p2=(pend1) in (\x1,\y2) -- (pend1);
%       % \draw[reverse arrowed] (pend) -- ++(0,25pt);
%       % \drawbox{p}
%       % \init[grow=up]([yshift=-30pt]myweak1){
%       %   \wire{\zeroary{\oc}}
%       % }
%       \drawbox{p}
%       \drawbox{pone}
%       \wirefromto{[xshift=5pt]ppal.pal}{[xshift=5pt]ppal.pal}{[yshift=-15pt,xshift=5pt]ppal.pal}{[yshift=-15pt,xshift=5pt]ppal.pal}
%       % \draw[rounded corners=3pt, arrowed] ([xshift=5pt]ppal.pal) |- ++(0,-15pt);
%     \end{proofnet}
%   }
% } \\
% \hline

$\infer[(par)]
{ R; \Gamma \vdash P_1 \parallel P_2 : \mathbf{B} }
{i=1,2 \qquad R;\Gamma \vdash P_i : \alpha_i }$
& \includegraphics{figures/translation/pdfs/translation-par.pdf} \\
\hline

\infer[(subst)]
{ R; \Gamma \vdash \varss{\sigma}{M} : (\alpha, e) }
{ R; \Gamma, x : A \vdash M : (\alpha,e) \qquad R; \Gamma \vdash V : (A,\emptyset) }
& \includegraphics{figures/translation/pdfs/translation-subst-var.pdf} \\
\hline

\infer[(subst\text{-}r\downarrow)]
{ R; \Gamma \vdash \substg{(r_i)}{(\mathcal{V}_i)}{M} : (\alpha, e) \qquad }
{ R; \Gamma \vdash M : (\alpha,e) \qquad R; \Gamma \vdash \mathcal{V}_i : (A_i,\emptyset) }
& \includegraphics{figures/translation/pdfs/translation-substr-down.pdf} \\
\hline

\infer[(subst\text{-}r\uparrow)]
{ R; \Gamma \vdash \substup{(r_i)}{(\mathcal{V}_i)}{M} : (\alpha, e) \qquad }
{ R; \Gamma \vdash M : (\alpha,e) \qquad R; \Gamma \vdash \mathcal{V}_i : (A_i,\emptyset) }
& \includegraphics{figures/translation/pdfs/translation-substr-up.pdf} \\
\hline
\end{longtable}
\end{center}

We proceed to give the properties satisfied by the translation.


==> paper-csl-long arxiv/parts/nets.tex <==
\section{Proof nets}
\label{section:nets}

In this section, we detail the proof nets that we are considering in the rest of
the paper. We do not attempt to give a full treatment of proof nets.
We recall the important notions and specify the system that we use. The
interested reader may find more details in~\cite{Pag08} for example. Proof nets are a
representation of proofs as multigraphs, where edges - called \emph{wires}
- correspond to the formulas, and nodes - \emph{cells} - correspond to the
rules.  We can decompose our system into three different layers:
\begin{description}
  \item[Multiplicative] The multiplicative fragment is
    composed of the conjunction $\otimes$ and the dual disjunction $\parr$.
    These connectors can express the linear implication $\multimap$ and are thus
    able to encode a linear $\lambda$-calculus, where all bound variables
    must occur exactly once in the body of an abstraction.
  \item[Exponential] The exponentials enable
    structural rules to be applied on particular formulas distinguished by the
    $\oc$ modality (its dual being $\wn$). Structural rules correspond to
    duplication (contraction) and erasure (weakening) : the multiplicative
    exponential fragment is the typical setting to interpret the
    $\lambda$-calculus.
  \item[Differential] Non determinism is expressed by using two rules from
    Differential {\LL}: cocontraction and coweakening.
    Semantically, contraction is thought as a family of diagonal morphisms
    $\mathit{cntr}_A : \oc A \to \oc A \otimes \oc A$, each one taking a
    resource $\oc A$ and duplicate it into a pair $\oc A \otimes \oc A$.
    Dually, cocontraction is a morphism going in the opposite direction, packing
    two resources of the same type into one : $\mathit{cocntr}_A : \oc A \otimes
    \oc A \to \oc A$.  What happens when the resulting resource is to be
    consumed ? Two incompatible possibilities : either the left one is used and
    the right one is erased, or vice-versa.  This corresponds to the rule
    $\red{nd}$ (see Table~\ref{figure:reduction}) in proof nets: the reduction
    produces the non-deterministic sum of the two outcomes.  Cocontraction will
    be used as an internalized non-deterministic sum. While weakening
    $\mathit{weak}_A : \oc A \to \mathbf{1}$ erases a resource, the dual
    coweakening produces a resource ex nihilo: $\mathit{coweak}_A : \mathbf{1}
    \to \oc A$.  This resource can be duplicated or erased, but any attempt to
    consume it will turn the whole net to $\mathbf{0}$. Coweakening produces a
    Pandora box with a $0$ inside. It is the neutral element of cocontraction.
\end{description}

% We define in this section the proof nets we use as a target of the translation.
% Proof nets are a representation of proofs as multigraphs, where pending edges -
% called here \emph{free wires} - correspond to conclusions, and nodes correspond
% to rules. We work in an extension of Multiplicative Exponential Linear Logic
% (MELL), to which we add the coweakening and cocontraction rules borrowed to
% Differential Linear Logic to represent non determinism.
%

One can define a correctness criterion to discriminate nets that are
well-behaved - the ones that are the representation of a valid proof - ensuring
termination and confluence of the reduction. We will not require it here (cf
Section~\ref{section:conclusion}). Without the correctness criterion, the full fledged reduction
of (differential) {\LL} is not even confluent, let alone terminating. We add
constraints in order to recover an suitable system that is confluent and
verifies a termination property (Theorem~\ref{theorem-nets-termination}). Let us now give the
definition of proof nets and their reduction:
% As mentioned in the introduction, the translation of concurrent processes
% naturally generate cycles, thus no correctness criterion is involved. To cope
% with this permissive setting, we restrict the reduction not only to be surface
% (no reduction inside boxes), but also close, meaning that only a box with no
% auxiliary doors can be subject to exponential reductions. Actually, we
% liberalize a bit the surface constraints to allow a few harmless reduction rules
% to happen at arbitrary depth. We prove that the resulting system is
% \emph{confluent}, and satisfies a termination-related property: a weakly
% normalizing term is actually strongly normalizing.

\begin{notation}
We recall some vocabulary of rewriting theory that we use in the following. A term of a language or a proof net $t$ is
\begin{description}
  \item[A normal form] if it can't be reduced further
  \item[Weakly normalizing] if there exists a
    normal form $n$ such that $t \to^\ast n$ 
  \item[Strongly normalizing] if it has no infinite
    reduction sequence
  \item[Confluent] if for all $u,u'$ such that $u \rredstar{} t \to^\ast u'$,
    there exists $v$ such that $u \to^\ast v \rredstar{} u'$
  \end{description}
  A rewriting relation is confluent if all terms are.
\end{notation}

\begin{definition}{Proof nets}\label{nets-definition-nets}\\
Given a countable set, whose elements are called ports, a proof net is given by
\begin{enumerate}
  \item A finite set of ports
  \item A finite set of cells. A cell is a finite non-empty sequence of pairwise
    distinct ports, and two cells have pairwise distinct ports.  The first port
    of a cell $c$ is called the {\emph principal port} and written $p(c)$, and
    the $(i+1)$th the $i$th auxiliary port noted $p_i(c)$.  The number of
    auxiliary ports is called the {\emph arity} of the cell. A port is free if
    it does not occur in a cell. 
  \item A labelling of cells by symbols amongst $\{ 1, \otimes, \parr, \wn, \oc
    \}$. We ask moreover that the arity respects the following table: 
    \begin{center}
      \begin{tabular}{c|ccccc}
        Symbol & $\parr$ & $\otimes$ & $\wn$ & $\oc$ & $\oc_p$  \\
        \hline
        Arity &  $2$ & $2$ & $0,1$ or $2$ & $0,1$ or $2$ & $i \geq 1$\\
      \end{tabular}
    \end{center}
  \item A partition of its ports into pairs called {\emph wires}. A wire with
    one (resp. two) free port is a free (resp. floating) wire.
  \item A labelling of wires by MELL formulas: $F \mathrel{::=} 1 \mid \bot
    \mid F \parr F \mid F \otimes F \mid \oc F \mid \wn F$. A wire $(p_1,p_2)$
    labelled by $F$ is identified with the reversed wire $(p_2,p_1)$ labelled by
    $F^\perp$. We will abusively confuse ports with the wire attached to them.
  \item A mapping from $\oc_p$ nodes - called exponential boxes - to proof nets
    with no floating wires and $n \geq 1$ free wires. The first one is labelled
    (assuming orientation toward the free port) by $A$ and the
    remaining ones by $\oc B_1,\ldots, \oc B_{n-1}$. The corresponding
    $\oc_p$ node must have $\oc{A}$ as principal port and $\oc B_1,\ldots,\oc
    B_{n-1}$ as auxiliary ports.
\end{enumerate}
\end{definition}

The different kind of cells are illustrated in Figure~\ref{figure:nets}.  We
directly represent $\oc_p$ cells as their associated proof net delimited by a
rectangular shape. We impose that labels of wires connected to a cell respect
the one given in Figure~\ref{figure:nets}, i.e that nets are \emph{well-typed}.

%%% ----------------------------------------------------------------
\begin{table}[tb]
\centering
\begin{minipage}{.74\linewidth}
\centering
\begin{tabular}{cccc}
  one & tensor & par & dereliction \\
  \includegraphics{figures/nets/pdfs/nets-one.pdf} &
  \includegraphics{figures/nets/pdfs/nets-tensor.pdf} &
  \includegraphics{figures/nets/pdfs/nets-par.pdf} &
  \includegraphics{figures/nets/pdfs/nets-der.pdf}  \\
  contraction & cocontraction & weakening & coweakening \\
  \includegraphics{figures/nets/pdfs/nets-contr.pdf} &
  \includegraphics{figures/nets/pdfs/nets-cocontr.pdf} &
  \includegraphics{figures/nets/pdfs/nets-weak.pdf} &
  \includegraphics{figures/nets/pdfs/nets-coweak.pdf} \\
\end{tabular}
% \caption{Cells}\label{figure:cells}
\end{minipage}
\begin{minipage}{.24\linewidth}
\centering
exponential box ($\oc_p$)
\includegraphics{figures/nets/pdfs/nets-box.pdf}
% \caption{Exponential box}\label{figure:box}
\end{minipage}
\caption{Cells and box}\label{figure:nets}
\end{table}
%%% ----------------------------------------------------------------

% % \tikzset{every wirelabel/.style={script,dist=2.5pt},angle/.style={isosceles triangle apex angle=#1}}
% \tikzvcenter{%
%   \proofset{bottom=10pt,straight}
%   \tikzset{every proofnet/.style={baseline=-.5ex},every wirelabel={script}}
%   \begin{tabular}%
% %   {@{}*{3}{P{.24\linewidth}@{}}P{.27\linewidth}@{}}
%   {h{-5pt}*{3}{h{5pt}c}@{}c@{}}
%    \tikztarget(one){\begin{proofnet}
%   \init[grow=left]{
%     \binary[wire=arrowed,wirelabel={[above]1},name=cell]{1}{}{}
%   }
%   \end{proofnet}}
%   &
%   \tikztarget(prooften){\begin{proofnet}
%     \init[grow=left]{
%     \binary[wire=arrowed,wirelabel={[above,at end]A\otimes B},name=cell]{\otimes}{
%       \wire[wire=arrowed,wirelabel={[below]A}]{}
%     }{
%       \wire[wire=arrowed,wirelabel={[above]B}]{}
%     }
%   }
%   \end{proofnet}}
%   &
%  \tikztarget(bot){\begin{proofnet}
%   \init[grow=left]{
%     \binary[wire=arrowed,wirelabel={[above]\bot},name=cell]{\bot}{}{}
%   }
%   \end{proofnet}}
%   &
%   \tikztarget(proofpar){\begin{proofnet}
%   \init[grow=left]{
%     \binary[wire=arrowed,wirelabel={[above,at end]A\parr B},name=cell]{\parr}{
%       \wire[wire=arrowed,wirelabel={[below]B}]{}
%     }{
%       \wire[wire=arrowed,wirelabel={[above]A}]{}
%     }
%   }
%   \end{proofnet}}
%   \\[-1ex]
%   one & \tikztarget(otimes){\normalsize tensor} & bottom & \tikztarget(parr){\normalsize par}\\[1ex]
%   \begin{proofnet}
%   \init[grow=left]{
%     \unary[normal,wire=arrowed,wirelabel={[above]\wn A},name=cell]{\wn}{
%       \wire[wire=arrowed,wirelabel={[above]A}]{}
%     }
%   }
% %   \checkbb
%   \end{proofnet}
%   &
%   \begin{proofnet}
%   \init[grow=left]{
%     \binary[wire=arrowed,wirelabel={[above]\wn A},name=cell]{\wn}{
%       \wire[wire=arrowed,wirelabel={[below]\wn A}]{}
%     }{
%       \wire[wire=arrowed,wirelabel={[above]\wn A}]{}
%     }
%   }
%   \end{proofnet}
%   &
%   \begin{proofnet}
%   \init[grow=left]{
%     \binary[wire=arrowed,wirelabel={[above]\wn A},name=cell]{\wn}{}{}
%   }
%   \end{proofnet}
%   &
%      \proofset{bottom=7.5pt}%
%      \tikzset{script/.append style={dist=2.5pt}}
%   \tikztarget(box){\begin{proofnet}
%   \init[grow=left]{
%     \boxpal[wire=arrowed,wirelabel={[above]\oc A},name=pal]{p}{
%       \nary[shape=rectangle,cell={net={22.5pt}{12pt}}, wire=arrowed,wirelabel={[above,script]A}]{\pi}{
%         {\wire[straight,wire=arrowed near start,wirelabel={[below,near start,script]\oc B_1}]{\point(a)
%         }},
%         {\wire[straight,wire=arrowed near start,wirelabel={[above,near start,script]\oc B_k}]{\point(b)
%         }}
%       }
%     }
%   }
%   \pdots[2.5pt](a)(b)
%   \drawbox[box={inner ysep=0pt,inner xsep=1pt},name=p] p
%   \init(a){
%     \wire[wire=railed]{\wire[bottom=10pt,inbox={},wire={arrowed,railed},wirelabel={[below,script,near start]\oc B_1}]{}}
%   }
%   \init(b){
%     \wire[wire=railed]{\wire[bottom=10pt,inbox={},wire={arrowed,railed},wirelabel={[above,script,near start]\oc B_k}]{}}
%   }
%   \end{proofnet}}
%   \\
%   \tikztarget(bottomleft){\normalsize dereliction\vphantom{g}}
%   &
%   contraction
%   &
%   weakening
%   &
%   box
%   \end{tabular}
% }
%
\subsection{Reduction}

The reduction rules are illustrated in Table~\ref{figure:reduction}. Notice that
the exponential reductions are required to operate on closed boxes (boxes
without auxiliary doors). $\red{er}$ and $\red{e}$ may be performed  at any
depth. All the other rules are only allowed at the surface: reduction inside boxes
is prohibited. 

\proofset{straight,bottom=5pt}
% \begin{gather*}
% \begin{aligned}
\begin{table}[tb]
\centering
\begin{minipage}{0.54\textwidth}
\centering
  $\begin{gathered}
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % multiplicative redex
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \tikztarget(multexp){\extm{multexp}{
    \begin{proofnet}[baseline=-.5ex]
      \init[grow=right]{
        \binary[bottom=2.5pt]{\parr}{
          \wire{}
        }{
          \wire{}
        }
      }
      \init[grow=left]{
        \binary[bottom=2.5pt]{\otimes}{
          \wire{}
        }{
          \wire{}
        }
      }
      \end{proofnet}
    \red m
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      % multiplicative reduct
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \begin{proofnet}[baseline=-.5ex,rotate=90]
      \draw (5pt,-10pt) -- ++(0,20pt);
      \draw (-5pt,-10pt) -- ++(0,20pt);
      \end{proofnet}
      \qquad\hspace{20pt}
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      % der vs box redex
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \begin{proofnet}[baseline=-.5ex]
      \init[grow=left]{
        \unary[flip]{\wn}{
        \boxpal{p}{
          \nary[shape=rectangle,cell={net={20pt}{12pt}}]{\pi}{}
        }
        }
      }
      \drawbox{p}
      \end{proofnet}
    \red e
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      %% der vs box reduct
      %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
      \begin{proofnet}[baseline=-.5ex]
      \init[grow=left]{
          \nary[shape=rectangle,cell={net={20pt}{12pt}}]{\pi}{}
      }
      \end{proofnet}
  }}
  \\[1ex]
  \tikzvcenter{\tikztarget(duperase){\extm{duperase}{
  \begin{proofnet}[baseline=-.5ex]
    \init[grow=right]{
      \binary{\wn}{\wire{}}{\wire{}}
    }
    \init[grow=left]{
      \boxpal[bottom=0pt]{p}{
        \nary[shape=rectangle,cell={net={17.5pt}{12pt}}]{\pi}{}
      }
    }
    \drawbox p
  \end{proofnet}
  \red {d} 
  \begin{proofnet}[baseline=-.5ex]
    \init[multi,grow=left,sep=8pt]{
      \boxpal[]{p}{
        \nary[shape=rectangle,cell={net={15pt}{12pt}}]{\pi}{}
      },
      \boxpal[]{q}{
        \nary[shape=rectangle,cell={net={15pt}{12pt}}]{\pi}{}
      }
    }
    \drawbox p
    \drawbox q
  \end{proofnet}
  \qquad\hspace{15pt}
  \begin{proofnet}[baseline=-.5ex]
    \init[grow=right]{
      \zeroary{\wn}
    }
    \init[grow=left]{
      \boxpal[bottom=0pt]{p}{
        \nary[shape=rectangle,cell={net={17.5pt}{12pt}}]{\pi}{}
      }
    }
    \drawbox p
    \end{proofnet}
  \red {er} 
  \epsilon
  }}}
  % \qquad
  % \tikzvcenter{\tikztarget(neutr){\extm{neutr}{
  % \begin{proofnet}[baseline=-.5ex]
  %   \init[grow=right]{
  %     \binary[very very small]{\wn}{\coord(c)}{\unary[very very small]{\wn}{\point(a)}}
  %   }
  %   \init(c){\wireupto(a){}}
  % \end{proofnet}
  % \red s
  % \begin{proofnet}[baseline=-.5ex,rotate=90]
  % \draw(0,0) -- ++(0,15pt);
  % \end{proofnet}
  % }}}
  \\[1ex]
  \tikzvcenter{\tikztarget(boxcompose){\extm{boxcompose}{
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % box vs box redex
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{proofnet}[baseline=-.5ex]
    \init[grow=left]{
      \boxpal{p}{
        \nary[shape=rectangle,cell={net={37.5pt}{12pt}}]{\pi}{
            \wire[inbox={}]{
              \boxpal q{
                \nary[shape=rectangle,cell={net={17.5pt}{12pt}},bottom=3pt]{\sigma}{
                  {\wire[wire=fake,inbox={},bottom=7.5pt]{\point(a)}}
                }
              }
            },,
          {
            \wireupto[straight,inbox={}](a){\coord(d)}
          },
          {
            \wireupto[straight,inbox={}](a){\coord(c)}
          }
      }
    }
    }
    \drawbox{p}
    \drawbox{q}
    \pdots[2pt](c)(d)
    \end{proofnet}
  \red c
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % box vs box reduct
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \begin{proofnet}[baseline=-.5ex]
    \init[grow=left]{
      \boxpal{p}{
        \nary[shape=rectangle,cell={net={37.5pt}{12pt}}]{\pi}{
            {\wire[inbox={},bottom=0pt]{
              \boxpal[] q{
                \nary[shape=rectangle,cell={net={17.5pt}{12pt}},bottom=3pt]{\sigma}{
                  {\wire[wire=fake,inbox={},bottom=12.5pt]{\point(a)}},
                }
              }
            }}
            ,,
          {
            \wireupto[straight,inbox={}](a){\coord(d)}
          },
          {
            \wireupto[straight,inbox={}](a){\coord(c)}
          }
      }
    }
    }
    \drawbox[inbox=p]{q}
    \drawbox{p}
    \pdots[2pt](c)(d)
    \end{proofnet}
  }}}
  %%%%%%
  \end{gathered}$
\end{minipage}
\begin{minipage}{0.44\linewidth}
  $\begin{gathered}
  % \qquad
  % \tikzvcenter{\tikztarget(weakborder){\extm{weakborder}{
  % \begin{proofnet}[baseline=-.5ex]
  %   \init[grow=right]{
  %     \binary[very very small,bottom=15pt]{\wn}{\wire[wire=fake]{\point(a)}}{}
  %   }
  %   \draw[railed] (7.5pt,12.5pt) coordinate (x)-- ++(0,-17.5pt) coordinate (y);
  %   \draw[densely dotted] (y) -- ++(0,-7.5pt);
  %   \draw (x)  -- ([xshift=-7.5pt]x-|a) coordinate (y);
  %   \draw[densely dotted] (y) -- (y-|a);
  % \end{proofnet}
  % \red s
  % \begin{proofnet}[baseline=-.5ex]
  %   \init[grow=right]{
  %     \binary[very very small]{\wn}{\wire[bottom=20pt,wire=fake]{\point(a)}}{}
  %   }
  %     \draw[railed] (22.5pt,12.5pt) coordinate (x)-- ++(0,-17.5pt) coordinate (y);
  %     \draw[densely dotted] (y) -- ++(0,-7.5pt);
  %     \draw (x) -- ([xshift=-7.5pt]x-|a) coordinate (y);
  %     \draw[densely dotted] (y) -- (y-|a);
  %   \end{proofnet}
  % }}}
  \tikztarget(choice){\extm{choice}{
    \begin{proofnet}[baseline=-.5ex]
      \init[grow=right]{\unary[flip]{\wn}{\binary{\oc}{\wire{}}{\wire{}}}}
    \end{proofnet}
    \red{nd} 
    \begin{proofnet}[baseline=-.5ex]
      \coordinate (m) at (-30pt,0);
      \init[grow=left,multi]{
        \unary{\wn}{\wireto(m){}},
        \zeroary{\wn}
      }
    \end{proofnet}
    +
    \begin{proofnet}[baseline=-.5ex]
      \coordinate (m) at (-30pt,0);
      \init[grow=left,multi]{
        \zeroary{\wn},
        \unary{\wn}{\wireto(m){}}
      }
    \end{proofnet}
    % \qquad
    % \begin{proofnet}[baseline=-.5ex]
    %   \init[grow=right]{\unary[flip]{\wn}{\zeroary{\oc}}}
    % \end{proofnet}
    % \red 0
    % 0
  }}
  \\[1ex]
  \tikztarget(bialgebra){\extm{bialgebra}{
    \begin{proofnet}[baseline=-.5ex]
      \init[grow=left]{\binary{\oc}{\wire{}}{\wire{}}}
      \init[grow=right]{\binary[bottom=0pt]{\wn}{\wire{}}{\wire{}}}
    \end{proofnet}
    \red {ba}
    \begin{proofnet}[baseline=-.5ex]
      \init[multi,grow=left]{
        {\binary{\oc}{\coord(a)}{\coord(b)}},
        {\binary{\oc}{\coord(c)}{\coord(d)}}
      }
      \ljoin ac[bottom=10pt,wires={,railed}]{\wn}{\wire{}}
      \rjoin bd[bottom=10pt,wires={railed,}]{\wn}{\wire{}}
    \end{proofnet}
    % &
  }}
  \\[1ex]
  \tikztarget(srules){\extm{srules}{
  \begin{aligned}
    \begin{proofnet}[baseline=-.5ex]
      \init[grow=left]{\zeroary{\oc}}
      \init[grow=right]{\binary[bottom=0pt]{\wn}{\wire{}}{\wire{}}}
    \end{proofnet}
    &\red {s_1}
    \begin{proofnet}[baseline=-.5ex]
      \init[multi,grow=left]{
        {\zeroary{\oc}},
        {\zeroary{\oc}}
      }
    \end{proofnet}
    &\hspace{20pt}
    \begin{proofnet}[baseline=-.5ex]
      \init[grow=left]{\binary{\oc}{\wire{}}{\wire{}}}
      \init[grow=right]{\zeroary[bottom=0pt]{\wn}}
    \end{proofnet}
    &\red {s_2}
    \begin{proofnet}[baseline=-.5ex]
      \init[multi,grow=right]{
        {\zeroary{\wn}},
        {\zeroary{\wn}}
      }
    \end{proofnet}
    \\
    \begin{proofnet}[baseline=-.5ex]
      \init[grow=left]{\zeroary{\oc}}
      \init[grow=right]{\zeroary[bottom=0pt]{\wn}}
    \end{proofnet}
    &\red \epsilon
    \epsilon
    \end{aligned}
  }}
  %%%%%%
  \end{gathered}$
\end{minipage}

\caption{Reduction rules}\label{figure:reduction}
\end{table}


%%%% OLD PART ON NON-SQUIGGLED ARROW AND STUFF %%%%% BEGIN 

% We define the structural reduction $\red s$ as the union of all rules, excepted
% the logical rules $\red m$ and $\red e$. The box reduction comprises the rules
% handling boxes : $\red{\text{box}} := \red e \cup \red d \cup \red{er} \cup \red
% c$.  Dually, $\red{\text{nbox}}$ is composed of all the rules except thes ones.
% Finally, we define the differential reduction as the union of all the
% aformentionned rules $\red {\text{diff}} := \red e \cup \red m \cup \red s$.
%
% % \newcommand*{\rred}[1]{\mathrel{\sur{\leftarrow}{\mathtt{#1}}}} % reversed red
% % many-steps reverse reduction
% % \newcommand*{\rredstar}[1]{\mathrel{^{\ast}{\sur{\leftarrow}{\mathtt{#1}}}}}
%
% The surface and closed reduction have a very strong commutation property as it
% does not contain any critical pair:
%
% \begin{property}{Diamond}\label{property-nets-diamond}\\
%   The rewriting relation $\redsurf$ has the diamond property: If
%   $\net{R}'
%   \rred{\text{diff}} \net{R} \redsurf \net{R}''$, then there exists
%   $\net S$ such that $\net{R}' \redsurf \net{S} \rred{\text{diff}}
%   \net{R}''$
% \end{property}
%
% In the context of non correct nets, where termination is not assured, the diamond
% property implies the following important fact:
%
% \begin{mcor}{Termination}\label{mcor-nets-termination}\\
%   A net is weakly normalizing if and only if it is strongly normalizing
% \end{mcor}
%

%%%% OLD PART ON NON-SQUIGGLED ARROW AND STUFF %%%%% END 

%%%% OLD SUBSECTION : rednsurf REDUCTION %%%%
% \subsection{Equivalence relation and $\rednsurf$ reduction}
We quotient the proof nets by associativity and commutativity of contraction and
cocontractions. We also include in the relation the neutrality of (co)weakening for
(co)contraction (Table~\ref{figure:equivalence}).
\proofset{straight,bottom=5pt}
% \begin{gather*}
% \begin{aligned}
\begin{table}[tb]
\centering
$\begin{gathered}
\\[2ex]
\tikztarget(equivwn){\extm{equivwn}{
\begin{proofnet}[baseline=-.5ex]
  \init[grow=right]{
    \binary{\wn}{\wire{}}{\wire{}}
  }
\end{proofnet}
  \equiv
\begin{proofnet}[baseline=-.5ex]
  \init[grow=right]{
    \binary{\wn}{\wire[bottom=10pt,straight=false,shift=11pt]{}}{\wire[bottom=10pt,straight=false,shift=-11pt,wire=railed]{}}
  }
\end{proofnet}
\quad\quad %SEP
\begin{proofnet}[baseline=-.5ex]
  \init[grow=right]{
    \binary{\wn}{\binary{\wn}{\wire{\point(a)}}{\wire{}}}{\coord(c)}
  }
  \init(c){\wireupto(a){}}
\end{proofnet}
  \equiv
\begin{proofnet}[baseline=-.5ex]
  \init[grow=right]{
    \binary{\wn}{\coord(c)}{\binary{\wn}{\wire{\point(a)}}{\wire{}}}
  }
  \init(c){\wireupto(a){}}
\end{proofnet}
\quad\quad %SEP
  \begin{proofnet}[baseline=-.5ex]
    \init[grow=right]{
      \binary{\wn}{\zeroary[name=weak]{\wn}}{\wireupto(weak.middle pax){}}
    }
  \end{proofnet}
\equiv
  \begin{proofnet}[baseline=-.5ex,rotate=90]
    \draw (0pt,-10pt) -- ++(0,20pt);
  \end{proofnet}
}}
\\[2ex]
\tikztarget(equivoc){\extm{equivoc}{
\begin{proofnet}[baseline=-.5ex]
  \init[grow=right]{
    \binary{\oc}{\wire{}}{\wire{}}
  }
\end{proofnet}
  \equiv
\begin{proofnet}[baseline=-.5ex]
  \init[grow=right]{
    \binary{\oc}{\wire[bottom=10pt,straight=false,shift=11pt]{}}{\wire[bottom=10pt,straight=false,shift=-11pt,wire=railed]{}}
  }
\end{proofnet}
\quad\quad%SEP
\begin{proofnet}[baseline=-.5ex]
  \init[grow=right]{
    \binary{\oc}{\binary{\oc}{\wire{\point(a)}}{\wire{}}}{\coord(c)}
  }
  \init(c){\wireupto(a){}}
\end{proofnet}
  \equiv
\begin{proofnet}[baseline=-.5ex]
  \init[grow=right]{
    \binary{\oc}{\coord(c)}{\binary{\oc}{\wire{\point(a)}}{\wire{}}}
  }
  \init(c){\wireupto(a){}}
\end{proofnet}
\quad\quad %SEP
  \begin{proofnet}[baseline=-.5ex]
    \init[grow=right]{
      \binary{\oc}{\zeroary[name=weak]{\oc}}{\wireupto(weak.middle pax){}}
    }
  \end{proofnet}
\equiv
  \begin{proofnet}[baseline=-.5ex,rotate=90]
    \draw (0pt,-10pt) -- ++(0,20pt);
  \end{proofnet}
}}
\end{gathered}$
\caption{Equivalence relation}\label{figure:equivalence}
\end{table}

%%%% OLD SUBSECTION : rednsurf REDUCTION %%%% BEGIN
% \subsection{Equivalence relation and $\rednsurf$ reduction}
% However, requiring all our rules to be surface turns out to be too restrictive
% for our purpose. More specifically, we need to handle the following cases:
%
% \begin{itemize}
%   \item (Garbage Collection). When a variable is not free in the body of an
%     abstraction, the substituted value is erased in the calculus. However, in
%     the term's translation the corresponding weakening is located inside an
%     exponential box. The weakening/bang corresponding redex is then locked and
%     can't be reduced until the box is opened or erased. Then only, all the
%     accumulated garbage become be available to
%     collection. We wish to avoid managing all these superfluous garbage and
%     perform directly erasure $\red{er}$ inside boxes: 
%
%     \begin{center}
%     $\begin{gathered}
%     \tikzvcenter{\tikztarget(boxequiv){\extm{boxequiv}{
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % Equiv weak-box - redex 
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \begin{proofnet}[baseline=-.5ex]
%       \init[multi,grow=left,sep=15pt]{
%         {\boxpal[name=ppal,cell={right=8pt}]{p}{
%             \nary[name=pi,shape=rectangle,cell={net={20pt}{12pt}}]{\pi}{
%               \wire[inbox={}]{\coord(pia)},
%               \wire[inbox={}]{\coord(pib)}
%             }
%         }},
%         {\flipped[inbox={p},name=weak1]{\wn}{}{
%           \boxpal[inbox={p}]{sn}{
%             \nary[name=sigman,shape=rectangle,cell={net={20pt}{12pt}}]{\sigma_n}{
%               {\wire[wire=fake,inbox={},bottom=12.5pt]{\point(a)}},
%               {\wire[wire=fake,inbox={},bottom=12.5pt]{\point(b)}}
%             }
%           }
%         }},
%         {\flipped[inbox={p},name=weak2]{\wn}{}{
%             \boxpal[inbox={p}]{s1}{
%             \nary[name=sigma1,shape=rectangle,cell={net={20pt}{12pt}}]{\sigma_1}{}
%           }
%         }}
%       }
%       \addtobox{p}(pi)
%       \addtobox{p}(s1)
%       \pdots[2.5pt](sigman)(sigma1)
%       \drawbox[name=s1]{s1}
%       \drawbox[name=sn]{sn}
%       \drawbox[box={inner ysep=8pt,inner xsep=5pt},name=p]{p}
%       \init(pia){
%         \wireupto(a){}
%       }
%       \init(pib){
%         \wireupto(a){}
%       }
%       \inetwire(ppal.pal)([xshift=-13pt]ppal.pal)
%     \end{proofnet}
%     \rednsurf
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % Equiv weak-box - reduct
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     \begin{proofnet}[baseline=-.5ex]
%       \init[grow=left]{
%         \boxpal{p}{
%           \nary[shape=rectangle,cell={net={20pt}{12pt}}]{\pi}{
%             \wire{\coord(pia1)},
%             \wire{\coord(pia2)}
%           }
%         }
%       }
%       \init(pia1){
%         \wire{\wire{}}
%       }
%       \init(pia2){
%         \wire{\wire{}}
%       }
%     \drawbox{p}
%     \end{proofnet}
%     }}}
%     \end{gathered}$
%     \end{center}
%
%   \item (Proxy variable). If a variable does appear, as in $\varss{x \mapsto
%     V}{x}$, we encounter a similar limitation of surface reduction. We would
%     like to perform (linear) substitution deep inside terms, which correspond  
%     to allow opening boxes by applying $\red{o}$ at any depth:
%     \begin{center}
%     $\begin{gathered}
%     \tikzvcenter{\tikztarget(boxequiv){\extm{boxequiv}{
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % Equiv closed-box - redex
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       \begin{proofnet}[baseline=-.5ex]
%         \init[grow=left]{
%           \boxpal[name=ppal,cell={right=8pt}]{p}{
%             \unary[name=der1,flip]{\wn}{
%               \boxpal[inbox={p}]{q}{
%                 \nary[name=pi,shape=rectangle,cell={net={20pt}{12pt}}]{\pi}{}
%               }
%             }
%           }
%         }
%         \addtobox{p}(pi)
%         \drawbox[name=q]{q}
%         \drawbox[box={inner ysep=8pt,inner xsep=5pt},name=p]{p}
%         \inetwire(ppal.pal)([xshift=-13pt]ppal.pal)
%       \end{proofnet}
%       \rednsurf
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     % Equiv closed-box - reduct
%     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%       \begin{proofnet}[baseline=-.5ex]
%         \init[grow=left]{
%           \boxpal{p}{
%             \nary[shape=rectangle,cell={net={20pt}{12pt}}]{\pi}{}
%           }
%         }
%         \drawbox{p}
%       \end{proofnet}
%     }}}
%     \end{gathered}$
%     \end{center}
% \end{itemize}
%%%% OLD SUBSECTION : rednsurf REDUCTION %%%% END

% Adding these two rules breaks the diamond property, as a reduction inside a box
% can not commute in one step with the duplication of the box which unvoidably
% duplicate all the redexes inside it. But the crucial properties required for our
% rewriting, confluence and the fact that weakly normalization
% implies strong normalization, are actually preserved as developped in the the
% coming subsection.

%%%% OLD STUFF : SQUIGGLED ARROW %%%% END

%%%% OLD STUFF : INTEGRATING LEADS TO THE REDUCTION %%% BEGIN

We denote by $\to$ the full reduction, extended to sums of nets in the same way
as in~\cite{ehrhard:hal-00150274}.

\begin{theorem}{Confluence}\label{theorem-nets-confluence}\\
  The reduction $\to$ is confluent.
\end{theorem}

%%%%%%%%%%%%%%%%%%%% --- EXTENDED --- %%%%%%%%%%%%%%%%%%%
\begin{proof}
  The reduction is similar in spirit to an orthogonal reduction in a term
  rewriting system.  In the same approach as the proof of confluence of the
  $\lambda$-caluclus, we can define a parallel reduction $\redpar$, which allow
  to perform an abritrary number of step in parallel (meaning that we can't
  reduce redexes that are created by other the other steps). This parallel
  reduction verifies $\to \subseteq
  \redpar \subseteq \to^\ast$. Then we prove that $\redpar$ has the diamond
  property, and the previous expression ensures that $\to^\ast \subseteq
  \redpar^\ast$, thus $\to^\ast$ is confluent.
\end{proof}

\subsection{Termination}
%%%%%%%%%%%%%%%%%% --- END EXTENDED --- %%%%%%%%%%%%%%%%%

\begin{theorem}\label{theorem-nets-termination}
  A net is weakly normalizing if and only if it is strongly
  normalizing.
\end{theorem}

%%%%%%%%%%%%%%%%%%%% --- EXTENDED --- %%%%%%%%%%%%%%%%%%%

\newcommand{\redsurf}{\rightharpoonup}
\newcommand{\redsurfinv}{\leftharpoonup}
\newcommand{\rednsurf}{\leadsto}
\newcommand{\rednsurfinv}{\leftharpoondown}
\tikzset{
  equiv/.style={
    draw=none,
    edge node={node [sloped, allow upside down, auto=false]{$\rednsurf^\ast$}}},
  equiv1step/.style={
    draw=none,
    edge node={node [sloped, allow upside down, auto=false]{$\rednsurf$}}},
  equiv01step/.style={
    draw=none,
    edge node={node [sloped, allow upside down,
      auto=false]{$\underline{\rednsurf}$}}},
  equivkstep/.style={
    draw=none,
    edge node={node [sloped, allow upside down,
      auto=false]{$\rednsurf^k$}}},
  equivkpstep/.style={
    draw=none,
    edge node={node [sloped, allow upside down,
    auto=false]{$\rednsurf^{k'}$}}},
  equals/.style={
    draw=none,
    edge node={node [sloped, allow upside down, auto=false]{$=$}}},
  reduceto/.style={
    draw=none,
    edge node={node [sloped, allow upside down, auto=false]{$\redsurf^\ast$}}},
  reduceto1step/.style={
    draw=none,
    edge node={node [sloped, allow upside down, auto=false]{$\redsurf$}}},
  reduceto1pstep/.style={
    draw=none,
    edge node={node [sloped, allow upside down, auto=false]{$\redsurf^+$}}},
  reducetokstep/.style={
    draw=none,
    edge node={node [sloped, allow upside down, auto=false]{$\redsurf^k$}}},
  reducetokpstep/.style={
    draw=none,
    edge node={node [sloped, allow upside down, auto=false]{$\redsurf^{k'}$}}}
}

To prove Theorem~\ref{theorem-nets-termination}, we proceed in two steps. First, we
consider the system where all reductions are restricted to the surface.
This reduction is constrained enough so that it verifies the diamond
property, which is known to implies the 
Theorem~\ref{theorem-nets-termination}. Then, we consider the non-surface
$\red{er}$ and $\red{e}$ reductions, that we write $\rednsurf$, and show that
adding it to $\redsurf$ does not invalid the theorem. In this subsection, we denote by
$\redsurf$ all the reductions rules of Figure~\ref{figure:reduction} applied
at the surface. We have the decomposition $\to$ = $\redsurf \cup \rednsurf$.
The following lemma shows that $\redsurf$ and $\rednsurf$ have a 
commutation property:

\begin{lemma}{Swapping}\label{lemma-nets-swapping}\\
  Let $\mathcal{S} \rednsurf^\ast \mathcal{R}$ and $\mathcal{R} \redsurf^+ \mathcal{R}'$. Then
  there exists $\mathcal{S'}$ such that

  \begin{center}
    \begin{tikzpicture}
      \matrix (m) [matrix of math nodes,row sep=2em,column sep=2em,minimum
        width=2em] 
      {
        \mathcal{R} & \mathcal{R}' \\
        \mathcal{S} & \mathcal{S'} \\
      };
      \path[-stealth, auto]
        (m-1-1) edge[reduceto1pstep] (m-1-2)
        (m-2-1) edge[reduceto1pstep] (m-2-2)
        (m-2-1) edge[equiv] (m-1-1)
        (m-2-2) edge[equiv] (m-1-2);
    \end{tikzpicture} 
  \end{center}
\end{lemma}

\begin{proof}Lemma~\ref{lemma-nets-swapping}\\
  By induction on both the length of the reduction $\mathcal{S} \rednsurf^\ast
  \mathcal{R}$ and $\mathcal{R} \to^+ \mathcal{R}'$. We consider the
  fundamental case where both reductions are one-step : 
  
  \begin{center}
    \begin{tikzpicture}
      \matrix (m) [matrix of math nodes,row sep=2em,column sep=2em,minimum
        width=2em] 
      {
        \mathcal{R} & \mathcal{R}' \\
        \mathcal{S} & \\
      };
      \path[-stealth, auto]
        (m-1-1) edge[reduceto1step] (m-1-2)
        (m-2-1) edge[equiv1step] (m-1-1);
    \end{tikzpicture} 
  \end{center}

  We make the following remarks:
  \begin{itemize}
    \item As $\rednsurf$ reduction happens inside boxes, and $\redsurf$ outside,
      we can put in a one-to-one correspondence the boxes at depth 0 - and thus
      the $\redsurf$-redexes - of $\mathcal{R}$ and $\mathcal{S}$ 
    \item If the reduction in $\mathcal{R}$ does not involve a box, it does not interact with
      $\rednsurf$, and the diagram can be closed as a square with one step reduction in every
      direction
    \item If the reduction in $\net R$ erases a box, we can erase the
      corresponding one in $\mathcal{S}$, which may delete the $\rednsurf$ redex
      involved reduced in $\net S$.  In any case we can reduce $\mathcal{S}$ to
      $\mathcal{S}'$ in one step by erasing this box and $\mathcal{S}'$ to
      $\mathcal{R}'$ by at most one $\rednsurf$ step.
    \item If the reduction in $\net R$ opens a box, we can open the
      corresponding one in $\net S$. If the $\rednsurf$-redex was at depth $1$
      in the same box, then it becomes a $\redsurf$-redex as it now appears at
      the surface. Otherwise, it can be performed in one $\rednsurf$ step. In
      any case, we can close the diagram by peforming either one $\redsurf$ step
      followed by one $\rednsurf$ step, or two $\redsurf$ steps.
  \end{itemize}

  In the cases listed above, the length of the reduction between
  $\mathcal{R}'$ and $\mathcal{S}'$ never exceeds one, hence we can always
  fill the following diagram :
    
    \begin{center}
      \begin{tikzpicture}
        \matrix (m) [matrix of math nodes,row sep=2em,column sep=2em,minimum
          width=2em] 
        {
          \mathcal{R} & \mathcal{R}' \\
          \mathcal{S} & \mathcal{S'} \\
        };
        \path[-stealth, auto]
          (m-1-1) edge[reduceto1step] (m-1-2)
          (m-2-1) edge[reduceto1pstep] (m-2-2)
          (m-2-1) edge[equiv1step] (m-1-1)
          (m-2-2) edge[equiv01step] (m-1-2);
      \end{tikzpicture} 
    \end{center}
  
  Where the bottom line does not involve duplication
  ($\mathcal{S}' \underline{\rednsurf} \mathcal{R}'$ if $\mathcal{S}' =
  \mathcal{R}'$ or $\mathcal{S'} \rednsurf \mathcal{R}'$).

  \begin{itemize}
    \item Duplication is the only $\redsurf$ reduction that can create new
      $\rednsurf$ redexes, but the bottom $\redsurf$ reduction requires exactly
      one step in $\mathcal{S}$. This corresponds to the
      following diagram: 
      
      \begin{center}
        \begin{tikzpicture}
          \matrix (m) [matrix of math nodes,row sep=2em,column sep=2em,minimum
            width=2em] 
          {
            \mathcal{R} & \mathcal{R}' \\
            \mathcal{S} & \mathcal{S'} \\
          };
          \path[-stealth, auto]
            (m-1-1) edge[reduceto1step] (m-1-2)
            (m-2-1) edge[reduceto1step] (m-2-2)
            (m-2-1) edge[equiv1step] (m-1-1)
            (m-2-2) edge[equiv] (m-1-2);
        \end{tikzpicture} 
      \end{center}
  \end{itemize}

  Let us now prove the lemma. We consider the two cases separately : let us assume that $\mathcal{R}
  \redsurf \mathcal{R'}$ is not a duplication.  We perform an induction
  on the length of the reduction $\mathcal{S} \rednsurf^k \mathcal{R}$. The
  induction hypothesis is that we can always fill the following diagram

  \begin{center}
      \begin{tikzpicture}
        \matrix (m) [matrix of math nodes,row sep=2em,column sep=2em,minimum
          width=2em] 
        {
          \mathcal{R} & \mathcal{R}' \\
          \mathcal{S} & \mathcal{S'} \\
        };
        \path[-stealth, auto]
          (m-1-1) edge[reduceto1step] (m-1-2)
          (m-2-1) edge[reduceto] (m-2-2)
          (m-2-1) edge[equivkstep] (m-1-1)
          (m-2-2) edge[equivkpstep] (m-1-2);
      \end{tikzpicture} 
  \end{center}

  With $k' \leq k$, and where the bottom reduction does not contain any
  duplication step.  The base case $k=0$ is trivially true. For the induction
  step, if we have $\mathcal{S} \rednsurf^k \mathcal{T} \rednsurf \mathcal{R}$,
  we use the first diagram of the remarks to get the middle line $T \redsurf^\ast
  T_p$.  Then, we apply the induction hypothesis on each reduction step $T_i \to
  T_{i+1}$, which we can do precisely because our IH states that the lengths
  $k_i$ of each reduction $S_i \rednsurf^{k_i} T_i$ verify $k_i \leq k_{i-1}
  \leq \ldots \leq k$. We paste all the diagrams and get 

  \begin{center}
      \begin{tikzpicture}
        \matrix (m) [matrix of math nodes,row sep=3em,column sep=1em,minimum
          width=1em] 
        {
          \mathcal{R} & & & \mathcal{R}' \\
          \mathcal{T} & \mathcal{T}_1 & \phantom{|}\ldots & \mathcal{T}_p \\
          \mathcal{S} & \mathcal{S}_1 & \phantom{|}\ldots & \mathcal{S}_p \\
        };
        \path[-stealth, auto]
          (m-1-1) edge[reduceto1step] (m-1-4)
          (m-2-1) edge[reduceto1step] (m-2-2)
          (m-2-2) edge[reduceto1step] (m-2-3)
          (m-2-3) edge[reduceto1step] (m-2-4)
          (m-3-1) edge[reduceto1step] (m-3-2)
          (m-3-2) edge[reduceto1step] (m-3-3)
          (m-3-3) edge[reduceto1step] (m-3-4)
          (m-2-1) edge[equiv1step] (m-1-1)
          (m-2-4) edge[equiv01step] (m-1-4)
          (m-3-1) edge[equiv] (m-2-1)
          (m-3-2) edge[equiv] (m-2-2)
          (m-3-4) edge[equiv] (m-2-4);
      \end{tikzpicture} 
  \end{center}

  The case of duplication is simpler as the step $\mathcal{R} \redsurf \mathcal{R}'$
  is reflected by just one step $\mathcal{S} \redsurf \mathcal{S}'$ in the second
  diagram of the remarks. Our IH is now that we can fill the diagram, without
  further assertion on the length of the $\rednsurf$ reduction. Indeed, if $\mathcal{S} \rednsurf^k \mathcal{T}
  \rednsurf \mathcal{R}$, we use the one-step diagram to get $\mathcal{T}'$ and
  apply the IH to fill the bottom part with $\mathcal{S}'$ : 

  \begin{center}
      \begin{tikzpicture}
        \matrix (m) [matrix of math nodes,row sep=2em,column sep=2em,minimum
          width=2em] 
        {
          \mathcal{R} & \mathcal{R}' \\
          \mathcal{T} & \mathcal{T}' \\
          \mathcal{S} & \mathcal{S}' \\
        };
        \path[-stealth, auto]
          (m-1-1) edge[reduceto1step] (m-1-2)
          (m-2-1) edge[reduceto1step] (m-2-2)
          (m-3-1) edge[reduceto1step] (m-3-2)
          (m-2-1) edge[equiv1step] (m-1-1)
          (m-3-1) edge[equivkstep] (m-2-1)
          (m-2-2) edge[equiv] (m-1-2)
          (m-3-2) edge[equiv] (m-2-2);
      \end{tikzpicture} 
  \end{center}

  Finally, we can perform a second induction on the length of the reduction
  $\mathcal{R} \to^+ \mathcal{R}'$ to get the final result.
\end{proof}

Writing a reduction $\net R \to^\ast S$ as blocks $\net R \rednsurf^\ast R_1
\redsurf^\ast R_2 \rednsurf^\ast \ldots \redsurf^\ast R_n$,
we can iterate Lemma~\ref{lemma-nets-swapping} to form a new reduction sequence with
only two distinct blocks:

\begin{lemma}{Standardization}\label{lemma-nets-standardization}\\
  Let $\net R \to^\ast \net S$. Then $\net R \redsurf^\ast \net{R}'
  \rednsurf^\ast \net S$. Moreover, if the original reduction contains at least
  one $\redsurf$ step, then $\net{R} \redsurf^+ \net{R}'$.
\end{lemma}

\begin{proof}Lemma~\ref{lemma-nets-standardization}\\
This follows from the previous lemma: we decompose the reduction $\net R
\to^\ast S$ as blocks $\net R \rednsurf^\ast R_1 \redsurf^\ast R_2
\rednsurf^\ast \ldots \redsurf^\ast R_n$, and iterate
\ref{lemma-nets-swapping} to gather the reductions into only two distinct
blocks.
\end{proof}

Lemma~\ref{lemma-nets-rednsurf-neutrality} follows from
the observation that as $\redsurf$ only acts on surface and $\rednsurf$
inside boxes, the latter can not interact with the redexes of the former.

\begin{lemma}{Neutrality of $\rednsurf$}\label{lemma-nets-rednsurf-neutrality}\\
  $\rednsurf$ does not create nor erase $\redsurf$-redexes. In
  particular, if $\net R \rednsurf^\ast \net{R}'$, then $\net{R}$ is
  $\redsurf$-normal if and only if $\net{R}'$ is.
\end{lemma}

We also need some properties about termination of the reduction $\redsurf$ and
$\rednsurf$ :

\begin{lemma}{Strong normalization for $\rednsurf$}\label{lemma-nets-termination-nsurf}\\
  $\rednsurf$ is strongly normalizing.
\end{lemma}

\begin{proof}
  It suffices to note that opening or deleting a box strictly decreases the
  total number of boxes in the net.
\end{proof}

\begin{lemma}\label{lemma-nets-termination-surf}
  Theorem~\ref{theorem-nets-termination} is true when replacing $\to$ with
$\redsurf$.
\end{lemma}

\begin{proof}
  The surface reduction satisfies the diamond property,
  which excludes the existence of a weakly normalizing term with an
  infinite reduction.
\end{proof}

We can finally prove Theorem~\ref{theorem-nets-termination}:

\begin{proof}Theorem~\ref{theorem-nets-termination}\\
  We prove two auxiliary properties:
\begin{description}
  \item[(a)] \textbf{$\to$-weak normalization implies $\redsurf$-weak
    normalization} \\
    Let $\net R$ be $\to$-weakly normalizing, $\net R \to^\ast \net N$ a
    reduction to its normal form. By \ref{lemma-nets-standardization}, we can write
    $\net R \redsurf^\ast \net S \rednsurf^\ast N$. $N$ being a
    $\to$-normal form, it is also a $\redsurf$-normal form, and by
    \ref{lemma-nets-rednsurf-neutrality} so is $\net S$. $\net R$ is thus a
    $\redsurf$-weakly normalizing.
  \item[(b)] \textbf{an infinite $\to$-reduction gives an infinite
    $\redsurf$-reduction}\\
    Let $\net R$ be a net with an infinite reduction, written $\net R \to^\ast
    \infty$. We will prove by induction that for any $n \geq 0$, there exists
    $\net{R}_n$ such that $R \redsurf^n \net{R}_n \to^\ast \infty$.
    \begin{itemize}
      \item Case $n = 0$\\
        We just take $\net{R}_0 = \net R$
      \item Inductive case\\ If $\net R \redsurf^n \net{R}_n \to^\ast \infty$,
        we take any infinite reduction starting from $\net{R}_n$. If the first
        step is $\net{R}_n \redsurf \net S$, then we take $\net{R}_{n+1} = \net
        S$. Otherwise, the first step is a $\rednsurf$ step, and we take the
        maximal block of $\rednsurf$ reduction starting from $\net{R}_n$. By
        \ref{lemma-nets-termination-nsurf}, this block must indeed be finite and we can write $\net{R}_n
        \rednsurf^\ast \net S \redsurf \net{S}' \to \infty$. By \ref{lemma-nets-swapping},
        we can swap the two blocks such that $\net{R}_n \redsurf \net{R}'
        \redsurf^\ast
        \net{R}'' \rednsurf^\ast \net{S}'$, and we take $\net{R}_{n+1} =
        \net{R}'$.
    \end{itemize}
\end{description}
From these two points follows that $\to$-weak normalization implies $\to$-strong
normalization. If a net is $\to$-weakly normalizing, then it is
$\redsurf$-weakly normalizing by (a). By
\ref{lemma-nets-termination-surf}, it is also $\redsurf$-strongly normalizing.
But by (b) it must be also $\to$-strongly normalizing.
\end{proof}
%%%%%%%%%%%%%%%%%% --- END EXTENDED --- %%%%%%%%%%%%%%%%%

%
% Summing up: 
% \begin{itemize}
%   \item A $\to$-weakly normalizing net is also $\redsurf$-weakly
%     normalizing.
%   \item Using the termination property for $\redsurf$, a $\redsurf$-weakly normalizing net is
%     $\redsurf$-strongly normalizing.
%   \item On the other hand, an infinite $\to$-reduction of a net $\net R$ can be
%     transformed to an infinite $\redsurf$-reduction using
%     \ref{lemma-nets-standardization}. Thus, a $\redsurf$-strongly normalizing
%     term must actually be $\to$-strongly normalizing.
% \end{itemize}
%
% From which we can conclude:
%
% \begin{theorem}{Termination for $\to$}\label{theorem-nets-termination}\\
%   A net is $\to$-weakly normalizing if and only if it is $\to$-strongly
%   normalizing.
% \end{theorem}
%
The next section focuses on a specific family of proof nets that play a key role
in the expression of communication primitives inside proof nets.

% \subsection{Integrating $\rednsurf$ to the reduction} % $\redsurf$ and $\rednsurf$}
%
% \tikzset{
%   equiv/.style={
%     draw=none,
%     edge node={node [sloped, allow upside down, auto=false]{$\rednsurf^\ast$}}},
%   equiv1step/.style={
%     draw=none,
%     edge node={node [sloped, allow upside down, auto=false]{$\rednsurf$}}},
%   equiv01step/.style={
%     draw=none,
%     edge node={node [sloped, allow upside down,
%       auto=false]{$\underline{\rednsurf}$}}},
%   equivkstep/.style={
%     draw=none,
%     edge node={node [sloped, allow upside down,
%       auto=false]{$\rednsurf^k$}}},
%   equivkpstep/.style={
%     draw=none,
%     edge node={node [sloped, allow upside down,
%     auto=false]{$\rednsurf^{k'}$}}},
%   equals/.style={
%     draw=none,
%     edge node={node [sloped, allow upside down, auto=false]{$=$}}},
%   reduceto/.style={
%     edge node={node[above right=0.5pt and 1.4em] {$\ast$}}},
%   reducetolong/.style={
%     edge node={node[above right=0.5pt and 4.35em] {$\ast$}}}
% }
%
% \newcommand{\redpar}{\Leftrightarrow}
%
% Confluence of $\to$ comes from the fact it is morally ``orthogonal''. We don't
% attempt at giving a definition of orthogonality, but one can define a parallel
% % relation $\redpar$ such that $\to \subseteq \redpar \subseteq \to^\ast$ and
% $\redpar$ enjoys the diamond property. As in the $\lambda$-calculus, we can
% conclude:
%
% \begin{theorem}{Confluence}\label{theorem-nets-confluence}\\
%   $\to$ is confluent.
% \end{theorem}
%
% % \begin{definition}{Parallel reduction}\label{definition-nets-parallel-reduction}\\
% %   The parallel reduction $\redpar$ is defined on nets as follow :
% % \end{definition}
% %
% % \begin{lemma}{$\redpar$ and $\to$}\label{lemma-nets-parallel-inclusion}\\
% %   We have $\to \subset \redpar \subset \to^\ast$.
% % \end{lemma}
% %
% % \begin{proof}\ref{lemma-nets-parallel-inclusion}\\
% % The inclusion $\to \subset \redpar$ is immediate. For the second, we proceed by
% % induction on the redex.
% % \end{proof}
% %
% % \begin{lemma}{Diamond for $\redpar$}\label{lemma-nets-parallel-diamond}\\
% %   $\redpar$ has the diamond property.
% % \end{lemma}
% %
% % \begin{proof}\ref{lemma-nets-parallel-diamond}\\
% %   TODO
% % \end{proof}
% %
% % We can conclude since by \ref{lemma-nets-parallel-inclusion}, we have
% % $\redpar^\ast = \to^\ast$, and the former is confluent by
% % \ref{lemma-nets-parallel-diamond}.
% %
%
% On the equivalence of weak and strong normalization, we already know that a
% $\redsurf$-weakly normalizing term is $\redsurf$-strongly normalizing. The
% main fact to rely on is that $\rednsurf$ interact nicely with
% $\redsurf$, as we can swap two consecutive blocks
% (\ref{lemma-nets-swapping}) of these reductions. Moreover $\rednsurf$ does not
% create nor erase $\redsurf$ redexes.
%
% \newcommand{\netenv}[1]{
%   \begin{center}
%     $\begin{gathered}
%       \tikzvcenter{
%         #1
%       }
%     \end{gathered}$
%   \end{center}
% }
%
% \begin{lemma}{Swapping}\label{lemma-nets-swapping}\\
%   Let $\mathcal{S} \rednsurf^\ast \mathcal{R}$ and $\mathcal{R} \to \mathcal{R}'$. Then
%   there exists $\mathcal{S'}$ such that
%
%   \begin{center}
%     \begin{tikzpicture}
%       \matrix (m) [matrix of math nodes,row sep=3em,column sep=4em,minimum
%         width=2em] 
%       {
%         \mathcal{R} & \mathcal{R}' \\
%         \mathcal{S} & \mathcal{S'} \\
%       };
%       \path[-stealth, auto]
%         (m-1-1) edge[reduceto] (m-1-2)
%         (m-2-1) edge[reduceto] (m-2-2)
%         (m-2-1) edge[equiv] (m-1-1)
%         (m-2-2) edge[equiv] (m-1-2);
%     \end{tikzpicture} 
%   \end{center}
% \end{lemma}
%
% Writing a reduction $\net R \to^\ast S$ as blocks $\net R \rednsurf^\ast R_1
% \redsurf^\ast R_2 \rednsurf^\ast \ldots \redsurf^\ast R_n$, we
% can iterate \ref{lemma-nets-swapping} to form a new reduction sequence with only
% two such blocks:
%
% \begin{lemma}{Standardization}\label{lemma-nets-standardization}\\
%   Let $\net R \to^\ast \net S$. Then $\net R {\redsurf}^\ast \net{R}'
%   \rednsurf^\ast \net S$. Moreover, if the original reduction contains at least
%   one $\redsurf$ step, then $\net{R} \redsurf^+ \net{R}'$.
% \end{lemma}
%
% Summing up: 
% \begin{itemize}
%   \item A $\to$-weakly normalizing net is also $\redsurf$-weakly
%     normalizing.
%   \item Using the termination property for $\redsurf$, a $\redsurf$-weakly normalizing net is
%     $\redsurf$-strongly normalizing.
%   \item On the other hand, an infinite $\to$-reduction of a net $\net R$ can be
%     transformed to an infinite $\redsurf$-reduction using
%     \ref{lemma-nets-standardization}. Thus, a $\redsurf$-strongly normalizing
%     term must actually be $\to$-strongly normalizing.
% \end{itemize}
%
% From which we can conclude:
%
% \begin{theorem}{Termination for $\to$}\label{theorem-nets-termination}\\
%   A net is $\to$-weakly normalizing if and only if it is $\to$-strongly
%   normalizing.
% \end{theorem}
%
%%%% OLD STUFF : INTEGRATING LEADS TO THE REDUCTION %%% END


==> paper-csl-long arxiv/parts/properties-termination.tex <==
\subsection{Termination}
\label{sec:lces-props:termination}

We proceed by reducibility. In this whole part, we will tune the reduction so
that the \rrulet{subst-r}{get} reduction becomes non-determinstic : instead of producing a
sum, one chose one term among the summands to be the reduct. We will prove
termination for this reduction, from which termination for the original one follows easily.
We first need to lay some definitions

\paragraph{}

The following definition attempts at formalizing the behavior of a term in an
"environment", ie as a subterm of a bigger one, where it can be exposed to
arbitrary incoming downward substitutions references. The usual defintion of
strongly computable terms for simply typed lambda calculus is not sufficient to
prove termination, because here separate subterms can affect each other
through references substitutions. Thus we need to add a property to the definition of SC
terms, namely that they are well-behaved when we put them in an environment of
other well-behaved terms : they only emit a finite number of strongly computable
terms.

An environment reduction abstract the enclosing context just as a sequence of
incoming downard substitutions.

\begin{mdef}{Environment reduction}\label{mdef-env-reduction}\\
  Let $\vdash M : (\alpha,e)$ be well typed (simple) term, Let $\seq{\multv{V}}$
  be a sequence of references substitutions such that $\refrawsd{}{\multv{V}_i}{M}$ is well typed that we write
  $\vdash (M,\seq{\multv{V}})$.  We call a $(M,\seq{\multv{V}})$-reduction a finite
  or infinite reduction sequence starting from $M$ where each rule is either a
  usual one or a rule $\to_i$ defined by $M \to_i
  \refrawsd{}{\multv{V}_i}{M}$.
\end{mdef}

We will also make use of another tool that compares two terms that have
essentially the same structure but differ in their downard references
substitutions. The main point is that if a term $M$ has more substitutions
available than $N$, then any reduction than can be performed in $N$ can be
performed in $M$. In particular, if $M$ is strongly normalizable, then so is
$N$.

\begin{mdef}{Reachability and associated pre-order}\\
  Let $M$ be a term, and $N$ an occurence of a subterm in $M$
  that is not under a lambda. We define
  $\reach{r}{M}$ the set of all reference substitutions that are in scope
  of this subterm in $M$, by
  \begin{itemize}
    \item If $M=N$ then $\reach{N}{M} = \emptyset$
    \item If $M=\refssd{s}{U}{M'}$ then $\reach{N}{M} = \multv{U}
      + \reach{N}{M'}$
    \item If $M=\varss{\sigma}{M'}$ then $\reach{N}{M} =
      \varsmetas{x}{V}{\reach{r}{M'}}$
    \item If $M = \refssu{s}{U}{M'}$ then $\reach{N}{M} =
      \reach{r}{M'}$
    \item If $M=\refssl{s}{U}{M_1\ M_2}$ or $M = M_1 \parallel M_2$, let $i$ be the index such that
      $N$ occurs in $M_i$, then $\reach{N}{M} = \reach{N}{M_i}$
  \end{itemize}

  We define the skeleton of a term $\skel{M}$ by removing all downward
  reference substitutions that are not under a lambda. We say that $M
  \rincl N$
  if :
  \begin{itemize}
    \item $\skel{M}$ = $\skel{N}$, and thus we can put in a one-to-one correspondance the occurences of
      $\get{r}$ and $\refssl{}{V}{M_1\ M_2}$ subterms of $M$ and $N$
    \item For all such $\get{r}$ occurences, $\reach{\get{r}}{M} \subseteq
      \reach{\get{r}}{N}$
    \item For all such $M' = \refssl{r}{V}{M_1\ M_2}$ corresponding to
      $N' = \refssl{s}{U}{N_1\ N_2}$, then $\reach{M'}{M} + \multv{V}
      \subseteq \reach{N'}{N} + \multv{U}$
  \end{itemize}

  Similarly, we say that $M \rdiff{V} N$ if the
  difference between reachability sets involved in the definition is somehow
  "bounded" by $\multv{V}$ :
  \begin{itemize}
    \item $\skel{M}$ = $\skel{N}$
    \item For all such $\get{r}$ occurences, $\reach{\get{r}}{M} \subseteq
      \reach{\get{r}}{N} \subseteq \reach{\get{r}}{M} + \multv{V}$
    \item For all such $M' = \refssl{s}{U}{M_1\ M_2}$ corresponding to
      $N' = \refssl{t}{W}{N_1\ N_2}$, then $\reach{M'}{M} + \multv{W} \subseteq
      \reach{N'}{N} + \multv{U} \subseteq \reach{M'}{M} + \multv{W} + \multv{V} $
  \end{itemize}

  $\rincl$ (resp. $\rdiff{V}$) is a partial pre-order on terms. The equivalence relation induced by
  these preorders is the same and is noted $\req$.
\end{mdef}

\begin{mlem}{Invariance by \rrulet{subst-r}{}
reductions}\label{mlem-ord-invariance}\\
Let $M \rincl N$ (resp. $M \rdiff{V} N$).
  \begin{itemize}
    \item If $M \to M'$ by a \rrulet{subst-r}{} rule except
      \rrulet{subst-r}{get} then $M' \rincl N$ (resp. $M' \rdiff{V} N$)
    \item If $N \to N'$ by a
      \rrulet{subst-r}{} by a \rrulet{subst-r}{} rule except
      \rrulet{subst-r}{get} then $M \rincl N'$ (resp. $M \rdiff{V} N'$).
  \end{itemize}
\end{mlem}

\begin{proof}
 Clearly, a \rrulet{subst-r}{} rule does not modify the skeleton, so $\skel{M} =
 \skel{M'} = \skel{N}$. It is also almost immediate to see that rules that
 propagate reference substitutions or \rrulet{subst-r}{val} that erases the ones
 only in scope of a value do not modify $\reach{\get{r}}{M}$ for an
 occurence $\get{r}$ in $M$, nor do they modify $\reach{M'}{M} + \multv{V}$ for
 $M' = \refssl{r}{V}{M_1\ M_2}$.
\end{proof}

\begin{mlem}{Simulation}\label{mlem-ord-simulation}\\
  Let $M \rincl N$ (resp. $M \rdiff{V} N$).
  \begin{enumerate}
    \item If $M \to M'$ then $\exists n \geq 0,\ N \to^n N'$ such that $M'
      \rincl N'$ (resp. $M' \rdiff{V} N'$). If the
      applied rule is not a \rrulet{subst-r}{} or is \rrulet{subst-r}{get}, then
      $n > 0$.
    \item Corollary. If $M \rincl N$, then if $N$ is strongly normalizing, so is
      $M$.
    \item Corollary. If $M \req N$, then $M$ is strongly normalizing iff $N$
      is.
  \end{enumerate}
\end{mlem}

\begin{proof}
  We will first prove that if $M = C[E[P]$, then $N \to^\ast C[E'[P']]$. One may
  just have to apply the rule \rrule{subst-r}{\parallel} until it
  is not possible anymore to get $N \to C[N']$. Then, $E[P]$ and $N'$ having the
  same skeleton,
  $N'$ can be written as $E'[P']$ where $E'$ is $E$ with
  additionnal downward references substitutions, and $P$ and $P'$ have the same
  skeleton and the same head constructor (if $P'$ have additionnal substitutions in
  head position one can always include it in $E'$ : we actually take the maximal $E'$
  that satisfies the decomposition).
  The reachability sets of subterms in $C$ (respectively $E$,$E'$) only depends
  on $C$ (resp. $C,E$ and $C,E'$). The reachability sets of subterms in $P$
  (resp. $P'$) are unions of substitutions occuring in $P,E$ (resp.
  $P',E'$) and $C$.

  \begin{itemize}
    \item If the rule is one of the \rrulet{subst-r}{} except
      \rrulet{subst-r}{get}, by \ref{mlem-ord-invariance}, $n=0$ works.
    \item \rrulet{subst-r}{get} : $P = \refssd{r}{V}{\get{r}} \to V \in
      \multv{V}(r)$ and $P =
      \refssd{r'}{V'}{\get{r}}$. $\multv{V}(r)$ is in $\reach{\get{r}}{N}$ so by iterated application of \rrulet{subst-r}{}
      rules except \rrulet{subst-r}{get} and \rrulet{subst-r}{val}, we can push
      (without modifying the skeleton nor the reachability sets) the
      corresponding substitutions down to $\get{r}$ in $P'$ and we can do the
      same reduction. All the other reachability sets of gets or application or
      left unmodified.
    \item $(\beta_v)$ : $P = \refssl{r}{V}{(\lambda x. Q)\ V} \to
      T = \refssd{r}{V}{\vars{x}{V}{Q}}$. Up to
      \rrulet{subst-r}{val} reductions, $P' = \refssl{r'}{V'}{(\lambda x. Q)\ V} \to
        T' = \refssd{r'}{V'}{\vars{x}{V}{Q}}$. The condition on reachabiliy sets for
        application in the defintion of $\rincl$ precisely ensures that all the
        gets and applications in $Q$ have the same reachability in
        $C[E[T]]$ and in $C[E'[T']]$.
  \end{itemize}

  \rrulet{subst}{} rules
  \begin{itemize}
    \item \rrulet{subst}{var} : $P = \varss{\sigma}{x} \to x$ or $V(x)$, and $P' =
      \varss{\sigma}{\refssd{r}{V}{x}} \to \varss{\sigma}{x} \to x$ or $V(x)$.
    \item \rrulet{subst}{app} : $P = \varss{\sigma}{\refssl{r}{V}{Q_1\ Q_2}} \to
      T = \refrawsl{\vect{r}}{(\varss{\sigma}{V})}{(\varss{\sigma}{Q_1})\
      (\varss{\sigma}{Q_2})}$. We have $P' =
      \varss{\sigma}{\refssl{r'}{V'}{(\refssl{s}{U}{Q'_1})\
      (\refssl{t}{W}{Q'_2})}} \to^\ast
      \refrawsl{r'}{\varss{\sigma}{V'}}{(\refrawsd{s}{\varss{\sigma}{U}}{\varss{\sigma}{Q_1}})\
      (\refrawsd{s}{\varss{t}{V}{W}}{\varss{\sigma}{Q_2}})}$. By definition of
      reachability sets, they are invariant by all the rule applied.
    \item We proceed the same way for other cases : the var substitution just
      go through the additionnal references substitutions, and by design,
      reachability sets are not modified.
  \end{itemize}

  \rrulet{subst-r'}{} rules
  \begin{itemize}
    \item Upward substitutions commute with downward ones without interacting.
      On the other hand, they can span new downward substitutions but in this
      case, they do it in the same way for both $P$ and $P'$ and thus do not
      modify the inclusion relation on reachability sets.
  \end{itemize}
\end{proof}
%
% \begin{mdef}{Completion}\label{mdef-completion}\\
% Let $ \vdash M,N : (\alpha,e)$,
% $\vect{r},\vect{\mathcal{V}}$ be respectively
% references and multivalues, we define the relation $\complrv$ by the following
% rules :
%   \begin{itemize}
%     \item $V \complrv V$
%     \item $M \complu{(r,\mathcal{V})+(s,\mathcal{U})} \refssd{r}{V}{N}$ if $M \compl{s}{U} N$
%     \item $\refssd{s}{U}{M'} \compl{r}{V} N$ if $M'
%       \complu{(r,\mathcal{V})+(s,\mathcal{U})} N$
%     \item $\refssl{s}{U}{M_1\ M_2} \complrv \refssl{s'}{U'}{N_1\ N_2}$ if $M_i
%       \complrv N_i$ and $(r,\multv{V}) + (s,\multv{U}) = (s',\multv{U}')$
%     \item $\varss{x}{U}{M} \compl{\emptyset}{\emptyset} \varss{x}{U}{M}$
%     \item $\refssu{s}{U}{M} \complrv \refssu{s}{U}{N}$ if $M \complrv N$
%     \item $M = M_1 \parallel M_2$ then $N = N_1 \parallel N_2$ with $M_i
%       \complrv N_i$
%   \end{itemize}
%   We extend this definition to context by adding the rule $[.] \complrv [.]$ for
%   any $(r,\mathcal{V})$.
% \end{mdef}
%
% \paragraph{}
% We need to prove a few lemma concerning completions.
%
% \begin{mlem}{Decomposition}\label{mlem-completion-decomposition}\\
% Let $M \complrv N$.
%
% \begin{enumerate}
%   \item If $M = C[E[M']]$ for some $M'$, then $N \to^\ast
%    C'[E'[N']]$ where $C[E] \compl{s}{U} C'[E']$ and $M' \compl{r'}{V'} N'$.
% Moreover, if $P \compl{r'}{V'} Q$ with the same type as $M'$ and $N'$ then $C[E[P]] \complrv C'[E'[Q]]$.
%   \item If $N = C[E[N']]$, then $M
%     \to^\ast
%     C'[E'[M']]$ where $C'[E'] \compl{s}{U} C[E]$ and $M' \compl{r'}{V'} N'$
%     such that for any $P \compl{r'}{V'} Q$ with the same type as $M'$ and $N'$ then $C'[E'[P]]
%     \complrv C[E[Q]]$
% \end{enumerate}
% \end{mlem}
%
% \begin{mlem}{Simulation}
% \label{mlem-completion-reduction-stability}\\
%   Let $M \complrv N$.
%   \begin{enumerate}
%     \item If $M \to M'$ then $N \to^\ast N'$ such that $M' \complrv
%       N'$. Moreover, if the applied reduction rule is not \rrule{subst-r}{} or
%       is \rrulet{subst-r}{get}, then $N \to^+ N'$.
%     \item If $(r,\multv{V}) = (\emptyset,\emptyset)$ and $N \to N'$ then $M
%       \to^+ M'$ such that $M' \compl{\emptyset}{\emptyset} N'$. Moreover,
%       if the applied reduction rule is not \rrule{subst-r}{} or is
%       \rrulet{subst-r}{get}, then $M \to^+ M'$.
%     \item Corollary : if $M \complrv N$, then $N$ is strongly normalizing
%       implies that $M$ is. Moreover, if $(r,\multv{V})=(\emptyset,\emptyset)$,
%       then $N$ is iff $M$ is.
%   \end{enumerate}
% \end{mlem}
%
% \begin{proof}
% The first lemma is proved by induction on the contexts (C,E), from the
% definition of $\complrv$.  For the second one, we proceed by case analysis on
% the reduction rule. We consider first \rrule{subst-r}{}
% rules. Thanks to the first lemma, we can ignore contexts and assume that
% $C=E=[]$.
% \begin{itemize}
%   \item $(\beta_v)$
%     \begin{enumerate}
%       \item $$M = \refssl{s}{U}{(\lambda x. M_1)\ V}$$
%         so $N = \refssd{t}{W}{\refssl{s'}{U'}{(\lambda x. M_1)\ V}}$ with $M_i
%         \compl{r'}{V'} N_i$, $(s',\mathcal{U}') = (s,\mathcal{U}) +
%         (r',\mathcal{V'})$ and $(r,\mathcal{V}) = (t,\mathcal{W}) + (r',\mathcal{V'})$.
%         Then $$N \to^2 N' = \refssd{t+s'}{W+U'}{\vars{x}{V}{M}}$$ and
%         $$M' = \refssd{s}{U}{\vars{x}{V}{M}} \complrv
%         N'$$.
%       \item
%         Conversely, if $N = \refssl{s}{U}{(\lambda x. N_1)\ V}$, then $M
%         = \refssd{t}{W}{\refssl{s'}{U'}{(\lambda x. M_1)\ V}}$
%         such that $M_1 \compl{t}{W} N_1$ and
%         $(s,\multv{U}) = (s',\multv{U'}) + (t,\multv{W})$. Then $M
%         \to^\ast \refssl{s}{\multv{U}}{(\lambda x . M_1)\ V} = N \to
%         N'$.
%     \end{enumerate}
%   \item \rrulet{subst-r}{get}
%     \begin{enumerate}
%       \item $M = \refssd{s}{U}{\get{t}}$, hence $N \to^\ast
%         \refssd{s'}{U'}{\get{t}}$ with $s,\mathcal{U} \subset s',\mathcal{U'}$.
%         Since $M' = \get{t}$ or $M' = U \in \multv{U}$, then $N \to^+ M'$.
%       \item If $(r,\multv{V})=(\emptyset,\emptyset)$ and $N =
%         \refssd{s}{U}{\get{t}}$ then $M \to^\ast \refssd{s}{U}{\get{t}}$, and
%         the statement is obviously true.
%     \end{enumerate}
% \end{itemize}
%
% Variables substitutions. If $N$ is a \rrulet{subst}{var} redex then
% $(r,\multv{V}) = (\emptyset, \emptyset)$, $N = M$ and there is nothing to prove.
% If $M$ is a redex, $N = \refssd{r}{V}{M}$. Then $N \to N' = \refssd{r}{V}{M'}$
% and $M' \complrv N'$.
%
% And finally upward substitutions.
% \begin{itemize}
%   \item \rrule{subst-r'}{\parallel}
%     \begin{enumerate}
%       \item
%         $M = (\refssu{s}{U}{M_1}) \parallel M_2$, then
%         $N \to^\ast {(\refssd{t}{W}{\refssu{s}{U}{N_1}}) \parallel
%         (\refssd{u}{X}{N_2})}$ with $M_1
%         \complu{(r,\multv{V}) - (t,\multv{W})} N_1$ and $M_2
%         \complu{(r,\multv{V}) - (u,\multv{X})} N_2$.
%         Then $M' = \refssu{s}{U}{(M_1 \parallel \refssd{s}{U}{M_2})}$, and $N \to^+ N'
%         = \refssu{s}{U}{(\refssd{t'}{W'}{N_1}) \parallel
%         (\refssd{u'}{X'}{N_2}})$ with $(t',\multv{W'}) = (t,\multv{W}) +
%         (s,\multv{U})$ and same for $(u,\multv{X})$. This gives us $M' \complrv
%         N'$.
%       \item A similar argument gives that $M \to M' \complrv N'$.
%     \end{enumerate}
% \end{itemize}
%
% The third point of the lemma is an almost immediate corollay of the first two.
% One just has to notice that an infinite reduction can not contain an infinite
% subsequence of \rrule{subst-r}{} (excluding \rrulet{subst-r}{get}) reductions,
% because these reductions always move references substitutions deeper.
% Technically, for any downard reference substitution $s$, let $d(s)$ be its
% depth in the AST, and $D$ the maximal depth of the term, then the multiset
% $[ D - d(s) \mid s \in M ]$ is a decreasing (for the usual well-ordered set of
% finite multisets over natural numbers) parameter of the reduction.
% \end{proof}
%
\begin{mdef}{Strongly computable terms}\label{mdef-strongly-computable}\\
  The set $\mathbf{SC}_R(\alpha,e)$ of strongly computable terms of type
$(\alpha,e)$ is defined by induction on (simple) terms.
Later, we will omit the $R$ or $(\alpha,e)$ when it is obvious from the context and
just write $M \in \mathbf{SC}$. Moreover, we abusively write $\multv{V} \subseteq
\mathbf{SC}$ for a substitutions to mean $\forall r, \multv{V}(r) \in
\mathbf{SC}_R(R(r),\emptyset)$.

\begin{itemize}
  \item $M \in \mathbf{SC}_R(\tau,e)$ where $\tau = \text{Unit} \mid \mathbf{B}$ if $R \vdash M :
    (\tau,e)$ and :
    \begin{itemize}
      \item (SN) $$\multv{V} \subseteq \mathbf{SC}_R
        \implies \refssd{r}{V}{M} \text{ is SN (strongely normalizable)}$$
      \item (WB)
        For any $r,\mathcal{V}$ such that $\vdash (M,r,\mathcal{V})$ and
        $\mathcal{V} \subseteq \mathbf{SC}_R$,
        for any $(M,\seq{\multv{V}})$ reduction $M = M_0 \to \ldots \to M_n$
        there exists $n_0 \geq 1$ such that for any $k \geq 1$ then
        \begin{enumerate}
          \item If $M_{k-1} = \refssu{}{U}{N} \to M_k$ is a
            \rrule{subst-r'}{\top} reduction then $\mathcal{U} \subseteq
            \mathbf{SC}$
          \item if $k \geq n_0$ then $M_{k-1} \to M_k$ is not \rrule{subst-r'}{\top}
        \end{enumerate}
    \end{itemize}
  \item $M \in \mathbf{SC}_R(A \sur{\to}{e_1} \alpha,e)$ if $R \vdash M :
    (A \sur{\to}{e_1} \alpha,e)$ with $e_1 \subseteq e = \{ r_i \}$ and
    \[
      N \in \mathbf{SC}_R(A,e) \implies M\ N \in \mathbf{SC}_R(\alpha,e)
    \]
\end{itemize}
\end{mdef}

\paragraph{}
% \begin{mlem}{Anti-reduction}\label{mlem-antired}\\
%   If $R \vdash M : (\alpha,e)$ and $M \to M' \in \mathbf{SC}(\alpha,e)$ then $M
%   \in \mathbf{SC}(\alpha,e)$
% \end{mlem}
%
% \begin{proof}
%   TODO
% \end{proof}

\begin{mlem}{Characterization}\label{mlem-charact}\\
  Let
  \begin{itemize}
    \item $\alpha = A_1 \sur{\to}{e_1} \ldots \sur{\to}{e_{n-1}} A_n
      \sur{\to}{e_n} \beta$ with $\beta = \text{Unit} \mid \mathbf{B}$
    \item $\vdash M : (\alpha,e)$
    \item $N_i \in \mathbf{SC}(A_i,e_i')$
    \item $\multv{U} \subseteq \mathbf{SC}$
  \end{itemize}
  with $\ptentre{i}{1}{n}, e'_i \subseteq e_i \subseteq e$ and $\dom{\multv{U}} \subseteq e$.
  We define
  \[
    \Lambda(M,\multv{U},\seq{N}) = \refssd{r}{\mathcal{U}}{M\ N_1\ \ldots\ N_n}
  \]
    Then $M \in \mathbf{SC}(\alpha,e)$ if and only if
  $\Lambda(M,\multv{U},\seq{N})$ is (SN) and (WB) for all $\multv{U},\seq{N}$
  satisfying the above conditions.
  In the following, we may conveniently omit some of the parameters
  $(M,\multv{U},\seq{N})$ of $\Lambda$.
\end{mlem}

\begin{proof}
  By induction on types.
\end{proof}

\begin{mlem}{Auxiliary results for soundness}\label{mlem-soundness-aux}\\
  Let $M,V \in \mathbf{SC},\ \multv{V} \subseteq \mathbf{SC}$ then
  \begin{enumerate}
    \item For any infinite reduction of $\Lambda(N)$, $N$ must be reduced at some
      point.
    \item If $\varss{\sigma}{N} \to M$ then $\varss{\sigma}{N} \in \mathbf{SC}$
    \item $\refssd{r}{V}{M} \in \mathbf{SC}$
    \item $\refssu{r}{V}{M} \in \mathbf{SC}$
    \item If $M \to M'$, then $M' \in \mathbf{SC}$
    \item $\varsmetas{x}{V}{\multv{V}} \subseteq \mathbf{SC}$
  \end{enumerate}
\end{mlem}

\begin{proof}


  \begin{enumerate}
    \item If the subterm $N$ is never reduced, the reducts of $\Lambda(N)$ are of
      the form $N\ N_1' \ldots N_n'$ (with some additionnal reference
      substitutions not written for conciseness) where each $N_i'$ can be seen as the result
      of an $(N_i,\seq{\multv{W}})$ reduction for some $\seq{\multv{W}}$ corresponding
      to the upward substitutions generated by the interaction with other
      subterms $N_1,\ldots,N_n$. All these subterms are (WB) and
      generate $\mathbf{SC}$ upward substitutions. $N_i$ being well behaved, there is a number of
      steps $n_i$ after wich the reduct $N'_i$ doesn't generate upward
      substitutions anymore. After $n= \vee n_i$ steps (actually one may have to take a
      bigger $n$ for the substitutions have to dispatch, but there is such a $n$), $N_i$ has reduced to some $P_i$
      and doesn't receive any downard substitution. If we gather all the downward substitutions
      delivered to $N_i$ (or, viewed as an $(N_i,\seq{\multv{W}})$ reduction, all
      the substitutions produced by $\to_i$ rules) as $\multv{X}$, then
      $N_i \rdiff{U} Q = \refssd{}{U}{N_i}$. Consider the first step of the
      $(N_i,\seq{\multv{W}})$ reduction $N_i \to N_i'$, either this is a usual step and then by
      \ref{mlem-ord-simulation} $Q \to^\ast Q'$ with $N_i'
      \rdiff{U} Q'$ or this is a $\to_j$ step and $N_i' = \refssd{}{Z}{N_i}$
      for some $\multv{Z} \subseteq \multv{U}$ and $N_i'
      \rdiffraw{\multv{U} \setminus \multv{Z}} Q$. By induction over the n firt
      steps, we get that $Q \to^\ast Q_0$ such that $P_i
      \req Q_0$. Since $N_i \in \mathbf{SC}$, $Q$ and all its reducts are
      (SN), and so is $P_i$ thus the reduction of $\Lambda(N)$ must be finite.

    \item Let $M' = \varss{\sigma}{M}$, consider an infinite reduction of
      $\Lambda(M')$.  By the previous point, the subterm $M'$ must be reduced,
      and $M$ is the only possible reduct. But the reduct of $\Lambda(M')$
      we get is reachable from $\Lambda(M)$ which is (SN) thus the reduction
      must be finite and $\Lambda(M')$ is (SN).

      Similarly, consider (for suitable $\seq{\multv{V}}$) a $(M',\seq{\multv{V}})$
      reduction. If $M'$ is never reduced, then no upward
      substitution is ever produced. If $M'$ is reduced at
      some point, then it is reduced to $M$ and thus produces a finite amount of
      $\mathbf{SC}$ upward substitutions since $M$ is (WB). Hence $M'$ is (WB).

    \item Consider $\Lambda(\refssd{r}{V}{M},\multv{U},\seq{N})$. Then
      $\Lambda(\refssd{r}{V}{M},\multv{U},\seq{N}) \rincl \Lambda(M,\multv{U} +
      \multv{V},\seq{N})$ but the latter is (SN), since $M$ is $\mathbf{SC}$. So is
      the former by \ref{mlem-ord-simulation}.
      For (WB), we can easily map a $(M',\seq{\multv{W'}})$ reduction to a
      $(M,\seq{\multv{W}})$ by just appending $\multv{V}$ to
      $\seq{\multv{W}}$ and
      start with a $\to_i$ reduction. Since $M \in \mathbf{SC}$, $M'$ is (WB).
    % \item For this one, we will use induction on types. Base case : for any
    %   adapted $(s,\multv{U})$, $\refssd{s}{U}{M'} \compl{\emptyset}{\emptyset}
    %   \refssd{t}{W}{M}$ where $(t,\multv{W}) = (s,\multv{U}) + (r,\multv{V})$. Since $M
    %   \in \mathbf{SC}$ then by definition  the latter is (SN). $M$ is well behaved, thus so is
    %   $M'$ : we can easily map a reduction sequence of $M'$ to a $M$ one by adding
    %   $(r,\multv{V})$ to the available references. Now, take $\alpha = A
    %   \sur{\to}{e} \beta$. By induction, $\refssd{r}{V}{N_i} \in \mathbf{SC}$,
    %   and $\Lambda(M,(r,\multv{V})+(s,\multv{U}),N_i)
    %   \compl{\emptyset}{\emptyset} \Lambda(M',(s,\multv{U}),\refssd{r}{V}{N_i})$
    %   $\Lambda(M')$. Assume that the reducts of $M'$ are never part of a
    %   $\beta_v$.  As before, there is a point from which no references
    %   substitutions are exchanged anymore, and the reducts of the $N_is$
    %   terminate, so the reducts of $M'$ must diverge. But we can map this
    %   divergent sequence to a divergent one of $\refssd{t}{W}{M}$ for some
    %   $(t,\multv{W})$ which is (SN). There is a contradiction and thus the
    %   reduction is finite. Now, if there is a $\beta_v$ reduction, then one of the reduct of a subterm must
    %   $\Lambda(M,(s,\multv{U})+(r,\multv{V}),N_i)
    %   \compl{\emptyset}{\emptyset} \Lambda(M',s,\multv{U},N_i)$ and thus the two have the same behavior
    %   in respect to divergence. Since $M \in \mathbf{SC}$, the two are (SN).

    \item Let $M' = \refssu{r}{V}{M}$. We proceed by induction on types. For
      base types, it is clear that $M'$ is (WB) iff $M$ is, and
      $\refssd{s}{U}{M'}$ has exactly the same reductions as $\refssd{s}{U}{M}$
      except for commutation of upward and downard substitutions, and a possible
      \rrule{subst}{\top}. Thus they are both (SN).
      Now, for $\alpha = A \sur{\to}{e_1} \alpha'$, consider an infinite reduction of
      $\Lambda(M',\multv{U},\seq{N})$. If the upward substitution is never
      reduced, we can map this to an infinite reduction of
      $\Lambda(M,\multv{U},\seq{N})$ for the same reasons as above, but the
      latter is (SN). Hence at some point the upward substitution must move up,
      so that the head term becomes $\refssu{r}{V}{\refssl{t}{W}{M''\
        (\refssd{r}{V}{N_1'}})}$ where $M''$ and $N_1'$ are reducts descendant
      from respectively $M$ and $N_1$. Using induction and points 5 and 3 of
      this lemma, $P = \refssl{t}{W}{M''\ (\refssd{r}{V}{N_1'}})$ is $\mathbf{SC}$. By
      induction, so is the new head redex, and the whole redex of $\Lambda$ is
      reachable from $\Lambda(\refssl{t}{W}{M\ N_1},\multv{U},\seq{N})$.

    \item This is straightforward from the definition of $\mathbf{SC}$ sets.
  \item Combining 2. and 4., using the fact that $\varsmetas{x}{V}{U}$ is the
      normal form of $\varss{\sigma}{U}$ using only \rrule{subst}{} rules, we get
      the result by induction on the length of the reduction.
  \end{enumerate}
\end{proof}

\begin{mlem}{Soundness}\label{mlem-soundness}\\
  If $R; x_1:A_1,\ldots,x_n:A_n \vdash M : (\alpha,e)$,
  $V_i \in \mathbf{SC}(A_i)$ and $\sigma : x_i \mapsto V_i$. Then
  $$\varss{\sigma}{M} \in \mathbf{SC}(\alpha,e)$$
\end{mlem}

\begin{proof}

  We perform the proof by induction.
  \begin{itemize}
    \item $M=x$ : $\varss{\sigma}{x}$ reduces to $\sigma(x) \in \mathbf{SC}$, and
      we apply \ref{mlem-soundness-aux}
    \item $M=\ast$ : $\varss{\sigma}{\ast} \to \ast$.
    \item $M=\lambda y.M'$ : $\varss{\sigma}{M} \to \lambda x .
      (\varss{\sigma}{M'})$. Consider an infinite reduction $\Lambda(\lambda x.
      (\varss{\sigma}{M'}))$. By \ref{mlem-soundness-aux} 1), at some point a
      $(\beta_v)$ must occur, replacing the head redex by $P =
      \refssd{s}{U}{\vars{y}{X}{\varss{\sigma}{M'}}}$ which is $\mathbf{SC}$ by
      induction \ref{mlem-soundness-aux} 3). But this term can be reached from
      $\Lambda(P,\multv{U},\refssd{}{V}{N_{i+1}})$ (for some
      $\multv{V}$ that are $\mathbf{SC}$, the ones emitted by the reduction of
      $N_1$) which is (SN). The same kind of
      argument show that $\Lambda(M,\multv{U},\seq{N})$ is (WB) : if the redex
      is not reduced, then all upgoing substitutions that come from $N_i$ must stop
      after a finite number of reductions and all contain $\mathbf{SC}$ terms,
      or the redex is reduced after a finite number of steps and from this point
      the term is a reduct of a (WB) one thus must be (WB) as well.

    \item $M = \get{r}$ : $\varss{\sigma}{\get{r}} \to \get{r}$. Let see that
      $\get{r} \in \mathbf{SC}$. Consider an infinite reduction of
      $\Lambda(\get{r})$. By \ref{mlem-soundness-aux} 1), the $\get{r}$ must be
      reduced at some point and from
      this point it is either replaced by a value from the substitution prefix,
      or by a value emitted by one of the $N_i$, all of these being
      $\mathbf{SC}$.
    \item $M = \varss{\tau}{M'}$, then $\varss{\sigma}{M} \to
      \varss{\mu}{M'}$. By \ref{mlem-soundness-aux},
      $\varsmetas{x}{V}{U} \in \mathbf{SC}$. $M'$ has a typing judgement of the form $x_1:A_1,\ldots,x_n : A_n, y_1 :
      B_1, \ldots, y_m : B_m \vdash M' : (\alpha,e)$. By induction,
      $\varss{\mu}{M'} \in
      \mathbf{SC}$.
    \item $M = \refssd{}{U}{M'}$ : $\varss{\sigma}{M} \to
      \refssd{}{\varsmetas{x}{V}{\multv{U}}}{\varss{\sigma}{M'}}$. By
      induction, $\varss{\sigma}{M'}$ is $\mathbf{SC}$ and by \ref{mlem-soundness-aux}
      so is $M$.
    \item $M = \refssu{r}{\mathcal{V}}{M'}$ : induction +
      \ref{mlem-soundness-aux}.
    \item $M = \refrawsl{(r_i)}{(\mathcal{V}_i)}{M_1\ M_2}$ : $\varss{\sigma}{M}
      \to M' = \refrawsl{r}{(\varss{\sigma}{\multv{V}})}{(\varss{\sigma}{M_1})\
      (\varss{\sigma}{M_2})}$. By induction and \ref{mlem-soundness-aux}, $\varss{\sigma}{M_i} \in \mathbf{SC}$
      and $\varss{x}{\multv{V}}$ are in $\mathbf{SC}$. Then by definition
      $M' \in \mathbf{SC}$.
    \item $M = M_1 \parallel M_2$ : $\vars{x}{V}{M} \to M'= M_1' \parallel M_2'$
      with $M_i' = \vars{x}{V}{M_i}$  and according to \ref{mlem-soundness-aux} it
      is sufficient to prove $M' \in \mathbf{SC}$. By induction, $M_i' \in
      \mathbf{SC}$. Let us take an $(M',r,\multv{V})$ reduction
      starting from $M'$. It can be associated to an $(M_i',r_i,\multv{V}_i)$
      reduction from the point of view of $M_i'$, where
      $r_i,\multv{V}_i$ are coming either from $(r,\multv{V})$ or from the
      upward substitution of $M'_{1-i}$, that are all in $\mathbf{SC}$. Since
      the $M_i$ are (WB), so is $M'$.
      Now, the proof is very similar to the first point of
      \ref{mlem-soundness-aux} : Take an $M'$ reduction, since $M'_i$ are (WB), after a finite
      number of steps, no more substitutions are exchanged. We can then smash
      all the substitutions received by $M'_i$ into a big one $(x,\multv{X})$
      and since $\refssd{x}{X}{M'_i}$ is (SN), then the reduction must be
      finite.
  \end{itemize}

\end{proof}


\begin{mlem}{Adequacy}\label{mlem-adequacy}\\
  If $M \in \mathbf{SC}(\alpha,e)$ then $M$ is strongly normalizable
\end{mlem}

\begin{proof}
  We will prove additionnally by induction on types that $\mathbf{SC}(\alpha)
  \neq \emptyset$ for any $\alpha$.
  \begin{itemize}
    \item For $\alpha = \texttt{Unit} \mid \mathbf{B}$ it is immediate : $\ast
      \in \mathbf{SC}(\texttt{Unit})$ and $\ast \parallel \ast \in
      \mathbf{SC}(\mathbf{B})$. If $M \in \mathbf{SC}(\alpha)$
      had an infinite reduction, then so would $\refsrawsd{r}{V}{M}$
    \item For $\alpha = A \to \alpha'$, by induction there exists $M_{\alpha'}
      \in \mathbf{SC}(\alpha')$, then $\lambda x . M_{\alpha'}$ for $x$ not free in
      $M_{\alpha'}$ is in $\mathbf{SC}(\alpha)$. If $M \in \mathbf{SC}(\alpha)$ did not terminate, so would $M\
      N$ for $N \in \mathbf{SC}(A)$ which exists since the latter set
      is not empty.
  \end{itemize}
\end{proof}

\begin{mthe}{Termination}\label{mthe-termination}\\
  All well-typed closed terms are strongly normalizing
\end{mthe}
\begin{proof}
  By conjunction of \ref{mlem-soundness} (with $n=0$) and \ref{mlem-adequacy}.
\end{proof}

\subsection{Termination strikes back}

We add a labelled reference substitution variable substitution to $\lamlang{aux} : \refssdbar{}{V}{M} \mid
\varsbar{x}{N}{M}$ such that $\varsbar{x}{N}{M}$ can't be reduced in either $N$
or by \rrulet{subst}{} rules (where $N$ is not a value). The labelled reference
substitution plays the same role in contexts : it forbids any reduction under
it, except for labelled reference substitutions.
We add the reduction rules \rrulet{subst-r}{} for $\refssdbar{}{V}{}$ for
labelled substitution, that can be
performed everywhere (included under a variable substitution) except under
abstraction : $J ::= [.] \mid J\ M \mid M\ J \mid \refssd{}{V}{J} \mid
\varss{\sigma}{J} \mid \vars{x}{N}{J}$.

We also add a $\beta$-rule to fire such labelled substitution :
\[
  (\beta_{V}') \refssl{}{V}{(\lambda x . M)\ N} \to
  \varsbar{x}{N}{\refssdbar{}{V}{M}}
\]

This corresponds to the additionnal reduction nets can do, and we will show that
going from a normal form in \lthis with these additionnal rules leads
to a new normal form that is (almost) normal in nets.

\begin{mdef}{$F$-normal forms}\label{mlem-progress-auxplus}\\
 Let $M$ be a normal form of the form $M_\text{norm}$, then $M$ reduces to a sum
 of terms in $\lamlang{aux+}$ that belongs to the
 following grammar of $F$-normal forms :
\begin{tabred}
  F_\text{norm} & ::= & \get{r} \mid \refssl{}{V}{F_\text{norm}\ V} \mid
  \refssl{}{V}{F_\text{norm}\ F_\text{norm}} \mid \varsbar{x}{F_\text{norm}}{M} \\
\end{tabred}
where the $M$ is in \lthis (contains no labelled substitution).
\end{mdef}

\begin{proof}
  By induction on the structure of $M$, with the additionnal hypthesis that only
  the additionnal rules are performed (no upward substitution) :
  \begin{itemize}
    \item $M = \get{r}$ : ok
    \item $M = \refssl{}{V}{M_\text{norm}\ V}$ : by induction, $M_\text{norm}$
      reduces to a sum of $F_\text{norm}$. Take one such $N$, then $M \to^\ast
      \refssl{}{V}{N_\text{norm}\ V}$ (because no rule \rrule{subst-r'}{\top} was
      used)
    \item $M = \refssl{}{V}{M_\text{norm}\ M'_\text{norm}}$ : we proceed as the
      previous case
    \item $M = \refssl{}{V}{V\ M_\text{norm}}$ : by induction, $M_\text{norm}$
      reduces to some $N$ in $F_\text{norm}$ grammar, so $M \to^\ast
      \refssl{}{V}{V\ N}$. Then, by inversion of typing rules, $V$ is of the
      form $\lambda x . P$ and we can apply the new $\beta$-reduction to get
      $\varsbar{x}{N}{\refssdbar{}{V}{P}}$. By pushing down $\refssdbar{}{V}{}$ in
      $P$, we can reduce it to a sum of $P_i$s where each $P_i$ do not contain
      labelled substitutions. Then $M \to^\ast \sum_i \vars{x}{N}{P_i}$ 
  \end{itemize}
\end{proof}

\begin{mlem}
$F$-normal forms are normal. 
\end{mlem}

\begin{proof}
  By induction : 
  \begin{itemize}
    \item $M = \get{r}$ : ok
    \item $M = \refssl{}{V}{F_\text{norm}\ V}$ : by induction, $F_\text{norm}$
      is normal, and values are not $F$-normal form, so the application can't create any
      $\beta$-redex.
    \item $M = \refssl{}{V}{M_\text{norm}\ M'_\text{norm}}$ : same as the
      previous case
    \item $M = \varsbar{x}{F_\text{normal}}{M}$ : The explicit substitution
      prevent any reduction except \rrulet{subst-r}{} ones for labelled
      reference substitution, but by definition, $M$ does not contain any.
  \end{itemize}
\end{proof}
\begin{mthe}{Adequacy}\label{mthe-adequacy-simulation-orig}\\
  Let $P$ be a term of \lamadio and $M = \widetilde{P}$ its translation in
  \lthis, if $M \to^\ast \sum_i M_i$ a normal form, then $\forall
  i, P \to^\ast P_i$ such that $M_i \rincl \widetilde{P_i}$. In other words, any
  term appearing in the normal form of the translation of $P$ is bounded by the
  translation of a reduct of $P$.
\end{mthe}

In particular, applied to values, this gives us

\begin{mcor}{Adequacy}\label{mcor-adequacy-simulation-orig}\\
  Let $P$ be a term of \lamadio, $M = \widetilde{P}$ its translation in
  \lthis such that $M \to^\ast M' + \mathbf{M''}$ a normal
  form.
  \begin{itemize}
    \item If $M' = V \parallel N$, then $P \to^\ast U \parallel Q$ with $V =
      \widetilde{U}$.
    \item In particular, if $M' = \parallel_i V_i$, then $P \to^\ast \parallel_i
      U_i$ with $V_i = \widetilde{U}_i$
  \end{itemize}
\end{mcor}

\begin{mlem}{}\label{mlem-preservation-values}
  Let $M$ be a term of \lamadio, if $M \to^\ast M'$ without using
  \rrulet{subst-r}{get}. We define $\text{NF}(M) = \{ T \mid T \text{ normal}
  \text{ and } M \to^\ast T \}$. Then $\text{NF}(M) = \text{NF}(M')$
\end{mlem}

\begin{proof}
  If we don't use \rrulet{subst-r}{get}, the two reduction (full and
  non-deterministic) coincide and we use the confluence in \lthis.
\end{proof}


\begin{mlem}{}\label{mlem-onestep-adequacy}
  Let $M = \widetilde{P}$ be the translation of a \lamadio term, such
  that $M \to M'$. Then there exists $M'',N'$, such that $M' \to^\ast M'' \rincl
  \widetilde{N'}$ and $N \to^{\{0,1\}} N'$, with all reductions from $M'$ to
  $M''$ not being \rrulet{subst-r}{get}.
\end{mlem}

\begin{proof}
  The only redexes in $M$ are either premises of \rrulet{subst-r'}{},
  $(\beta_v)$ or \rrulet{subst-r}{get}.
  In the first case, it corresponds to a reducible set whose reduction can be
  carried on in $M'$ by pushing the upward substitution to the top and pushing
  down the corresponding generated downward substitutions, to obtain the translation of
  $N'$ which is $N$ where we the set is reduced. We can proceed the same way
  with $(\beta_v)$ : this corresponds to a $\beta$-redex in $N$, where $N'$ is
  the result of reducing it, and $M''$ is obtained by pushing down the generated
  substitutions (variable and refenreces).
  \\
  Finally, if the reduction rule is \rrulet{subst-r}{get}, then either it
  choosed one of the available values and it corresponds exactly to a get
  reduction $N \to N'$, or it threw away available values, in which case $N =
  N'$, $M' = M''$ and clearly $M'' \rincl \widetilde{N'}$.
\end{proof}

\begin{proof}\ref{mthe-adequacy-simulation-orig}\\
  We proceed by induction on $\eta (M)$, the length of the longest reduction
  starting from $M$. If $\eta (M) = 0$, ie $M$ is a normal form, this is
  trivially true.
  \\
  To prove the induction step, consider a reduct $M'$ of $M$. We use
  \ref{mlem-onestep-adequacy} to get $M' \to^\ast M'' \rincl \widetilde{P'}$ for some reduct
  $P'$ of $P$, such that the reduction to $M''$ doesn't use
  \rrulet{subst-r}{get}. Thus, by \ref{mlem-preservation-values},
  $\text{NF}(M'') = \text{NF}(M')$. By induction on $M''$, $\forall T \in
  \text{NF}(M''), \exists Q, P \to^\ast Q \text{ and } T \rincl \widetilde{Q}$.
  But this true for any reduct $M'$, and we have $\text{NF}(M) = \bigcup_{M \to
  M'} \text{NF}(M')$, hence this is true for $M$.
\end{proof}


==> paper-csl-long arxiv/parts/properties-type.tex <==
\begin{mlem}{Critical pairs}\label{mlem-critical-pairs}\\
  We write $G_1 \# G_2$ for two contexts $G_1,G_2$ if $G_1 \neq G_2$, and each one
  is not a prefix of the other, ie $\forall G, G_1 \neq G_2[G]$ and $G_2 \neq
  G_1[G]$. In the following, we write the reduction rules as
  $S[N] \to S[N'] + \mathbf{M'}$, where $\mathbf{M}'$ is equals to $\mathbf{0}$ unless when
  \rrulet{subst-r}{get} occurs where it may have additionnal terms.
  \paragraph{}
  If $\mathbf{M} \to \mathbf{M_1}$ and $\mathbf{M} \to \mathbf{M_2}$ with
  $\mathbf{M_1} \neq \mathbf{M_2}$, then one of the assertion holds :
  \begin{enumerate}
    \item The two rules are of the form $S_i[N_i] \to S_i[N_i'] + \mathbf{M}'_i$
      with $S_1 \# S_2, \mathbf{M} = S_i[N_i] = \sum_i N_i$
    \item The two rules are of the form $S[C_i[N_i]] \to S_i[C_i[N_i']] +
      \mathbf{M}'_i$
      with $C_1 \# C_2, C_i[N_i] = \parallel_i N_i$
    \item The two rules are of the form $S[C[N_1]] \to S[C[N_1']]$ and
      $S[C[C_2[N_2]]] \to S_2[C[C_2[N_2']]] + \mathbf{M}'_2$,
      the first rule being \rrule{subst-r'}{\parallel}.
    \item The two rules are of the form $S[C[H[H_i[N_i]]] \to
      S_i[C[H[H_i[N_i']]]] + \mathbf{M}_i'$ with $H_1 = \refssl{r}{V}{H_1'[.]\ H_2'[N_2]}$ and $H_2
      = \refssl{r}{V}{H_1'[N_1]\ H_2'[.]}$, $N_i \to N_i'$, where $H_i$ is a
      context of type $E$ or $F$.
    \item The two rules are of the form $S[C[H[N_1]]] \to S[C[H[N_1']]$ and
      $S[C[H[H_2[N_2]]]] \to S_2[C[H[H_2[N_2']]]] + \mathbf{M}'_2$, with one
      of the following :
      \begin{enumerate}
        % \item $N_1 = \varss{\sigma}{H'}$ and the first rule applied is either
        %   \rrulet{subst}{app} or \rrulet{subst}{subst-r'} and the second is of
        %   type \rrule{subst}{\ldots} or \rrule{subst-r}{\ldots}
        \item $N_1 = \refssd{r}{V}{M'}$ and the applied rule is
          \rrule{subst-r}{app}, \rrule{subst-r}{subst-r'} or
          \rrule{subst-r}{merge}%  or \rrule{subst-r}{\ldots}
        \item $N_1 = \refssl{r}{V}{(\refssu{s}{U}{P})\
        H_2'[N_2]}$ or $N_1 = \refssl{r}{V}{H_2'[N_2]\
          (\refssu{s}{U}{P})}$
        \item  $N_1 = \refssl{r}{V}{(\refssu{s}{U}{H_2'[N_2]})\
          P}$ or $N_1 = \refssl{r}{V}{P\
          (\refssu{s}{U}{H_2'[N_2]})}$
        \item $C = H = [.]$, $N_1 = \refssu{r}{V}{H_2[N_2]}$ and the first rule
          used is \rrule{subst-r'}{\top}
      \end{enumerate}
  \end{enumerate}
\end{mlem}

\begin{proof}
We can write $\mathbf{M}$ in a unique way
(modulo structual rules) as a sum of parallel of simple terms :
$$\mathbf{M} = \sum_k M_k,\  M_k = \parallel_{i} M^i_k$$
\begin{itemize}
  \item The two reductions rules have a premise of the form $S[N_i]$.
    Identifying the terms of both sums, we can write $S_1 = [.] + \sum_{k \neq
    k_1} M_k$ and $S_2 = [.] + \sum_{k \neq k_2} M_k$. If $k_1 \neq k_2$ we are in
    the case (1), or $S_1=S_2$.

  \item If one of the rule used (let say the first one) is
    \rrule{subst-r'}{\top}, then $M_{k_1} =
    \refssu{r}{V}{M_{k_1}'}$. Since $\mathbf{M_1} \neq
    \mathbf{M_2}$, the second rule can't be the same and is of the form
    $H[T] \to H[T']$ where $H ::= E \mid F$ and $H =
    \refssu{r}{V}{H'}$. This is the case (5d) of the lemma.

  \item Otherwise, the premises of the two rules have the form $S[C_1[H_1[P_1]]]
    \to S[C_1[H_1[P_1']]] + \mathbf{M'}_1$ and $S[C_2[H_2[P_2]]] \to
    S[C_2[H_2[P_2']]] + \mathbf{M'}_2$.  If $C_1 \# C_2$, we are in case (2). If
    not, then either $C_1=C_2$ or $C_2=C_1[C_2'],C_2' \neq [.]$ but the only
    rule that matches a parallel is \rrule{subst-r'}{\parallel}, and this is
    case (3). We assume from now on that $C_1=C_2$. We decompose $H_1$ and $H_2$
    by their greatest common prefix, such that $H_1=H[H_1']$ and $H_2=H[H_2']$
    with either $H_1' = H_2' = [.]$, or $H_1' = [.],\ H_2' \neq [.]$, or $H_1 \#
    H_2$. The former is excluded since the reducts $\mathbf{N_1}$ and
    $\mathbf{N_2}$ are assumed differents, and no rule have overlapping redex on
    base cases (when $C$ and $E/F/G$ are empty).  \\
  \item
    If $H_1' \# H_2'$, since $H_1'[P_1]
    = H_2'[P_2]$, then $H_1$ must be of the form
    $\refssl{r}{V}{H_1''\ R}$, $H_2 =
    \refssl{r}{V}{L\ H_2''}$ with $L = H_1''[P_1]$ and $R =
    H_2''[P_2]$. This is case (4).
  \item
    Assume now that one of the two (let say $H_1'$) is $[.]$.
    Then $P_1$ and $H_2'$ have a common prefix. If $P_1$ is an application,
    it can't be the premise of the $(\beta_v)$ rule with $P_1 =
    \refssl{r}{U}{(\lambda x . M)\ V}$, because then $H_2' =
    \refssl{r}{U}{H_2''\ V}$ or $H_2' =
    \refssl{r}{U}{(\lambda x . M)\ H_2''}$ but no non-empty context
    verifies $H_2''[P_2] = V$ for a value $V$. Thus it must be the premise of
    \rrulet{subst-r'}{app}, and this corresponds to cases (5b) and (5c).

  \item
    If $P_1$ is not an application, since it must be both the premise of a rule
    and prefix of the context $H_2'$, the only remaining possibility is $P_1 =
    \refssd{r}{V}{\widetilde{P}_1}$. Then $\widetilde{P}_1$ can't be a value
    $y,\ast,\lambda y. \_$ or $\get{r}, \_ \parallel \_,
    \refssu{s}{U}{\_}$, because these constructors can't be in $H_2'$, which
    must be of type $F$ : we are in case (5a).
\end{itemize}

\end{proof}

\subsection{Weak confluence}

\begin{mlem}{Weak confluence}\label{mlem-weak-confluence}\\
  Let $\mathbf{M}$ be a term such that $\mathbf{M} \to
  \mathbf{M_1}$ and $\mathbf{M} \to \mathbf{M_2}$. Then
  $$\exists \mathbf{M'}, \mathbf{M_1} \to^\ast \mathbf{M'} \text{ and }
  \mathbf{M_2} \to^\ast \mathbf{M'}$$
\end{mlem}

\begin{proof}
We can write $\mathbf{M},\mathbf{M_1}$ and $\mathbf{M_2}$ in a unique way
(modulo structual rules) as a sum of parallel of simple terms :
$$\mathbf{M} = \sum_k M_k,\ \mathbf{M_1} = \sum_k M^1_k,\
\mathbf{M_2} = \sum_k M^2_k$$
Let us process all the possible cases of \ref{mlem-critical-pairs}, assuming that $\mathbf{N_1} \neq \mathbf{N_2}$:
\begin{enumerate}
  \item We have $S_1 \# S_2$, by identifying each terms, $\exists k_1 \neq k_2, S_i =
    [.] + \sum_{k \neq k_i}$, and we have
    \begin{tabred}
      \mathbf{M}_1 & = & \sum_{k \neq k_1} M_k + N_1' + \mathbf{M}'_1 \\
        & \to & \sum_{k \neq k_1,k_2} M_k + N_1' + N_2' + \mathbf{M}'_1 +
          \mathbf{M}'_2
    \end{tabred}
    as well as $\mathbf{M_2}$.
  \item Let write $C_i[N_i] = \parallel_{l \in
      \mathcal{L}} P_l$. Then
    there exists $\mathcal{L}_1, \mathcal{L}_2 \subseteq \mathcal{L}$. Since
    $C_1 \# C_2$, we have $\mathcal{L}_1 \neq \mathcal{L}_2$ and $\mathcal{L}_1
    \not \subseteq \mathcal{L}_2$ and $\mathcal{L}_2 \not \subseteq
    \mathcal{L}_1$, such that $C_i = [.] \parallel (\parallel_{l
      \in \mathcal{L}_i} P_l)$ and $N_i = \parallel_{l \notin \mathcal{L}_i} P_l$.
    The only rule that has a parallel of terms as premise is
    \rrule{subst-r'}{\parallel}. Thus $\mathcal{L}_i$ are either singletons (if
    the corresponding rule is not \rrule{subst-r'}{\parallel}) or have size two. If
    they are disjoint, then $\mathcal{L}_2 \subseteq \mathcal{L} \setminus
    \mathcal{L}_1$ and :
    \begin{tabred}
      \mathbf{M}_1 & = & S[N_1' \parallel (\parallel_{l \notin \mathcal{L}_1} P_l)] + \mathbf{M}'_1 \\
        & = &
          S[N_1' \parallel N_2 \parallel (\parallel_{l \notin \mathcal{L}_1 \cup
            \mathcal{L}_2} P_l)] + \mathbf{M}'_1 \\
        & \to &
          S[N_1' \parallel N_2' \parallel (\parallel_{l \notin \mathcal{L}_1 \cup
          \mathcal{L}_2} P_l)] +
          \mathbf{M}'_1 + \mathbf{M}'_2 \\
    \end{tabred}
    as do $\mathbf{M_2}$.\\
    The only remaining case is if both rules are \rrule{subst-r'}{\parallel} and
    $\mathcal{L}_1 \cap \mathcal{L}_2 = \{ l_0 \}$. We write $\mathcal{L}_1 = \{
    l_1, l_0 \}, \mathcal{L}_2 = \{ l_2, l_0 \}$ and $\mathcal{L_3} =
    \mathcal{L} \setminus \{ l_0, l_1, l_2 \}$. If $P_{l_0} =
    \refssu{r}{V}{P'}$ is the "active" upward substitution in both reduction, we
    have
    \begin{tabred}
      C_1[N_1'] & = & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P')}
        \parallel P_{l_2} \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
        & \to & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P' \parallel
          \refssd{r}{V}{P_{l_2}})} \parallel (\parallel_{l \neq \mathcal{L}_3}
          P_l) \\
    \end{tabred}
    If $P_{l_0}$ is the "passive" term in both reductions, with $P_{l_1} =
    \refssu{r}{V}{P_{l_1}'}$ and  $P_{l_2} = \refssu{s}{U}{P_{l_2}'}$, then
    \begin{tabred}
      C_1[N_1'] & = & \refssu{r}{V}{(P'_{l_1} \parallel \refssd{r}{V}{P_{l_0}})}
      \parallel \refssu{s}{U}{P'_{l_2}} \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
      & \to^\ast & P_{l_1} \parallel
        (\refssd{r}{V}{P_{l_0}}) \parallel
        (\refssd{r}{V}{\refssu{s}{U}{P'_{l_2}}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{r}{V}{P_l}) \\
      & \to & P_{l_1} \parallel
        (\refssd{r}{V}{P_{l_0}}) \parallel
        (\refssu{s}{U}{\refssd{r}{V}{P'_{l_2}}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{r}{V}{P_l}) \\
        & \to^\ast & (\refssd{s}{U}{P_{l_1}}) \parallel
        (\refssd{t}{W}{P_{l_0}}) \parallel
        (\refssd{r}{V}{P'_{l_2}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{t}{W}{P_l}) \\
    \end{tabred}
    using repeated \rrule{subst-r'}{\parallel}, \rrule{subst-r'}{\top},
    \rrulet{subst-r}{subst-r'} and
    \rrule{subst-r}{merge}.
    \\
    Finally, if $P_{l_0}$ is active in of the two (let say the first) and
    passive in the other, meaning that $P_{l_0} =
    \refssu{r}{V}{P_{l_0}'},P_{l_2} = \refssu{s}{U}{P_{l_2}'}$, then

    \begin{tabred}
      C_1[N_1'] & = & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P_{l_0}')}
      \parallel (\refssu{s}{U}{P_{l_2}}) \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
        & \to & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P' \parallel
          \refssd{r}{V}{P_{l_2}})} \parallel (\parallel_{l \neq \mathcal{L}_3}
          P_l) \\
    \end{tabred}
    \begin{tabred}
      C_1[N_1'] & = & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P'_{l_0})}
      \parallel \refssu{s}{U}{P'_{l_2}} \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
      & \to^\ast & (\refssd{r}{V}{P_{l_1}}) \parallel
        P'_{l_0} \parallel
        (\refssd{r}{V}{\refssu{s}{U}{P'_{l_2}}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{r}{V}{P_l}) \\
      & \to &  (\refssd{r}{V}{P_{l_1}}) \parallel
        P'_{l_0} \parallel
        (\refssu{s}{U}{\refssd{r}{V}{P_{l_2}}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{r}{V}{P_l}) \\
        & \to^\ast & (\refssd{t}{W}{P_{l_1}}) \parallel
        (\refssd{s}{U}{P_{l_0}}) \parallel
        (\refssd{r}{V}{P_{l_2}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{t}{W}{P_l}) \\
    \end{tabred}
    On the other side,
    \begin{tabred}
      C_2[N_2'] & = & P_{l_1} \parallel
        \refssu{s}{U}{( (\refssd{s}{U}{\refssu{r}{V}{P'_{l_0}}}) \parallel
        P'_{l_2})}
        \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
      & \to^\ast & (\refssd{s}{U}{P_{l_1}}) \parallel
        (\refssd{s}{U}{\refssu{r}{V}{P'_{l_0}}}) \parallel P'_{l_2} \\
      & &
          \parallel (\parallel_{l \neq \mathcal{L}_3}
          \refssd{s}{U}{P_l}) \\
      & \to & (\refssd{s}{U}{P_{l_1}}) \parallel
        (\refssu{r}{V}{\refssd{s}{U}{P'_{l_0}}}) \parallel P'_{l_2} \\
      & &
          \parallel (\parallel_{l \neq \mathcal{L}_3}
          \refssd{s}{U}{P_l}) \\
      & \to^\ast & (\refssd{t}{W}{P_{l_1}})
        \parallel (\refssd{s}{U}{P'_{l_0}})
        \parallel (\refssd{r}{V}{P'_{l_2}}) \\
      & &
          \parallel (\parallel_{l \neq \mathcal{L}_3}
          \refssd{t}{W}{P_l}) \\
    \end{tabred}

  \item
    $C_2 = \refssu{r}{V}{Q} \parallel C_2'$. Let write $C = \parallel_{l} P_l$
    and $C_2 = [.] \parallel P'$.
    then $C[N_1'] = \refssu{r}{V}{(Q \parallel \refssd{r}{V}{(N_2 \parallel P')})}$.
    \begin{itemize}
      \item Either $N_2 = \refssu{s}{U}{N_2'} \parallel Q'$ and
        \begin{tabred}
          C[N_1'] & \to^\ast & Q \parallel
            \refssd{r}{V}{((\refssu{s}{U}{N_2'}) \parallel Q')}
            \parallel (\parallel_{l} \refssd{r}{V}{P_l}) \\
          & \to^\ast & Q \parallel
            (\refssu{s}{U}{\refssd{r}{V}{N_2'}}) \parallel (\refssd{r}{V}{Q'})
            \parallel (\parallel_{l} \refssd{r}{V}{P_l}) \\
          & \to^\ast & (\refssd{s}{U}{Q})
          \parallel (\refssd{r}{V}{N_2'})
          \parallel (\refssd{t}{W}{Q'})
          \parallel (\parallel_{l} \refssd{t}{W}{P_l}) \\
        \end{tabred}
        and
        \begin{tabred}
          C[C_2[N_2']] & = & (\refssu{r}{V}{Q})
            \parallel \refssu{s}{U}{(N_2' \parallel \refssd{s}{U}{Q'})}
            \parallel (\parallel_{l} P_l) \\
          & \to^\ast &
            (\refssd{s}{U}{\refssu{r}{V}{Q}}) \parallel
            N_2' \parallel (\refssd{s}{U}{Q'})
            \parallel (\parallel_{l} \refssd{s}{U}{P_l}) \\
          & \to^\ast &
            (\refssd{s}{U}{Q}) \parallel
            (\refssd{r}{V}{N_2'}) \\
          & &
            \parallel (\refssd{t}{W}{Q'})
            \parallel (\parallel_l \refssd{t}{W}{P_l}) \\
        \end{tabred}
      \item Otherwise, $N_2$ is a premise of the form $E[Q']$ and
        $S[C[C_2[E[Q']]] \to S[C[C_2[E[Q'']]]] + \mathbf{M}_2'$. Then
        \begin{tabred}
          \mathbf{M_1} & \to^\ast & S[Q \parallel
            \refssd{r}{V}{E[Q']}
            \parallel (\parallel_{l} \refssd{r}{V}{P_l})] \\
          & \to & S[Q \parallel
            \refssd{r}{V}{E[Q']}
            \parallel (\parallel_{l} \refssd{r}{V}{P_l})] + \mathbf{M_2}' \\
        \end{tabred}
        On the other side,
        \begin{tabred}
          \mathbf{M_2} & = & S[(\refssu{r}{V}{Q}) \parallel
            E[Q''] \parallel
            (\parallel_{l} P_l)] + \mathbf{M_2}' \\
          & \to^\ast & S[Q \parallel
            (\refssd{r}{V}{E[Q'']}) \parallel
            (\parallel_{l} \refssd{r}{V}{P_l})] + \mathbf{M_2}' \\
        \end{tabred}
    \end{itemize}

  \item
    \begin{tabred}
      S[C[H[H_1[N_1']]]] + \mathbf{M}'_1 & = &
        S[C[H[\refssl{r}{V}{H_1'[N_1']\ H_2'[N_2]}]]] + \mathbf{M}'_1 \\
      & \to &
        S[C[H[\refssl{r}{V}{H_1'[N_1']\ H_2'[N_2']}]]] + \mathbf{M}'_1 +
        \mathbf{M}'_2 \\
    \end{tabred}

  \item
    \begin{enumerate}
      \item The applied rule is either :
        \begin{itemize}
          \item \rrulet{subst-r}{app} and $H_2 = \refssl{s}{U}{H_2'\ Q}$ or $H_2
            = \refssl{s}{U}{Q\ H_2'}$
          \item \rrulet{subst-r}{subst-r'} and $H_2 = \refssu{s}{U}{H_2'}$
          \item \rrulet{subst-r}{merge} and $H_2 = \refssd{s}{V}{H_2'}$
        \end{itemize}
        In the three cases, it is clear that the reductions are independant :
        the first one can be performed in $\mathbf{M_2}$ and vice-versa to get a
        common reduct.
      \item
      \item
      \item \ldots The same argument applies to the other four cases.
    \end{enumerate}
  % \item
  %   If $P_1 = \refssd{r}{V}{\widetilde{P}_1}$, then
  %   $\widetilde{P}_1$ can't be a value $y,\ast,\lambda y. \_$ or
  %   $\get{r}, \_ \parallel \_, \refssu{s}{U}{\_}$, because
  %   these constructors can't be in $H_2'$.
  %   \begin{itemize}
  %     \item If $\widetilde{P}_1 = \refssl{s}{U}{X\ Y}$ then $H_2'$
  %       must be of type $F$ and thus $H_2'[P_2]$ can't be the premise of the
  %       $(\beta_v)$ rule. It follows that $H_2' =
  %       \refssl{s}{U}{H_2''\ Y}$ (or  $H_2' =
  %       \refssl{s}{U}{X\ H_2''}$). Then
  %       \begin{gather*}
  %         P_1 \to \refssl{t}{W}{(\refssd{r}{V}{H_2''[P_2]})\
  %         (\refsd{r}{V}{Y})} \\
  %         \to \refssl{t}{W}{(\refssd{r}{V}{H_2''[P_2']})\
  %         (\refssd{r}{V}{Y})}
  %       \end{gather*}
  %       And the other way around :
  %       \begin{gather*}
  %         H_2'[P_2] \to
  %         \refssd{r}{V}{\refssl{s}{U}{H_2''[P_2']\ Y}} \\
  %         \to \refssl{t}{W}{(\refssd{r}{V}{H_2''[P_2']})\
  %         (\refssd{r}{V}{Y})}
  %       \end{gather*}
  %     \item If $\widetilde{P}_1 = \text{set}(r,V)$ then TODO [changer la
  %       reduction pour propager les substitutions dans les SUBSTUP]
  %     \item If $\widetilde{P}_1 = \substv{s}{\mathcal{U}}{X}$ then $H_2' =
  %       \substv{s}{\mathcal{U}}{H_2''}$ thus
  %       \begin{gather*}
  %         P_1 \to \refssd{r}{V}{\substv{s}{\mathcal{U}}{H_2''[P_2]}}\\
  %         \to \substv{t}{\mathcal{W}}{H_2''[P_2]} \to
  %         \substv{t}{\mathcal{W}}{H_2''[P_2']}
  %       \end{gather*}
  %       Symetrically,
  %       \begin{gather*}
  %         P_1 \to \refssd{r}{V}{\substv{s}{\mathcal{U}}{H_2''[P_2]}}\\
  %         \to \refssd{r}{V}{\substv{s}{\mathcal{U}}{H_2''[P_2']}}\\
  %         \to \substv{t}{\mathcal{W}}{H_2''[P_2']}
  %       \end{gather*}
  %   \end{itemize}
  % \item
  %   We treat the case $P_1 = \varss{\sigma}{\widetilde{P}_1}$ exactly as the
  %   previous one.
\end{enumerate}

\end{proof}

\subsection{Type soundness}

\begin{mlem*}{Subject reduction}\label{mlem-subject-reduction}\\
  Let $R;\Gamma \vdash M : (\alpha,e)$ be a typing judgement, and assume that $M
  \rightarrow M'$. Then $R;\Gamma \vdash M' : (\alpha,e)$.
\end{mlem*}

\begin{proof}
  Case analysis on the reduction rule used :
\paragraph{Main reduction rules}
\begin{itemize}
  \item ($\beta_v$) Then the typing derivation of $M$ is of the form :
  \begin{mathpar}
    \inferrule* [Right=(subst-r)] {
      R;\Gamma \vdash \text{Reg}_r B \qquad \forall U \in \mathcal{U}:\ R;\Gamma
      \vdash U : (B,\emptyset) \qquad
      \inferrule* [Right=(app)] {
        \inferrule* [Right=(lam),rightskip=-4em] {
          R; \Gamma, x : A \vdash M : (\alpha, e)
        }
        {R; \Gamma \vdash (\lambda x. M) : (A \sur{\to}{e}, \emptyset)}
        R;\Gamma \vdash V : (A,\emptyset)
      }
      {R; \Gamma \vdash (\lambda x. M)\ V : (\alpha,e) }
    }
    { R;\Gamma \vdash \refssl{r}{U}{(\lambda x. M)\ V} : (\alpha,e)}
  \end{mathpar}
  Then one can form the derivation
  \begin{mathpar}
    \inferrule* [Right=(subst-r)] {
      R;\Gamma \vdash \text{Reg}_r B
      \qquad
      \forall U \in \mathcal{U}:\ R;\Gamma \vdash U : (B,\emptyset)
      \qquad
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash V : (A,\emptyset)
        \qquad
        R;\Gamma,x:A \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \vars{x}{V}{M} : (\alpha,e) }
    }
    { R;\Gamma \vdash \refssd{r}{U}{\vars{x}{V}{M}} : (\alpha,e) }
    %       \\
    % \inferrule* [Right=(subst)] {
    %   \inferrule* [Left=(weak)] {
    %     R;\Gamma \vdash V: (A, \emptyset)
    %   }
    %   { R;\Gamma,x:A \vdash V : (A,\emptyset) }
    %   \qquad
    %   \inferrule* [Right=(subst-r)] {
    %     \inferrule* [Left=(weak)] {
    %     }
    %     { R;\Gamma,x:A \vdash \text{Reg}_r B }
    %     \qquad
    %     \inferrule* [Right=(weak)] {
    %       \forall U \in \mathcal{U}:\ R;\Gamma \vdash U : (B,\emptyset)
    %     }
    %     {\forall U \in \mathcal{U}:\ R;\Gamma,x:A \vdash U : (B,\emptyset)}
    %     \qquad
    %     R;\Gamma,x:A \vdash M : (\alpha,e)
    %   }
    %   {R;\Gamma,x:A \vdash \substdown{r}{\mathcal{U}}{M}}
    % }
    % { R;\Gamma \vdash \varss{\sigma}{\substdown {r}{\mathcal{U}}{M}} : (\alpha,e) }
  \end{mathpar}
  using the admissibility of generalized weakening.
  % \item (\texttt{set})
  %   \begin{mathpar}
  %     \inferrule* {
  %       R;\Gamma \vdash r : \text{Reg}_r A
  %       \qquad
  %       R;\Gamma \vdash V : (A,\emptyset)
  %     }
  %     { R;\Gamma \vdash \text{set}(r,V) : (\text{Unit}, \{ r \}) }
  %   \end{mathpar}
  %   That we use to build the derivation
  %   \begin{mathpar}
  %     \inferrule* [Left=(subst-r)] {
  %       \inferrule* [Left=(unit)] { }
  %       { R;\Gamma \vdash \ast : (\text{Unit}, \emptyset) }
  %       \qquad
  %       R;\Gamma \vdash r : \text{Reg}_r A
  %       \qquad
  %       R;\Gamma \vdash V : (A, \emptyset)
  %     }
  %     { R;\Gamma \vdash \substup{r}{[V]}{\ast} }
  %   \end{mathpar}
\end{itemize}

\paragraph{Variables substitutions}
\begin{itemize}
  \item ($\texttt{subst}_\texttt{var}$)
    We have
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_i) : (A_i,\emptyset)
        \qquad
        \inferrule* [Right=(var)] { }
        { R;\Gamma' \vdash y : (B,\emptyset) }
      }
      { R;\Gamma \vdash \varss{\sigma}{y} : (B,\emptyset) }
    \end{mathpar}
    with $\Gamma' = \Gamma,x_1 : A_1,\ldots,x_n:A_n$ if $i$ ranges over $1
    \ldots n$. We have
    \begin{mathpar}
      \inferrule* [Right=(var)] { }
      { R;\Gamma \vdash y : (B,\emptyset) }
    \end{mathpar}
    if $\sigma$ is undefined at $y$ or
    \begin{mathpar}
      R;\Gamma \vdash \sigma(y) : (A_{i_0},\emptyset)
    \end{mathpar}
    if $\exists i_0, x_{i_0} = y$ and thus $A_{i_0}=B$.
  \item \rrulet{subst}{unit} : just apply the \trule{unit} typing rule.
  \item \rrulet{subst}{app}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma' \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \mathcal{V}(r_i):\ R;\Gamma' \vdash V : (A_i, \emptyset)
        \inferrule* [Right=(app)] {
          R;\Gamma' \vdash M : (C \sur{\to}{e_1} \alpha, e_2)
          \qquad
          R;\Gamma' \vdash N : (C,e_3)
        }
        { R;\Gamma' \vdash M\ N : (\alpha,e) }
      }
      { R;\Gamma' \vdash \refssl{}{V}{M\ N} }
      \\
      \inferrule* [Left=(subst)] {
        R;\Gamma' \vdash \sigma(x_j) : (B_j, \emptyset)
        \qquad
        R;\Gamma' \vdash \refssl{}{V}{M\ N}
      }
      { R;\Gamma \vdash \varss{\sigma}{\refssl{}{V}{M\ N}} : (\alpha,e)
      }
    \end{mathpar}
    With $\Gamma' = \Gamma,x_1:A_1,\ldots,x_n:A_n$ and $e_1 \cup e_2 \cup e_3 = e$. We can derive

    \begin{mathpar}
      \inferrule* [Right=(app)] {
        \inferrule* [Left=(subst)] {
            R;\Gamma \vdash \sigma(x_j) : (B_j,\emptyset)
            \qquad
            R;\Gamma' \vdash M : (C \sur{\to}{e_1} \alpha, e_2)
          }
          { R;\Gamma \vdash \varss{\sigma}{M} : (C \sur{\to}{e_1} \alpha, e_2)
          }
          \qquad
          \inferrule* [Right=(subst)] {
            R;\Gamma \vdash \sigma(x_j): (B_j,\emptyset)
            \qquad
            R;\Gamma' \vdash N : (C,e_3)
          }
          { R;\Gamma \vdash \varss{\sigma}{N} : (C,e_3) }
        }
        { R;\Gamma \vdash (\varss{\sigma}{M})\ (\varss{\sigma}{N}) : (\alpha,e) }
    \end{mathpar}
    For any $V \in \multv{V}(r_i)$, one has
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_j) : (B_j,\emptyset)
        \qquad
        R;\Gamma' \vdash V : (A_i,\emptyset)
      }
      { R;\Gamma \vdash \varss{\sigma}{V} : (A_i,\emptyset) }
    \end{mathpar}
    And finally
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash P : (\alpha,e)
        \qquad
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \mathcal{V}(r_i):\ R;\Gamma \vdash \varss{\sigma}{V} : (A_i,\emptyset)
      }
      { R;\Gamma \vdash
        \refrawsl{}{\varss{\sigma}{\multv{V}}}{(\varss{\sigma}{M})\
        (\varss{\sigma}{N})}
      }
    \end{mathpar}
  \item \rrule{subst}{\lambda} :
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_i) : (A_i, \emptyset)
        \qquad
        \inferrule* [Right=(lam)] {
          R;\Gamma',y:A \vdash M : (\alpha, e)
        }
        { R;\Gamma' \vdash \lambda y . M : (A \sur{\to}{e} \alpha, \emptyset)
        }
      }
      { R;\Gamma \vdash \varss{\sigma}{\lambda y. M} :  (A \sur{\to}{e} \alpha, \emptyset) }
    \end{mathpar}
    then we just swap the two rules :
    \begin{mathpar}
      \inferrule* [Right=(lam)] {
        \qquad
        \inferrule* [Right=(subst)] {
          \inferrule* [Left=(weak)] {
            R;\Gamma \vdash \sigma(x_i) : (A_i, \emptyset)
          }
          { R;\Gamma,y:A \vdash \sigma(x_i) : (A_i, \emptyset) }
          \qquad
          R;\Gamma',y:A \vdash M : (\alpha, e)
        }
        { R;\Gamma,y:A \vdash \varss{\sigma}{M} : (\alpha, \emptyset)
        }
      }
      { R;\Gamma \vdash \lambda y . (\varss{\sigma}{M}) :  (A \sur{\to}{e} \alpha, \emptyset) }
    \end{mathpar}
  \item \rrulet{subst}{get} :
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_i): (A_i, \emptyset)
        \qquad
        \inferrule* [Right=(get)] {
          R;\Gamma' \vdash r : \text{Reg}_r B
        }
        { R;\Gamma' \vdash \get{r} : (B, \{ r \}) }
      }
      { R;\Gamma \vdash \varss{\sigma}{\get{r}} : (B, \{ r \}) }
    \end{mathpar}
    We can juste recast the get rule without the weakened $x_i$s :
    \begin{mathpar}
      \inferrule* [Right=(get)] {
        R;\Gamma \vdash r : \text{Reg}_r B
      }
      { R;\Gamma \vdash \get{r} : (B, \{ r \}) }
    \end{mathpar}
  % \item \rrulet{subst}{set} :
  %   \begin{mathpar}
  %     \inferrule* [Right=(subst)] {
  %       R;\Gamma \vdash V : (A, \emptyset)
  %       \qquad
  %       \inferrule* [Right=(set)] {
  %         R;\Gamma,x:A \vdash r : \text{Reg}_r B
  %         \qquad
  %         R;\Gamma,x:A \vdash U : (B,\emptyset)
  %       }
  %       { R;\Gamma,x:A \vdash \text{set}(r,U) : (\text{Unit}, \{ r \}) }
  %     }
  %     { R;\Gamma \vdash \varss{\sigma}{\text{set}(r,U)} : (\text{Unit}, \{ r \}) }
  %   \end{mathpar}
  %   Then
  %   \begin{mathpar}
  %     \inferrule* [Right=(set)] {
  %       R;\Gamma,x:A \vdash r : \text{Reg}_r B
  %       \qquad
  %       \inferrule* [Right=(subst)] {
  %         R;\Gamma \vdash V : (A, \emptyset)
  %         \qquad
  %         R;\Gamma,x:A \vdash U : (B,\emptyset)
  %       }
  %       { R;\Gamma \vdash \varss{\sigma}{U} : (B, \emptyset) }
  %     }
  %     { R;\Gamma,x:A \vdash \text{set}(r,\varss{\sigma}{U}) : (\text{Unit}, \{ r \}) }
  %   \end{mathpar}
  \item \rrule{subst}{\parallel} :
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_j): (A_j, \emptyset)
        \qquad
        \inferrule* [Right=(par)] {
          i = 1,2
          \qquad
          R;\Gamma' \vdash M_i : (\alpha_i, e_i)
        }
        { R;\Gamma' \vdash M_1 \parallel M_2 : (\mathbf{B},e) }
      }
      { R;\Gamma \vdash \varss{\sigma}{M_1 \parallel M_2} : (\mathbf{B},e) }
    \end{mathpar}
    Then
    \begin{mathpar}
      \inferrule* [Right=(par)] {
        i=1,2
        \qquad
        \inferrule* [Right=(subst)] {
          R;\Gamma \vdash \sigma(x_j) : (A_j, \emptyset)
          \qquad
          R;\Gamma' \vdash M_i : (\alpha_i, e_i)
        }
        { R;\Gamma \vdash \varss{\sigma}{M_i} : (\alpha_i, e_i) }
      }
      { R;\Gamma \vdash (\varss{\sigma}{M_1}) \parallel (\varss{\sigma}{M_2}) : (\mathbf{B},e) }
    \end{mathpar}
  \item \rrule{subst}{subst-r} :
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_j): (A_j,\emptyset)
        \qquad
        \inferrule* [Right=(subst-r)] {
          R;\Gamma' \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall U \in \mathcal{U}(r_i):\ R;\Gamma' \vdash U : (A_i, \emptyset)
          \qquad
          R;\Gamma' \vdash M : (\alpha,e)
        }
        { R;\Gamma' \vdash \refssd{}{\mathcal{U}}{M} : (\alpha,e) }
      }
      { R;\Gamma \vdash \varss{\sigma}{\refssd{}{\mathcal{U}}{M}} : (\alpha,e) }
    \end{mathpar}
    Then for any $U \in \mathcal{U}(r_i)$
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma' \vdash U : (A_i, \emptyset)
      }
      { R;\Gamma \vdash \varss{\sigma}{U} : (A_i,\emptyset) }
    \end{mathpar}
    It follows
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall U \in \multv{U}(r_i):\
          R;\Gamma \vdash U : (A_i, \emptyset)
        \qquad
        \inferrule* [Right=(subst)] {
          R;\Gamma \vdash \sigma(x_j) : (A_j,\emptyset)
          \qquad
          R;\Gamma' \vdash M : (\alpha,e)
          }
          { R;\Gamma \vdash \vars{\sigma}{M} : (\alpha,e) }
        }
        { R;\Gamma \vdash
          \refssd{}{\varss{\sigma}{\multv{U}}}{\varss{\sigma}{M}} : (\alpha,e) }
    \end{mathpar}
  \item \rrule{subst}{subst-r'} : exactly as the previous case (the typing rules
    and reduction rules being similar)
  \item \rrule{subst}{merge}
    We need a simple substitution lemma to handle this case of the meta
    substitution.
    Let $\Gamma_{\mathcal{I}} = \bullet_{i \in
    \mathcal{I}} x_i : A_i$ and $\Gamma_{\mathcal{J}} = \bullet_{j \in
    \mathcal{J}} x_j : A_j$ where $\bullet$ is the list concatenation.
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        \forall U \in \mathcal{U}(r_j):\ R;\Gamma \vdash U : (A_j,\emptyset)
        \qquad
        \inferrule* [Right=(subst)] {
          \forall V \in \mathcal{V}(r_i):\
          R;\Gamma,\Gamma_\mathcal{J} \vdash V : (A_i,\emptyset)
          \qquad
          R;\Gamma,\Gamma_\mathcal{J},\Gamma_\mathcal{I} \vdash M : (\alpha,e)
        }
        { R;\Gamma_\mathcal{J} \vdash \vars{(x_i)}{(V_i)}{M} : (\alpha,e) }
      }
      { R;\Gamma \vdash \vars{(y_j)}{(U_j)}{\vars{(x_i)}{(U_i)}{M}} : (\alpha,e) }
    \end{mathpar}
    Then we have
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        \forall V \in \mathcal{V}_i:\ R;\Gamma \vdash \varmetas{(y_j)}{(U_j)}{V} : (A_i,\emptyset)
        \qquad
        \forall U \in \mathcal{U}_j:\ R;\Gamma \vdash U : (A_j,\emptyset)
        \qquad
        R;\Gamma,\Gamma_\mathcal{J},\Gamma_\mathcal{I} \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \vars{(z_i)}{(W_i)}{M} : (\alpha,e) }
    \end{mathpar}
    \emph{TODO : TO COMPLETE}
\end{itemize}

\paragraph{Downward references substitutions}
\begin{itemize}
  \item \rrulet{subst-r}{val}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall U \in \mathcal{U}(r_i):\ R;\Gamma \vdash U : (A_i,\emptyset)
        \qquad
        \inferrule* [Right=(sub)] {
          R;\Gamma \vdash V : (A,\emptyset)
        }
        { R;\Gamma \vdash V : (A,\{r\}) }
      }
      { R;\Gamma \vdash \refssd{}{U}{V} : (A,e) }
    \end{mathpar}
    Then we just reuse the typing derivation of
    \begin{mathpar}
      \inferrule* [Right=(sub)] {
        R;\Gamma \vdash V : (A,\emptyset)
      }
      { R;\Gamma \vdash V : (A,\{r\}) }
    \end{mathpar}
  % \item \rrulet{subst-r}{set}
  %   We assume $s \neq r$. When $s = r$, then the application of \trule{sub} is
  %   not needed anymore.
  %   \begin{mathpar}
  %     \inferrule* [Right=(subst-r)] {
  %       R;\Gamma \vdash r : \text{Reg}_r B
  %       \qquad
  %       \forall U \in \mathcal{U}:\ R;\Gamma \vdash U : (B,\emptyset)
  %       \qquad
  %       \inferrule* [Right=(sub)] {
  %         \inferrule* [Right=(set)] {
  %           R;\Gamma \vdash s : \text{Reg}_s A
  %           \qquad
  %           R;\Gamma \vdash V : (A,\emptyset)
  %         }
  %         { R;\Gamma \vdash \text{set}(s,V) : (\text{Unit},\{s\}) }
  %       }
  %       { R;\Gamma \vdash \text{set}(s,V) : (\text{Unit},\{s,r\}) }
  %     }
  %     { R;\Gamma \vdash \substdown{r}{U}{\text{set}(s,V)} : (\text{Unit},\{r,s\}) }
  %   \end{mathpar}
  %   As for the previous case, we have then
  %   \begin{mathpar}
  %     \inferrule* [Right=(sub)] {
  %       R;\Gamma \vdash \text{set}(s,V) : (\text{Unit},\{r\})
  %     }
  %     { R;\Gamma \vdash \text{set}(s,V) : (\text{Unit},\{r,s\}) }
  %   \end{mathpar}
  \item \rrule{subst-r}{\parallel}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall U \in \mathcal{U}(r_i):\ R;\Gamma \vdash U : (A_i,\emptyset)
        \qquad
        \inferrule* [Right=(par)] {
          R;\Gamma \vdash M_i : (\alpha_i,e_i)
        }
        { R;\Gamma \vdash M_1 \parallel M_2 : (\mathbf{B},e) }
      }
      { R;\Gamma \vdash \refssd{}{U}{M_1 \parallel M_2} :
      (\mathbf{B},e) }
    \end{mathpar}
    Then we commute the two rules
    \begin{mathpar}
      \inferrule* [Right=(par)] {
        \inferrule* [Right=(subst-r)] {
          R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall U \in \mathcal{U}(r_i) :\ R;\Gamma \vdash U : (A_i,\emptyset)
          \qquad
          R;\Gamma \vdash M_i : (\alpha_i,e)
        }
        { R;\Gamma \vdash \refssd{}{U}{M_i} : (\alpha_i,e) }
      }
      { R;\Gamma \vdash (\refssd{}{U}{M_1}) \parallel
      (\refsd{}{U}{M_2}) : (\mathbf{B},e) }
    \end{mathpar}
  \item \rrulet{subst-r}{subst-r'}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \refssu{}{V}{M} : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \mathcal{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash \refssd{}{V}{M} : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{U}{\refssu{}{V}{M}} : (\alpha,e) }
    \end{mathpar}
    We just swap the two rules
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{U}{M} : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \mathcal{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash \refssd{}{U}{M} : (\alpha,e)
      }
      { R;\Gamma \vdash \refssu{}{V}{\refssd{}{U}{M}} : (\alpha,e) }
      \\
    \end{mathpar}
  \item \rrule{subst-r-merge}{}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{V}{M} : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash \refssd{}{V}{M} : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{U}{\refssd{}{V}{M}} : (\alpha,e) }
    \end{mathpar}
    Then we have
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_k : \text{Reg}_{r_k} A_k
        \qquad
        \forall W \in (\multv{U} + \multv{V})(x_k):\ R;\Gamma \vdash W : (A_k,\emptyset)
        \qquad
        R;\Gamma \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \refrawsd{}{\multv{V},\multv{U}}{M} : (\alpha,e) }
    \end{mathpar}
  \item \rrule{subst-r-app}{}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        \inferrule* [Right=(app)] {
          R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha,e_2)
          \qquad
          R;\Gamma \vdash N : (A,e_3)
        }
        { R;\Gamma \vdash M\ N : (\alpha,e) }
      }
      { R;\Gamma \vdash \refssl{}{V}{M\ N} : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash \refssl{}{V}{M\ N} : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{U}{\refssl{}{V}{M\ N}} : (\alpha,e) }
    \end{mathpar}
    That we can turn into
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha,e_2)
      }
      { R;\Gamma \vdash \refssd{}{U}{M} : (A \sur{\to}{e_1} \alpha,e_2) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash N : (A,e_3)
      }
      { R;\Gamma \vdash \refssd{}{U}{N} : (A,e_3) }
      \\
      \inferrule* [Right=(app)] {
        R;\Gamma \vdash \refssd{}{U}{M} : (A \sur{\to}{e_1} \alpha,e_2)
        \qquad
        R;\Gamma \vdash \refssd{}{U}{N} : (A,e_3)
      }
      { R;\Gamma \vdash (\refssd{}{U}{M})\ (\refssd{}{U}{N})  : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_k : \text{Reg}_{r_k} A_k
        \qquad
        \forall W \in (\multv{V} + \multv{U})(r_i):\ R;\Gamma \vdash W : (C_i,\emptyset)
        \qquad
        R;\Gamma \vdash (\refssd{}{U}{M})\ (\refssd{}{U}{N}) : (\alpha,e)
      }
      { R;\Gamma \vdash \refssl{}{W}{(\refssd{}{U}{M})\ (\refssd{}{U}{N})}
      }
    \end{mathpar}
  \item \rrulet{subst-r}{get}
    Write $\mathbf{S} = M_1 + \ldots + M_n + []$, with $n \geq 0$. The
    derivation tree of $P = C[E[\refssd{}{V}{\get{r}}]]$
    is of the form
    \begin{mathpar}
      \inferrule* {
        \inferrule* {
          \inferrule* [Right=(subst)] {
            R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
            \qquad
            \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
            \qquad
            R;\Gamma \vdash \get{r} : (A,e)
          }
          { R;\Gamma \vdash \refssd{}{V}{\get{r}} : (A,e) }
        }
        { [\ldots] }
      }
      { R;\Gamma' \vdash P : (\alpha,e') }
    \end{mathpar}
    And of the full term :
    \begin{mathpar}
        \inferrule* [Right=(sum)] {
          \ptentre{i}{1}{n}\ R;\Gamma \vdash M_i : (\alpha,e')
          \qquad
          R;\Gamma \vdash P : (\alpha,e')
        }
        { R;\Gamma \vdash S[P] : (\alpha,e') }
    \end{mathpar}
    To get the first term of the reduct, we just remove the subst rule :
    \begin{mathpar}
      \inferrule* [Right=(sum)] {
        \ptentre{i}{1}{n}\ R;\Gamma \vdash M_i : (\alpha,e')
        \qquad
        \inferrule* {
          \inferrule* { R;\Gamma \vdash \get{r} : (A,e) }
          { [\ldots] }
        }
        { R;\Gamma' \vdash C[E[\get{r}]] : (\alpha,e') }
      }
      { R;\Gamma' \vdash S[C[E[\get{r}]]] : (\alpha,e') }
    \end{mathpar}
    Now if $\multv{V}$ is undefined at $r$ we are done. Otherwise, we substitute
    $\get{r}$ by a value $V \in \multv{V}(r)$ :
    \begin{mathpar}
      \inferrule* {
        \inferrule* {
          \inferrule* [Right=(sub)] {
            R;\Gamma \vdash V : (A,\emptyset)
          }
          { R;\Gamma \vdash V : (A,e) }
        }
        { [\ldots] }
      }
      { R;\Gamma' \vdash C[E[V]] : (\alpha,e') }
    \end{mathpar}
    And we can finally derive
    \begin{mathpar}
      \inferrule* [Right=(sum)] {
        \forall V \in \mathcal{V}_{i_0}:\ R;\Gamma' \vdash C[E[V]] : (\alpha,e')
        \qquad
        R;\Gamma' \vdash S[C[E[\get{r}]]] : (\alpha,e')
      }
      { R;\Gamma' \vdash S[C[E[\get{r}]]] + \sum_{V \in
        \multv{V}(r)}C[E[V]] : (\alpha,e') }
    \end{mathpar}

\end{itemize}

\paragraph{Upward references substitutions}
\begin{itemize}
  \item \rrule{subst-r'}{\parallel}
    \begin{mathpar}
      \inferrule* [Right=(par)] {
        R;\Gamma \vdash M : (\alpha_1,e_1)
        \qquad
        \inferrule* [Right=(subst-r)] {
          R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
          \qquad
          R;\Gamma \vdash N : (\alpha_2,e_2)
        }
        { R;\Gamma \vdash \refssu{}{V}{N} : (\alpha_2,e_2) }
      }
      { R;\Gamma \vdash M \parallel (\refssu{}{V}{N}) :
      (\mathbf{B},e) }
    \end{mathpar}
    Then we have
    \begin{mathpar}
      \inferrule* [Right=(par)] {
        \inferrule* [Left=(subst-r)] {
          R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
          \qquad
          R;\Gamma \vdash M : (\alpha_1,e_1)
        }
        { R;\Gamma \vdash (\refssd{}{V}{M}) : (\alpha_1,e_2) }
        \qquad
        R;\Gamma \vdash N : (\alpha_2,e_2)
      }
      { R;\Gamma \vdash (\refssd{}{V}{M}) \parallel N :
        (\mathbf{B},e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V_i : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash (\refssd{}{V}{M}) \parallel N :
        (\mathbf{B},e)
      }
      { R;\Gamma \vdash
        \refssu{}{V}{(\refssd{}{V}{M}) \parallel N} :
        (\mathbf{B},e) }
    \end{mathpar}
  \item \rrulet{subst-r'}{app-left}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash M : (A \sur{\to}{e_2} \alpha,e_3)
      }
      { R;\Gamma \vdash \refssu{}{V}{M} : (A \sur{\to}{e_2}
          \alpha,e_3) }
      \\
      \inferrule* [Right=(app)] {
        R;\Gamma \vdash (\refssu{}{V}{M})\ : (B \sur{\to}{e_1}
        \alpha,e_2)
        \qquad
        R;\Gamma \vdash N : (A,e_3)
      }
      { R;\Gamma \vdash (\refssu{}{V}{M})\ N : (\alpha,e) }

      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash (\refssu{}{V}{M})\ N : (\alpha,e)
      }
      { R;\Gamma \vdash \refssl{}{U}{(\refssu{}{V}{M})\
        N} : (\alpha,e) }
    \end{mathpar}
    That we turn to
    \begin{mathpar}
      \inferrule* [Right=(app)] {
        R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha,e_2)
        \qquad
        \inferrule* [Right=(subst-r)] {
          R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
          \qquad
          R;\Gamma \vdash N : (A,e_3)
        }
        { R;\Gamma \vdash \refssd{}{V}{N} : (A,e_3) }
      }
      { R;\Gamma \vdash M\ (\refssd{}{V}{N}) : (\alpha,e) }
      \\
      \inferrule* [Right=(subt-r)] {
        R;\Gamma \vdash r_k : \text{Reg}_{r_k} C_k
        \qquad
        \forall W \in (\multv{V} + \multv{U})(r_k):\ R;\Gamma \vdash W : (C_k,\emptyset)
        \qquad
        R;\Gamma \vdash M\ (\refrawsd{}{\multv{U},\multv{V}}{N}) : (\alpha,e)
      }
      { R;\Gamma \vdash  \refrawsl{}{\multv{U},\multv{V}}{M\ (\refssd{}{V}{N})
        } : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_k : \text{Reg}_{r_k} C_k
        \qquad
        \forall W \in (\multv{U} + \multv{V})(r_k):\ R;\Gamma \vdash W : (C_k,\emptyset)
        \qquad
        R;\Gamma \vdash \refrawsl{}{\multv{U},\multv{V}}{M\ (\refssd{}{V}{N})} :
        (\alpha,e)
      }
      { R;\Gamma \vdash \refssu{}{\multv{V}}{\refrawsl{}{\multv{U},\multv{V}}{M\ (\refssd{}{V}{N})
        }}  : (\alpha,e) }
    \end{mathpar}
  \item \rrulet{subst-r'}{app-right} : same as \rrulet{subst-r'}{app-left}
  \item \rrule{subst-r'}{\top}
    Assume that $\mathbf{S} = M_1 + \ldots + M_n + []$, with $n \geq 0$, then we
    have
      \begin{mathpar}
        \inferrule* [Right=(subst-r)] {
          R;\Gamma \vdash r_j : \text{Reg}_{r_j} A_j
          \qquad
          \forall V \in \multv{V}(r_j):\ R;\Gamma \vdash V : (A_j,\emptyset)
          \qquad
          R;\Gamma \vdash M : (\alpha,e)
        }
        { R;\Gamma \vdash \refssu{}{V}{M} : (\alpha,e) }
        \\
        \inferrule* [Right=(sum)] {
          \ptentre{i}{1}{n}\ R;\Gamma \vdash M_i : (\alpha,e)
          \qquad
          R;\Gamma \vdash \refssu{}{V}{M} : (\alpha,e)
        }
        { R;\Gamma \vdash S[\refssu{}{V}{M}] : (\alpha,e) }
      \end{mathpar}
      We juste have to remove the \rrulet{subst-r}{} rule to get the result :
      \begin{mathpar}
        \inferrule* [Right=(sum)] {
          \ptentre{i}{1}{n}\ R;\Gamma \vdash M_i : (\alpha,e)
          \qquad
          R;\Gamma \vdash M : (\alpha,e)
        }
        { R;\Gamma \vdash S[M] : (\alpha,e) }
      \end{mathpar}
\end{itemize}
\end{proof}

\begin{mlem*}{Progress}\label{mlem-progress}\\
  Let $R \vdash \mathbf{M} : (A,e)$ be a typable program that does not reduce
  further. Then $\mathbf{M} =
  \sum_{i=1}^n (M^i_1 \parallel \ldots \parallel M^i_{l_i})$ where $M^i_1$ is
  either a value or of the form
  $$ M_{\text{norm}} ::= \get{r} \mid
  \refssl{r}{V}{M_{\text{norm}}\ V} \mid \refssl{r}{V}{V\
    M_{\text{norm}}} \mid \refssl{r}{V}{M_{\text{norm}}\
    M_{\text{norm}}} $$
\end{mlem*}

\begin{proof}
  By recurrence on $\mathbf{M}$. First assume that $\mathbf{M} = M$ :
  \begin{itemize}
    \item If $M$ is a value or $M = \get{r}$, there is nothing to do
    \item If $M = \varss{\sigma}{M'}$, then there is always a \rrulet{subst}{}
      rule that can be applied whatever $M'$ is.
    \item If $M = \refssd{r}{V}{M'}$, we can use a \rrulet{subst-r}{} rule
      unless $M' = \varss{\sigma}{M''}$. But then, by the previous case, $M'$
      reduces hence so does $M = F[M']$.
    \item If $M = \refssl{r}{V}{P\ Q}$, we have the type derivation
      \begin{mathpar}
        \inferrule* [Right=(subst-r)] {
          \inferrule* [Right=(app)] {
            R; \vdash P : (A \sur{\to}{e_1} \alpha,e_2)
            \qquad
            R; \vdash Q : (A,e_3)
          }
          { R; \vdash P\ Q : (\alpha,e) }
        }
        { R; \vdash \refssl{r}{V}{P\ Q} : (\alpha,e) }
      \end{mathpar}
      If $P \to P'$ by any rule
      excepted \rrule{subst-r'}{\top}, $M = E[P]$ with $E =
      \refssl{r}{V}{[.]\ Q}$ and thus $M$ also reduces. The same
      applies to $Q$. \\
      Assume now that $P \to P'$ by \rrule{subst-r'}{\top}, meaning that $P =
      \refssu{r}{V}{P'}$. Then we can apply
      \rrulet{subst-r'}{app-left} to $M$. Similarly, we can apply
      \rrulet{subst-r'}{app-right} if $Q = \substup{r}{\mathcal{V}}{Q'}$.
      Thus by induction $P$ and $Q$ are themselves either values, of the form $M_\text{norm}$, or a
      parallel of values and $M_\text{norm}$ forms. It is immediate that neither
      $P$ or $Q$ can be of the form $M_1 \parallel M_2$ (they would have to be
      typed by $\mathbf{B}$ and coudn't be applied or applied to), thus $P$ and
      $Q$ are either values or $M_\text{norm}$.
      \\
      Now, if both are values (note that $P$ and $Q$ must be closed terms), the only way for $P$ to have
      type $A \sur{\to}{e_1} \alpha$ is to be an abstraction, but then $M$ would
      reduce by $(\beta_v)$. Thus one of them is of the form $M_\text{norm}$ and
      so is $M$.
    % \item If $M = \text{set}(r,V)$ then it reduces by \rrule{set}{}.
    \item if $M = \refssu{r}{V}{M'}$ then it reduces by
      \rrule{subst-r'}{\top}.
    \item if $M = P \parallel Q$, assume that $P \to P'$ by any
      rule excepted \rrule{subst-r'}{\top}, then so would $M$, taking $E =[.]$
      and $C = [.] \parallel Q$. Same for $Q$.
      \\
      Now if $P = \refssu{r}{V}{P'}$ (or $Q$), then $M$ reduces by
      \rrule{subst-r'}{\parallel}. Thus $P$ and $Q$ does not reduce, and by
      induction, are of
      the form $\parallel_i M_i$ with $M_i$ a value or of the form $M_\text{norm}$, hence so
      is $M$.
  \end{itemize}
  Finally, if $\mathcal{M} = \sum M_i$, then $\mathcal{M}$ is normal if and
  only if each $M_i$ is and the induction hypothesis immediatly gives the result.
\end{proof}


==> paper-csl-long arxiv/parts/simulation-languages.tex <==
\section{Simulation}

\subsection{Definitions and lemmas}

\newcommand{\vstore}{\multv{V}_S}
\newcommand{\strans}{$\overline{\phantom{M}}^S$}
\newcommand{\sleq}{\rightsquigarrow_s}

\begin{mdef}{Translation of \lamadio in \lthis}\\
    Let $M$ be a term and $S$ be a store of \lamadio.
    S can be written as
    \[
      S = r_1 \Leftarrow V^1_1 \parallel \ldots \parallel r_1
      \Leftarrow V^1_{k_1} \parallel \ldots \parallel r_n \Leftarrow
      V^n_1 \parallel \ldots \parallel r_n \Leftarrow
      V^n_{k_n}
    \]
    Let $\multv{V}_S : r_i \mapsto [V^i_1, \ldots, V^i_{k_i}]$.
  We define the translation of $M$ under $S$ by
    \begin{itemize}
      \item If $M = V$ or $M = \text{set}(s,V)$ then $\overline{M}^S = M$
      \item If $M = N\ N'$ then $\overline{M}^S = \refsrawsl{r}{\vstore}(\overline{N}^S)\
        (\overline{N'}^S)$
      \item If $M = \get{s}$ then $\overline{M}^S =
        \refsrawsd{r}{\vstore}{\get{s}}$
      \item If $M = N \parallel N'$ then $\overline{M}^S = \overline{N}^S
        \parallel \overline{N'}^S$
    \end{itemize}

    In fact, one can see that $\overline{M}^S$ is the normal form of
    $\refsrawsd{r}{\vstore}{M}$ for the reduction defined by all
    \rrulet{subst-r}{} rules except \rrulet{subst-r}{get}.

    We extend it to contexts $E,F$ and $G$ by adding the rule $\overline{[.]}^S = [.]$.
    \\
    Finally, for any program $P = M \parallel S$, we define $\overline{P} =
    \overline{M}^S$.
    If $P = M$ then $\overline{P} = \overline{M} = M$.
  \end{mdef}

  % Originally put restrictions like $M$ and $N$ must not be parallel,
  % or that some reduction on parallel must not be used, but now I don't
  % see why this would be the case, so just removing
  \begin{mlem}{Context reduction}\label{mlem-ctxt-red}\\
    Let $M,N$ be terms of \lthis such that $M \to^\ast N$ without using
    \rrule{subst-r}{\top}, then for any
    context $C$ and $E$, $C[E[M]] \to^\ast C[E[N]]$ using the same reduction
    rules.
  \end{mlem}

  \begin{mlem}{Context decomposition}\label{mlem-ctxt-decomp}\\
    Let $P$ be a program of \lamadio,
    \begin{itemize}
      \item $P = C[E[M]] \text{ with } C = [.] \text{ or } C = [.] \parallel N \implies
        \overline{P} = P$
      \item $P = C[E[M]] \text{ with } C = [.] \parallel N \parallel S \implies
        \overline{P} = \overline{E}^S[\overline{M}^S] \parallel \overline{N}^S$
    \end{itemize}
  \end{mlem}

  \begin{proof}
    This is an easy induction following the definition of \strans.
  \end{proof}

  \begin{mlem}{Substitution for \strans}\label{mlem-subst}\\
    Let $M,M'$ be terms, $V$ a value and $S$ a
    store of \lamadio. Then
    \[
      \overline{M[x/V]}^S = \overline{M}^S[x/V]
    \]
  \end{mlem}
  \begin{proof}
    By induction
  \end{proof}

  \begin{mlem}{Absorption}\label{mlem-absorption}\\
    Let $M$ be a term and $S = S' \parallel r \Leftarrow V$ be a store of
    \lamadio, $C$ and $E$ be context of \lthis, and $\multv{V}
    : r \mapsto [V]$. Then
    $$C[E[\refssd{}{V}{\overline{M}^{S'}}]] \to_\texttt{aux}^\ast
    C[E[\overline{M}^{S}]]$$
  \end{mlem}

  \begin{proof} By induction on $M$, using the definition of
    \strans and the \texttt{subst-r} reductions.
  \end{proof}

  \begin{mlem}{Diffusion}\label{mlem-diffusion}\\
    Let $N$ be a term, $E$ a context, $S = S' \parallel r \Leftarrow V$ a store of
    \lamadio and $\multv{V} : r \mapsto [V]$. Let $M$ be a term of \lthis. Then
    \begin{equation}\label{mlem-diff-eq1}
      \overline{E}^{S'}[\refssu{}{V}{M}]
      \to_\texttt{aux}^\ast \refssu{}{V}{\overline{E}^S[M]}
    \end{equation}
    \begin{equation}\label{mlem-diff-eq2}
      \refssu{}{V}{M} \parallel \overline{N}^{S'}
      \to_\texttt{aux}^\ast \refssu{}{V}{(M \parallel
      \overline{N}^S)}
    \end{equation}
    \begin{equation}\label{mlem-diff-eq3}
      \overline{E}^{S'}[\refssu{}{V}{M}] \parallel \overline{N}^{S'}
      \to_\texttt{aux}^\ast \refssu{}{V}{\overline{E}^S[M] \parallel
      \overline{N}^S}
    \end{equation}
    using only rules \rrulet{subst-r}{} or \rrulet{subst-r'}{}.
  \end{mlem}

  \begin{proof}
    \begin{itemize}

      \item For (\ref{mlem-diff-eq1}), we work by induction on $E$. As we
        will need \ref{mlem-ctxt-red}, we add the induction hypothesis
        that the rule $(\texttt{subst-r'}_\top)$ is not used.
        \begin{itemize}
          \item $\overline{E}^{S'} = [.]$ nothing to do
          \item $\overline{E}^{S'} = \refssl{s}{U}{\overline{E'}^{S'}\
          \overline{M'}^{S'}}$\\
            By IH, $\overline{E'}^{S'}[\refssu{}{V}{M}] \to^\ast
            \refssu{}{V}{\overline{E'}^{S}[M]}$ using no
            \rrule{subst-r'}{\top} rules.
            We use \ref{mlem-ctxt-red} and get
            $$\overline{E}^{S'}[\refssu{}{V}{M}] \to^\ast
            \refssl{s}{U}{(\refssu{}{V}{\overline{E'}^{S}[M]})
            \ \overline{M'}^{S'}}$$
            We then apply \rrulet{subst-r'}{lapp} to get
            $$\overline{E}^{S'}[\refssu{}{V}{M}] \to^\ast \refssu{}{V}{\refssl{t}{W}{(\overline{E'}^{S}[M])
            \ (\refssd{}{V}{\overline{M'}^{S'}})}}$$
            Using \ref{mlem-absorption}, we get that the right part of the
            application reduces to $\overline{M'}^S$. Finally, by definition of
            \strans, the right hand side is $\refssu{}{V}{\overline{E}^S[M]}$.
          \item Other cases are treated alike
         \end{itemize}
    \item To prove (\ref{mlem-diff-eq2}), we apply
      \rrule{subst-r'}{\parallel}. We then use
      \ref{mlem-absorption} on $\refssd{}{V}{\overline{N}^{S'}}$ to get
      $\overline{N}^S$ and \ref{mlem-ctxt-red} with $C = M \parallel [.]$
      to get the desired result.
    \item Finally, we prove (\ref{mlem-diff-eq3}) by combining the two results. We
      first use the strenghtened version of $(\ref{mlem-diff-eq1})$, so we can
      apply \ref{mlem-ctxt-red} and get
      $$\overline{E}^{S'}[\refssu{}{V}{M}] \parallel \overline{N}^{S'}
      \to^\ast \refssu{}{V}{M}{\overline{E}^S[M]} \parallel \overline{N}^{S'}$$.
      We use (\ref{mlem-diff-eq2}) with $M' = E[M]$ to get the result.
    \end{itemize}
  \end{proof}

  Our reduction have the drawback of not reducing under abstractions, such that
  some of the variable substitution propagation will be delayed until the
  corresponding lambda will be applied (or forever). To cope with this subtelty,
  we introduce a relation on terms of \lthis that morally states that a
  term $M$ is related to $N$ if $M$ is the same as $N$ up to some pending
  substitutions hidden under lambdas, such that if we could reduce these
  subtitution under abstraction $M$ would actually reduce to $N$.

  \begin{mdef}{Substitution order}\label{mdef-substitution-equivalence}\\
    We define $\sleq$ as :
    \begin{itemize}
      \item $x \sleq x$, $\get r \sleq \get r$, $\set r V \sleq \set r V$
      \item $\refssl{}{V}{M\ N} \sleq \refssl{}{V}{M'\ N'}$
        or $M \parallel N \sleq M' \parallel N'$ iff $M \sleq M'$ and $N \sleq N'$
      \item $\lambda x.M \sleq \lambda x.M'$ if $M =
        \varss{\sigma_1}{\varss{\ldots}{\varss{\sigma_n}{N}}}$ such that
        $N\{\sigma_1,\ldots,\sigma_n\} = N$.
      \item $\refssd{}{V}{M} \sleq \refssd{}{V}{M'}$ or $\refssu{}{V}{M}
        \sleq \refssu{}{V}{M'}$ iff $M \sleq M'$
    \end{itemize}
  \end{mdef}

  \begin{mlem}{Properties of the substitution
    order}\label{mlem-substitution-equivalence-prop}\\
    $\sleq$ is a simulation order, meaning that if $M \sleq N$ and $M \to
    M'$, then $N \to^\ast N'$ with $M' \sleq N'$
  \end{mlem}

  We can now state the following result modulo this equivalence

  \begin{mlem}{Explicit substitution}\label{mlem-expl-subst}\\
    Let $P = C[E[\varss{\sigma}{M}]]$ with $M$ containing no explicit
    substitutions nor upward reference substitution.
    Then $$P \to_\texttt{aux}^\ast P' \sleq C[E[\varmetas{x}{V}{M}]]$$
  \end{mlem}

  \begin{proof}
    By induction on $M$.
    \begin{itemize}
      \item Neutral \\
        If $M=\ast$, $M=\get{r}$ or $M=y$ with $y \neq x$, then
        $\varmetas{x}{V}{M}=M$. If we apply \rrulet{subst}{unit} (resp.
        \rrulet{subst}{get},\rrulet{subst}{var}) we also get
        that $$C[E[\varss{\sigma}{M}]] \to_\text{aux} C[E[M]]$$
      \item $M=x$ \\
        $\varmetas{x}{V}{M}=V$. By \rrulet{subst}{var},
        $$C[E[\varss{\sigma}{x}]] \to_\text{aux} C[E[V]]$$
      \item $M=\lambda y. M'$ \\
        $\varmetas{x}{V}{M}=\lambda y.(\varmetas{x}{V}{M'})$. By
        \rrule{subst}{\lambda},
        $$C[E[\varss{\sigma}{\lambda y. M'}]] \to_\text{aux}
        C[E[\lambda y. (\varss{\sigma}{M'})]]
        \sleq C[E[\lambda y.(M'\{\sigma\})]]$$
      \item \ldots \\
        The remaining cases are treated similarly, the reduction rules being
        designed to make this lemma work.
        TODO : explain why we don't care about reference substitution, that
        cannot have free variables in the translation
        % There is a little subtelty, depending on how the substitution
        % $\varmetas{M}{x}{V}$ is defined with respect to references substitutions, ie when $M =
        % \refssd{r}{\mathcal{V}}{M'}$ for example. Actually, the
        % variables appearing in $\mathcal{V}$ should not be bound by any lambda because these
        % values have been emitted by sets, and sets can't be reduced under
        % lambdas. Thus all substitutions of bound variables in $\mathcal{V}$
        % already occured, and only globally free variables can remain. We define $M[x/V]$ to be
        % $\substvg{r}{\mathcal{V}}{(M'[x/V])}$, which matches the reduction rule
        % $\texttt{subst}_{\texttt{subst}_\texttt{r}}$, and this case is treated
        % as others.
    \end{itemize}
  \end{proof}

\subsection{One-step simulation}
  We prove now the technical result that will give the main theorem, which is
  contained in this lemma :

  \begin{mthe}{One-step simulation}\label{mthe-simulation}\\
    Let $P,Q$ be \lamadio programs such that $P
    \rightarrow_\texttt{orig} Q$. Then
    $$\overline{P} \rightarrow_\texttt{aux}^\ast M \sleq \overline{Q}$$
  \end{mthe}

  \begin{proof}\ref{mthe-simulation}\\
    By case analysis on the reduction rule applied :
    \begin{description}
      \item[$\beta_v$] We have $P = E[(\lambda x. M)\ V] \parallel N \parallel
        S$ and $Q = E[\varmetas{x}{V}M] \parallel N \parallel S$. Let
        By ~\ref{mlem-ctxt-decomp}, $\overline{P} =
        \overline{E}^S[\refrawsl{r}{\vstore}{\lambda x. M
        \ V}] \parallel \overline{N}^S$ and $\overline{Q} =
          \overline{E}^S[\overline{\varmetas{x}{V}{M}}^S] \parallel \overline{N}^S$. Then, by
        one application of $\beta_v$ in \lthis, we have $\overline{P}
        \rightarrow_\texttt{aux} Q_0 =
        \overline{E}^S[\varss{\sigma}{\refrawsd{}{\vstore}{M}}] \parallel
        \overline{N}^S$.
        We apply \ref{mlem-absorption} with to deduce
        $Q_0 \to^\ast Q_1 = \overline{E}^S[\varss{\sigma}{\overline{M}^S}]
        \parallel \overline{N}^S$. Using \ref{mlem-expl-subst} and
        \ref{mlem-subst}, we get $Q_1
        \to^\ast Q_2 \sleq \overline{E}^S[\overline{\varmetas{x}{V}{M}}^S] \parallel
        \overline{N}^S=\overline{Q}$.
      \item[get] We have $P = E[\get{r}] \parallel N \parallel S$ with
        $S=S' \parallel
        r \Leftarrow V$, and $Q = E[V] \parallel N \parallel S$.
        By \ref{mlem-ctxt-decomp},
        $\overline{P} = \overline{E}^S[\refssd{}{V}{\get{r}}]
        \parallel \overline{N}^S$ and $\overline{Q} = \overline{E}^S[V]
        \parallel \overline{N}^S$.
        The rule \rrulet{subst-r}{get} gives $\overline{P} \to_\text{aux}
        \overline{E}^S[V] \parallel \overline{N}^S = \overline{Q}$.
      \item[set] We have $P = E[\set r V] \parallel N \parallel S'$ and $Q = E[\ast]
        \parallel N \parallel S$ with $S = S' \parallel r \Leftarrow V$. By
        \ref{mlem-ctxt-decomp}, $\overline{P} =
        \overline{E}^{S'}[\refssu{}{V}{\ast}]
        \parallel \overline{N}^{S'}$ and $\overline{Q} = \overline{E}^S[\ast]
        \parallel \overline{N}^S = \overline{E[\ast] \parallel N}^S$.
        We apply \ref{mlem-diffusion} to get
        $P \to^\ast \refssu{}{V}{(\overline{E}^S[\ast] \parallel
        \overline{N}^S)}$ and then use the rule \rrule{subst-r}{\top} to get
        rid of the toplevel reference substitution.
    \end{description}
  \end{proof}


==> paper-csl-long arxiv/parts/simulation-nets.tex <==
\section{Simulation of $\lamlang{aux}$ in nets}

\subsection{Nets}

\subsection{Definition}
We consider MELL Interaction Nets with co-contraction and co-weakening. Formulas
are
\begin{equation*}
  A,B ::= \mathbf{1} \mid \bot \mid \oc{A} \mid
  \wn{A} \mid A \otimes B \mid A \parr B
\end{equation*}

Nets are build using the following cells

\begin{center}
  \includegraphics{translation/asy/pdf/components.pdf}
\end{center}

Using the following reductions rules :

\begin{center}
\begin{longtable}{|c|c|c|}
\hline
Rule & Redex & Reduced net \\
\hline
\multicolumn{3}{c|}{MLL reductions} \\
\hline
$\otimes / \parr$ & \includegraphics{translation/asy/pdf/reduction-partensor-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-partensor-right.pdf} \\
\hline
\multicolumn{3}{c|}{Exponential reductions} \\
\hline
$\oc / \wn{d}$ & \includegraphics{translation/asy/pdf/reduction-derprom-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-derprom-right.pdf} \\
\hline
$\oc / \wn{w}$ & \includegraphics{translation/asy/pdf/reduction-weakprom-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-weakprom-right.pdf} \\
\hline
$\oc / \wn{c}$ & \includegraphics{translation/asy/pdf/reduction-contprom-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-contprom-right.pdf} \\
\hline
\multicolumn{3}{|c|}{Non-determinstic reduction} \\
\hline
$\oc{c} / \wn{d}$ & \includegraphics{translation/asy/pdf/reduction-dercocontr-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-dercocontr-right.pdf}\\
\hline
\multicolumn{3}{|c|}{Co-reductions} \\
\hline
$\oc{c} / \wn{c}$ &
\includegraphics{translation/asy/pdf/reduction-contcocontr-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-contcocontr-right.pdf} \\
\hline
$\oc{c} / \wn{w}$ &
\includegraphics{translation/asy/pdf/reduction-coweakcont-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-coweakcont-right.pdf} \\
\hline
$\oc{w} / \wn{c}$ &
\includegraphics{translation/asy/pdf/reduction-weakcocontr-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-weakcocontr-right.pdf} \\
\hline
$\oc{w} / \wn{w}$ &
\includegraphics{translation/asy/pdf/reduction-weakcoweak-left.pdf} &
$\epsilon$ \\
\hline
$\oc{w} / \wn{d}$ &
\includegraphics{translation/asy/pdf/reduction-dercoweak-left.pdf} &
$0$ \\

\end{longtable}
\end{center}

\subsection{Simulation}

  \begin{mlem}{Base case}\label{mlem-simu-base-case}\\
    Let $R \vdash M : (\alpha,e)$ be a typing derivation, such that $M \to M'$
    by a base reduction (without contexts). For any $e' \supset e$, $R \vdash M
    : (\alpha,e')$ by adding \trule{sub} to the typing derivation of $M$, and by subject reduction, $R \vdash M' :
    (\alpha,e')$. Then $$\mathcal{C}(M) \to^\ast \mathcal{C}(M')$$
  \end{mlem}

  \begin{mthe}{Simulation}\label{mthe-simu-aux-nets}\\
    Let $R \vdash M : (\alpha,e)$. If $M \to M'$, then $\mathcal{C}(M) \to
    \mathcal{C}{M'}$.
  \end{mthe}


==> paper-csl-long arxiv/parts/translation-nets.tex <==
\section{Translation of $\lamlang{aux}$ in nets}

We translate the full typing derivation of a term into a MELL+Cocon interaction
net.
\begin{center}
\begin{longtable}{|c|c|}
\hline
Typing derivation of & Translation \\
\hline
$\infer[(var)]{\Gamma,x : A \vdash x : (A,\emptyset)}{}$
& \includegraphics{translation/asy/pdf/var.pdf} \\
\hline

$\infer[(unit)]{\Gamma \vdash \ast : (\texttt{Unit},\emptyset)}{}$
 & \includegraphics{translation/asy/pdf/unit.pdf} \\
\hline

$\infer[(lam)]
{ R;\Gamma \vdash \lambda{x}.M : (A \sur{\to}{e} \alpha, \emptyset) }
{ R;x:A,\Gamma \vdash M : (\alpha,e) }$
& \includegraphics{translation/asy/pdf/abstraction.pdf} \\
\hline

$\infer[(app)]
{ R;\Gamma \vdash M\ N : (\alpha, e=e_1 \cup e_2 \cup e_3) }
{ R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha, e_2)
\qquad R;\Gamma \vdash N : (A,e_3)}$
  & \includegraphics{translation/asy/pdf/application.pdf} \\
\hline

$\infer[(get)]
{ R;\Gamma \vdash \get{r} : (A,\{ r \}) }
{ R \vdash \Gamma }$
 & \includegraphics{translation/asy/pdf/get.pdf} \\
\hline

$\infer[(set)]
{ R;\Gamma \vdash set(r,V) : (\text{Unit},\{ r \}) }
{ R \vdash r:\text{Reg}_r\ A \qquad R;\Gamma \vdash V : (A,\emptyset) }$
 & \includegraphics{translation/asy/pdf/set.pdf}\\
\hline

$\infer[(par)]
{ R; \Gamma \vdash P_1 \parallel P_2 : \mathbf{B} }
{i=1,2 \qquad R;\Gamma \vdash P_i : \alpha_i }$
  & \includegraphics{translation/asy/pdf/parallel.pdf} \\
\hline

\infer[(subst)]
{ R; \Gamma \vdash \varss{\sigma}{M} : (\alpha, e) }
{ R; \Gamma, x : A \vdash M : (\alpha,e) \qquad R; \Gamma \vdash V : (A,\emptyset) }
  & \includegraphics{translation/asy/pdf/substv.pdf} \\
\hline

\infer[(subst\text{-}r\downarrow)]
{ R; \Gamma \vdash \substg{(r_i)}{(\mathcal{V}_i)}{M} : (\alpha, e) \qquad }
{ R; \Gamma \vdash M : (\alpha,e) \qquad R; \Gamma \vdash \mathcal{V}_i : (A_i,\emptyset) }
  & \includegraphics{translation/asy/pdf/substr.pdf} \\

\infer[(subst\text{-}r\uparrow)]
{ R; \Gamma \vdash \substup{(r_i)}{(\mathcal{V}_i)}{M} : (\alpha, e) \qquad }
{ R; \Gamma \vdash M : (\alpha,e) \qquad R; \Gamma \vdash \mathcal{V}_i : (A_i,\emptyset) }
  & \includegraphics{translation/asy/pdf/substr-up.pdf} \\
\hline
\end{longtable}
\end{center}

\paragraph{}
  Where
\begin{center}
\begin{tabular}{ccc}
\hline
\includegraphics{translation/asy/pdf/mycombox.pdf} & $=$
& \includegraphics{translation/asy/pdf/mycombox-expanded.pdf} \\
\hline
\includegraphics{translation/asy/pdf/myappbox.pdf} & $=$
& \includegraphics{translation/asy/pdf/myappbox-expanded.pdf} \\
\hline
\end{tabular}
\end{center}

For a net $M^\bullet$, we define its closed form $\mathcal{C}(M^\bullet)$ by cutting the free
wires corresponding to effects with weakening and coweakening cells :
\begin{center}
  \includegraphics{translation/asy/pdf/closed.pdf}
\end{center}

By extension, we define the translation $M^\bullet$ (and thus
$\mathcal{C}(M^\bullet))$ of a term $M$
of $\lamlang{orig}$ by $M^\bullet = \overline{M}^\bullet$.


==> paper-csl-long arxiv/parts/typing.tex <==
\begin{section}{Type and effect system}

\subsection{Types and effects}

%%% TYPE SYSTEM WITH POLARITY
\begin{comment}
\begin{center}
\begin{tabular}{lrcl}
  -effects & $e,e'$ & $\subset$ & $\{r,r^-,r^+,s,s^-,s^+,\ldots\}$ \\
  -types & $\alpha$ & $::=$ & $\mathbf{B} \mid A$ \\
  -values types & $A$ & $::=$ & $\text{Unit} \mid A \sur{\to}{e} \alpha
  \mid \text{Reg}_r A$ \\
  -variable contexts & $\Gamma$ & $::=$ & $x_1 : A_1,\ldots,x_n : A_n$ \\
  -region contexts & $R$ & $::=$ & $r_1 : A_1,\ldots,r_n : U_n$ \\
\end{tabular}
\paragraph{}
\end{center}
\end{comment}
%%% END TYPE SYSTEM WITH POLARITY

\begin{center}
\begin{tabular}{lrcl}
  -effects & $e,e'$ & $\subset$ & $\{r_1,r_2,\ldots\}$ \\
  -types & $\alpha$ & $::=$ & $\mathbf{B} \mid A$ \\
  -values types & $A$ & $::=$ & $\text{Unit} \mid A \sur{\to}{e} \alpha
  \mid \text{Reg}_r A$ \\
  -variable contexts & $\Gamma$ & $::=$ & $x_1 : A_1,\ldots,x_n : A_n$ \\
  -region contexts & $R$ & $::=$ & $r_1 : A_1,\ldots,r_n : A_n$ \\
\end{tabular}
\paragraph{}
\end{center}

\subsection{Stratification and context formation}

\paragraph{Stratification Rules}

\begin{gather*}
\infer[]
{\emptyset \vdash}{}
\qquad
\infer[]
{ R,r:A \vdash }
{ R \vdash A \qquad r \notin \text{dom}(R) }
\\
\\
\infer[]
{ R \vdash Unit }
{ R \vdash }
\qquad
\infer[]
{ R \vdash \mathbf{B}}
{ R \vdash }
\\
\\
\infer[]
{ R \vdash A \sur{\rightarrow}{e} \alpha }
{ R \vdash A \qquad R \vdash \alpha \qquad e \subseteq \text{dom}(R)}
\qquad
\infer[]
{ R \vdash \text{Reg}_r A }
{ R \vdash \qquad r : A \in R }
\end{gather*}

\paragraph{Stratification conditions}
Note that these typing rules are equivalent to the following conditions :
\begin{mlem*}{Stratification conditions}\\
  A type and effect $\alpha$ (or $\emptyset$) are well-formed
  under a reference context $R = r_1:A_1,\ldots,r_n:A_n$, meaning
  that the judgement
  \begin{equation*}
    R \vdash \alpha
  \end{equation*}
  holds, if and only if :
  \begin{itemize}
    \item
      $\text{Eff}(A_1,\ldots,A_n,\alpha) \subseteq \text{dom}(R)$
    \item
      There exists a total ordering $\leq_R$ on dom$(R)$ such that\\
      $\ptentre{i}{1}{n},\ \text{Eff}(A_i) \subseteq \dcl{\{r_i\}}
        \setminus \{ r_i \}$
  \end{itemize}
\end{mlem*}

\paragraph{}
where

\begin{tabular}{rcl}
  $\text{dom}(R)$ & $=$ & $\{ r_1,\ldots,r_n \}$ \\
  $\text{Eff}(U)$ & $=$ & $\emptyset$ \\
  $\text{Eff}(\mathbf{B})$ & $=$ & $\emptyset$ \\
  $\text{Eff}(A \sur{\to}{e} \alpha)$ & $=$ &
  $\text{Eff}(A) \cup e \cup \text{Eff}(\alpha)$
\end{tabular}

\paragraph{Type equations}

Let $R = r_1 : A_1, \ldots, r_n : A_n$. To each reference $r_i$ we
associate a type variable $X_{r_i}$.
We define the type equations
\begin{itemize}
  \item $\text{unit}^\bullet=\oc{1}$
  \item $\mathbf{B}^\bullet=?$
  \item $(A \sur{\to}{\{s_1, \ldots, s_m\}} \alpha)^\bullet = \oc{((A^\bullet
      \otimes X_{s_1} \ldots \otimes X_{s_m}) \multimap (X_{s_1} \otimes \ldots
      \otimes X_{s_m} \otimes \alpha^\bullet))}$
  \item $X_{r_i} = {A_i}^\bullet$
\end{itemize}

These equations are solvable if and only if $R \vdash \ $.


\subsection{Typing rules for \lamadio}

\begin{gather*}
\infer[(var)]
{R;\Gamma,x : A \vdash x : (A,\emptyset)}
{R \vdash \Gamma,x : A}
\\
\\
\infer[(unit)]
{R;\Gamma \vdash \ast : (\texttt{Unit},\emptyset)} {R \vdash \Gamma}
\\
\\
\infer[(reg)]
{R;\Gamma \vdash r : Reg_r{A}}
{R \vdash \Gamma \qquad r : A \in R}
\\
\\
\infer[(lam)]
{ R;\Gamma \vdash \lambda{x}.M : (A \sur{\to}{e} \alpha,\emptyset) }
{ R;\Gamma,x : A \vdash M : (\alpha,e) }
\\
\\
\infer[(app)]
{ R; \Gamma\vdash M\ N : (\alpha, e_1 \cup e_2 \cup e_3) }
{ R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha, e_2) \qquad R;\Gamma \vdash N : (A,e_3) }
\\
\\
\infer[(get)]
{ R;\Gamma \vdash \get{r} : (A,\{ r \}) }
{ R;\Gamma \vdash \text{Reg}_r{A} }
\\
\\
\infer[(set)]
{ R;\Gamma \vdash set(r,V) : (\text{Unit},\{ r \}) }
{ R;\Gamma \vdash r : \text{Reg}_r{A} \qquad R;\Gamma \vdash V : (A,\emptyset) }
\\
\\
\infer[(store)]
{ R;\Gamma \vdash r \Leftarrow V : (\mathbf{B},\emptyset) }
{ r : A \in R \qquad R;\Gamma \vdash V : (A,\emptyset) }
\\
\\
\infer[(par1)]
{ R;\Gamma \vdash P \parallel S : (\alpha,\emptyset) }
{ R;\Gamma \vdash P : (\alpha,e) \qquad R;\Gamma \vdash S : (\mathbf{B},\emptyset) }
\\
\\
\infer[(par2)]
{ R;\Gamma \vdash P_1 \parallel P_2 : (\mathbf{B},e_1 \cup e_2) }
{i=1,2 \qquad R;\Gamma \vdash P_i : (\alpha_i,e_i) }
\end{gather*}

\subsection{Typing rules for \lthis}

\begin{gather*}
\infer[(var)]
{R;\Gamma,x : A \vdash x : (A,\emptyset)}
{R \vdash \Gamma,x : A}
\\
\\
\infer[(unit)]
{R;\Gamma \vdash \ast : (\texttt{Unit},\emptyset)} {R \vdash \Gamma}
% \\
% \\
% \infer[(mval)]
% {R;\Gamma \vdash [V^s_1,\ldots,V^s_n] : (A, \emptyset)}
% {R;\Gamma \vdash V^s_i : (A,\emptyset) }
\\
\\
\infer[(reg)]
{R;\Gamma \vdash r : Reg_r{A}}
{R \vdash \Gamma \qquad r : A \in R}
\\
\\
\infer[(lam)]
{ R;\Gamma \vdash \lambda{x}.M : (A \sur{\to}{e} \alpha,\emptyset) }
{ R;\Gamma,x : A \vdash M : (\alpha,e) }
\\
\\
\infer[(app)]
{ R; \Gamma\vdash M\ N : (\alpha, e_1 \cup e_2 \cup e_3) }
{ R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha, e_2) \qquad R;\Gamma \vdash N : (A,e_3) }
\\
\\
\infer[(get)]
{ R;\Gamma \vdash \get{r} : (A,\{ r \}) }
{ R;\Gamma \vdash \text{Reg}_r{A} }
\\
\\
% \infer[(set)]
% { R;\Gamma \vdash \text{set(r,V)} : (\text{Unit},\{ r \}) }
% { R;\Gamma \vdash r : \text{Reg}_r{A} \qquad R;\Gamma \vdash V : (A,\emptyset) }
% \\
% \\
\infer[(subst)]
{ R; \Gamma \vdash \vars{x_i}{V_i}{M} : (\alpha, e) }
{ i=(1,\ldots,n) \qquad
  R; \Gamma, x_1 : A_1, \ldots, x_n : A_n \vdash M : (\alpha,e) \qquad
  R; \Gamma \vdash V_i : (A,\emptyset) }
\\
\\
\infer[(subst\text{-}r)]
{ R; \Gamma \vdash \sind{r_i / \mathscr{E}_i}{M}{\uparrow \mid \downarrow \mid
\lambda} (\alpha, e) \qquad }
{ R; \Gamma \vdash r_i : \text{Reg}_{r_i} A_i \qquad
  R; \Gamma \vdash M : (\alpha,e) \qquad
  r_i \in e \qquad
  R; \Gamma \vdash V \in \mathscr{E}_i : (A_i,\emptyset) }
\\
\\
\infer[(par)]
{ R;\Gamma \vdash M_1 \parallel M_2 : (\mathbf{B},e_1 \cup e_2) }
{i=1,2 \qquad R;\Gamma \vdash M_i : (\alpha_i,e_i) }
\\
\\
\infer[(sum)]
{ R;\Gamma \vdash \mathbf{M}_1 + \mathbf{M}_2 : (\alpha,e) }
{i=1,2 \qquad R;\Gamma \vdash \mathbf{M_i} : (\alpha,e) }
\end{gather*}

\subsection{Subtyping induced by effect containment}

\begin{gather*}
\infer[(ref)]
{R \vdash \alpha \leq \alpha}{}
\\
\\
\infer[(arrow)]
{ R \vdash A \sur{\to}{e} \alpha \leq A' \sur{\to}{e'}
\alpha' }
{ \qquad R \vdash (\alpha,e) \leq (\alpha',e') }
\\
\\
\infer[(cont)]
{ R \vdash (\alpha,e) \leq (\alpha',e') }
{ e \subset e' \subset \text{dom}(R) \qquad R \vdash \alpha \leq \alpha' }
\\
\\
\infer[(sub)]
{ R;\Gamma \vdash M : (\alpha',e') }
{ R;\Gamma \vdash M : (\alpha,e) \qquad R \vdash (\alpha,e) \leq (\alpha',e') }
\end{gather*}

\end{section}


==> parts/language-ces.tex <==
\subsection{A language with explicit substitutions: \lthis}

\lthis\ is a $\lambda$-calculus with explicit substitutions for both variables
and references, non deterministic sum and parallel composition. It serves as an
intermediate language between \lamadio\ and nets, easing the proofs of simulation
and termination.

%

The language {\lthis} has two kinds of variables: term variables (simply named
{\em variables}) represented with $x,y,\ldots$, and {\em references},
represented with $r,r',\ldots$.  Substitutions are represented by partial
functions with finite support. Variable substitutions, denoted with Greek
letters $\sigma,\tau,\ldots$, map variables to values. Reference substitutions,
denoted with calligraphic uppercase letters $\multv{V},\multv{U},\ldots$,
map references to {\em finite multisets} of values. Multisets reflect the
non-determinism, as multiple writes may have been performed on the same
reference. They are represented with the symbol $\mathcal{E}$.
%
The language consists
of values, terms and sums of terms, representing non-determinism.
\begin{center}
\begin{tabular}{llll}
  -values & $V$ & $::=$ & $x \mid \ast \mid \lambda x.M$ \\
  -terms & $M$ & $::=$ & $V \mid \varss{\sigma}{M} \mid
                         \refssl{r}{V}{(M\,M)} \mid \get{r}
\mid \refssd{r}{V}{M} \mid \refssu{r}{V}{M} \mid M \parallel M$ \\
  -sums & $\mathbf{M}$ & $::=$ & $\mathbf{0} \mid M \mid \mathbf{M} +
  \mathbf{M}$ \\
\end{tabular}
\end{center}
The construct $\varss{\sigma}{M}$ stands for the explicit substitutions
of variables in $M$ under the substitution $\sigma$. There are three
constructs for explicit substitutions for references:
$\refssd{r}{V}{M}$ and $\refssu{r}{V}{M}$ are respectively the
downward and upward references substitutions, while
$\refssl{r}{V}{(M\,M)}$ is the $\lambda$-substitution. The reason for
which the language needs three distinct notations is explained in the
next section while presenting the reduction rules.

Terms are considered modulo the same kind of equivalence relation as \lamadio.
The sum is idempotent, associative and commutative, while the parallel
composition is associative and commutative.


\begin{remark}
  The three constructs $\refssd{r}{V}{}$, $\refssu{r}{V}{}$ and
  $\refssl{r}{V}{}$ encapsulate the assignments in terms and in stores
  presented in Section~\ref{sec:intro}: there is no need anymore for
  ${\rm set}(r,V)$ and $r\Leftarrow V$. See
  Section~\ref{sec:discussion} for a discussion of this aspect.
\end{remark}

\begin{notation}
  Reference substitutions will be sometimes written
  with the notation $[\store r V]$ to mean $[\multv{V}]$ with $\multv{V} : r
  \mapsto [V]$.
\end{notation}

We will not describe \lthis\ more in detail. A complete formulation of the
reduction together with a type system and a proof of termination may be found in
\cite{paper-esop}. The reduction and typing rules are included in
Appendix~\ref{appendix:lces}.

%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Reduction of \lthis}
%
% We adopt a weak call-by-value reduction where the reduction order of
% an application is not specified. It is weak in the sense that no
% reduction occurs under abstractions.
%
% Although in a general setting non-determinism and call-by-value taken together
% may break confluence even when collecting all possible
% outcomes~\cite{deLiguoroP95},
% this phenomenon doesn't happen here. Indeed, we can't reduce under
% abstractions, and the only non-deterministic construct $\get{r}$ must be reduced
% before being duplicated, avoiding problematic interactions between
% $\beta$-reduction and non-deterministic choice.
%
% The language {{\lthis}} is equipped with the reduction defined
% in Table~\ref{fig:lth-red-rules}. The rules make use of several notations
% that we lay out below.
% Rules devoted to dispatching substitutions are referred as
% \emph{structural rules}. The \emph{variable} (resp. \emph{downward},
% \emph{upward}) \emph{structural rules} consist in \rrulet{subst}{}
% (resp.  \rrulet{subst-r}{}, \rrulet{subst-r'}{}) rules excluding
% \rrulet{subst}{var} (resp.  \rrulet{subst-r}{get},
% \rrule{subst-r}{\top}). An in-depth discussion about these rules follows.
%
%
%
% %%% -------------------------------------------------------------------
% \begin{table}[tb]
% \centering
% \begin{minipage}{.49\linewidth}
% \centering
% \begin{tabular}{rcl}
% $M \parallel M'$ & = & $M' \parallel M$ \\
% $(M \parallel M') \parallel M''$ & = & $M \parallel (M' \parallel M'')$ \\
% $\mathbf{M} + \mathbf{M}'$ & = & $\mathbf{M}' + \mathbf{M}$ \\
% $(\mathbf{M} + \mathbf{M}') + \mathbf{M}''$ & = & $\mathbf{M} + (\mathbf{M}' +
% \mathbf{M}'')$ \\
% $\mathbf{M} + \mathbf{M}$ = $\mathbf{M} + \mathbf{0}$ & = & $\mathbf{M}$
% \mynl
% \end{tabular}
% \caption{Structural Rules}\label{fig:lth-struct-rules}
% \end{minipage}
% \begin{minipage}{.49\linewidth}
% \centering
% \begin{tabular}{lcl}
% ~\\
% $E$ & $::=$ & $[.] \mid \refssl{r}{V}{E\ M} \mid
%   \refssl{r}{V}{M\ E}\mid{} $ \\
% & & $\refssd{r}{V}{E}
%   \mid \refssu{r}{V}{E}$ \\
% $C$ & $::=$ & $[.] \mid (C \parallel M) \mid (M \parallel C)$ \\
% $\mathbf{S}$ & $::=$ & $[.] \mid \mathbf{S} + \mathbf{M} \mid \mathbf{M} +
% \mathbf{S}$ \mynl
% \end{tabular}
% \caption{Evaluation Contexts}\label{fig:lth-eval-context}
% \end{minipage}
% \end{table}
% %%%-------------------------------------------------------------------
%
%
%
% %%%-------------------------------------------------------------------
% \begin{table}[!p]
% \begin{center}
% \begin{tabular}{lrcl}
% \hline
% \multicolumn{4}{|c|}{{\bf (a)}~$\beta$-reduction} \\
% \hline
% $(\beta_v)$ & $\refssl{r}{U}{((\lambda x.M)\,V)}$ & $\rightarrow$ &
% $\refssd{r}{U}{(\varss{\sigma}{M})}$ \\
% \\
% \multicolumn{4}{l}{If $M \rightarrow M'$ with rule $(\beta_v)$, then
%   $\mathbf{S}[C[E[M]]] \rightarrow \mathbf{S}[C[E[M']]]$}\\
% \\
% \hline
% \multicolumn{4}{|c|}{{\bf (b)}~Variable Substitutions} \\
% \hline
% \rrulet{subst}{var} & $\varss{\sigma}{x}$
% & $\to$ & $\sigma(x)$ if defined, or $x$ otherwise\\
% \rrulet{subst}{unit} & $\varss{\sigma}{\ast}$
% & $\to$ & $\ast$ \\
% \rrulet{subst}{app} & $\varss{\sigma}{\refssl{}{V}{(M\,N)}}$ & $\to$
% & $\refrawsl{}{\varss{\sigma}{\multv{V}}}{((\varss{\sigma}{M})\,(\varss{\sigma}{N}))}$ \\
% \rrule{subst}{\lambda} & $\varss{\sigma}{(\lambda y.M)}$ & $\to$
%   & $\lambda y.(\varss{\sigma}{M})$ \\
% \rrulet{subst}{get} & $\varss{\sigma}{\get{r}}$ & $\to$
%  & $\get{r}$ \\
% \rrule{subst}{\parallel} & $\varss{\sigma}{(M \parallel M')}$ & $\to$
% & $(\varss{\sigma}{M}) \parallel (\varss{\sigma}{M'})$ \\
% \rrulet{subst}{subst-r} &
% $\varss{\sigma}{( \refssd{r}{V}{M} )}$ & $\to$
% & $\refsrawsd{}{\metas{\sigma}{\multv{V}}}{\varss{\sigma}{M}}$ \\
% \rrulet{subst}{subst-r'} &
% $\varss{\sigma}{( \refssu{r}{V}{M} )}$ & $\to$
% & $\refsrawsu{}{\metas{\sigma}{\multv{V}}}{\varss{\sigma}{M}}$ \\
% \rrulet{subst}{merge} & $\varss{\tau}{\varss{\sigma}{M}}$ & $\to$ &
% $\varss{\sigma,\tau}{M}$
% % & & & \\[-2ex]
% %  & \multicolumn{3}{c}{
% %   where $W_i =
% %   \begin{cases*}
% %     V_i & \text{if $i \in \mathcal{I}$} \\
% %     \varmetas{(x_k)_{k \in \mathcal{I}}}{(V_k)_{k \in \mathcal{I}}}{U_i} & \text{if $i \in \mathcal{J}$} \\
% %   \end{cases*}$} \\
% \mynl
% \multicolumn{4}{l}{Congruence case: }\\
% \multicolumn{4}{l}{If $M \rightarrow M'$ by any of the previous rules, then
%   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% \\
% \hline
%   \multicolumn{4}{|c|}{{\bf (c)}~Downward Reference Substitutions} \\
% \hline
% \rrulet{subst-r}{val} & $\refssd{}{V}{V}$
% & $\to$ & $V$ \\
% \rrule{subst-r}{\parallel} & $\refssd{}{V}{(M
% \parallel M')}$ & $\to$
% & $(\refssd{}{V}{M}) \parallel (\refssd{}{V}{M'})$ \\
% \rrulet{subst-r}{subst-r'} &
% $\refssd{r}{V}{\refssu{s}{U}{M}}$ & $\to$
% & $\refssu{s}{U}{\refssd{r}{V}{M}}$ \\
%  & & & \\
% \rrulet{subst-r}{merge} &
% $\refssd{}{V}{\refssd{}{U}{M}}$ & $\to$
% & $\refsrawsd{}{\multv{U},\multv{V}}{M}$ \\
% \rrulet{subst-r}{app} &
% $\refssd{}{V}{\refssl{}{U}{(M\,N)}}$ & $\to$
% & $\refsrawsl{}{\multv{U},\multv{V}}{(\refssd{}{V}{M})\ (\refssd{}{V}{N})}$ \mynl
% \multicolumn{4}{l}{Congruence cases:}\\
% \multicolumn{4}{l}{If $M \rightarrow M'$ by any of the previous rules, then
%   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \mynl
% \multicolumn{4}{l}{Finally:}\\
% \rrulet{subst-r}{get} &
% $\mathbf{S}[C[E[\refssd{}{V}{\get{r}}]]]$ & $\to$
% & $\mathbf{S}[C[E[\get{r}]]] + \sum_{V \in \multv{V}(r)}
% C[E[V]]$ \\
% \\
% \hline
% \multicolumn{4}{|c|}{{\bf (d)}~Upward Reference Substitutions} \\
% \hline
% \rrule{subst-r'}{\parallel} & $(\refssu{r}{V}{M}) \parallel N$
% & $\to$ & $\refssu{r}{V}{(M \parallel (\refssd{r}{V}{N}))}$ \\
%  & & & \\
% \rrulet{subst-r'}{lapp} &
% $\refssl{}{U}{((\refssu{}{V}{M})\,N)}$ & $\to$ &
% $\refssu{}{V}{\refsrawsl{}{\multv{U},\multv{V}}{(M\,(\refssd{}{V}{N}))}}$ \\
% \rrulet{subst-r'}{rapp} &
% $\refssl{}{U}{(M\,(\refssu{}{V}{N}))}$ & $\to$ &
% $\refssu{}{V}{\refsrawsl{}{\multv{U},\multv{V}}{((\refssd{}{V}{M})\,N)}}$ \mynl
% \multicolumn{4}{l}{Congruence case:}\\
% \multicolumn{4}{l}{If $M \rightarrow M'$ by any of the previous rules, then
%   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \mynl
% \multicolumn{4}{l}{Finally:}\\
% \rrule{subst-r'}{\top} & $\mathbf{S}[\refssu{r}{V}{M}]$
% & $\to$ & $\mathbf{S}[M]$
% \end{tabular}
% \end{center}
% \caption{Reduction Rules}\label{fig:lth-red-rules}
% \end{table}
% %%%-------------------------------------------------------------------
%
%
% \begin{notation}\label{not:context}\rm
%   the contexts $E$, $C$ and $\mathbf{S}$ are defined in
%   Table~\ref{fig:lth-eval-context}. The context $E$ stands for a usual
%   call-by-value applicative context, $C$ picks a thread, while
%   $\mathbf{S}$ picks a term in a non-deterministic sum. Note how
%   $E$ does not enforce any reduction order on an application.
% \end{notation}
% %
% \begin{notation}\label{not:subst}\rm
%   Given a variable substitution $\sigma$ and a value $V$, we define
%   the value $\metas{\sigma}V$ as follows:
%   $\metas{\sigma}{(\lambda x . M)} = \lambda x .
%   (\varss{\sigma}{M})$,
%   $\metas{\sigma}{(x)} = \sigma(x)$ if $\sigma$ is defined at $x$ or
%   $\metas{\sigma}{(x)} = x$ if not, and
%   $\metas{\sigma}{(\ast)} = \ast$.
% \end{notation}
% %
% \begin{notation}\label{not:subst2}\rm
%   We use the
%    notation $\multv{X} = \multv{V},\multv{W}$ for the juxtaposition of
%    references substitutions. It is defined by
%    %
%    $\multv{X}(r) =
%    \multv{V}(r) + \multv{W}(r)$ if both are defined and where $+$ is the union of multisets,
%    $\multv{V}(r)$ if only $\multv{V}$ is defined, and
%    $\multv{W}(r)$ if only $\multv{W}$ is defined.
%    %
%    We use the same notation for the
%    composition of variable substitutions, defined by
%    %
%    $(\sigma,\tau)(x) =
%      \metas{\tau}{\sigma(x)}$ if both are defined,
%      $\sigma(x)$ if only $\sigma$ is defined
%      $\tau(x)$  if only $\tau$ is defined.
%    %
%    Finally, we define
%    $\metas{\sigma}{\multv{V}} : r \mapsto [ \metas{\sigma}{V_i} \mid V_i \in
%    \multv{V}(r) ]$.
% \end{notation}
%
% We now give some explanations on the rules of Table~\ref{fig:lth-red-rules}.
%
% \paragraph*{(a) $\beta$-reduction}
% %
% If one forgets the $\lambda$-substitution explained below in
% Subsection (d), this set of rules encapsulates the call-by-value
% behavior of the language: only values can be substituted in the body
% of abstractions, and this happens within a thread in a call-by-value
% applicative context.
%
% \paragraph*{(b) Variable Substitutions}
%
% A variable
% substitution can be seen as a message emitted by a $\beta$-redex and
% dispatched through the term seen as a tree. The substitution flows
% from the redex downward the term-tree until it reaches the occurrence
% of a variable. The occurrence is then replaced, or not, depending on
% the variable to be substituted. The rules in
% Table~\ref{fig:lth-red-rules}(a) are an operational formalization of
% this step-by-step procedure.
% %
% Consider for example the reduction of the term
% $(\lambda x . x\ y\ z)\ (\lambda x . x)$. The redex triggers with
% $(\beta_v)$ the substitution of all occurrences of $x$ in what was the
% body of the lambda-abstraction. The substitution goes down the
% corresponding sub-term and performs the substitution when it reaches an
% occurrence of $x$.
% %
% \begin{center}
% \scalebox{.8}{%
% \begin{tabular}{ccccc}
%   \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$(\lambda x . x\ y\ z)\ (\lambda x.x)$};
%     \node[draw=none] (M) at (-1,-1)
%       {$\lambda x. x\ y\ z$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (X) at (-1,-3)
%       {$x$};
%     \node[draw=none] (N) at (1,-1)
%       {$(\lambda x. x)$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (M) at (0,0)
%     {$\varss{x \mapsto (\lambda x. x)}{x\ y\ z}$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$x$};
%
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (M) at (0,0)
%       {$x\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%     {$\varss{x \mapsto (\lambda x. x)}{\ldots}$};
%     \node[draw=none] (X) at (0,-2)
%       {$x$};
%
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (M) at (0,0)
%       {$x\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$\varss{x \mapsto (\lambda x. x)}{x}$};
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (M) at (0,0)
%       {$(\lambda x. x)\ y\ z$};
%     \node[draw=none] (M2) at (0,-1)
%       {$\ldots$};
%     \node[draw=none] (X) at (0,-2)
%       {$\lambda x. x$};
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (X);
%   \end{tikzpicture}
% \end{tabular}%
% } % END SCALEBOX
% \end{center}
%
% % \begin{remark}
% \paragraph{Remark}
% On rules \rrulet{subst}{subst-r} and \rrulet{subst}{subst-r'}.
% %
% When composing or swapping substitutions, non-values may appear in
% unfortunate places: take for example
% $\varss{\sigma}{(\refssu{}{V}{\ast})}$, its reduction should be
% $\refrawsu{}{\multv{V'}}{(\varss{\sigma}{\ast})}$ where
% $\multv{V}'(r) = [ \varss{\sigma}{V} \mid V \in \multv{V}(r) ]$ when
% $\multv{V}(r)$ is defined. But $\varss{\sigma}{V}$ are not necessarily
% values and should then be able to be reduced inside
% substitutions. However, note that that $\varss{\sigma}{V}$ always
% reduces in one step to the value $\metas{\sigma}{V}$. To avoid
% additional complexity, we perform this reduction at the same time,
% whence the use of $\metas{\sigma}{V}$ instead of $\varss{\sigma}{V}$
% in the actual rules.
% % \end{remark}
%
%
% \paragraph*{(c) Downward Reference Substitutions}
%
% An {\setw} can occur anywhere within a term and it must be able to reach a
% {\getw} located in an arbitrary position. In a language such
% as~\cite{Amadio2009}, as discussed in Section~\ref{sec:amadio}
% the solution is to keep all assignments in a global
% store. When a {\getw} gets evaluated, the value for the reference is
% taken from the store.  This approach is very global in nature: the
% store is ``visible'' by every subterm.
%
% The language {{\lthis}} features a step-by-step decomposition of
% reference assignments akin to term variable substitutions: an
% assignment follows the branches of the term-tree, actively seeking a
% {\getw}.
% %
% We therefore introduce two sorts of reference substitutions: one that
% goes downward (indicated by $\downarrow$), similar to variable
% substitutions, and one that goes upward (indicated by $\uparrow$). Starting from
% an \setw, the latter climbs up the tree up to the root. The rules in
% Table~\ref{fig:lth-red-rules}(c) describes the former while the rules in
% Table~\ref{fig:lth-red-rules}(d) describes the latter.
%
% % \begin{remark}
% \paragraph{Remark}
%   In Table~\ref{fig:lth-red-rules}, the rule \rrulet{subst-r}{get} is
%   the central case of the reduction of reference substitutions. It
%   says that whenever a downward substitution reaches a $\get{r}$, then
%   it generates a non deterministic sum of all the available values for
%   the reference $r$ (if $\multv{V}$ is undefined at $r$, then this sum
%   is understood as a neutral element $\mathbf{0}$) plus a term where
%   the substitution was discarded but the $\get{r}$ is left
%   unreduced. To see why this ``remainder'' is necessary, consider the
%   term $\refsrawsd{}{\store r V_2}{\refsrawsd{}{\store r V_1}{\get{r}}}$.  If we
%   omit the remainder, the term could reduce to
%   $\refrawsd{}{\store r V_2}{V_1}$ and finally to $V_1$. But another
%   reduction is possible: one can first reduce the term to
%   $\refsrawsd{}{\store{r}{V_1},\store{r}{V_2}}{\get{r}}$ and then to $V_1 + V_2$.  The
%   $\get{r}$ must not be greedy: when it meets a substitution, it has
%   to consider the possibility that other substitutions will be
%   available later. This aspect will be crucial when considering the
%   proof of strong normalization of the language in
%   Section~\ref{sec:term}.
% % \end{remark}
%
% \paragraph*{(d) Upward Reference Substitutions}
%
% Each time an upward reference substitution goes through a multi-ary constructor --
% as an application or a parallel composition -- it propagates downward
% substitutions in all the children of the constructor except the one
% it comes from, while continuing its ascension. Eventually, all the
% leafs are reached by a corresponding downward substitution. To
% illustrate the idea, consider a term $M\ N$ where $M$ contains a
% $\get{r}$ somewhere and $N$ an {\setw} $\refrawsu{}{\store r V}{\ast}$. The reduction of explicit
% substitutions would go as follows.
%
% \begin{center}
% \scalebox{.8}{%
% \begin{tabular}{cccc}
%   % \begin{tikzpicture}[yscale=\mytikshrink]
%   %   \node[draw=none] (MN) at (0,0)
%   %     {$M\ N$};
%   %   \node[draw=none] (M) at (-1,-1)
%   %     {$M$};
%   %   \node[draw=none] (M2) at (-1,-2)
%   %     {$\ldots$};
%   %   \node[draw=none] (G) at (-1,-3)
%   %     {$\text{get}(r)$};
%   %   \node[draw=none] (N) at (1,-1)
%   %     {$M$};
%   %   \node[draw=none] (N2) at (1,-2)
%   %     {$\ldots$};
%   %   \node[draw=none] (S) at (1,-3)
%   %     {$\set{r}{V}$};
%   %
%   %   \draw[-,>=latex] (MN) -- (M);
%   %   \draw[-,>=latex] (MN) -- (N);
%   %   \draw[-,>=latex] (M) -- (M2);
%   %   \draw[-,>=latex] (M2) -- (G);
%   %   \draw[-,>=latex] (N) -- (N2);
%   %   \draw[-,>=latex] (N2) -- (S);
%   % \end{tikzpicture}
%   %
%   \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\refrawsu{}{\store r V}{\ast}$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\refrawsu{}{\store r V}{\ldots}$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$M\ N$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$\refrawsu{}{\store r V}{N}$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture} \\
%
%   \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$\refrawsu{}{\store r V}{(M\ N)}$};
%     \node[draw=none] (M) at (-1,-1)
%       {$\refrawsd{}{\store r V}{M}$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$\refrawsu{}{\store r V}{(M\ N)}$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\refrawsd{}{\store r V}{\ldots}$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\text{get}(r)$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$\refrawsu{}{\store r V}{(M\ N)}$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$\refrawsd{}{\store r V}{\get r}$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
%
%   & \begin{tikzpicture}[yscale=\mytikshrink]
%     \node[draw=none] (MN) at (0,0)
%       {$\refrawsu{}{\store r V}{(M\ N)}$};
%     \node[draw=none] (M) at (-1,-1)
%       {$M$};
%     \node[draw=none] (M2) at (-1,-2)
%       {$\ldots$};
%     \node[draw=none] (G) at (-1,-3)
%       {$V$};
%     \node[draw=none] (N) at (1,-1)
%       {$N$};
%     \node[draw=none] (N2) at (1,-2)
%       {$\ldots$};
%     \node[draw=none] (S) at (1,-3)
%       {$\ast$};
%
%     \draw[-,>=latex] (MN) -- (M);
%     \draw[-,>=latex] (MN) -- (N);
%     \draw[-,>=latex] (M) -- (M2);
%     \draw[-,>=latex] (M2) -- (G);
%     \draw[-,>=latex] (N) -- (N2);
%     \draw[-,>=latex] (N2) -- (S);
%   \end{tikzpicture}
% \end{tabular}%
% } % END SCALEBOX
% \end{center}
%
%
%
% One last subtlety in the movement of reference substitutions concerns
% $\lambda$-abstractions. As made explicit in
% Table~\ref{fig:lth-red-rules}(a), the language is call-by-value:
% reduction does not happen under $\lambda$-abstractions. In particular, a
% read within the body of a $\lambda$-abstraction should only be accessible
% by an assignment when the $\lambda$-abstraction is opened: we have a
% natural notion of pure and impure terms. Pure terms are terms that
% won't produce any effect when reduced, and in particular, all values
% are expected to be pure terms since they can't reduce further. This is
% highlighted by rule \rrulet{subst-r}{val}: when encountering a pure
% term, a reference substitution vanishes. But the case of abstraction
% is more subtle: computational effects frozen in its body are freed
% when the abstraction is applied. If one implements naively the
% reduction rules of reference substitutions, then the following example
% doesn't behave as expected:
% $\refssd{}{V}{((\lambda x. \get{r})\ \ast)} \to
% (\refssd{}{V}{(\lambda x .  \get{r})})\ (\refssd{}{V}{\ast}) \to
% (\lambda x .  \get{r})\ \ast \to \get{r}$.
% We end up with an orphan $\get{r}$ despite the fact that a substitution was
% available at the beginning.
% The problem is that the substitution diffuses through the application,
% then encounters two pure terms and vanishes.
%
% In an application, the left term eventually exposes the body of an
% abstraction, and this body should be able to use any substitution that
% was in its scope. The $\lambda$-substitution $[-]_\lambda$ is a
% special stationary reference substitution attached to an
% application. Its goal is precisely to record all the substitutions
% that went down through it with Rules \rrulet{subst-r'}{lapp} and
% \rrulet{subst-r'}{rapp}. When the application is finally reduced with
% a $\beta_v$-rule, this substitution will turn to a downward one and
% feed the $\get{r}$'s that were hidden in the abstraction's
% body.
%
% % \begin{remark}
% \paragraph{Remark}
%   An alternative approach to $\lambda$-substitution would be to make
%   downward substitutions not vanish (i.e. getting rid of Rule
%   \rrulet{subst-r}{val}). In this situation, values would be handled
%   with their whole context of references assignment. Apart from the
%   heavy syntactical cost of carrying around a lot of similar and
%   possibly useless substitutions, the idea that hidden effects are
%   released at application appears more natural regarding type and
%   effect systems, as the one we introduce in Section~\ref{sec:type}.
% % \end{remark}
%
% % \begin{remark}
% \paragraph{Remark}
%   Rule \rrule{subst-r'}{\top} acts as a garbage
%   collection to eliminating top-level upward substitutions. While not
%   necessary, this will greatly ease the statement and proof of lemmas
%   and theorems (such as Lemma~\ref{lemma-progress}).
% % \end{remark}
%
% %
% % \paragraph{Terms}
% %
% % We define $\finsup{A}{B}$ as the set of partial functions $f : A \rightharpoonup
% % B$ with finite
% % support. Substitutions will be represented by such functions, mapping a finite
% % set of variable (resp. locations) to a value (resp. a multiset of values).
% % We write $\fmset{A}$ for the finite multisets of elements of $A$, or in other
% % word, $\finsup{A}{\mathbb{N}}$.
% %
% % \vspace{0.5cm}
% %
% % \begin{tabular}{llll}
% %   -variables & \multicolumn{3}{l}{$x,y,\ldots$} \\
% %   -regions & \multicolumn{3}{l}{$r,r',\ldots$} \\
% %   -values & $V$ & $::=$ & $x \mid \ast \mid \lambda x.M$ \\
% %   % csubst values & $V^s$ & $::=$ & $V \mid \varss{x}{V}{V^s}$ \\
% %   -rsubsts & $\mathcal{V}$ & : & $\finsup{\text{regions}}{\text{values}}$ \\
% %   -vsubsts & $\sigma$ & : & $\finsup{\text{variables}}{\fmset{\text{values}}}$ \\
% %   -terms & $M$ & $::=$ & $V \mid \varss{\sigma}{M} \mid \refssl{r}{V}{M\ M} \mid
% %   \get{r} \mid \text{set}(r,V)$ \\
% %   & & & $\mid \refssd{r}{V}{M} \mid \refssu{r}{V}{M} \mid M \parallel M$ \\
% %   -sums & $\mathbf{M}$ & $::=$ & $\mathbf{0} \mid M \mid \mathbf{M} +
% %   \mathbf{M}$ \\
% % \end{tabular}
% %
% % \paragraph{}
% % We will use the synctatic sugar $\varss{\sigma}{\multv{V}} = \multv{V}'$ where
% % $\multv{V}'(r) = \{ \varss{\sigma}{V_i} \mid V_i \in \multv{V}(r) \}$.
% %
% % \paragraph{}
% % For a value $V$, we define a meta substitution $\varmetas{(x_k)}{(U_k)}{V}$ by
% % the normal form of $\vars{(x_k)}{(U_k)}{V}$ which is :
% % \begin{itemize}
% %   \item $\varmetas{(x_k)}{(U_k)}{y} = U_k$ if $\exists k, y = x_k$, or $y$
% %     otherwise
% %   \item $\varmetas{(x_k)}{(U_k)}{\ast} = \ast$
% %   \item $\varmetas{(x_k)}{(U_k)}{(\lambda y . M)} = \lambda y .
% %     (\vars{(x_k)}{(U_k)}{M})$
% % \end{itemize}
% %
% % \subsection{Reduction}
% % We adopt a weak CBV reduction, where the reduction order of an application is not
% % specified (nor left-to-right neither right-to-left). The sum is idempotent,
% % associative and commutative, with $\mathbf{0}$ as neutral element. The parallel
% % composition is associative and commutative.
% % \begin{center}
% % \begin{tabular}{rcl}
% % \hline
% % \multicolumn{3}{|c|}{Structural rules} \\
% % \hline
% % $M \parallel M'$ & = & $M' \parallel M$ \\
% % $\mathbf{M} + \mathbf{M}'$ & = & $\mathbf{M}' + \mathbf{M}$ \\
% % $(\mathbf{M} + \mathbf{M}') + \mathbf{M}''$ & = & $\mathbf{M} + (\mathbf{M}' +
% % \mathbf{M}'')$ \\
% % $(M \parallel M') \parallel M''$ & = & $M \parallel (M' \parallel M'')$ \\
% % $\mathbf{M} + \mathbf{0}$ & = & $\mathbf{M}$ \\
% % \end{tabular}
% % \end{center}
% %
% % \paragraph{}
% % \begin{center}
% % \begin{tabular}{lcl}
% % \hline
% % \multicolumn{3}{|c|}{Evaluation contexts} \\
% % \hline
% % % $E$ & $::=$ & $[.] \mid \refssl{r}{V}{E\ M} \mid
% % %   \refssl{r}{V}{M\ E}$ \\
% % $E$ & $::=$ & $[.] \mid \refssl{r}{V}{E\ M} \mid
% %   \refssl{r}{V}{M\ E} $ \\
% % & & $\refssd{r}{V}{E}
% %   \mid \refssu{r}{V}{E}$ \\
% % % $G$ & $::=$ & $[.] \mid \refssl{r}{V}{G\ M} \mid
% % %   \refssl{r}{V}{M\ G} \mid \varss{\sigma}{G}$ \\
% % $C$ & $::=$ & $[.] \mid (C \parallel M) \mid (M \parallel C)$ \\
% % $\mathbf{S}$ & $::=$ & $[.] \mid \mathbf{S} + \mathbf{M} \mid \mathbf{M} +
% % \mathbf{S}$ \\
% % \end{tabular}
% % \end{center}
% %
% % \paragraph{}
% % \begin{center}
% % \begin{tabular}{lrcl}
% % \hline
% % \multicolumn{4}{|c|}{Reduction rules (main)} \\
% % \hline
% %
% % $(\beta_v)$ & $\refssl{r}{U}{(\lambda x.M)\ V}$ & $\rightarrow$ &
% % $\refssd{r}{U}{\varss{\sigma}{M}}$ \\
% %
% % % $(\texttt{\text{set}})$ & $\text{set}(r,V)$ & $\rightarrow$ & $
% % % \substup{(r)}{([V])}{\ast}$ \\
% % \\
% %
% % \hline
% % \multicolumn{4}{c}{If $M \rightarrow M'$ by any of the previous rules, then
% %   $\mathbf{S}[C[E[M]]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% %
% % \end{tabular}
% % \paragraph{}
% % \begin{tabular}{lrcl}
% %
% % \hline
% % \multicolumn{4}{|c|}{Reduction rules (variables substitutions)} \\
% % \hline
% % \rrulet{subst}{var} & $\varss{\sigma}{x}$
% % & $\to$ & $\sigma(x)$ if defined, or $x$ otherwise\\
% %
% % \rrulet{subst}{unit} & $\varss{\sigma}{\ast}$
% % & $\to$ & $\ast$ \\
% %
% % \rrulet{subst}{app} & $\varss{\sigma}{\refssl{}{V}{M\
% % N}}$ & $\to$
% % & $\refrawsl{}{(\varss{\sigma}{\multv{V}})}{(\varss{\sigma}{M})\
% % (\varss{\sigma}{N})}$ \\
% %
% % \rrule{subst}{\lambda} & $\varss{\sigma}{\lambda y.M}$ & $\to$
% %   & $\lambda y.(\varss{\sigma}{M})$ \\
% %
% % \rrulet{subst}{get} & $\varss{\sigma}{\get{r}}$ & $\to$
% %  & $\get{r}$ \\
% %
% % % $(\texttt{subst}_\texttt{set})$ & $\varss{\sigma}{\text{set}(r,U)}$ & $\to$
% % %  & $\text{set}(r,\varss{\sigma}{U})$ \\
% %
% % \rrule{subst}{\parallel} & $\varss{\sigma}{M \parallel M'}$ & $\to$
% % & $(\varss{\sigma}{M}) \parallel (\varss{\sigma}{M'})$ \\
% %
% % \rrulet{subst}{subst-r} &
% % $\varss{\sigma}{( \refssd{r}{V}{M} )}$ & $\to$
% % & $\refsrawsd{}{\varss{\sigma}{\multv{V}}}{\varss{\sigma}{M}}$ \\
% %
% % \rrulet{subst}{subst-r'} &
% % $\varss{\sigma}{( \refssu{r}{V}{M} )}$ & $\to$
% % & $\refsrawsu{}{\varss{\sigma}{\multv{V}}}{\varss{\sigma}{M}}$ \\
% %
% % \rrulet{subst}{merge} & $\vars{(x_i)_{i \in \mathcal{I}}}{(V_i)_{i \in
% % I}}{\vars{(y_i)_{i \in \mathcal{J}}}{(U_i)_{i \in \mathcal{J}}}{M}}$ & $\to$
% % & $\vars{(z_i)_{i \in \mathcal{I} \cup \mathcal{J}}}{(W_i)_{i \in \mathcal{I} \cup \mathcal{J}}}{M}$ \\
% % & & & \\
% %  & \multicolumn{3}{c}{
% %   $\mathcal{W}_i =
% %   \begin{cases*}
% %     V_i & \text{if $i \in \mathcal{I}$} \\
% %     \varmetas{(x_k)_{k \in \mathcal{I}}}{(V_k)_{k \in \mathcal{I}}}{U_i} & \text{if $i \in \mathcal{J}$} \\
% %   \end{cases*}$} \\
% % \\
% %
% % \\
% % \hline
% % \multicolumn{4}{c}{If $M \rightarrow M'$ by any of the previous rules, then
% %   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% %
% % \end{tabular}
% % \paragraph{}
% % \begin{tabular}{lrcl}
% %
% % \hline
% % \multicolumn{4}{|c|}{Reduction rules (downward references substitutions)} \\
% % \hline
% %
% % \rrulet{subst-r}{val} & $\refssd{}{V}{V}$
% % & $\to$ & $V$ \\
% %
% % % $(\texttt{subst-r}_\texttt{set})$ &
% % % $\refssd{r}{V}{\text{set}(s,V)}$ & $\to$ &
% % % $\text{set}(s,V)$ \\
% %
% % \rrule{subst-r}{\parallel} & $\refssd{}{V}{M
% % \parallel M'}$ & $\to$
% % & $(\refssd{}{V}{M}) \parallel (\refssd{}{V}{M'})$ \\
% %
% % \rrulet{subst-r}{subst-r'} &
% % $\refssd{r}{V}{\refssu{s}{U}{M}}$ & $\to$
% % & $\refssu{s}{U}{\refssd{r}{V}{M}}$ \\
% %
% %  & & & \\
% %
% % \rrulet{subst-r}{merge} &
% % $\refssd{}{V}{\refssd{}{U}{M}}$ & $\to$
% % & $\refsrawsd{}{\multv{U},\multv{V}}{M}$ \\
% % % \rrulet{subst-r}{merge} & \multicolumn{3}{l}{
% % %  $\substdown{(r_i)_{i \in \mathcal{I}}} {(\mathcal{U}_i)_{i \in \mathcal{I}}} {(
% % %     \substdown{(r_j)_{j \in \mathcal{J}}} {(\mathcal{V}_j)_{j \in \mathcal{J}}} {M}
% % %   )}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\to$
% % %     $\substdown{(r_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {(\mathcal{W}_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {M}$} \\
% % % \\
% %
% % \rrulet{subst-r}{app} &
% % $\refssd{}{V}{\refssl{}{U}{M\ N}}$ & $\to$
% % & $\refsrawsl{}{\multv{V},\multv{U}}{(\refssd{}{V}{M})\ (\refssd{}{V}{N})}$ \\
% % % \rrulet{subst-r}{app} & \multicolumn{3}{l}{
% % %  $\substdown{(r_i)_{i \in \mathcal{I}}} {(\mathcal{U}_i)_{i \in \mathcal{I}}} {(
% % %     \substl{(r_j)_{j \in \mathcal{J}}} {(\mathcal{V}_j)_{j \in \mathcal{J}}}{M\ N}
% % %   )}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\to \text{subst}^\lambda \ {(r_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %     ={(\mathcal{W}_i)_{i \in \mathcal{I}\cup\mathcal{J}}} \text{ in }$} \\
% % %     & \multicolumn{3}{l}{
% % %       $\phantom{\to C[G[}(\substdown{(r_i)_{i \in \mathcal{I}}}{(\mathcal{U}_i)_{i
% % %         \in \mathcal{I}}}{M})
% % %       \ (\substdown{(r_i)_{i \in \mathcal{I}}}{(\mathcal{U}_i)_{i
% % %         \in \mathcal{I}}}{N})$} \\
% % %  & & & \\
% % %  & \multicolumn{3}{c}{
% % %   $\mathcal{W}_i =
% % %   \begin{cases*}
% % %     \mathcal{U}_i & \text{if $i \in \mathcal{I} \setminus (\mathcal{I} \cap \mathcal{J})$} \\
% % %     \mathcal{V}_i & \text{if $i \in \mathcal{J} \setminus (\mathcal{I} \cap \mathcal{J})$} \\
% % %     \mathcal{U}_i + \mathcal{V}_i & \text{if $i \in \mathcal{I} \cap \mathcal{J}$}
% % %   \end{cases*}$} \\
% % % \\
% % % \hline
% %
% % \multicolumn{4}{c}{If $M \rightarrow M'$ by any of the previous rules, then
% %   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% %
% % \\
% % \rrulet{subst-r}{get} &
% % $\mathbf{S}[C[E[\refssd{}{V}{\get{r}}]]]$ & $\to$
% % & $\mathbf{S}[C[E[\get{r}]]] + \sum_{V \in \multv{V}(r)}
% % C[E[V]]$ \\
% %
% % \end{tabular}
% % \paragraph{}
% % \begin{tabular}{lrcl}
% %
% % \hline
% % \multicolumn{4}{|c|}{Reduction rules (upward references substitutions)} \\
% % \hline
% %
% %
% % % $(\texttt{subst-r'}_\texttt{$\parallel$})$ & $M \parallel (\refssu{r}{V}{N})$
% % % & $\to$ & $\refssu{r}{V}{(\refssd{r}{V}{M}) \parallel N}$ \\
% %
% % \rrule{subst-r'}{\parallel} & $(\refssu{r}{V}{M}) \parallel N$
% % & $\to$ & $\refssu{r}{V}{M \parallel (\refssd{r}{V}{N})}$ \\
% %  & & & \\
% %
% % \rrulet{subst-r'}{lapp} &
% % $\refssl{}{U}{(\refssu{}{V}{M})\ N}$ & $\to$ &
% % $\refssu{}{V}{\refsrawsl{}{\multv{V},\multv{U}}{M\ (\refssd{}{V}{N})}}$ \\
% %
% % % \rrulet{subst-r'}{lapp} & \multicolumn{3}{l}{
% % %  $\substl{(r_i)_{i \in \mathcal{I}}} {(\mathcal{U}_i)_{i \in \mathcal{I}}} {
% % %     (\substup{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in \mathcal{J}}}
% % %     {M})\ N}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\to\ \substup{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in
% % %       \mathcal{J}}}{}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\phantom{\to\ }
% % %       \substl{(r_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {(\mathcal{W}_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {M\ (\substdown{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in
% % %         \mathcal{J}}}{N})}$} \\
% % %  & & & \\
% %
% % \rrulet{subst-r'}{rapp} &
% % $\refssl{}{U}{M\ (\refssu{}{V}{N})}$ & $\to$ &
% % $\refssu{}{V}{\refsrawsl{}{\multv{V},\multv{U}}{(\refssd{}{V}{M})\ N}}$ \\
% %
% % % \rrulet{subst-r'}{rapp} & \multicolumn{3}{l}{
% % %  $\substl{(r_i)_{i \in \mathcal{I}}} {(\mathcal{U}_i)_{i \in \mathcal{I}}} {
% % %     M\ (\substup{(r_j)_{j \in \mathcal{J}}} {(\mathcal{V}_j)_{j \in \mathcal{J}}}
% % %     {N}
% % %   )}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\to\ \substup{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in
% % %       \mathcal{J}}}{}$} \\
% % %   & \multicolumn{3}{l}{
% % %     $\phantom{\to\ C[E[}
% % %       \substl{(r_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {(\mathcal{W}_i)_{i \in \mathcal{I}\cup\mathcal{J}}}
% % %       {(\substdown{(r_j)_{j \in \mathcal{J}}}{(\mathcal{V}_j)_{j \in
% % %         \mathcal{J}}}{M})\ N}$} \\
% % %  & & & \\
% %
% % % ****** EST-CE QU'IL FAUDRAIT UN MERGE POUR SUBST UP ÉGALEMENT ??? ****** %
% % \\
% %
% % \hline
% % \multicolumn{4}{c}{If $M \rightarrow M'$ by any of the previous rules, then
% %   $\mathbf{S}[C[E[M]] \rightarrow \mathbf{S}[C[E[M']]]$} \\
% % \\
% % \rrule{subst-r'}{\top} & $\mathbf{S}[\refssu{r}{V}{M}]$
% % & $\to$ & $\mathbf{S}[M]$ \\
% %
% % \end{tabular}
% %
% % \end{center}
% %
% % \subsection{ }
% %
% % In [US], we define a type system for \lthis and gives proof for the following
% % statements:
% %
% % \begin{theorem}{Type soundness}\\
% %   Typing is preserved by reduction.
% % \end{theorem}
% %
% % \begin{theorem}{Confluence}\\
% %   \lthis\ is confluent on well-typed terms.
% % \end{theorem}
% %
% % \begin{theorem}{Termination}\\
% %   Well typed terms are strongly normalizing.
% % \end{theorem}
% %
% % \subsection{Simulation}
% %
% % \newcommand{\vstore}{\multv{V}_S}
% % \newcommand{\strans}{$\overline{\phantom{M}}^S$}
% % \newcommand{\sleq}{\rightsquigarrow_s}
% %
% % The intermediate language \lthis\ is capable of simulating \lamadio. Moreover, a
% % result of adequacy is proven, in the sense that it does not produce more values
% % than the original \lamadio\ term.
% %
% % \begin{definition}{Translation of \lamadio in \lthis}\\
% %     Let $M$ be a term and $S$ be a store of \lamadio.
% %     S can be written as
% %     \[
% %       S = r_1 \Leftarrow V^1_1 \parallel \ldots \parallel r_1
% %       \Leftarrow V^1_{k_1} \parallel \ldots \parallel r_n \Leftarrow
% %       V^n_1 \parallel \ldots \parallel r_n \Leftarrow
% %       V^n_{k_n}
% %     \]
% %     Let $\multv{V}_S : r_i \mapsto [V^i_1, \ldots, V^i_{k_i}]$.
% %   We define the translation of $M$ under $S$ by
% %     \begin{itemize}
% %       \item If $M = V$ or $M = \text{set}(s,V)$ then $\overline{M}^S = M$
% %       \item If $M = N\ N'$ then $\overline{M}^S = \refsrawsl{r}{\vstore}(\overline{N}^S)\
% %         (\overline{N'}^S)$
% %       \item If $M = \get{s}$ then $\overline{M}^S =
% %         \refsrawsd{r}{\vstore}{\get{s}}$
% %       \item If $M = N \parallel N'$ then $\overline{M}^S = \overline{N}^S
% %         \parallel \overline{N'}^S$
% %     \end{itemize}
% %
% %     In fact, one can see that $\overline{M}^S$ is the normal form of
% %     $\refsrawsd{r}{\vstore}{M}$ for the reduction defined by all
% %     \rrulet{subst-r}{} rules except \rrulet{subst-r}{get}.
% %
% %     We extend it to contexts $E,F$ and $G$ by adding the rule $\overline{[.]}^S = [.]$.
% %     \\
% %     Finally, for any program $P = M \parallel S$, we define $\overline{P} =
% %     \overline{M}^S$.
% %     If $P = M$ then $\overline{P} = \overline{M} = M$.
% %   \end{definition}
% %
% %   % Originally put restrictions like $M$ and $N$ must not be parallel,
% %   % or that some reduction on parallel must not be used, but now I don't
% %   % see why this would be the case, so just removing
% %   % \begin{lemma}{Context reduction}\label{lemma-ctxt-red}\\
% %   %   Let $M,N$ be terms of \lthis such that $M \to^\ast N$ without using
% %   %   \rrule{subst-r}{\top}, then for any
% %   %   context $C$ and $E$, $C[E[M]] \to^\ast C[E[N]]$ using the same reduction
% %   %   rules.
% %   % \end{lemma}
% %   %
% %   % \begin{lemma}{Context decomposition}\label{lemma-ctxt-decomp}\\
% %   %   Let $P$ be a program of \lamadio,
% %   %   \begin{itemize}
% %   %     \item $P = C[E[M]] \text{ with } C = [.] \text{ or } C = [.] \parallel N \implies
% %   %       \overline{P} = P$
% %   %     \item $P = C[E[M]] \text{ with } C = [.] \parallel N \parallel S \implies
% %   %       \overline{P} = \overline{E}^S[\overline{M}^S] \parallel \overline{N}^S$
% %   %   \end{itemize}
% %   % \end{lemma}
% %   %
% %   % \begin{proof}
% %   %   This is an easy induction following the definition of \strans.
% %   % \end{proof}
% %   %
% %   % \begin{lemma}{Substitution for \strans}\label{lemma-subst}\\
% %   %   Let $M,M'$ be terms, $V$ a value and $S$ a
% %   %   store of \lamadio. Then
% %   %   \[
% %   %     \overline{M[x/V]}^S = \overline{M}^S[x/V]
% %   %   \]
% %   % \end{lemma}
% %   % \begin{proof}
% %   %   By induction
% %   % \end{proof}
% %   %
% %   % \begin{lemma}{Absorption}\label{lemma-absorption}\\
% %   %   Let $M$ be a term and $S = S' \parallel r \Leftarrow V$ be a store of
% %   %   \lamadio, $C$ and $E$ be context of \lthis, and $\multv{V}
% %   %   : r \mapsto [V]$. Then
% %   %   $$C[E[\refssd{}{V}{\overline{M}^{S'}}]] \to_\texttt{aux}^\ast
% %   %   C[E[\overline{M}^{S}]]$$
% %   % \end{lemma}
% %   %
% %   % \begin{proof} By induction on $M$, using the definition of
% %   %   \strans and the \texttt{subst-r} reductions.
% %   % \end{proof}
% %   %
% %   % \begin{lemma}{Diffusion}\label{lemma-diffusion}\\
% %   %   Let $N$ be a term, $E$ a context, $S = S' \parallel r \Leftarrow V$ a store of
% %   %   \lamadio and $\multv{V} : r \mapsto [V]$. Let $M$ be a term of \lthis. Then
% %   %   \begin{equation}\label{lemma-diff-eq1}
% %   %     \overline{E}^{S'}[\refssu{}{V}{M}]
% %   %     \to_\texttt{aux}^\ast \refssu{}{V}{\overline{E}^S[M]}
% %   %   \end{equation}
% %   %   \begin{equation}\label{lemma-diff-eq2}
% %   %     \refssu{}{V}{M} \parallel \overline{N}^{S'}
% %   %     \to_\texttt{aux}^\ast \refssu{}{V}{(M \parallel
% %   %     \overline{N}^S)}
% %   %   \end{equation}
% %   %   \begin{equation}\label{lemma-diff-eq3}
% %   %     \overline{E}^{S'}[\refssu{}{V}{M}] \parallel \overline{N}^{S'}
% %   %     \to_\texttt{aux}^\ast \refssu{}{V}{\overline{E}^S[M] \parallel
% %   %     \overline{N}^S}
% %   %   \end{equation}
% %   %   using only rules \rrulet{subst-r}{} or \rrulet{subst-r'}{}.
% %   % \end{lemma}
% %   %
% %   % \begin{proof}
% %   %   \begin{itemize}
% %   %
% %   %     \item For (\ref{lemma-diff-eq1}), we work by induction on $E$. As we
% %   %       will need \ref{lemma-ctxt-red}, we add the induction hypothesis
% %   %       that the rule $(\texttt{subst-r'}_\top)$ is not used.
% %   %       \begin{itemize}
% %   %         \item $\overline{E}^{S'} = [.]$ nothing to do
% %   %         \item $\overline{E}^{S'} = \refssl{s}{U}{\overline{E'}^{S'}\
% %   %         \overline{M'}^{S'}}$\\
% %   %           By IH, $\overline{E'}^{S'}[\refssu{}{V}{M}] \to^\ast
% %   %           \refssu{}{V}{\overline{E'}^{S}[M]}$ using no
% %   %           \rrule{subst-r'}{\top} rules.
% %   %           We use \ref{lemma-ctxt-red} and get
% %   %           $$\overline{E}^{S'}[\refssu{}{V}{M}] \to^\ast
% %   %           \refssl{s}{U}{(\refssu{}{V}{\overline{E'}^{S}[M]})
% %   %           \ \overline{M'}^{S'}}$$
% %   %           We then apply \rrulet{subst-r'}{lapp} to get
% %   %           $$\overline{E}^{S'}[\refssu{}{V}{M}] \to^\ast \refssu{}{V}{\refssl{t}{W}{(\overline{E'}^{S}[M])
% %   %           \ (\refssd{}{V}{\overline{M'}^{S'}})}}$$
% %   %           Using \ref{lemma-absorption}, we get that the right part of the
% %   %           application reduces to $\overline{M'}^S$. Finally, by definition of
% %   %           \strans, the right hand side is $\refssu{}{V}{\overline{E}^S[M]}$.
% %   %         \item Other cases are treated alike
% %   %        \end{itemize}
% %   %   \item To prove (\ref{lemma-diff-eq2}), we apply
% %   %     \rrule{subst-r'}{\parallel}. We then use
% %   %     \ref{lemma-absorption} on $\refssd{}{V}{\overline{N}^{S'}}$ to get
% %   %     $\overline{N}^S$ and \ref{lemma-ctxt-red} with $C = M \parallel [.]$
% %   %     to get the desired result.
% %   %   \item Finally, we prove (\ref{lemma-diff-eq3}) by combining the two results. We
% %   %     first use the strenghtened version of $(\ref{lemma-diff-eq1})$, so we can
% %   %     apply \ref{lemma-ctxt-red} and get
% %   %     $$\overline{E}^{S'}[\refssu{}{V}{M}] \parallel \overline{N}^{S'}
% %   %     \to^\ast \refssu{}{V}{M}{\overline{E}^S[M]} \parallel \overline{N}^{S'}$$.
% %   %     We use (\ref{lemma-diff-eq2}) with $M' = E[M]$ to get the result.
% %   %   \end{itemize}
% %   % \end{proof}
% %
% %   Our reduction have the drawback of not reducing under abstractions, such that
% %   some of the variable substitution propagation will be delayed until the
% %   corresponding lambda will be applied (or forever). To cope with this subtelty,
% %   we introduce a relation on terms of \lthis\ that morally states that a
% %   term $M$ is related to $N$ if $M$ is the same as $N$ up to some pending
% %   substitutions hidden under lambdas, such that if we could reduce these
% %   subtitution under abstraction $M$ would actually reduce to $N$.
% %
% %   \begin{definition}{Substitution order}\label{definition-substitution-equivalence}\\
% %     We define $\sleq$ as :
% %     \begin{itemize}
% %       \item $x \sleq x$, $\get r \sleq \get r$, $\set r V \sleq \set r V$
% %       \item $\refssl{}{V}{M\ N} \sleq \refssl{}{V}{M'\ N'}$
% %         or $M \parallel N \sleq M' \parallel N'$ iff $M \sleq M'$ and $N \sleq N'$
% %       \item $\lambda x.M \sleq \lambda x.M'$ if $M =
% %         \varss{\sigma_1}{\varss{\ldots}{\varss{\sigma_n}{N}}}$ such that
% %         $N\{\sigma_1,\ldots,\sigma_n\} = N$.
% %       \item $\refssd{}{V}{M} \sleq \refssd{}{V}{M'}$ or $\refssu{}{V}{M}
% %         \sleq \refssu{}{V}{M'}$ iff $M \sleq M'$
% %     \end{itemize}
% %   \end{definition}
% %
% %   \begin{lemma}{Properties of the substitution
% %     order}\label{lemma-substitution-equivalence-prop}\\
% %     $\sleq$ is a simulation order, meaning that if $M \sleq N$ and $M \to
% %     M'$, then $N \to^\ast N'$ with $M' \sleq N'$
% %   \end{lemma}
% %
% %   We can now state the following result modulo this equivalence
% %
% %   \begin{lemma}{Explicit substitution}\label{lemma-expl-subst}\\
% %     Let $P = C[E[\varss{\sigma}{M}]]$ with $M$ containing no explicit
% %     substitutions nor upward reference substitution.
% %     Then $$P \to_\texttt{aux}^\ast P' \sleq C[E[\varmetas{x}{V}{M}]]$$
% %   \end{lemma}
% %
% %   % \begin{proof}
% %   %   By induction on $M$.
% %   %   \begin{itemize}
% %   %     \item Neutral \\
% %   %       If $M=\ast$, $M=\get{r}$ or $M=y$ with $y \neq x$, then
% %   %       $\varmetas{x}{V}{M}=M$. If we apply \rrulet{subst}{unit} (resp.
% %   %       \rrulet{subst}{get},\rrulet{subst}{var}) we also get
% %   %       that $$C[E[\varss{\sigma}{M}]] \to_\text{aux} C[E[M]]$$
% %   %     \item $M=x$ \\
% %   %       $\varmetas{x}{V}{M}=V$. By \rrulet{subst}{var},
% %   %       $$C[E[\varss{\sigma}{x}]] \to_\text{aux} C[E[V]]$$
% %   %     \item $M=\lambda y. M'$ \\
% %   %       $\varmetas{x}{V}{M}=\lambda y.(\varmetas{x}{V}{M'})$. By
% %   %       \rrule{subst}{\lambda},
% %   %       $$C[E[\varss{\sigma}{\lambda y. M'}]] \to_\text{aux}
% %   %       C[E[\lambda y. (\varss{\sigma}{M'})]]
% %   %       \sleq C[E[\lambda y.(M'\{\sigma\})]]$$
% %   %     \item \ldots \\
% %   %       The remaining cases are treated similarly, the reduction rules being
% %   %       designed to make this lemma work.
% %   %       TODO : explain why we don't care about reference substitution, that
% %   %       cannot have free variables in the translation
% %   %       % There is a little subtelty, depending on how the substitution
% %   %       % $\varmetas{M}{x}{V}$ is defined with respect to references substitutions, ie when $M =
% %   %       % \refssd{r}{\mathcal{V}}{M'}$ for example. Actually, the
% %   %       % variables appearing in $\mathcal{V}$ should not be bound by any lambda because these
% %   %       % values have been emitted by sets, and sets can't be reduced under
% %   %       % lambdas. Thus all substitutions of bound variables in $\mathcal{V}$
% %   %       % already occured, and only globally free variables can remain. We define $M[x/V]$ to be
% %   %       % $\substvg{r}{\mathcal{V}}{(M'[x/V])}$, which matches the reduction rule
% %   %       % $\texttt{subst}_{\texttt{subst}_\texttt{r}}$, and this case is treated
% %   %       % as others.
% %   %   \end{itemize}
% %   % \end{proof}
% %   %
% % \subsection{One-step simulation}
% %   We prove now the technical result that will give the main theorem, which is
% %   contained in this lemma :
% %
% %   \begin{theorem}{One-step simulation}\label{theorem-simulation}\\
% %     Let $P,Q$ be \lamadio programs such that $P
% %     \rightarrow_\texttt{orig} Q$. Then
% %     $$\overline{P} \rightarrow_\texttt{aux}^\ast M \sleq \overline{Q}$$
% %   \end{theorem}
% %
% %   From which, thanks to \ref{lemma-substitution-equivalence-prop}, we easily deduce
% %
% %   \begin{theorem}{Simulation}\label{theorem-simulation}\\
% %     Let $P,Q$ be \lamadio programs such that $P
% %     \rightarrow_\texttt{orig}^\ast Q$. Then
% %     $$\overline{P} \rightarrow_\texttt{aux}^\ast M \sleq \overline{Q}$$
% %   \end{theorem} 
% %
% %   % \begin{proof}\ref{theorem-simulation}\\
% %   %   By case analysis on the reduction rule applied :
% %   %   \begin{description}
% %   %     \item[$\beta_v$] We have $P = E[(\lambda x. M)\ V] \parallel N \parallel
% %   %       S$ and $Q = E[\varmetas{x}{V}M] \parallel N \parallel S$. Let
% %   %       By ~\ref{lemma-ctxt-decomp}, $\overline{P} =
% %   %       \overline{E}^S[\refrawsl{r}{\vstore}{\lambda x. M
% %   %       \ V}] \parallel \overline{N}^S$ and $\overline{Q} =
% %   %         \overline{E}^S[\overline{\varmetas{x}{V}{M}}^S] \parallel \overline{N}^S$. Then, by
% %   %       one application of $\beta_v$ in \lthis, we have $\overline{P}
% %   %       \rightarrow_\texttt{aux} Q_0 =
% %   %       \overline{E}^S[\varss{\sigma}{\refrawsd{}{\vstore}{M}}] \parallel
% %   %       \overline{N}^S$.
% %   %       We apply \ref{lemma-absorption} with to deduce
% %   %       $Q_0 \to^\ast Q_1 = \overline{E}^S[\varss{\sigma}{\overline{M}^S}]
% %   %       \parallel \overline{N}^S$. Using \ref{lemma-expl-subst} and
% %   %       \ref{lemma-subst}, we get $Q_1
% %   %       \to^\ast Q_2 \sleq \overline{E}^S[\overline{\varmetas{x}{V}{M}}^S] \parallel
% %   %       \overline{N}^S=\overline{Q}$.
% %   %     \item[get] We have $P = E[\get{r}] \parallel N \parallel S$ with
% %   %       $S=S' \parallel
% %   %       r \Leftarrow V$, and $Q = E[V] \parallel N \parallel S$.
% %   %       By \ref{lemma-ctxt-decomp},
% %   %       $\overline{P} = \overline{E}^S[\refssd{}{V}{\get{r}}]
% %   %       \parallel \overline{N}^S$ and $\overline{Q} = \overline{E}^S[V]
% %   %       \parallel \overline{N}^S$.
% %   %       The rule \rrulet{subst-r}{get} gives $\overline{P} \to_\text{aux}
% %   %       \overline{E}^S[V] \parallel \overline{N}^S = \overline{Q}$.
% %   %     \item[set] We have $P = E[\set r V] \parallel N \parallel S'$ and $Q = E[\ast]
% %   %       \parallel N \parallel S$ with $S = S' \parallel r \Leftarrow V$. By
% %   %       \ref{lemma-ctxt-decomp}, $\overline{P} =
% %   %       \overline{E}^{S'}[\refssu{}{V}{\ast}]
% %   %       \parallel \overline{N}^{S'}$ and $\overline{Q} = \overline{E}^S[\ast]
% %   %       \parallel \overline{N}^S = \overline{E[\ast] \parallel N}^S$.
% %   %       We apply \ref{lemma-diffusion} to get
% %   %       $P \to^\ast \refssu{}{V}{(\overline{E}^S[\ast] \parallel
% %   %       \overline{N}^S)}$ and then use the rule \rrule{subst-r}{\top} to get
% %   %       rid of the toplevel reference substitution.
% %   %   \end{description}
% %   % \end{proof}


==> parts/language-properties.tex <==
\section{Properties of $\lamlang{aux}$}

\input{parts/properties-type}
\input{parts/properties-termination}


==> parts/nets-simulation.tex <==
\section{Simulation}

We are now equipped to state the simulation result. The one step simulation
result, which bears all the technical content, states that a one step reduction
in \lthis can be simulated by a many step reduction in nets, up to some
administrative reductions.

\begin{lemma}{One step simulation}\label{lemma-nets-simulation-onestep}\\
  Let $\vdash M : (\alpha,e)$ be closed well-typed term of \lthis
  . If $M \to N$, then $M^\bullet \to^\ast N^\bullet$.
\end{lemma}

\begin{theorem}{Simulation}\label{theorem-nets-simulation}\\
  Let $\vdash M : (\alpha,e)$ be a closed well-typed term of \lthis.
  If $M \to^\ast N$, then $M^\bullet \to^\ast N^\bullet$. 
\end{theorem}

\subsection{Nets context}

In order to prove simulation, it will be handy to manipulate the translation of
not only terms, but contexts. We add a typing rule for the hole

\begin{definition}{Hole typing rule}\label{definition-nets-simulation-typehole}\\
\[
  \infer[(hole)]
  {R,[.] : (\alpha,e) \vdash [.] : (\alpha,e)}
  {R \vdash (\alpha,e)}
\]
\end{definition}

\begin{center}
  \begin{tabular}{|c|c|}
    
  \end{tabular}
\end{center}

$[.]$ can be seen just as a special distinguished variable in the typing
derivation. From this, we use the usual rule to build derivations of typed
contexts. A context can then be translated to a net, with a special interface
determined by $\alpha$ and $e$, labelling free ports. This is what we call net
contexts. The substitution of nets consists in plugging the translation of term
of this type in this interface. 

\begin{definition}{Hole translation}\label{definition-nets-simulation-holetrans}\\
  We define the translation of a typed hole $R \vdash [.] : (\alpha,e)$
as 

\begin{center}
  \begin{tabular}{DD}
  \[
    \infer[(hole)]
    {R,[.] : (\alpha,e) \vdash [.] : (\alpha,e)}
    {R \vdash (\alpha,e)}
  \]
   & 
    \includegraphics{figures/translation/pdfs/translation-hole.pdf} \\
  \end{tabular}
\end{center}


We can then carry on and use the usual term translation to build the
translation of a context $(C[E])^\bullet$, which is a net of the form

\begin{center}
  \includegraphics{figures/translation/pdfs/translation-context.pdf}
\end{center}


The substitution of $M^\bullet$, or of any net with a compatible interface for
that matter, in $(C[E])^\bullet$ is defined by just connecting the free wires of
the substituted net to the corresponding free wire of the context hole :

\begin{center}
  \includegraphics{figures/translation/pdfs/translation-context-subst.pdf}
\end{center}

\end{definition}

The fundamental property of net contexts and net substitutions is that the substitution commutes to the translation, in the
following sense :

\begin{theorem}{Nets substitution}\label{theorem-nets-simulation-commutation}\\
  Let $ \vdash [.] : (\alpha,e)$ be a typed hole, $[.] : (\alpha,e) \vdash C[E]
  : (\beta,e')$ a typed context, and $ \vdash M : (\alpha,e)$ a term. Then :
\[
  (C[E[M]])^\bullet = (C[E])^\bullet[M^\bullet]
\]
\end{theorem}

The proof is an easy induction: the base case when $C[E] = [.]$ is immediate,
and by definition of the context translation, so is the inductive case.

The very definition of net reduction immediately entails that if $M^\bullet
\to^\ast N^\bullet$ then $(C[E])^\bullet[M^\bullet] \to^\ast
(C[E])^\bullet[N^\bullet]$. Together with
\ref{theorem-nets-simulation-commutation}, this ensures that we can focus on the case
where $C = E = [.]$, as the general case follows seamlessly.

% \subsection{Reference substitutions}
%
% We state and prove a few lemma about the reduction of the translation of reference
% substitutions.
%
% TODO
%
% \subsection{Variable substitutions reductions}
%
% Let us show the simulation for \rrulet{subst}{} rules, involving mainly
% duplication. Thanks to the previous theorem, we can assume that contexts are
% empty without loss of generality. We consider only closed terms. Indeed, since 
% reduction contexts $S,C,E$ do not bind variables, all the terms appearing in the
% premise of a rule ($V$,$M$,$\multv{V}$,\ldots) are thus closed terms, and we can
% omit their context. For each rule, we write the translation of the premise
% followed by its reduction in nets, that match the conclusion.
%
% The fundamental rule is the variable one.
%
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrulet{subst}{var} ($\sigma(x)$ undefined)
%     & \includegraphics{figures/simulation/pdfs/subst-var-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-var-reduct.pdf} \\
%
%     \rrulet{subst}{var} ($\sigma(x)$ defined)
%     & \includegraphics{figures/simulation/pdfs/subst-var-2-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-var-2-reduct.pdf} \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% When reaching a $\get{r}$ or a $\ast$, the substitution simply vanishes.
% \begin{center}
%  \begin{longtable}{lDED}
%     \rrulet{subst}{unit}
%     & \includegraphics{figures/simulation/pdfs/subst-unit-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-unit-reduct.pdf} \\
%   \end{longtable} 
% \end{center}
%
% \paragraph{}
% The \rrulet{subst}{app}, \rrulet{subst}{subst-r} and \rrulet{subst}{subst-r'}
% perform a duplication and make use of \ref{REDUCTION-SUBST-SUBSTR} to propagate
% the substitution inside reference substitutions.
%
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrulet{subst}{app}
%     & \multicolumn{3}{D}{
%       \includegraphics{figures/simulation/pdfs/subst-app-redex.pdf}
%     } \\
%
%     $\to^\ast$
%     & \multicolumn{3}{D}{
%       \includegraphics{figures/simulation/pdfs/subst-app-reduct.pdf}
%     } \\
%
%     \rrulet{subst}{subst-r}
%     & \includegraphics{figures/simulation/pdfs/subst-substr-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-substr-reduct.pdf} \\
%
%     \rrulet{subst}{subst-r'}
%     & \includegraphics{figures/simulation/pdfs/subst-substrp-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-substrp-reduct.pdf} \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% The \rrule{subst}{\parallel} just duplicate the variable substitution to the two
% threads
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrule{subst}{\parallel}
%     & \includegraphics{figures/simulation/pdfs/subst-par-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-par-reduct.pdf} \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% Finally, the \rrulet{subst}{merge} distributes the outter substitution to both
% the term and the inner substitution.
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrulet{subst}{merge}
%     & \includegraphics{figures/simulation/pdfs/subst-merge-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/subst-merge-reduct.pdf} \\
%   \end{longtable}
% \end{center}
%
% \subsection{Downward reference substitutions reductions}
%
% The propagation of references substitutions relies on the behavior of routing
% area, and especially the Transit lemma (\ref{lemma-route-transit}). The
% fundamental case is the non deterministic reduction happening when reducing a
% $\get{r}$ whose redex is 
% \begin{center}
%   \begin{longtable}{lD}
%     \rrulet{subst-r}{get}
%     & \includegraphics{figures/simulation/pdfs/substr-get-redex.pdf} \\
%   \end{longtable}
% \end{center}
%
% Then for each $V$ in the image of $\multv{V}$, there will be exactly one summand
% of the following form
%
% \begin{center}
%   \begin{longtable}{DED}
%     \includegraphics{figures/simulation/pdfs/substr-get-reduct-1-1.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substr-get-reduct-1-2.pdf} \\
%   \end{longtable}
% \end{center}
%
% The remaining term does indeed reduce to the translation of $\get{r}$:
% \begin{center}
%   \begin{longtable}{DED}
%     \includegraphics{figures/simulation/pdfs/substr-get-reduct-2-1.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substr-get-reduct-2-2.pdf} \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% \rrulet{subst-r}{val}, \rrule{subst-r}{\parallel} and \rrulet{subst-r}{app} are
% just direct application of the Transit lemma.
%
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrulet{subst-r}{val}
%     & \includegraphics{figures/simulation/pdfs/substr-val-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substr-val-reduct.pdf} \\
%
%     \rrule{subst-r}{\parallel}
%     & \includegraphics{figures/simulation/pdfs/substr-par-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substr-par-reduct.pdf} \\
%
%     \rrulet{subst-r}{app}
%     & \multicolumn{3}{D}{
%       \includegraphics{figures/simulation/pdfs/substr-app-redex.pdf}
%     } \\
%     $\to^\ast$
%     & \multicolumn{3}{D}{
%       \includegraphics{figures/simulation/pdfs/substr-app-reduct.pdf}
%     } \\
%   \end{longtable}
% \end{center}
%
% \paragraph{}
% \rrulet{subst-r}{merge} and \rrulet{subst-r}{subst-r'} amount to nothing in nets, as the translation
% already identifies the redex and the reduct of these rules.
%
% \begin{center}
%   \begin{longtable}{lDlD}
%     \rrulet{subst-r}{subst-r'}
%     & \includegraphics{figures/simulation/pdfs/substr-substrp-both.pdf}
%     & \rrulet{subst-r}{merge}
%     & \includegraphics{figures/simulation/pdfs/substr-merge-both.pdf} \\
%   \end{longtable}
% \end{center}
%
% \subsection{Upward reference substitutions reduction}
% As for downward substitutions, the main ingredient is the Transit lemma applies
% to our specific routing area $\delta$ and $\gamma$.
%
% \begin{center}
%   \begin{longtable}{lDED}
%     \rrule{subst-r'}{\parallel}
%     & \includegraphics{figures/simulation/pdfs/substrp-par-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substrp-par-reduct.pdf} \\
%
%     \rrulet{subst-r'}{lapp}
%     & \includegraphics{figures/simulation/pdfs/substrp-lapp-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substrp-lapp-reduct.pdf} \\
%
%     \rrulet{subst-r'}{rapp}
%     & \includegraphics{figures/simulation/pdfs/substrp-rapp-redex.pdf}
%     & $\to^\ast$
%     & \includegraphics{figures/simulation/pdfs/substrp-rapp-reduct.pdf} \\
%   \end{longtable}
% \end{center}


==> parts/nets-termination.tex <==
\newcommand{\labelsubst}[2]{|{#1}|_{#2}}
\newcommand{\lthisplus}{$\lamlang{cES+}$}

\section{Termination}

We introduced an intermediate language \lthis and showed its termination.
However, a few steps may remain to eventually reach a normal form. The first
step is to collect and merge all the routing areas that are created and
connected during the translation. Doing so, we separate the net between a part
that closely follows the translated term structure, and a big routing area which
connects various substerms to enable communication through references between
them. Once this is done, the only remaining possible redexes are dereliction,
introduced by $\get r$, facing the cocontraction tree of a input of the routing
area. A non deterministic reduction can occur, but these gets will never be fed
anything after that : there is no available assignment in the original term.
Hence, after these two steps, the nets are constrained enough to ensure that no
more redex appear. This is the essence of the proof of
\ref{lemma-nets-termination-sn}.

We first define the list of constraints that the non-routing part of the net
will satisfy :

\begin{definition}{Separability}\label{definition-nets-termination-separability}\\
  Let $\mathcal{R}$ be the translation of a \lthis or \lthisplus
  term, then $\mathcal{R}$ is say te be \emph{separable} if 
  can be reduced to the following form :

  \begin{center}
    \tikzvcenter{
      \begin{proofnet}
        % Communication box
        \node[net={40pt}{40pt}] (box) {\mathbf{R}};
        % Remaining part of the net
        \init[grow=left]([xshift=15ex]box.east){
          \nary[shape=rectangle,cell={net={40pt}{30pt}},name=sigma]{\mathcal{S}}{
            \point(sigmai1),
            \point(sigmao1),
            \point(sigmain),
            \point(sigmaon)
          }
        }
        % Box coordinates
        \coordinate (i1) at ([yshift=-13pt]box.east);
        \coordinate (o1) at ([yshift=-8pt]box.east);
        \coordinate (in) at ([yshift=8pt]box.east);
        \coordinate (on) at ([yshift=13pt]box.east);
        \coordinate (i0) at ([yshift=-3pt]box.west);
        \coordinate (o0) at ([yshift=2pt]box.west);
        % Sigma coordinates
        \coordinate (sigmai1) at ([yshift=-13pt]sigma.north);
        \coordinate (sigmao1) at ([yshift=-8pt]sigma.north);
        \coordinate (sigmain) at ([yshift=8pt]sigma.north);
        \coordinate (sigmaon) at ([yshift=13pt]sigma.north);
        % Connect box and sigma
        \init[grow=up]{ 
          \wirefromto{sigmai1}{sigmai1}{i1}{i1}
          \wirefromto{sigmain}{sigmain}{in}{in}
          \wirefromto{sigmao1}{sigmao1}{o1}{o1}
          \wirefromto{sigmaon}{sigmaon}{on}{on}
          \wirefromto{[xshift=-10pt]i0}{[xshift=-10pt]i0}{i0}{i0}
          \wirefromto{[xshift=-10pt]o0}{[xshift=-10pt]o0}{o0}{o0}
        }
        %
        \pdots[2pt]([xshift=10pt]o1)([xshift=10pt]in)
      \end{proofnet}
    }
  \end{center}
  where $\mathbf{R}$ is a routing area and $\mathcal{S}$ a net with free wires labelled by
  $i_1,\ldots,i_n,o_1,\ldots,o_m,O$, satisfying :
  \begin{itemize}
    \item There is no redex in $\mathcal{S}$
    \item $i_1,\ldots,i_m$ are either connected to the auxiliary port of a
      $\otimes$ cell, or to the principal port of a dereliction
    \item $o_1,\ldots,o_n,O$ are either connected to a
      $\parr$ cell, or to the principal door of an open box
  \end{itemize}

\end{definition}

The following lemma states that the translation of any open term is separable.
The main reason is that constructors as application, substitution, parallel,
etc. preserve separability. But the translation of values with free variables
are obviously separable.  This comes from the fact that we pushed weakening deep
inside atoms' exponential boxes, so any pending variable that is not bound
forces an auxiliary door on all the boxes, blocking further reduction.

\begin{lemma}{Open terms separability}\label{lemma-nets-termination-otsep}\\
  Let $\Gamma,x:A \vdash M : (\alpha,e)$ a \lthis well-typed term, then its
  translation $M^\bullet$ is separable. 
\end{lemma}

% \begin{proof}\ref{lemma-nets-termination-ostep}\\
% \begin{description}
%   \item[Values] As stated above, we can first observe that the translation of $\ast$, of a
%     variable $x$ and an abstraction all statisfy the separability conditions.
%     Their general form is :
%
%     % \begin{center}
%     %   \includegraphics{}
%     % \end{center}
%
%     Which is normal, and the box $R$ is just a juxtaposition of $0$-communication
%     areas, corresponding to references introduced by subtyping in $e$. Thus $m = n
%     = 0$. The net is normal, and its output $O$ is the the principal door of an
%     open box.
%   \item[Get] It is almost the same as for values, except that the output $o$
%     corresponding to the get's reference is connected to a dereliction, which is
%     allowed in (blah).
%   \item[Application] By induction, $M^\bullet$, $N^\bullet$ and $\multv{V}$ are
%     separable, thus can be decomposed in the following way :
%
%     % \begin{center}
%     %   \includegraphics{}
%     % \end{center}
%
%     We can merge all the communcation boxes in the left circle together. All the 
%     inputs or outputs previously connected to one of the small area immediatly
%     satisfies the condition (blah) by IH. The two remaining
%     wires $i_0$ and $o_0$ are respectively connected to the auxiliary port of
%     a par and the auxiliary port of a cocontraction, thus satisfy (blah). We take
%     the right circle to be our second part $\mathcal{S}$.
%     $\mathcal{S}_N$, $\mathcal{S}_M$ and $\mathcal{S}_\multv{V}$ are normal by IH.
%     $O$ is the conclusion of par, hence satisfies (blah). It only remains to see
%     that the wole net contained in the circle is normal, but the only redex that
%     could appear is the connection of a dereliction to $M^\bullet$. But by (blah),
%     $O_M$ is either the conclusion of an open box or a par, and thus the whole net
%     is normal indeed, and (blah) is verified.
%   \item[Parallel] Similar to application
%   \item[Variable substitution] As for application, we apply the IH on
%     $M^\bullet$ and $V^\bullet$, merge the routing areas, and just check that the
%     connection of $V^\bullet$ to $M^\bullet$ can't create new redexes. Indeed, by
%     (blah), the outpout $O_V$ can't be part of any redex.
%   \item[Reference substitutions] Again the same technique is applied, and we see
%     that the resulting net and routing area satisfies the conditions.
% \end{description}
%
% \end{proof}

Finally, the main result we rely on as explained above is the following one :

\begin{lemma}{Normal form separability}\label{lemma-nets-termination-nfsep}\\
  The translation of a \lthisplus normal form is separable
\end{lemma}

% \begin{proof}{\ref{lemma-nets-termination-sn}}\\
%   We apply \ref{lemma-nets-termination-nfsep} to reduce the translation of $F$ to
%   a routing area connected to $\mathcal{S}$ satisfying $P$. $\mathcal{S}$ and
%   $\routarea R$ are normal. The potential ones must take place at the interface
%   of $\routarea{R}$ and $\mathcal{S}$. The inputs of $\routarea{R}$ are
%   connected to $\mathcal{S}$, being either connected to a par or the conclusion
%   of an open box, and thus can't form any redex with (co)weakenings and
%   (co)contractions of $\routarea R$.
%
%   The output of $\routarea R$ are connected to the auxiliary port of a tensor,
%   or to a dereliction. Only the latter may form a new redex. If the output of
%   $\mathbf{R}$ is a coweakening, then everything reduces to $\mathbf{0}$. If it
%   is just a wire, then the dereliction is connected through this wire to an
%   input of $\routarea R$ which again can't be part of any redex. The only
%   remaining case is when the output of $\routarea R$ is a cocontraction tree.
%   Then we can perform the non-deterministic reduction, and we go back to exactly
%   the two previous cases as the dereliction is finally connected to a leaf of
%   the tree of an input.
%
%   Hence, after we performed finitely many dereliction/cocontraction reductions,
%   we finally get a normal form, which either $\mathbf{0}$, or a sum of the
%   previous net $\mathbf{S}$ connected to simpler routing area $\routarea{R}_i$.
% \end{proof}

Which leads us to the main result :

\begin{theorem}{Termination for nets}\\
  The translation of a well typed term of \lthis\ terminates.
\end{theorem}


==> parts/properties-termination.tex <==
\subsection{Termination}
\label{sec:lces-props:termination}

We proceed by reducibility. In this whole part, we will tune the reduction so
that the \rrulet{subst-r}{get} reduction becomes non-determinstic : instead of producing a
sum, one chose one term among the summands to be the reduct. We will prove
termination for this reduction, from which termination for the original one follows easily.
We first need to lay some definitions

\paragraph{}

The following definition attempts at formalizing the behavior of a term in an
"environment", ie as a subterm of a bigger one, where it can be exposed to
arbitrary incoming downward substitutions references. The usual defintion of
strongly computable terms for simply typed lambda calculus is not sufficient to
prove termination, because here separate subterms can affect each other
through references substitutions. Thus we need to add a property to the definition of SC
terms, namely that they are well-behaved when we put them in an environment of
other well-behaved terms : they only emit a finite number of strongly computable
terms.

An environment reduction abstract the enclosing context just as a sequence of
incoming downard substitutions.

\begin{mdef}{Environment reduction}\label{mdef-env-reduction}\\
  Let $\vdash M : (\alpha,e)$ be well typed (simple) term, Let $\seq{\multv{V}}$
  be a sequence of references substitutions such that $\refrawsd{}{\multv{V}_i}{M}$ is well typed that we write
  $\vdash (M,\seq{\multv{V}})$.  We call a $(M,\seq{\multv{V}})$-reduction a finite
  or infinite reduction sequence starting from $M$ where each rule is either a
  usual one or a rule $\to_i$ defined by $M \to_i
  \refrawsd{}{\multv{V}_i}{M}$.
\end{mdef}

We will also make use of another tool that compares two terms that have
essentially the same structure but differ in their downard references
substitutions. The main point is that if a term $M$ has more substitutions
available than $N$, then any reduction than can be performed in $N$ can be
performed in $M$. In particular, if $M$ is strongly normalizable, then so is
$N$.

\begin{mdef}{Reachability and associated pre-order}\\
  Let $M$ be a term, and $N$ an occurence of a subterm in $M$
  that is not under a lambda. We define
  $\reach{r}{M}$ the set of all reference substitutions that are in scope
  of this subterm in $M$, by
  \begin{itemize}
    \item If $M=N$ then $\reach{N}{M} = \emptyset$
    \item If $M=\refssd{s}{U}{M'}$ then $\reach{N}{M} = \multv{U}
      + \reach{N}{M'}$
    \item If $M=\varss{\sigma}{M'}$ then $\reach{N}{M} =
      \varsmetas{x}{V}{\reach{r}{M'}}$
    \item If $M = \refssu{s}{U}{M'}$ then $\reach{N}{M} =
      \reach{r}{M'}$
    \item If $M=\refssl{s}{U}{M_1\ M_2}$ or $M = M_1 \parallel M_2$, let $i$ be the index such that
      $N$ occurs in $M_i$, then $\reach{N}{M} = \reach{N}{M_i}$
  \end{itemize}

  We define the skeleton of a term $\skel{M}$ by removing all downward
  reference substitutions that are not under a lambda. We say that $M
  \rincl N$
  if :
  \begin{itemize}
    \item $\skel{M}$ = $\skel{N}$, and thus we can put in a one-to-one correspondance the occurences of
      $\get{r}$ and $\refssl{}{V}{M_1\ M_2}$ subterms of $M$ and $N$
    \item For all such $\get{r}$ occurences, $\reach{\get{r}}{M} \subseteq
      \reach{\get{r}}{N}$
    \item For all such $M' = \refssl{r}{V}{M_1\ M_2}$ corresponding to
      $N' = \refssl{s}{U}{N_1\ N_2}$, then $\reach{M'}{M} + \multv{V}
      \subseteq \reach{N'}{N} + \multv{U}$
  \end{itemize}

  Similarly, we say that $M \rdiff{V} N$ if the
  difference between reachability sets involved in the definition is somehow
  "bounded" by $\multv{V}$ :
  \begin{itemize}
    \item $\skel{M}$ = $\skel{N}$
    \item For all such $\get{r}$ occurences, $\reach{\get{r}}{M} \subseteq
      \reach{\get{r}}{N} \subseteq \reach{\get{r}}{M} + \multv{V}$
    \item For all such $M' = \refssl{s}{U}{M_1\ M_2}$ corresponding to
      $N' = \refssl{t}{W}{N_1\ N_2}$, then $\reach{M'}{M} + \multv{W} \subseteq
      \reach{N'}{N} + \multv{U} \subseteq \reach{M'}{M} + \multv{W} + \multv{V} $
  \end{itemize}

  $\rincl$ (resp. $\rdiff{V}$) is a partial pre-order on terms. The equivalence relation induced by
  these preorders is the same and is noted $\req$.
\end{mdef}

\begin{mlem}{Invariance by \rrulet{subst-r}{}
reductions}\label{mlem-ord-invariance}\\
Let $M \rincl N$ (resp. $M \rdiff{V} N$).
  \begin{itemize}
    \item If $M \to M'$ by a \rrulet{subst-r}{} rule except
      \rrulet{subst-r}{get} then $M' \rincl N$ (resp. $M' \rdiff{V} N$)
    \item If $N \to N'$ by a
      \rrulet{subst-r}{} by a \rrulet{subst-r}{} rule except
      \rrulet{subst-r}{get} then $M \rincl N'$ (resp. $M \rdiff{V} N'$).
  \end{itemize}
\end{mlem}

\begin{proof}
 Clearly, a \rrulet{subst-r}{} rule does not modify the skeleton, so $\skel{M} =
 \skel{M'} = \skel{N}$. It is also almost immediate to see that rules that
 propagate reference substitutions or \rrulet{subst-r}{val} that erases the ones
 only in scope of a value do not modify $\reach{\get{r}}{M}$ for an
 occurence $\get{r}$ in $M$, nor do they modify $\reach{M'}{M} + \multv{V}$ for
 $M' = \refssl{r}{V}{M_1\ M_2}$.
\end{proof}

\begin{mlem}{Simulation}\label{mlem-ord-simulation}\\
  Let $M \rincl N$ (resp. $M \rdiff{V} N$).
  \begin{enumerate}
    \item If $M \to M'$ then $\exists n \geq 0,\ N \to^n N'$ such that $M'
      \rincl N'$ (resp. $M' \rdiff{V} N'$). If the
      applied rule is not a \rrulet{subst-r}{} or is \rrulet{subst-r}{get}, then
      $n > 0$.
    \item Corollary. If $M \rincl N$, then if $N$ is strongly normalizing, so is
      $M$.
    \item Corollary. If $M \req N$, then $M$ is strongly normalizing iff $N$
      is.
  \end{enumerate}
\end{mlem}

\begin{proof}
  We will first prove that if $M = C[E[P]$, then $N \to^\ast C[E'[P']]$. One may
  just have to apply the rule \rrule{subst-r}{\parallel} until it
  is not possible anymore to get $N \to C[N']$. Then, $E[P]$ and $N'$ having the
  same skeleton,
  $N'$ can be written as $E'[P']$ where $E'$ is $E$ with
  additionnal downward references substitutions, and $P$ and $P'$ have the same
  skeleton and the same head constructor (if $P'$ have additionnal substitutions in
  head position one can always include it in $E'$ : we actually take the maximal $E'$
  that satisfies the decomposition).
  The reachability sets of subterms in $C$ (respectively $E$,$E'$) only depends
  on $C$ (resp. $C,E$ and $C,E'$). The reachability sets of subterms in $P$
  (resp. $P'$) are unions of substitutions occuring in $P,E$ (resp.
  $P',E'$) and $C$.

  \begin{itemize}
    \item If the rule is one of the \rrulet{subst-r}{} except
      \rrulet{subst-r}{get}, by \ref{mlem-ord-invariance}, $n=0$ works.
    \item \rrulet{subst-r}{get} : $P = \refssd{r}{V}{\get{r}} \to V \in
      \multv{V}(r)$ and $P =
      \refssd{r'}{V'}{\get{r}}$. $\multv{V}(r)$ is in $\reach{\get{r}}{N}$ so by iterated application of \rrulet{subst-r}{}
      rules except \rrulet{subst-r}{get} and \rrulet{subst-r}{val}, we can push
      (without modifying the skeleton nor the reachability sets) the
      corresponding substitutions down to $\get{r}$ in $P'$ and we can do the
      same reduction. All the other reachability sets of gets or application or
      left unmodified.
    \item $(\beta_v)$ : $P = \refssl{r}{V}{(\lambda x. Q)\ V} \to
      T = \refssd{r}{V}{\vars{x}{V}{Q}}$. Up to
      \rrulet{subst-r}{val} reductions, $P' = \refssl{r'}{V'}{(\lambda x. Q)\ V} \to
        T' = \refssd{r'}{V'}{\vars{x}{V}{Q}}$. The condition on reachabiliy sets for
        application in the defintion of $\rincl$ precisely ensures that all the
        gets and applications in $Q$ have the same reachability in
        $C[E[T]]$ and in $C[E'[T']]$.
  \end{itemize}

  \rrulet{subst}{} rules
  \begin{itemize}
    \item \rrulet{subst}{var} : $P = \varss{\sigma}{x} \to x$ or $V(x)$, and $P' =
      \varss{\sigma}{\refssd{r}{V}{x}} \to \varss{\sigma}{x} \to x$ or $V(x)$.
    \item \rrulet{subst}{app} : $P = \varss{\sigma}{\refssl{r}{V}{Q_1\ Q_2}} \to
      T = \refrawsl{\vect{r}}{(\varss{\sigma}{V})}{(\varss{\sigma}{Q_1})\
      (\varss{\sigma}{Q_2})}$. We have $P' =
      \varss{\sigma}{\refssl{r'}{V'}{(\refssl{s}{U}{Q'_1})\
      (\refssl{t}{W}{Q'_2})}} \to^\ast
      \refrawsl{r'}{\varss{\sigma}{V'}}{(\refrawsd{s}{\varss{\sigma}{U}}{\varss{\sigma}{Q_1}})\
      (\refrawsd{s}{\varss{t}{V}{W}}{\varss{\sigma}{Q_2}})}$. By definition of
      reachability sets, they are invariant by all the rule applied.
    \item We proceed the same way for other cases : the var substitution just
      go through the additionnal references substitutions, and by design,
      reachability sets are not modified.
  \end{itemize}

  \rrulet{subst-r'}{} rules
  \begin{itemize}
    \item Upward substitutions commute with downward ones without interacting.
      On the other hand, they can span new downward substitutions but in this
      case, they do it in the same way for both $P$ and $P'$ and thus do not
      modify the inclusion relation on reachability sets.
  \end{itemize}
\end{proof}
%
% \begin{mdef}{Completion}\label{mdef-completion}\\
% Let $ \vdash M,N : (\alpha,e)$,
% $\vect{r},\vect{\mathcal{V}}$ be respectively
% references and multivalues, we define the relation $\complrv$ by the following
% rules :
%   \begin{itemize}
%     \item $V \complrv V$
%     \item $M \complu{(r,\mathcal{V})+(s,\mathcal{U})} \refssd{r}{V}{N}$ if $M \compl{s}{U} N$
%     \item $\refssd{s}{U}{M'} \compl{r}{V} N$ if $M'
%       \complu{(r,\mathcal{V})+(s,\mathcal{U})} N$
%     \item $\refssl{s}{U}{M_1\ M_2} \complrv \refssl{s'}{U'}{N_1\ N_2}$ if $M_i
%       \complrv N_i$ and $(r,\multv{V}) + (s,\multv{U}) = (s',\multv{U}')$
%     \item $\varss{x}{U}{M} \compl{\emptyset}{\emptyset} \varss{x}{U}{M}$
%     \item $\refssu{s}{U}{M} \complrv \refssu{s}{U}{N}$ if $M \complrv N$
%     \item $M = M_1 \parallel M_2$ then $N = N_1 \parallel N_2$ with $M_i
%       \complrv N_i$
%   \end{itemize}
%   We extend this definition to context by adding the rule $[.] \complrv [.]$ for
%   any $(r,\mathcal{V})$.
% \end{mdef}
%
% \paragraph{}
% We need to prove a few lemma concerning completions.
%
% \begin{mlem}{Decomposition}\label{mlem-completion-decomposition}\\
% Let $M \complrv N$.
%
% \begin{enumerate}
%   \item If $M = C[E[M']]$ for some $M'$, then $N \to^\ast
%    C'[E'[N']]$ where $C[E] \compl{s}{U} C'[E']$ and $M' \compl{r'}{V'} N'$.
% Moreover, if $P \compl{r'}{V'} Q$ with the same type as $M'$ and $N'$ then $C[E[P]] \complrv C'[E'[Q]]$.
%   \item If $N = C[E[N']]$, then $M
%     \to^\ast
%     C'[E'[M']]$ where $C'[E'] \compl{s}{U} C[E]$ and $M' \compl{r'}{V'} N'$
%     such that for any $P \compl{r'}{V'} Q$ with the same type as $M'$ and $N'$ then $C'[E'[P]]
%     \complrv C[E[Q]]$
% \end{enumerate}
% \end{mlem}
%
% \begin{mlem}{Simulation}
% \label{mlem-completion-reduction-stability}\\
%   Let $M \complrv N$.
%   \begin{enumerate}
%     \item If $M \to M'$ then $N \to^\ast N'$ such that $M' \complrv
%       N'$. Moreover, if the applied reduction rule is not \rrule{subst-r}{} or
%       is \rrulet{subst-r}{get}, then $N \to^+ N'$.
%     \item If $(r,\multv{V}) = (\emptyset,\emptyset)$ and $N \to N'$ then $M
%       \to^+ M'$ such that $M' \compl{\emptyset}{\emptyset} N'$. Moreover,
%       if the applied reduction rule is not \rrule{subst-r}{} or is
%       \rrulet{subst-r}{get}, then $M \to^+ M'$.
%     \item Corollary : if $M \complrv N$, then $N$ is strongly normalizing
%       implies that $M$ is. Moreover, if $(r,\multv{V})=(\emptyset,\emptyset)$,
%       then $N$ is iff $M$ is.
%   \end{enumerate}
% \end{mlem}
%
% \begin{proof}
% The first lemma is proved by induction on the contexts (C,E), from the
% definition of $\complrv$.  For the second one, we proceed by case analysis on
% the reduction rule. We consider first \rrule{subst-r}{}
% rules. Thanks to the first lemma, we can ignore contexts and assume that
% $C=E=[]$.
% \begin{itemize}
%   \item $(\beta_v)$
%     \begin{enumerate}
%       \item $$M = \refssl{s}{U}{(\lambda x. M_1)\ V}$$
%         so $N = \refssd{t}{W}{\refssl{s'}{U'}{(\lambda x. M_1)\ V}}$ with $M_i
%         \compl{r'}{V'} N_i$, $(s',\mathcal{U}') = (s,\mathcal{U}) +
%         (r',\mathcal{V'})$ and $(r,\mathcal{V}) = (t,\mathcal{W}) + (r',\mathcal{V'})$.
%         Then $$N \to^2 N' = \refssd{t+s'}{W+U'}{\vars{x}{V}{M}}$$ and
%         $$M' = \refssd{s}{U}{\vars{x}{V}{M}} \complrv
%         N'$$.
%       \item
%         Conversely, if $N = \refssl{s}{U}{(\lambda x. N_1)\ V}$, then $M
%         = \refssd{t}{W}{\refssl{s'}{U'}{(\lambda x. M_1)\ V}}$
%         such that $M_1 \compl{t}{W} N_1$ and
%         $(s,\multv{U}) = (s',\multv{U'}) + (t,\multv{W})$. Then $M
%         \to^\ast \refssl{s}{\multv{U}}{(\lambda x . M_1)\ V} = N \to
%         N'$.
%     \end{enumerate}
%   \item \rrulet{subst-r}{get}
%     \begin{enumerate}
%       \item $M = \refssd{s}{U}{\get{t}}$, hence $N \to^\ast
%         \refssd{s'}{U'}{\get{t}}$ with $s,\mathcal{U} \subset s',\mathcal{U'}$.
%         Since $M' = \get{t}$ or $M' = U \in \multv{U}$, then $N \to^+ M'$.
%       \item If $(r,\multv{V})=(\emptyset,\emptyset)$ and $N =
%         \refssd{s}{U}{\get{t}}$ then $M \to^\ast \refssd{s}{U}{\get{t}}$, and
%         the statement is obviously true.
%     \end{enumerate}
% \end{itemize}
%
% Variables substitutions. If $N$ is a \rrulet{subst}{var} redex then
% $(r,\multv{V}) = (\emptyset, \emptyset)$, $N = M$ and there is nothing to prove.
% If $M$ is a redex, $N = \refssd{r}{V}{M}$. Then $N \to N' = \refssd{r}{V}{M'}$
% and $M' \complrv N'$.
%
% And finally upward substitutions.
% \begin{itemize}
%   \item \rrule{subst-r'}{\parallel}
%     \begin{enumerate}
%       \item
%         $M = (\refssu{s}{U}{M_1}) \parallel M_2$, then
%         $N \to^\ast {(\refssd{t}{W}{\refssu{s}{U}{N_1}}) \parallel
%         (\refssd{u}{X}{N_2})}$ with $M_1
%         \complu{(r,\multv{V}) - (t,\multv{W})} N_1$ and $M_2
%         \complu{(r,\multv{V}) - (u,\multv{X})} N_2$.
%         Then $M' = \refssu{s}{U}{(M_1 \parallel \refssd{s}{U}{M_2})}$, and $N \to^+ N'
%         = \refssu{s}{U}{(\refssd{t'}{W'}{N_1}) \parallel
%         (\refssd{u'}{X'}{N_2}})$ with $(t',\multv{W'}) = (t,\multv{W}) +
%         (s,\multv{U})$ and same for $(u,\multv{X})$. This gives us $M' \complrv
%         N'$.
%       \item A similar argument gives that $M \to M' \complrv N'$.
%     \end{enumerate}
% \end{itemize}
%
% The third point of the lemma is an almost immediate corollay of the first two.
% One just has to notice that an infinite reduction can not contain an infinite
% subsequence of \rrule{subst-r}{} (excluding \rrulet{subst-r}{get}) reductions,
% because these reductions always move references substitutions deeper.
% Technically, for any downard reference substitution $s$, let $d(s)$ be its
% depth in the AST, and $D$ the maximal depth of the term, then the multiset
% $[ D - d(s) \mid s \in M ]$ is a decreasing (for the usual well-ordered set of
% finite multisets over natural numbers) parameter of the reduction.
% \end{proof}
%
\begin{mdef}{Strongly computable terms}\label{mdef-strongly-computable}\\
  The set $\mathbf{SC}_R(\alpha,e)$ of strongly computable terms of type
$(\alpha,e)$ is defined by induction on (simple) terms.
Later, we will omit the $R$ or $(\alpha,e)$ when it is obvious from the context and
just write $M \in \mathbf{SC}$. Moreover, we abusively write $\multv{V} \subseteq
\mathbf{SC}$ for a substitutions to mean $\forall r, \multv{V}(r) \in
\mathbf{SC}_R(R(r),\emptyset)$.

\begin{itemize}
  \item $M \in \mathbf{SC}_R(\tau,e)$ where $\tau = \text{Unit} \mid \mathbf{B}$ if $R \vdash M :
    (\tau,e)$ and :
    \begin{itemize}
      \item (SN) $$\multv{V} \subseteq \mathbf{SC}_R
        \implies \refssd{r}{V}{M} \text{ is SN (strongely normalizable)}$$
      \item (WB)
        For any $r,\mathcal{V}$ such that $\vdash (M,r,\mathcal{V})$ and
        $\mathcal{V} \subseteq \mathbf{SC}_R$,
        for any $(M,\seq{\multv{V}})$ reduction $M = M_0 \to \ldots \to M_n$
        there exists $n_0 \geq 1$ such that for any $k \geq 1$ then
        \begin{enumerate}
          \item If $M_{k-1} = \refssu{}{U}{N} \to M_k$ is a
            \rrule{subst-r'}{\top} reduction then $\mathcal{U} \subseteq
            \mathbf{SC}$
          \item if $k \geq n_0$ then $M_{k-1} \to M_k$ is not \rrule{subst-r'}{\top}
        \end{enumerate}
    \end{itemize}
  \item $M \in \mathbf{SC}_R(A \sur{\to}{e_1} \alpha,e)$ if $R \vdash M :
    (A \sur{\to}{e_1} \alpha,e)$ with $e_1 \subseteq e = \{ r_i \}$ and
    \[
      N \in \mathbf{SC}_R(A,e) \implies M\ N \in \mathbf{SC}_R(\alpha,e)
    \]
\end{itemize}
\end{mdef}

\paragraph{}
% \begin{mlem}{Anti-reduction}\label{mlem-antired}\\
%   If $R \vdash M : (\alpha,e)$ and $M \to M' \in \mathbf{SC}(\alpha,e)$ then $M
%   \in \mathbf{SC}(\alpha,e)$
% \end{mlem}
%
% \begin{proof}
%   TODO
% \end{proof}

\begin{mlem}{Characterization}\label{mlem-charact}\\
  Let
  \begin{itemize}
    \item $\alpha = A_1 \sur{\to}{e_1} \ldots \sur{\to}{e_{n-1}} A_n
      \sur{\to}{e_n} \beta$ with $\beta = \text{Unit} \mid \mathbf{B}$
    \item $\vdash M : (\alpha,e)$
    \item $N_i \in \mathbf{SC}(A_i,e_i')$
    \item $\multv{U} \subseteq \mathbf{SC}$
  \end{itemize}
  with $\ptentre{i}{1}{n}, e'_i \subseteq e_i \subseteq e$ and $\dom{\multv{U}} \subseteq e$.
  We define
  \[
    \Lambda(M,\multv{U},\seq{N}) = \refssd{r}{\mathcal{U}}{M\ N_1\ \ldots\ N_n}
  \]
    Then $M \in \mathbf{SC}(\alpha,e)$ if and only if
  $\Lambda(M,\multv{U},\seq{N})$ is (SN) and (WB) for all $\multv{U},\seq{N}$
  satisfying the above conditions.
  In the following, we may conveniently omit some of the parameters
  $(M,\multv{U},\seq{N})$ of $\Lambda$.
\end{mlem}

\begin{proof}
  By induction on types.
\end{proof}

\begin{mlem}{Auxiliary results for soundness}\label{mlem-soundness-aux}\\
  Let $M,V \in \mathbf{SC},\ \multv{V} \subseteq \mathbf{SC}$ then
  \begin{enumerate}
    \item For any infinite reduction of $\Lambda(N)$, $N$ must be reduced at some
      point.
    \item If $\varss{\sigma}{N} \to M$ then $\varss{\sigma}{N} \in \mathbf{SC}$
    \item $\refssd{r}{V}{M} \in \mathbf{SC}$
    \item $\refssu{r}{V}{M} \in \mathbf{SC}$
    \item If $M \to M'$, then $M' \in \mathbf{SC}$
    \item $\varsmetas{x}{V}{\multv{V}} \subseteq \mathbf{SC}$
  \end{enumerate}
\end{mlem}

\begin{proof}


  \begin{enumerate}
    \item If the subterm $N$ is never reduced, the reducts of $\Lambda(N)$ are of
      the form $N\ N_1' \ldots N_n'$ (with some additionnal reference
      substitutions not written for conciseness) where each $N_i'$ can be seen as the result
      of an $(N_i,\seq{\multv{W}})$ reduction for some $\seq{\multv{W}}$ corresponding
      to the upward substitutions generated by the interaction with other
      subterms $N_1,\ldots,N_n$. All these subterms are (WB) and
      generate $\mathbf{SC}$ upward substitutions. $N_i$ being well behaved, there is a number of
      steps $n_i$ after wich the reduct $N'_i$ doesn't generate upward
      substitutions anymore. After $n= \vee n_i$ steps (actually one may have to take a
      bigger $n$ for the substitutions have to dispatch, but there is such a $n$), $N_i$ has reduced to some $P_i$
      and doesn't receive any downard substitution. If we gather all the downward substitutions
      delivered to $N_i$ (or, viewed as an $(N_i,\seq{\multv{W}})$ reduction, all
      the substitutions produced by $\to_i$ rules) as $\multv{X}$, then
      $N_i \rdiff{U} Q = \refssd{}{U}{N_i}$. Consider the first step of the
      $(N_i,\seq{\multv{W}})$ reduction $N_i \to N_i'$, either this is a usual step and then by
      \ref{mlem-ord-simulation} $Q \to^\ast Q'$ with $N_i'
      \rdiff{U} Q'$ or this is a $\to_j$ step and $N_i' = \refssd{}{Z}{N_i}$
      for some $\multv{Z} \subseteq \multv{U}$ and $N_i'
      \rdiffraw{\multv{U} \setminus \multv{Z}} Q$. By induction over the n firt
      steps, we get that $Q \to^\ast Q_0$ such that $P_i
      \req Q_0$. Since $N_i \in \mathbf{SC}$, $Q$ and all its reducts are
      (SN), and so is $P_i$ thus the reduction of $\Lambda(N)$ must be finite.

    \item Let $M' = \varss{\sigma}{M}$, consider an infinite reduction of
      $\Lambda(M')$.  By the previous point, the subterm $M'$ must be reduced,
      and $M$ is the only possible reduct. But the reduct of $\Lambda(M')$
      we get is reachable from $\Lambda(M)$ which is (SN) thus the reduction
      must be finite and $\Lambda(M')$ is (SN).

      Similarly, consider (for suitable $\seq{\multv{V}}$) a $(M',\seq{\multv{V}})$
      reduction. If $M'$ is never reduced, then no upward
      substitution is ever produced. If $M'$ is reduced at
      some point, then it is reduced to $M$ and thus produces a finite amount of
      $\mathbf{SC}$ upward substitutions since $M$ is (WB). Hence $M'$ is (WB).

    \item Consider $\Lambda(\refssd{r}{V}{M},\multv{U},\seq{N})$. Then
      $\Lambda(\refssd{r}{V}{M},\multv{U},\seq{N}) \rincl \Lambda(M,\multv{U} +
      \multv{V},\seq{N})$ but the latter is (SN), since $M$ is $\mathbf{SC}$. So is
      the former by \ref{mlem-ord-simulation}.
      For (WB), we can easily map a $(M',\seq{\multv{W'}})$ reduction to a
      $(M,\seq{\multv{W}})$ by just appending $\multv{V}$ to
      $\seq{\multv{W}}$ and
      start with a $\to_i$ reduction. Since $M \in \mathbf{SC}$, $M'$ is (WB).
    % \item For this one, we will use induction on types. Base case : for any
    %   adapted $(s,\multv{U})$, $\refssd{s}{U}{M'} \compl{\emptyset}{\emptyset}
    %   \refssd{t}{W}{M}$ where $(t,\multv{W}) = (s,\multv{U}) + (r,\multv{V})$. Since $M
    %   \in \mathbf{SC}$ then by definition  the latter is (SN). $M$ is well behaved, thus so is
    %   $M'$ : we can easily map a reduction sequence of $M'$ to a $M$ one by adding
    %   $(r,\multv{V})$ to the available references. Now, take $\alpha = A
    %   \sur{\to}{e} \beta$. By induction, $\refssd{r}{V}{N_i} \in \mathbf{SC}$,
    %   and $\Lambda(M,(r,\multv{V})+(s,\multv{U}),N_i)
    %   \compl{\emptyset}{\emptyset} \Lambda(M',(s,\multv{U}),\refssd{r}{V}{N_i})$
    %   $\Lambda(M')$. Assume that the reducts of $M'$ are never part of a
    %   $\beta_v$.  As before, there is a point from which no references
    %   substitutions are exchanged anymore, and the reducts of the $N_is$
    %   terminate, so the reducts of $M'$ must diverge. But we can map this
    %   divergent sequence to a divergent one of $\refssd{t}{W}{M}$ for some
    %   $(t,\multv{W})$ which is (SN). There is a contradiction and thus the
    %   reduction is finite. Now, if there is a $\beta_v$ reduction, then one of the reduct of a subterm must
    %   $\Lambda(M,(s,\multv{U})+(r,\multv{V}),N_i)
    %   \compl{\emptyset}{\emptyset} \Lambda(M',s,\multv{U},N_i)$ and thus the two have the same behavior
    %   in respect to divergence. Since $M \in \mathbf{SC}$, the two are (SN).

    \item Let $M' = \refssu{r}{V}{M}$. We proceed by induction on types. For
      base types, it is clear that $M'$ is (WB) iff $M$ is, and
      $\refssd{s}{U}{M'}$ has exactly the same reductions as $\refssd{s}{U}{M}$
      except for commutation of upward and downard substitutions, and a possible
      \rrule{subst}{\top}. Thus they are both (SN).
      Now, for $\alpha = A \sur{\to}{e_1} \alpha'$, consider an infinite reduction of
      $\Lambda(M',\multv{U},\seq{N})$. If the upward substitution is never
      reduced, we can map this to an infinite reduction of
      $\Lambda(M,\multv{U},\seq{N})$ for the same reasons as above, but the
      latter is (SN). Hence at some point the upward substitution must move up,
      so that the head term becomes $\refssu{r}{V}{\refssl{t}{W}{M''\
        (\refssd{r}{V}{N_1'}})}$ where $M''$ and $N_1'$ are reducts descendant
      from respectively $M$ and $N_1$. Using induction and points 5 and 3 of
      this lemma, $P = \refssl{t}{W}{M''\ (\refssd{r}{V}{N_1'}})$ is $\mathbf{SC}$. By
      induction, so is the new head redex, and the whole redex of $\Lambda$ is
      reachable from $\Lambda(\refssl{t}{W}{M\ N_1},\multv{U},\seq{N})$.

    \item This is straightforward from the definition of $\mathbf{SC}$ sets.
  \item Combining 2. and 4., using the fact that $\varsmetas{x}{V}{U}$ is the
      normal form of $\varss{\sigma}{U}$ using only \rrule{subst}{} rules, we get
      the result by induction on the length of the reduction.
  \end{enumerate}
\end{proof}

\begin{mlem}{Soundness}\label{mlem-soundness}\\
  If $R; x_1:A_1,\ldots,x_n:A_n \vdash M : (\alpha,e)$,
  $V_i \in \mathbf{SC}(A_i)$ and $\sigma : x_i \mapsto V_i$. Then
  $$\varss{\sigma}{M} \in \mathbf{SC}(\alpha,e)$$
\end{mlem}

\begin{proof}

  We perform the proof by induction.
  \begin{itemize}
    \item $M=x$ : $\varss{\sigma}{x}$ reduces to $\sigma(x) \in \mathbf{SC}$, and
      we apply \ref{mlem-soundness-aux}
    \item $M=\ast$ : $\varss{\sigma}{\ast} \to \ast$.
    \item $M=\lambda y.M'$ : $\varss{\sigma}{M} \to \lambda x .
      (\varss{\sigma}{M'})$. Consider an infinite reduction $\Lambda(\lambda x.
      (\varss{\sigma}{M'}))$. By \ref{mlem-soundness-aux} 1), at some point a
      $(\beta_v)$ must occur, replacing the head redex by $P =
      \refssd{s}{U}{\vars{y}{X}{\varss{\sigma}{M'}}}$ which is $\mathbf{SC}$ by
      induction \ref{mlem-soundness-aux} 3). But this term can be reached from
      $\Lambda(P,\multv{U},\refssd{}{V}{N_{i+1}})$ (for some
      $\multv{V}$ that are $\mathbf{SC}$, the ones emitted by the reduction of
      $N_1$) which is (SN). The same kind of
      argument show that $\Lambda(M,\multv{U},\seq{N})$ is (WB) : if the redex
      is not reduced, then all upgoing substitutions that come from $N_i$ must stop
      after a finite number of reductions and all contain $\mathbf{SC}$ terms,
      or the redex is reduced after a finite number of steps and from this point
      the term is a reduct of a (WB) one thus must be (WB) as well.

    \item $M = \get{r}$ : $\varss{\sigma}{\get{r}} \to \get{r}$. Let see that
      $\get{r} \in \mathbf{SC}$. Consider an infinite reduction of
      $\Lambda(\get{r})$. By \ref{mlem-soundness-aux} 1), the $\get{r}$ must be
      reduced at some point and from
      this point it is either replaced by a value from the substitution prefix,
      or by a value emitted by one of the $N_i$, all of these being
      $\mathbf{SC}$.
    \item $M = \varss{\tau}{M'}$, then $\varss{\sigma}{M} \to
      \varss{\mu}{M'}$. By \ref{mlem-soundness-aux},
      $\varsmetas{x}{V}{U} \in \mathbf{SC}$. $M'$ has a typing judgement of the form $x_1:A_1,\ldots,x_n : A_n, y_1 :
      B_1, \ldots, y_m : B_m \vdash M' : (\alpha,e)$. By induction,
      $\varss{\mu}{M'} \in
      \mathbf{SC}$.
    \item $M = \refssd{}{U}{M'}$ : $\varss{\sigma}{M} \to
      \refssd{}{\varsmetas{x}{V}{\multv{U}}}{\varss{\sigma}{M'}}$. By
      induction, $\varss{\sigma}{M'}$ is $\mathbf{SC}$ and by \ref{mlem-soundness-aux}
      so is $M$.
    \item $M = \refssu{r}{\mathcal{V}}{M'}$ : induction +
      \ref{mlem-soundness-aux}.
    \item $M = \refrawsl{(r_i)}{(\mathcal{V}_i)}{M_1\ M_2}$ : $\varss{\sigma}{M}
      \to M' = \refrawsl{r}{(\varss{\sigma}{\multv{V}})}{(\varss{\sigma}{M_1})\
      (\varss{\sigma}{M_2})}$. By induction and \ref{mlem-soundness-aux}, $\varss{\sigma}{M_i} \in \mathbf{SC}$
      and $\varss{x}{\multv{V}}$ are in $\mathbf{SC}$. Then by definition
      $M' \in \mathbf{SC}$.
    \item $M = M_1 \parallel M_2$ : $\vars{x}{V}{M} \to M'= M_1' \parallel M_2'$
      with $M_i' = \vars{x}{V}{M_i}$  and according to \ref{mlem-soundness-aux} it
      is sufficient to prove $M' \in \mathbf{SC}$. By induction, $M_i' \in
      \mathbf{SC}$. Let us take an $(M',r,\multv{V})$ reduction
      starting from $M'$. It can be associated to an $(M_i',r_i,\multv{V}_i)$
      reduction from the point of view of $M_i'$, where
      $r_i,\multv{V}_i$ are coming either from $(r,\multv{V})$ or from the
      upward substitution of $M'_{1-i}$, that are all in $\mathbf{SC}$. Since
      the $M_i$ are (WB), so is $M'$.
      Now, the proof is very similar to the first point of
      \ref{mlem-soundness-aux} : Take an $M'$ reduction, since $M'_i$ are (WB), after a finite
      number of steps, no more substitutions are exchanged. We can then smash
      all the substitutions received by $M'_i$ into a big one $(x,\multv{X})$
      and since $\refssd{x}{X}{M'_i}$ is (SN), then the reduction must be
      finite.
  \end{itemize}

\end{proof}


\begin{mlem}{Adequacy}\label{mlem-adequacy}\\
  If $M \in \mathbf{SC}(\alpha,e)$ then $M$ is strongly normalizable
\end{mlem}

\begin{proof}
  We will prove additionnally by induction on types that $\mathbf{SC}(\alpha)
  \neq \emptyset$ for any $\alpha$.
  \begin{itemize}
    \item For $\alpha = \texttt{Unit} \mid \mathbf{B}$ it is immediate : $\ast
      \in \mathbf{SC}(\texttt{Unit})$ and $\ast \parallel \ast \in
      \mathbf{SC}(\mathbf{B})$. If $M \in \mathbf{SC}(\alpha)$
      had an infinite reduction, then so would $\refsrawsd{r}{V}{M}$
    \item For $\alpha = A \to \alpha'$, by induction there exists $M_{\alpha'}
      \in \mathbf{SC}(\alpha')$, then $\lambda x . M_{\alpha'}$ for $x$ not free in
      $M_{\alpha'}$ is in $\mathbf{SC}(\alpha)$. If $M \in \mathbf{SC}(\alpha)$ did not terminate, so would $M\
      N$ for $N \in \mathbf{SC}(A)$ which exists since the latter set
      is not empty.
  \end{itemize}
\end{proof}

\begin{mthe}{Termination}\label{mthe-termination}\\
  All well-typed closed terms are strongly normalizing
\end{mthe}
\begin{proof}
  By conjunction of \ref{mlem-soundness} (with $n=0$) and \ref{mlem-adequacy}.
\end{proof}

\subsection{Termination strikes back}

We add a labelled reference substitution variable substitution to $\lamlang{aux} : \refssdbar{}{V}{M} \mid
\varsbar{x}{N}{M}$ such that $\varsbar{x}{N}{M}$ can't be reduced in either $N$
or by \rrulet{subst}{} rules (where $N$ is not a value). The labelled reference
substitution plays the same role in contexts : it forbids any reduction under
it, except for labelled reference substitutions.
We add the reduction rules \rrulet{subst-r}{} for $\refssdbar{}{V}{}$ for
labelled substitution, that can be
performed everywhere (included under a variable substitution) except under
abstraction : $J ::= [.] \mid J\ M \mid M\ J \mid \refssd{}{V}{J} \mid
\varss{\sigma}{J} \mid \vars{x}{N}{J}$.

We also add a $\beta$-rule to fire such labelled substitution :
\[
  (\beta_{V}') \refssl{}{V}{(\lambda x . M)\ N} \to
  \varsbar{x}{N}{\refssdbar{}{V}{M}}
\]

This corresponds to the additionnal reduction nets can do, and we will show that
going from a normal form in \lthis with these additionnal rules leads
to a new normal form that is (almost) normal in nets.

\begin{mdef}{$F$-normal forms}\label{mlem-progress-auxplus}\\
 Let $M$ be a normal form of the form $M_\text{norm}$, then $M$ reduces to a sum
 of terms in $\lamlang{aux+}$ that belongs to the
 following grammar of $F$-normal forms :
\begin{tabred}
  F_\text{norm} & ::= & \get{r} \mid \refssl{}{V}{F_\text{norm}\ V} \mid
  \refssl{}{V}{F_\text{norm}\ F_\text{norm}} \mid \varsbar{x}{F_\text{norm}}{M} \\
\end{tabred}
where the $M$ is in \lthis (contains no labelled substitution).
\end{mdef}

\begin{proof}
  By induction on the structure of $M$, with the additionnal hypthesis that only
  the additionnal rules are performed (no upward substitution) :
  \begin{itemize}
    \item $M = \get{r}$ : ok
    \item $M = \refssl{}{V}{M_\text{norm}\ V}$ : by induction, $M_\text{norm}$
      reduces to a sum of $F_\text{norm}$. Take one such $N$, then $M \to^\ast
      \refssl{}{V}{N_\text{norm}\ V}$ (because no rule \rrule{subst-r'}{\top} was
      used)
    \item $M = \refssl{}{V}{M_\text{norm}\ M'_\text{norm}}$ : we proceed as the
      previous case
    \item $M = \refssl{}{V}{V\ M_\text{norm}}$ : by induction, $M_\text{norm}$
      reduces to some $N$ in $F_\text{norm}$ grammar, so $M \to^\ast
      \refssl{}{V}{V\ N}$. Then, by inversion of typing rules, $V$ is of the
      form $\lambda x . P$ and we can apply the new $\beta$-reduction to get
      $\varsbar{x}{N}{\refssdbar{}{V}{P}}$. By pushing down $\refssdbar{}{V}{}$ in
      $P$, we can reduce it to a sum of $P_i$s where each $P_i$ do not contain
      labelled substitutions. Then $M \to^\ast \sum_i \vars{x}{N}{P_i}$ 
  \end{itemize}
\end{proof}

\begin{mlem}
$F$-normal forms are normal. 
\end{mlem}

\begin{proof}
  By induction : 
  \begin{itemize}
    \item $M = \get{r}$ : ok
    \item $M = \refssl{}{V}{F_\text{norm}\ V}$ : by induction, $F_\text{norm}$
      is normal, and values are not $F$-normal form, so the application can't create any
      $\beta$-redex.
    \item $M = \refssl{}{V}{M_\text{norm}\ M'_\text{norm}}$ : same as the
      previous case
    \item $M = \varsbar{x}{F_\text{normal}}{M}$ : The explicit substitution
      prevent any reduction except \rrulet{subst-r}{} ones for labelled
      reference substitution, but by definition, $M$ does not contain any.
  \end{itemize}
\end{proof}
\begin{mthe}{Adequacy}\label{mthe-adequacy-simulation-orig}\\
  Let $P$ be a term of \lamadio and $M = \widetilde{P}$ its translation in
  \lthis, if $M \to^\ast \sum_i M_i$ a normal form, then $\forall
  i, P \to^\ast P_i$ such that $M_i \rincl \widetilde{P_i}$. In other words, any
  term appearing in the normal form of the translation of $P$ is bounded by the
  translation of a reduct of $P$.
\end{mthe}

In particular, applied to values, this gives us

\begin{mcor}{Adequacy}\label{mcor-adequacy-simulation-orig}\\
  Let $P$ be a term of \lamadio, $M = \widetilde{P}$ its translation in
  \lthis such that $M \to^\ast M' + \mathbf{M''}$ a normal
  form.
  \begin{itemize}
    \item If $M' = V \parallel N$, then $P \to^\ast U \parallel Q$ with $V =
      \widetilde{U}$.
    \item In particular, if $M' = \parallel_i V_i$, then $P \to^\ast \parallel_i
      U_i$ with $V_i = \widetilde{U}_i$
  \end{itemize}
\end{mcor}

\begin{mlem}{}\label{mlem-preservation-values}
  Let $M$ be a term of \lamadio, if $M \to^\ast M'$ without using
  \rrulet{subst-r}{get}. We define $\text{NF}(M) = \{ T \mid T \text{ normal}
  \text{ and } M \to^\ast T \}$. Then $\text{NF}(M) = \text{NF}(M')$
\end{mlem}

\begin{proof}
  If we don't use \rrulet{subst-r}{get}, the two reduction (full and
  non-deterministic) coincide and we use the confluence in \lthis.
\end{proof}


\begin{mlem}{}\label{mlem-onestep-adequacy}
  Let $M = \widetilde{P}$ be the translation of a \lamadio term, such
  that $M \to M'$. Then there exists $M'',N'$, such that $M' \to^\ast M'' \rincl
  \widetilde{N'}$ and $N \to^{\{0,1\}} N'$, with all reductions from $M'$ to
  $M''$ not being \rrulet{subst-r}{get}.
\end{mlem}

\begin{proof}
  The only redexes in $M$ are either premises of \rrulet{subst-r'}{},
  $(\beta_v)$ or \rrulet{subst-r}{get}.
  In the first case, it corresponds to a reducible set whose reduction can be
  carried on in $M'$ by pushing the upward substitution to the top and pushing
  down the corresponding generated downward substitutions, to obtain the translation of
  $N'$ which is $N$ where we the set is reduced. We can proceed the same way
  with $(\beta_v)$ : this corresponds to a $\beta$-redex in $N$, where $N'$ is
  the result of reducing it, and $M''$ is obtained by pushing down the generated
  substitutions (variable and refenreces).
  \\
  Finally, if the reduction rule is \rrulet{subst-r}{get}, then either it
  choosed one of the available values and it corresponds exactly to a get
  reduction $N \to N'$, or it threw away available values, in which case $N =
  N'$, $M' = M''$ and clearly $M'' \rincl \widetilde{N'}$.
\end{proof}

\begin{proof}\ref{mthe-adequacy-simulation-orig}\\
  We proceed by induction on $\eta (M)$, the length of the longest reduction
  starting from $M$. If $\eta (M) = 0$, ie $M$ is a normal form, this is
  trivially true.
  \\
  To prove the induction step, consider a reduct $M'$ of $M$. We use
  \ref{mlem-onestep-adequacy} to get $M' \to^\ast M'' \rincl \widetilde{P'}$ for some reduct
  $P'$ of $P$, such that the reduction to $M''$ doesn't use
  \rrulet{subst-r}{get}. Thus, by \ref{mlem-preservation-values},
  $\text{NF}(M'') = \text{NF}(M')$. By induction on $M''$, $\forall T \in
  \text{NF}(M''), \exists Q, P \to^\ast Q \text{ and } T \rincl \widetilde{Q}$.
  But this true for any reduct $M'$, and we have $\text{NF}(M) = \bigcup_{M \to
  M'} \text{NF}(M')$, hence this is true for $M$.
\end{proof}


==> parts/properties-type.tex <==
\begin{mlem}{Critical pairs}\label{mlem-critical-pairs}\\
  We write $G_1 \# G_2$ for two contexts $G_1,G_2$ if $G_1 \neq G_2$, and each one
  is not a prefix of the other, ie $\forall G, G_1 \neq G_2[G]$ and $G_2 \neq
  G_1[G]$. In the following, we write the reduction rules as
  $S[N] \to S[N'] + \mathbf{M'}$, where $\mathbf{M}'$ is equals to $\mathbf{0}$ unless when
  \rrulet{subst-r}{get} occurs where it may have additionnal terms.
  \paragraph{}
  If $\mathbf{M} \to \mathbf{M_1}$ and $\mathbf{M} \to \mathbf{M_2}$ with
  $\mathbf{M_1} \neq \mathbf{M_2}$, then one of the assertion holds :
  \begin{enumerate}
    \item The two rules are of the form $S_i[N_i] \to S_i[N_i'] + \mathbf{M}'_i$
      with $S_1 \# S_2, \mathbf{M} = S_i[N_i] = \sum_i N_i$
    \item The two rules are of the form $S[C_i[N_i]] \to S_i[C_i[N_i']] +
      \mathbf{M}'_i$
      with $C_1 \# C_2, C_i[N_i] = \parallel_i N_i$
    \item The two rules are of the form $S[C[N_1]] \to S[C[N_1']]$ and
      $S[C[C_2[N_2]]] \to S_2[C[C_2[N_2']]] + \mathbf{M}'_2$,
      the first rule being \rrule{subst-r'}{\parallel}.
    \item The two rules are of the form $S[C[H[H_i[N_i]]] \to
      S_i[C[H[H_i[N_i']]]] + \mathbf{M}_i'$ with $H_1 = \refssl{r}{V}{H_1'[.]\ H_2'[N_2]}$ and $H_2
      = \refssl{r}{V}{H_1'[N_1]\ H_2'[.]}$, $N_i \to N_i'$, where $H_i$ is a
      context of type $E$ or $F$.
    \item The two rules are of the form $S[C[H[N_1]]] \to S[C[H[N_1']]$ and
      $S[C[H[H_2[N_2]]]] \to S_2[C[H[H_2[N_2']]]] + \mathbf{M}'_2$, with one
      of the following :
      \begin{enumerate}
        % \item $N_1 = \varss{\sigma}{H'}$ and the first rule applied is either
        %   \rrulet{subst}{app} or \rrulet{subst}{subst-r'} and the second is of
        %   type \rrule{subst}{\ldots} or \rrule{subst-r}{\ldots}
        \item $N_1 = \refssd{r}{V}{M'}$ and the applied rule is
          \rrule{subst-r}{app}, \rrule{subst-r}{subst-r'} or
          \rrule{subst-r}{merge}%  or \rrule{subst-r}{\ldots}
        \item $N_1 = \refssl{r}{V}{(\refssu{s}{U}{P})\
        H_2'[N_2]}$ or $N_1 = \refssl{r}{V}{H_2'[N_2]\
          (\refssu{s}{U}{P})}$
        \item  $N_1 = \refssl{r}{V}{(\refssu{s}{U}{H_2'[N_2]})\
          P}$ or $N_1 = \refssl{r}{V}{P\
          (\refssu{s}{U}{H_2'[N_2]})}$
        \item $C = H = [.]$, $N_1 = \refssu{r}{V}{H_2[N_2]}$ and the first rule
          used is \rrule{subst-r'}{\top}
      \end{enumerate}
  \end{enumerate}
\end{mlem}

\begin{proof}
We can write $\mathbf{M}$ in a unique way
(modulo structual rules) as a sum of parallel of simple terms :
$$\mathbf{M} = \sum_k M_k,\  M_k = \parallel_{i} M^i_k$$
\begin{itemize}
  \item The two reductions rules have a premise of the form $S[N_i]$.
    Identifying the terms of both sums, we can write $S_1 = [.] + \sum_{k \neq
    k_1} M_k$ and $S_2 = [.] + \sum_{k \neq k_2} M_k$. If $k_1 \neq k_2$ we are in
    the case (1), or $S_1=S_2$.

  \item If one of the rule used (let say the first one) is
    \rrule{subst-r'}{\top}, then $M_{k_1} =
    \refssu{r}{V}{M_{k_1}'}$. Since $\mathbf{M_1} \neq
    \mathbf{M_2}$, the second rule can't be the same and is of the form
    $H[T] \to H[T']$ where $H ::= E \mid F$ and $H =
    \refssu{r}{V}{H'}$. This is the case (5d) of the lemma.

  \item Otherwise, the premises of the two rules have the form $S[C_1[H_1[P_1]]]
    \to S[C_1[H_1[P_1']]] + \mathbf{M'}_1$ and $S[C_2[H_2[P_2]]] \to
    S[C_2[H_2[P_2']]] + \mathbf{M'}_2$.  If $C_1 \# C_2$, we are in case (2). If
    not, then either $C_1=C_2$ or $C_2=C_1[C_2'],C_2' \neq [.]$ but the only
    rule that matches a parallel is \rrule{subst-r'}{\parallel}, and this is
    case (3). We assume from now on that $C_1=C_2$. We decompose $H_1$ and $H_2$
    by their greatest common prefix, such that $H_1=H[H_1']$ and $H_2=H[H_2']$
    with either $H_1' = H_2' = [.]$, or $H_1' = [.],\ H_2' \neq [.]$, or $H_1 \#
    H_2$. The former is excluded since the reducts $\mathbf{N_1}$ and
    $\mathbf{N_2}$ are assumed differents, and no rule have overlapping redex on
    base cases (when $C$ and $E/F/G$ are empty).  \\
  \item
    If $H_1' \# H_2'$, since $H_1'[P_1]
    = H_2'[P_2]$, then $H_1$ must be of the form
    $\refssl{r}{V}{H_1''\ R}$, $H_2 =
    \refssl{r}{V}{L\ H_2''}$ with $L = H_1''[P_1]$ and $R =
    H_2''[P_2]$. This is case (4).
  \item
    Assume now that one of the two (let say $H_1'$) is $[.]$.
    Then $P_1$ and $H_2'$ have a common prefix. If $P_1$ is an application,
    it can't be the premise of the $(\beta_v)$ rule with $P_1 =
    \refssl{r}{U}{(\lambda x . M)\ V}$, because then $H_2' =
    \refssl{r}{U}{H_2''\ V}$ or $H_2' =
    \refssl{r}{U}{(\lambda x . M)\ H_2''}$ but no non-empty context
    verifies $H_2''[P_2] = V$ for a value $V$. Thus it must be the premise of
    \rrulet{subst-r'}{app}, and this corresponds to cases (5b) and (5c).

  \item
    If $P_1$ is not an application, since it must be both the premise of a rule
    and prefix of the context $H_2'$, the only remaining possibility is $P_1 =
    \refssd{r}{V}{\widetilde{P}_1}$. Then $\widetilde{P}_1$ can't be a value
    $y,\ast,\lambda y. \_$ or $\get{r}, \_ \parallel \_,
    \refssu{s}{U}{\_}$, because these constructors can't be in $H_2'$, which
    must be of type $F$ : we are in case (5a).
\end{itemize}

\end{proof}

\subsection{Weak confluence}

\begin{mlem}{Weak confluence}\label{mlem-weak-confluence}\\
  Let $\mathbf{M}$ be a term such that $\mathbf{M} \to
  \mathbf{M_1}$ and $\mathbf{M} \to \mathbf{M_2}$. Then
  $$\exists \mathbf{M'}, \mathbf{M_1} \to^\ast \mathbf{M'} \text{ and }
  \mathbf{M_2} \to^\ast \mathbf{M'}$$
\end{mlem}

\begin{proof}
We can write $\mathbf{M},\mathbf{M_1}$ and $\mathbf{M_2}$ in a unique way
(modulo structual rules) as a sum of parallel of simple terms :
$$\mathbf{M} = \sum_k M_k,\ \mathbf{M_1} = \sum_k M^1_k,\
\mathbf{M_2} = \sum_k M^2_k$$
Let us process all the possible cases of \ref{mlem-critical-pairs}, assuming that $\mathbf{N_1} \neq \mathbf{N_2}$:
\begin{enumerate}
  \item We have $S_1 \# S_2$, by identifying each terms, $\exists k_1 \neq k_2, S_i =
    [.] + \sum_{k \neq k_i}$, and we have
    \begin{tabred}
      \mathbf{M}_1 & = & \sum_{k \neq k_1} M_k + N_1' + \mathbf{M}'_1 \\
        & \to & \sum_{k \neq k_1,k_2} M_k + N_1' + N_2' + \mathbf{M}'_1 +
          \mathbf{M}'_2
    \end{tabred}
    as well as $\mathbf{M_2}$.
  \item Let write $C_i[N_i] = \parallel_{l \in
      \mathcal{L}} P_l$. Then
    there exists $\mathcal{L}_1, \mathcal{L}_2 \subseteq \mathcal{L}$. Since
    $C_1 \# C_2$, we have $\mathcal{L}_1 \neq \mathcal{L}_2$ and $\mathcal{L}_1
    \not \subseteq \mathcal{L}_2$ and $\mathcal{L}_2 \not \subseteq
    \mathcal{L}_1$, such that $C_i = [.] \parallel (\parallel_{l
      \in \mathcal{L}_i} P_l)$ and $N_i = \parallel_{l \notin \mathcal{L}_i} P_l$.
    The only rule that has a parallel of terms as premise is
    \rrule{subst-r'}{\parallel}. Thus $\mathcal{L}_i$ are either singletons (if
    the corresponding rule is not \rrule{subst-r'}{\parallel}) or have size two. If
    they are disjoint, then $\mathcal{L}_2 \subseteq \mathcal{L} \setminus
    \mathcal{L}_1$ and :
    \begin{tabred}
      \mathbf{M}_1 & = & S[N_1' \parallel (\parallel_{l \notin \mathcal{L}_1} P_l)] + \mathbf{M}'_1 \\
        & = &
          S[N_1' \parallel N_2 \parallel (\parallel_{l \notin \mathcal{L}_1 \cup
            \mathcal{L}_2} P_l)] + \mathbf{M}'_1 \\
        & \to &
          S[N_1' \parallel N_2' \parallel (\parallel_{l \notin \mathcal{L}_1 \cup
          \mathcal{L}_2} P_l)] +
          \mathbf{M}'_1 + \mathbf{M}'_2 \\
    \end{tabred}
    as do $\mathbf{M_2}$.\\
    The only remaining case is if both rules are \rrule{subst-r'}{\parallel} and
    $\mathcal{L}_1 \cap \mathcal{L}_2 = \{ l_0 \}$. We write $\mathcal{L}_1 = \{
    l_1, l_0 \}, \mathcal{L}_2 = \{ l_2, l_0 \}$ and $\mathcal{L_3} =
    \mathcal{L} \setminus \{ l_0, l_1, l_2 \}$. If $P_{l_0} =
    \refssu{r}{V}{P'}$ is the "active" upward substitution in both reduction, we
    have
    \begin{tabred}
      C_1[N_1'] & = & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P')}
        \parallel P_{l_2} \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
        & \to & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P' \parallel
          \refssd{r}{V}{P_{l_2}})} \parallel (\parallel_{l \neq \mathcal{L}_3}
          P_l) \\
    \end{tabred}
    If $P_{l_0}$ is the "passive" term in both reductions, with $P_{l_1} =
    \refssu{r}{V}{P_{l_1}'}$ and  $P_{l_2} = \refssu{s}{U}{P_{l_2}'}$, then
    \begin{tabred}
      C_1[N_1'] & = & \refssu{r}{V}{(P'_{l_1} \parallel \refssd{r}{V}{P_{l_0}})}
      \parallel \refssu{s}{U}{P'_{l_2}} \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
      & \to^\ast & P_{l_1} \parallel
        (\refssd{r}{V}{P_{l_0}}) \parallel
        (\refssd{r}{V}{\refssu{s}{U}{P'_{l_2}}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{r}{V}{P_l}) \\
      & \to & P_{l_1} \parallel
        (\refssd{r}{V}{P_{l_0}}) \parallel
        (\refssu{s}{U}{\refssd{r}{V}{P'_{l_2}}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{r}{V}{P_l}) \\
        & \to^\ast & (\refssd{s}{U}{P_{l_1}}) \parallel
        (\refssd{t}{W}{P_{l_0}}) \parallel
        (\refssd{r}{V}{P'_{l_2}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{t}{W}{P_l}) \\
    \end{tabred}
    using repeated \rrule{subst-r'}{\parallel}, \rrule{subst-r'}{\top},
    \rrulet{subst-r}{subst-r'} and
    \rrule{subst-r}{merge}.
    \\
    Finally, if $P_{l_0}$ is active in of the two (let say the first) and
    passive in the other, meaning that $P_{l_0} =
    \refssu{r}{V}{P_{l_0}'},P_{l_2} = \refssu{s}{U}{P_{l_2}'}$, then

    \begin{tabred}
      C_1[N_1'] & = & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P_{l_0}')}
      \parallel (\refssu{s}{U}{P_{l_2}}) \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
        & \to & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P' \parallel
          \refssd{r}{V}{P_{l_2}})} \parallel (\parallel_{l \neq \mathcal{L}_3}
          P_l) \\
    \end{tabred}
    \begin{tabred}
      C_1[N_1'] & = & \refssu{r}{V}{(\refssd{r}{V}{P_{l_1}} \parallel P'_{l_0})}
      \parallel \refssu{s}{U}{P'_{l_2}} \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
      & \to^\ast & (\refssd{r}{V}{P_{l_1}}) \parallel
        P'_{l_0} \parallel
        (\refssd{r}{V}{\refssu{s}{U}{P'_{l_2}}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{r}{V}{P_l}) \\
      & \to &  (\refssd{r}{V}{P_{l_1}}) \parallel
        P'_{l_0} \parallel
        (\refssu{s}{U}{\refssd{r}{V}{P_{l_2}}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{r}{V}{P_l}) \\
        & \to^\ast & (\refssd{t}{W}{P_{l_1}}) \parallel
        (\refssd{s}{U}{P_{l_0}}) \parallel
        (\refssd{r}{V}{P_{l_2}}) \\
      & &
        \parallel (\parallel_{l \neq \mathcal{L}_3}
        \refssd{t}{W}{P_l}) \\
    \end{tabred}
    On the other side,
    \begin{tabred}
      C_2[N_2'] & = & P_{l_1} \parallel
        \refssu{s}{U}{( (\refssd{s}{U}{\refssu{r}{V}{P'_{l_0}}}) \parallel
        P'_{l_2})}
        \parallel (\parallel_{l \neq \mathcal{L}_3} P_l) \\
      & \to^\ast & (\refssd{s}{U}{P_{l_1}}) \parallel
        (\refssd{s}{U}{\refssu{r}{V}{P'_{l_0}}}) \parallel P'_{l_2} \\
      & &
          \parallel (\parallel_{l \neq \mathcal{L}_3}
          \refssd{s}{U}{P_l}) \\
      & \to & (\refssd{s}{U}{P_{l_1}}) \parallel
        (\refssu{r}{V}{\refssd{s}{U}{P'_{l_0}}}) \parallel P'_{l_2} \\
      & &
          \parallel (\parallel_{l \neq \mathcal{L}_3}
          \refssd{s}{U}{P_l}) \\
      & \to^\ast & (\refssd{t}{W}{P_{l_1}})
        \parallel (\refssd{s}{U}{P'_{l_0}})
        \parallel (\refssd{r}{V}{P'_{l_2}}) \\
      & &
          \parallel (\parallel_{l \neq \mathcal{L}_3}
          \refssd{t}{W}{P_l}) \\
    \end{tabred}

  \item
    $C_2 = \refssu{r}{V}{Q} \parallel C_2'$. Let write $C = \parallel_{l} P_l$
    and $C_2 = [.] \parallel P'$.
    then $C[N_1'] = \refssu{r}{V}{(Q \parallel \refssd{r}{V}{(N_2 \parallel P')})}$.
    \begin{itemize}
      \item Either $N_2 = \refssu{s}{U}{N_2'} \parallel Q'$ and
        \begin{tabred}
          C[N_1'] & \to^\ast & Q \parallel
            \refssd{r}{V}{((\refssu{s}{U}{N_2'}) \parallel Q')}
            \parallel (\parallel_{l} \refssd{r}{V}{P_l}) \\
          & \to^\ast & Q \parallel
            (\refssu{s}{U}{\refssd{r}{V}{N_2'}}) \parallel (\refssd{r}{V}{Q'})
            \parallel (\parallel_{l} \refssd{r}{V}{P_l}) \\
          & \to^\ast & (\refssd{s}{U}{Q})
          \parallel (\refssd{r}{V}{N_2'})
          \parallel (\refssd{t}{W}{Q'})
          \parallel (\parallel_{l} \refssd{t}{W}{P_l}) \\
        \end{tabred}
        and
        \begin{tabred}
          C[C_2[N_2']] & = & (\refssu{r}{V}{Q})
            \parallel \refssu{s}{U}{(N_2' \parallel \refssd{s}{U}{Q'})}
            \parallel (\parallel_{l} P_l) \\
          & \to^\ast &
            (\refssd{s}{U}{\refssu{r}{V}{Q}}) \parallel
            N_2' \parallel (\refssd{s}{U}{Q'})
            \parallel (\parallel_{l} \refssd{s}{U}{P_l}) \\
          & \to^\ast &
            (\refssd{s}{U}{Q}) \parallel
            (\refssd{r}{V}{N_2'}) \\
          & &
            \parallel (\refssd{t}{W}{Q'})
            \parallel (\parallel_l \refssd{t}{W}{P_l}) \\
        \end{tabred}
      \item Otherwise, $N_2$ is a premise of the form $E[Q']$ and
        $S[C[C_2[E[Q']]] \to S[C[C_2[E[Q'']]]] + \mathbf{M}_2'$. Then
        \begin{tabred}
          \mathbf{M_1} & \to^\ast & S[Q \parallel
            \refssd{r}{V}{E[Q']}
            \parallel (\parallel_{l} \refssd{r}{V}{P_l})] \\
          & \to & S[Q \parallel
            \refssd{r}{V}{E[Q']}
            \parallel (\parallel_{l} \refssd{r}{V}{P_l})] + \mathbf{M_2}' \\
        \end{tabred}
        On the other side,
        \begin{tabred}
          \mathbf{M_2} & = & S[(\refssu{r}{V}{Q}) \parallel
            E[Q''] \parallel
            (\parallel_{l} P_l)] + \mathbf{M_2}' \\
          & \to^\ast & S[Q \parallel
            (\refssd{r}{V}{E[Q'']}) \parallel
            (\parallel_{l} \refssd{r}{V}{P_l})] + \mathbf{M_2}' \\
        \end{tabred}
    \end{itemize}

  \item
    \begin{tabred}
      S[C[H[H_1[N_1']]]] + \mathbf{M}'_1 & = &
        S[C[H[\refssl{r}{V}{H_1'[N_1']\ H_2'[N_2]}]]] + \mathbf{M}'_1 \\
      & \to &
        S[C[H[\refssl{r}{V}{H_1'[N_1']\ H_2'[N_2']}]]] + \mathbf{M}'_1 +
        \mathbf{M}'_2 \\
    \end{tabred}

  \item
    \begin{enumerate}
      \item The applied rule is either :
        \begin{itemize}
          \item \rrulet{subst-r}{app} and $H_2 = \refssl{s}{U}{H_2'\ Q}$ or $H_2
            = \refssl{s}{U}{Q\ H_2'}$
          \item \rrulet{subst-r}{subst-r'} and $H_2 = \refssu{s}{U}{H_2'}$
          \item \rrulet{subst-r}{merge} and $H_2 = \refssd{s}{V}{H_2'}$
        \end{itemize}
        In the three cases, it is clear that the reductions are independant :
        the first one can be performed in $\mathbf{M_2}$ and vice-versa to get a
        common reduct.
      \item
      \item
      \item \ldots The same argument applies to the other four cases.
    \end{enumerate}
  % \item
  %   If $P_1 = \refssd{r}{V}{\widetilde{P}_1}$, then
  %   $\widetilde{P}_1$ can't be a value $y,\ast,\lambda y. \_$ or
  %   $\get{r}, \_ \parallel \_, \refssu{s}{U}{\_}$, because
  %   these constructors can't be in $H_2'$.
  %   \begin{itemize}
  %     \item If $\widetilde{P}_1 = \refssl{s}{U}{X\ Y}$ then $H_2'$
  %       must be of type $F$ and thus $H_2'[P_2]$ can't be the premise of the
  %       $(\beta_v)$ rule. It follows that $H_2' =
  %       \refssl{s}{U}{H_2''\ Y}$ (or  $H_2' =
  %       \refssl{s}{U}{X\ H_2''}$). Then
  %       \begin{gather*}
  %         P_1 \to \refssl{t}{W}{(\refssd{r}{V}{H_2''[P_2]})\
  %         (\refsd{r}{V}{Y})} \\
  %         \to \refssl{t}{W}{(\refssd{r}{V}{H_2''[P_2']})\
  %         (\refssd{r}{V}{Y})}
  %       \end{gather*}
  %       And the other way around :
  %       \begin{gather*}
  %         H_2'[P_2] \to
  %         \refssd{r}{V}{\refssl{s}{U}{H_2''[P_2']\ Y}} \\
  %         \to \refssl{t}{W}{(\refssd{r}{V}{H_2''[P_2']})\
  %         (\refssd{r}{V}{Y})}
  %       \end{gather*}
  %     \item If $\widetilde{P}_1 = \text{set}(r,V)$ then TODO [changer la
  %       reduction pour propager les substitutions dans les SUBSTUP]
  %     \item If $\widetilde{P}_1 = \substv{s}{\mathcal{U}}{X}$ then $H_2' =
  %       \substv{s}{\mathcal{U}}{H_2''}$ thus
  %       \begin{gather*}
  %         P_1 \to \refssd{r}{V}{\substv{s}{\mathcal{U}}{H_2''[P_2]}}\\
  %         \to \substv{t}{\mathcal{W}}{H_2''[P_2]} \to
  %         \substv{t}{\mathcal{W}}{H_2''[P_2']}
  %       \end{gather*}
  %       Symetrically,
  %       \begin{gather*}
  %         P_1 \to \refssd{r}{V}{\substv{s}{\mathcal{U}}{H_2''[P_2]}}\\
  %         \to \refssd{r}{V}{\substv{s}{\mathcal{U}}{H_2''[P_2']}}\\
  %         \to \substv{t}{\mathcal{W}}{H_2''[P_2']}
  %       \end{gather*}
  %   \end{itemize}
  % \item
  %   We treat the case $P_1 = \varss{\sigma}{\widetilde{P}_1}$ exactly as the
  %   previous one.
\end{enumerate}

\end{proof}

\subsection{Type soundness}

\begin{mlem*}{Subject reduction}\label{mlem-subject-reduction}\\
  Let $R;\Gamma \vdash M : (\alpha,e)$ be a typing judgement, and assume that $M
  \rightarrow M'$. Then $R;\Gamma \vdash M' : (\alpha,e)$.
\end{mlem*}

\begin{proof}
  Case analysis on the reduction rule used :
\paragraph{Main reduction rules}
\begin{itemize}
  \item ($\beta_v$) Then the typing derivation of $M$ is of the form :
  \begin{mathpar}
    \inferrule* [Right=(subst-r)] {
      R;\Gamma \vdash \text{Reg}_r B \qquad \forall U \in \mathcal{U}:\ R;\Gamma
      \vdash U : (B,\emptyset) \qquad
      \inferrule* [Right=(app)] {
        \inferrule* [Right=(lam),rightskip=-4em] {
          R; \Gamma, x : A \vdash M : (\alpha, e)
        }
        {R; \Gamma \vdash (\lambda x. M) : (A \sur{\to}{e}, \emptyset)}
        R;\Gamma \vdash V : (A,\emptyset)
      }
      {R; \Gamma \vdash (\lambda x. M)\ V : (\alpha,e) }
    }
    { R;\Gamma \vdash \refssl{r}{U}{(\lambda x. M)\ V} : (\alpha,e)}
  \end{mathpar}
  Then one can form the derivation
  \begin{mathpar}
    \inferrule* [Right=(subst-r)] {
      R;\Gamma \vdash \text{Reg}_r B
      \qquad
      \forall U \in \mathcal{U}:\ R;\Gamma \vdash U : (B,\emptyset)
      \qquad
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash V : (A,\emptyset)
        \qquad
        R;\Gamma,x:A \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \vars{x}{V}{M} : (\alpha,e) }
    }
    { R;\Gamma \vdash \refssd{r}{U}{\vars{x}{V}{M}} : (\alpha,e) }
    %       \\
    % \inferrule* [Right=(subst)] {
    %   \inferrule* [Left=(weak)] {
    %     R;\Gamma \vdash V: (A, \emptyset)
    %   }
    %   { R;\Gamma,x:A \vdash V : (A,\emptyset) }
    %   \qquad
    %   \inferrule* [Right=(subst-r)] {
    %     \inferrule* [Left=(weak)] {
    %     }
    %     { R;\Gamma,x:A \vdash \text{Reg}_r B }
    %     \qquad
    %     \inferrule* [Right=(weak)] {
    %       \forall U \in \mathcal{U}:\ R;\Gamma \vdash U : (B,\emptyset)
    %     }
    %     {\forall U \in \mathcal{U}:\ R;\Gamma,x:A \vdash U : (B,\emptyset)}
    %     \qquad
    %     R;\Gamma,x:A \vdash M : (\alpha,e)
    %   }
    %   {R;\Gamma,x:A \vdash \substdown{r}{\mathcal{U}}{M}}
    % }
    % { R;\Gamma \vdash \varss{\sigma}{\substdown {r}{\mathcal{U}}{M}} : (\alpha,e) }
  \end{mathpar}
  using the admissibility of generalized weakening.
  % \item (\texttt{set})
  %   \begin{mathpar}
  %     \inferrule* {
  %       R;\Gamma \vdash r : \text{Reg}_r A
  %       \qquad
  %       R;\Gamma \vdash V : (A,\emptyset)
  %     }
  %     { R;\Gamma \vdash \text{set}(r,V) : (\text{Unit}, \{ r \}) }
  %   \end{mathpar}
  %   That we use to build the derivation
  %   \begin{mathpar}
  %     \inferrule* [Left=(subst-r)] {
  %       \inferrule* [Left=(unit)] { }
  %       { R;\Gamma \vdash \ast : (\text{Unit}, \emptyset) }
  %       \qquad
  %       R;\Gamma \vdash r : \text{Reg}_r A
  %       \qquad
  %       R;\Gamma \vdash V : (A, \emptyset)
  %     }
  %     { R;\Gamma \vdash \substup{r}{[V]}{\ast} }
  %   \end{mathpar}
\end{itemize}

\paragraph{Variables substitutions}
\begin{itemize}
  \item ($\texttt{subst}_\texttt{var}$)
    We have
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_i) : (A_i,\emptyset)
        \qquad
        \inferrule* [Right=(var)] { }
        { R;\Gamma' \vdash y : (B,\emptyset) }
      }
      { R;\Gamma \vdash \varss{\sigma}{y} : (B,\emptyset) }
    \end{mathpar}
    with $\Gamma' = \Gamma,x_1 : A_1,\ldots,x_n:A_n$ if $i$ ranges over $1
    \ldots n$. We have
    \begin{mathpar}
      \inferrule* [Right=(var)] { }
      { R;\Gamma \vdash y : (B,\emptyset) }
    \end{mathpar}
    if $\sigma$ is undefined at $y$ or
    \begin{mathpar}
      R;\Gamma \vdash \sigma(y) : (A_{i_0},\emptyset)
    \end{mathpar}
    if $\exists i_0, x_{i_0} = y$ and thus $A_{i_0}=B$.
  \item \rrulet{subst}{unit} : just apply the \trule{unit} typing rule.
  \item \rrulet{subst}{app}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma' \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \mathcal{V}(r_i):\ R;\Gamma' \vdash V : (A_i, \emptyset)
        \inferrule* [Right=(app)] {
          R;\Gamma' \vdash M : (C \sur{\to}{e_1} \alpha, e_2)
          \qquad
          R;\Gamma' \vdash N : (C,e_3)
        }
        { R;\Gamma' \vdash M\ N : (\alpha,e) }
      }
      { R;\Gamma' \vdash \refssl{}{V}{M\ N} }
      \\
      \inferrule* [Left=(subst)] {
        R;\Gamma' \vdash \sigma(x_j) : (B_j, \emptyset)
        \qquad
        R;\Gamma' \vdash \refssl{}{V}{M\ N}
      }
      { R;\Gamma \vdash \varss{\sigma}{\refssl{}{V}{M\ N}} : (\alpha,e)
      }
    \end{mathpar}
    With $\Gamma' = \Gamma,x_1:A_1,\ldots,x_n:A_n$ and $e_1 \cup e_2 \cup e_3 = e$. We can derive

    \begin{mathpar}
      \inferrule* [Right=(app)] {
        \inferrule* [Left=(subst)] {
            R;\Gamma \vdash \sigma(x_j) : (B_j,\emptyset)
            \qquad
            R;\Gamma' \vdash M : (C \sur{\to}{e_1} \alpha, e_2)
          }
          { R;\Gamma \vdash \varss{\sigma}{M} : (C \sur{\to}{e_1} \alpha, e_2)
          }
          \qquad
          \inferrule* [Right=(subst)] {
            R;\Gamma \vdash \sigma(x_j): (B_j,\emptyset)
            \qquad
            R;\Gamma' \vdash N : (C,e_3)
          }
          { R;\Gamma \vdash \varss{\sigma}{N} : (C,e_3) }
        }
        { R;\Gamma \vdash (\varss{\sigma}{M})\ (\varss{\sigma}{N}) : (\alpha,e) }
    \end{mathpar}
    For any $V \in \multv{V}(r_i)$, one has
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_j) : (B_j,\emptyset)
        \qquad
        R;\Gamma' \vdash V : (A_i,\emptyset)
      }
      { R;\Gamma \vdash \varss{\sigma}{V} : (A_i,\emptyset) }
    \end{mathpar}
    And finally
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash P : (\alpha,e)
        \qquad
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \mathcal{V}(r_i):\ R;\Gamma \vdash \varss{\sigma}{V} : (A_i,\emptyset)
      }
      { R;\Gamma \vdash
        \refrawsl{}{\varss{\sigma}{\multv{V}}}{(\varss{\sigma}{M})\
        (\varss{\sigma}{N})}
      }
    \end{mathpar}
  \item \rrule{subst}{\lambda} :
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_i) : (A_i, \emptyset)
        \qquad
        \inferrule* [Right=(lam)] {
          R;\Gamma',y:A \vdash M : (\alpha, e)
        }
        { R;\Gamma' \vdash \lambda y . M : (A \sur{\to}{e} \alpha, \emptyset)
        }
      }
      { R;\Gamma \vdash \varss{\sigma}{\lambda y. M} :  (A \sur{\to}{e} \alpha, \emptyset) }
    \end{mathpar}
    then we just swap the two rules :
    \begin{mathpar}
      \inferrule* [Right=(lam)] {
        \qquad
        \inferrule* [Right=(subst)] {
          \inferrule* [Left=(weak)] {
            R;\Gamma \vdash \sigma(x_i) : (A_i, \emptyset)
          }
          { R;\Gamma,y:A \vdash \sigma(x_i) : (A_i, \emptyset) }
          \qquad
          R;\Gamma',y:A \vdash M : (\alpha, e)
        }
        { R;\Gamma,y:A \vdash \varss{\sigma}{M} : (\alpha, \emptyset)
        }
      }
      { R;\Gamma \vdash \lambda y . (\varss{\sigma}{M}) :  (A \sur{\to}{e} \alpha, \emptyset) }
    \end{mathpar}
  \item \rrulet{subst}{get} :
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_i): (A_i, \emptyset)
        \qquad
        \inferrule* [Right=(get)] {
          R;\Gamma' \vdash r : \text{Reg}_r B
        }
        { R;\Gamma' \vdash \get{r} : (B, \{ r \}) }
      }
      { R;\Gamma \vdash \varss{\sigma}{\get{r}} : (B, \{ r \}) }
    \end{mathpar}
    We can juste recast the get rule without the weakened $x_i$s :
    \begin{mathpar}
      \inferrule* [Right=(get)] {
        R;\Gamma \vdash r : \text{Reg}_r B
      }
      { R;\Gamma \vdash \get{r} : (B, \{ r \}) }
    \end{mathpar}
  % \item \rrulet{subst}{set} :
  %   \begin{mathpar}
  %     \inferrule* [Right=(subst)] {
  %       R;\Gamma \vdash V : (A, \emptyset)
  %       \qquad
  %       \inferrule* [Right=(set)] {
  %         R;\Gamma,x:A \vdash r : \text{Reg}_r B
  %         \qquad
  %         R;\Gamma,x:A \vdash U : (B,\emptyset)
  %       }
  %       { R;\Gamma,x:A \vdash \text{set}(r,U) : (\text{Unit}, \{ r \}) }
  %     }
  %     { R;\Gamma \vdash \varss{\sigma}{\text{set}(r,U)} : (\text{Unit}, \{ r \}) }
  %   \end{mathpar}
  %   Then
  %   \begin{mathpar}
  %     \inferrule* [Right=(set)] {
  %       R;\Gamma,x:A \vdash r : \text{Reg}_r B
  %       \qquad
  %       \inferrule* [Right=(subst)] {
  %         R;\Gamma \vdash V : (A, \emptyset)
  %         \qquad
  %         R;\Gamma,x:A \vdash U : (B,\emptyset)
  %       }
  %       { R;\Gamma \vdash \varss{\sigma}{U} : (B, \emptyset) }
  %     }
  %     { R;\Gamma,x:A \vdash \text{set}(r,\varss{\sigma}{U}) : (\text{Unit}, \{ r \}) }
  %   \end{mathpar}
  \item \rrule{subst}{\parallel} :
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_j): (A_j, \emptyset)
        \qquad
        \inferrule* [Right=(par)] {
          i = 1,2
          \qquad
          R;\Gamma' \vdash M_i : (\alpha_i, e_i)
        }
        { R;\Gamma' \vdash M_1 \parallel M_2 : (\mathbf{B},e) }
      }
      { R;\Gamma \vdash \varss{\sigma}{M_1 \parallel M_2} : (\mathbf{B},e) }
    \end{mathpar}
    Then
    \begin{mathpar}
      \inferrule* [Right=(par)] {
        i=1,2
        \qquad
        \inferrule* [Right=(subst)] {
          R;\Gamma \vdash \sigma(x_j) : (A_j, \emptyset)
          \qquad
          R;\Gamma' \vdash M_i : (\alpha_i, e_i)
        }
        { R;\Gamma \vdash \varss{\sigma}{M_i} : (\alpha_i, e_i) }
      }
      { R;\Gamma \vdash (\varss{\sigma}{M_1}) \parallel (\varss{\sigma}{M_2}) : (\mathbf{B},e) }
    \end{mathpar}
  \item \rrule{subst}{subst-r} :
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma \vdash \sigma(x_j): (A_j,\emptyset)
        \qquad
        \inferrule* [Right=(subst-r)] {
          R;\Gamma' \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall U \in \mathcal{U}(r_i):\ R;\Gamma' \vdash U : (A_i, \emptyset)
          \qquad
          R;\Gamma' \vdash M : (\alpha,e)
        }
        { R;\Gamma' \vdash \refssd{}{\mathcal{U}}{M} : (\alpha,e) }
      }
      { R;\Gamma \vdash \varss{\sigma}{\refssd{}{\mathcal{U}}{M}} : (\alpha,e) }
    \end{mathpar}
    Then for any $U \in \mathcal{U}(r_i)$
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        R;\Gamma' \vdash U : (A_i, \emptyset)
      }
      { R;\Gamma \vdash \varss{\sigma}{U} : (A_i,\emptyset) }
    \end{mathpar}
    It follows
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall U \in \multv{U}(r_i):\
          R;\Gamma \vdash U : (A_i, \emptyset)
        \qquad
        \inferrule* [Right=(subst)] {
          R;\Gamma \vdash \sigma(x_j) : (A_j,\emptyset)
          \qquad
          R;\Gamma' \vdash M : (\alpha,e)
          }
          { R;\Gamma \vdash \vars{\sigma}{M} : (\alpha,e) }
        }
        { R;\Gamma \vdash
          \refssd{}{\varss{\sigma}{\multv{U}}}{\varss{\sigma}{M}} : (\alpha,e) }
    \end{mathpar}
  \item \rrule{subst}{subst-r'} : exactly as the previous case (the typing rules
    and reduction rules being similar)
  \item \rrule{subst}{merge}
    We need a simple substitution lemma to handle this case of the meta
    substitution.
    Let $\Gamma_{\mathcal{I}} = \bullet_{i \in
    \mathcal{I}} x_i : A_i$ and $\Gamma_{\mathcal{J}} = \bullet_{j \in
    \mathcal{J}} x_j : A_j$ where $\bullet$ is the list concatenation.
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        \forall U \in \mathcal{U}(r_j):\ R;\Gamma \vdash U : (A_j,\emptyset)
        \qquad
        \inferrule* [Right=(subst)] {
          \forall V \in \mathcal{V}(r_i):\
          R;\Gamma,\Gamma_\mathcal{J} \vdash V : (A_i,\emptyset)
          \qquad
          R;\Gamma,\Gamma_\mathcal{J},\Gamma_\mathcal{I} \vdash M : (\alpha,e)
        }
        { R;\Gamma_\mathcal{J} \vdash \vars{(x_i)}{(V_i)}{M} : (\alpha,e) }
      }
      { R;\Gamma \vdash \vars{(y_j)}{(U_j)}{\vars{(x_i)}{(U_i)}{M}} : (\alpha,e) }
    \end{mathpar}
    Then we have
    \begin{mathpar}
      \inferrule* [Right=(subst)] {
        \forall V \in \mathcal{V}_i:\ R;\Gamma \vdash \varmetas{(y_j)}{(U_j)}{V} : (A_i,\emptyset)
        \qquad
        \forall U \in \mathcal{U}_j:\ R;\Gamma \vdash U : (A_j,\emptyset)
        \qquad
        R;\Gamma,\Gamma_\mathcal{J},\Gamma_\mathcal{I} \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \vars{(z_i)}{(W_i)}{M} : (\alpha,e) }
    \end{mathpar}
    \emph{TODO : TO COMPLETE}
\end{itemize}

\paragraph{Downward references substitutions}
\begin{itemize}
  \item \rrulet{subst-r}{val}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall U \in \mathcal{U}(r_i):\ R;\Gamma \vdash U : (A_i,\emptyset)
        \qquad
        \inferrule* [Right=(sub)] {
          R;\Gamma \vdash V : (A,\emptyset)
        }
        { R;\Gamma \vdash V : (A,\{r\}) }
      }
      { R;\Gamma \vdash \refssd{}{U}{V} : (A,e) }
    \end{mathpar}
    Then we just reuse the typing derivation of
    \begin{mathpar}
      \inferrule* [Right=(sub)] {
        R;\Gamma \vdash V : (A,\emptyset)
      }
      { R;\Gamma \vdash V : (A,\{r\}) }
    \end{mathpar}
  % \item \rrulet{subst-r}{set}
  %   We assume $s \neq r$. When $s = r$, then the application of \trule{sub} is
  %   not needed anymore.
  %   \begin{mathpar}
  %     \inferrule* [Right=(subst-r)] {
  %       R;\Gamma \vdash r : \text{Reg}_r B
  %       \qquad
  %       \forall U \in \mathcal{U}:\ R;\Gamma \vdash U : (B,\emptyset)
  %       \qquad
  %       \inferrule* [Right=(sub)] {
  %         \inferrule* [Right=(set)] {
  %           R;\Gamma \vdash s : \text{Reg}_s A
  %           \qquad
  %           R;\Gamma \vdash V : (A,\emptyset)
  %         }
  %         { R;\Gamma \vdash \text{set}(s,V) : (\text{Unit},\{s\}) }
  %       }
  %       { R;\Gamma \vdash \text{set}(s,V) : (\text{Unit},\{s,r\}) }
  %     }
  %     { R;\Gamma \vdash \substdown{r}{U}{\text{set}(s,V)} : (\text{Unit},\{r,s\}) }
  %   \end{mathpar}
  %   As for the previous case, we have then
  %   \begin{mathpar}
  %     \inferrule* [Right=(sub)] {
  %       R;\Gamma \vdash \text{set}(s,V) : (\text{Unit},\{r\})
  %     }
  %     { R;\Gamma \vdash \text{set}(s,V) : (\text{Unit},\{r,s\}) }
  %   \end{mathpar}
  \item \rrule{subst-r}{\parallel}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall U \in \mathcal{U}(r_i):\ R;\Gamma \vdash U : (A_i,\emptyset)
        \qquad
        \inferrule* [Right=(par)] {
          R;\Gamma \vdash M_i : (\alpha_i,e_i)
        }
        { R;\Gamma \vdash M_1 \parallel M_2 : (\mathbf{B},e) }
      }
      { R;\Gamma \vdash \refssd{}{U}{M_1 \parallel M_2} :
      (\mathbf{B},e) }
    \end{mathpar}
    Then we commute the two rules
    \begin{mathpar}
      \inferrule* [Right=(par)] {
        \inferrule* [Right=(subst-r)] {
          R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall U \in \mathcal{U}(r_i) :\ R;\Gamma \vdash U : (A_i,\emptyset)
          \qquad
          R;\Gamma \vdash M_i : (\alpha_i,e)
        }
        { R;\Gamma \vdash \refssd{}{U}{M_i} : (\alpha_i,e) }
      }
      { R;\Gamma \vdash (\refssd{}{U}{M_1}) \parallel
      (\refsd{}{U}{M_2}) : (\mathbf{B},e) }
    \end{mathpar}
  \item \rrulet{subst-r}{subst-r'}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \refssu{}{V}{M} : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \mathcal{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash \refssd{}{V}{M} : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{U}{\refssu{}{V}{M}} : (\alpha,e) }
    \end{mathpar}
    We just swap the two rules
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{U}{M} : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \mathcal{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash \refssd{}{U}{M} : (\alpha,e)
      }
      { R;\Gamma \vdash \refssu{}{V}{\refssd{}{U}{M}} : (\alpha,e) }
      \\
    \end{mathpar}
  \item \rrule{subst-r-merge}{}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{V}{M} : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash \refssd{}{V}{M} : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{U}{\refssd{}{V}{M}} : (\alpha,e) }
    \end{mathpar}
    Then we have
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_k : \text{Reg}_{r_k} A_k
        \qquad
        \forall W \in (\multv{U} + \multv{V})(x_k):\ R;\Gamma \vdash W : (A_k,\emptyset)
        \qquad
        R;\Gamma \vdash M : (\alpha,e)
      }
      { R;\Gamma \vdash \refrawsd{}{\multv{V},\multv{U}}{M} : (\alpha,e) }
    \end{mathpar}
  \item \rrule{subst-r-app}{}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        \inferrule* [Right=(app)] {
          R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha,e_2)
          \qquad
          R;\Gamma \vdash N : (A,e_3)
        }
        { R;\Gamma \vdash M\ N : (\alpha,e) }
      }
      { R;\Gamma \vdash \refssl{}{V}{M\ N} : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash \refssl{}{V}{M\ N} : (\alpha,e)
      }
      { R;\Gamma \vdash \refssd{}{U}{\refssl{}{V}{M\ N}} : (\alpha,e) }
    \end{mathpar}
    That we can turn into
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha,e_2)
      }
      { R;\Gamma \vdash \refssd{}{U}{M} : (A \sur{\to}{e_1} \alpha,e_2) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash N : (A,e_3)
      }
      { R;\Gamma \vdash \refssd{}{U}{N} : (A,e_3) }
      \\
      \inferrule* [Right=(app)] {
        R;\Gamma \vdash \refssd{}{U}{M} : (A \sur{\to}{e_1} \alpha,e_2)
        \qquad
        R;\Gamma \vdash \refssd{}{U}{N} : (A,e_3)
      }
      { R;\Gamma \vdash (\refssd{}{U}{M})\ (\refssd{}{U}{N})  : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_k : \text{Reg}_{r_k} A_k
        \qquad
        \forall W \in (\multv{V} + \multv{U})(r_i):\ R;\Gamma \vdash W : (C_i,\emptyset)
        \qquad
        R;\Gamma \vdash (\refssd{}{U}{M})\ (\refssd{}{U}{N}) : (\alpha,e)
      }
      { R;\Gamma \vdash \refssl{}{W}{(\refssd{}{U}{M})\ (\refssd{}{U}{N})}
      }
    \end{mathpar}
  \item \rrulet{subst-r}{get}
    Write $\mathbf{S} = M_1 + \ldots + M_n + []$, with $n \geq 0$. The
    derivation tree of $P = C[E[\refssd{}{V}{\get{r}}]]$
    is of the form
    \begin{mathpar}
      \inferrule* {
        \inferrule* {
          \inferrule* [Right=(subst)] {
            R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
            \qquad
            \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
            \qquad
            R;\Gamma \vdash \get{r} : (A,e)
          }
          { R;\Gamma \vdash \refssd{}{V}{\get{r}} : (A,e) }
        }
        { [\ldots] }
      }
      { R;\Gamma' \vdash P : (\alpha,e') }
    \end{mathpar}
    And of the full term :
    \begin{mathpar}
        \inferrule* [Right=(sum)] {
          \ptentre{i}{1}{n}\ R;\Gamma \vdash M_i : (\alpha,e')
          \qquad
          R;\Gamma \vdash P : (\alpha,e')
        }
        { R;\Gamma \vdash S[P] : (\alpha,e') }
    \end{mathpar}
    To get the first term of the reduct, we just remove the subst rule :
    \begin{mathpar}
      \inferrule* [Right=(sum)] {
        \ptentre{i}{1}{n}\ R;\Gamma \vdash M_i : (\alpha,e')
        \qquad
        \inferrule* {
          \inferrule* { R;\Gamma \vdash \get{r} : (A,e) }
          { [\ldots] }
        }
        { R;\Gamma' \vdash C[E[\get{r}]] : (\alpha,e') }
      }
      { R;\Gamma' \vdash S[C[E[\get{r}]]] : (\alpha,e') }
    \end{mathpar}
    Now if $\multv{V}$ is undefined at $r$ we are done. Otherwise, we substitute
    $\get{r}$ by a value $V \in \multv{V}(r)$ :
    \begin{mathpar}
      \inferrule* {
        \inferrule* {
          \inferrule* [Right=(sub)] {
            R;\Gamma \vdash V : (A,\emptyset)
          }
          { R;\Gamma \vdash V : (A,e) }
        }
        { [\ldots] }
      }
      { R;\Gamma' \vdash C[E[V]] : (\alpha,e') }
    \end{mathpar}
    And we can finally derive
    \begin{mathpar}
      \inferrule* [Right=(sum)] {
        \forall V \in \mathcal{V}_{i_0}:\ R;\Gamma' \vdash C[E[V]] : (\alpha,e')
        \qquad
        R;\Gamma' \vdash S[C[E[\get{r}]]] : (\alpha,e')
      }
      { R;\Gamma' \vdash S[C[E[\get{r}]]] + \sum_{V \in
        \multv{V}(r)}C[E[V]] : (\alpha,e') }
    \end{mathpar}

\end{itemize}

\paragraph{Upward references substitutions}
\begin{itemize}
  \item \rrule{subst-r'}{\parallel}
    \begin{mathpar}
      \inferrule* [Right=(par)] {
        R;\Gamma \vdash M : (\alpha_1,e_1)
        \qquad
        \inferrule* [Right=(subst-r)] {
          R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
          \qquad
          R;\Gamma \vdash N : (\alpha_2,e_2)
        }
        { R;\Gamma \vdash \refssu{}{V}{N} : (\alpha_2,e_2) }
      }
      { R;\Gamma \vdash M \parallel (\refssu{}{V}{N}) :
      (\mathbf{B},e) }
    \end{mathpar}
    Then we have
    \begin{mathpar}
      \inferrule* [Right=(par)] {
        \inferrule* [Left=(subst-r)] {
          R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
          \qquad
          R;\Gamma \vdash M : (\alpha_1,e_1)
        }
        { R;\Gamma \vdash (\refssd{}{V}{M}) : (\alpha_1,e_2) }
        \qquad
        R;\Gamma \vdash N : (\alpha_2,e_2)
      }
      { R;\Gamma \vdash (\refssd{}{V}{M}) \parallel N :
        (\mathbf{B},e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V_i : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash (\refssd{}{V}{M}) \parallel N :
        (\mathbf{B},e)
      }
      { R;\Gamma \vdash
        \refssu{}{V}{(\refssd{}{V}{M}) \parallel N} :
        (\mathbf{B},e) }
    \end{mathpar}
  \item \rrulet{subst-r'}{app-left}
    \begin{mathpar}
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
        \qquad
        \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
        \qquad
        R;\Gamma \vdash M : (A \sur{\to}{e_2} \alpha,e_3)
      }
      { R;\Gamma \vdash \refssu{}{V}{M} : (A \sur{\to}{e_2}
          \alpha,e_3) }
      \\
      \inferrule* [Right=(app)] {
        R;\Gamma \vdash (\refssu{}{V}{M})\ : (B \sur{\to}{e_1}
        \alpha,e_2)
        \qquad
        R;\Gamma \vdash N : (A,e_3)
      }
      { R;\Gamma \vdash (\refssu{}{V}{M})\ N : (\alpha,e) }

      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_j : \text{Reg}_{r_j} B_j
        \qquad
        \forall U \in \multv{U}(r_j):\ R;\Gamma \vdash U : (B_j,\emptyset)
        \qquad
        R;\Gamma \vdash (\refssu{}{V}{M})\ N : (\alpha,e)
      }
      { R;\Gamma \vdash \refssl{}{U}{(\refssu{}{V}{M})\
        N} : (\alpha,e) }
    \end{mathpar}
    That we turn to
    \begin{mathpar}
      \inferrule* [Right=(app)] {
        R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha,e_2)
        \qquad
        \inferrule* [Right=(subst-r)] {
          R;\Gamma \vdash r_i : \text{Reg}_{r_i} A_i
          \qquad
          \forall V \in \multv{V}(r_i):\ R;\Gamma \vdash V : (A_i,\emptyset)
          \qquad
          R;\Gamma \vdash N : (A,e_3)
        }
        { R;\Gamma \vdash \refssd{}{V}{N} : (A,e_3) }
      }
      { R;\Gamma \vdash M\ (\refssd{}{V}{N}) : (\alpha,e) }
      \\
      \inferrule* [Right=(subt-r)] {
        R;\Gamma \vdash r_k : \text{Reg}_{r_k} C_k
        \qquad
        \forall W \in (\multv{V} + \multv{U})(r_k):\ R;\Gamma \vdash W : (C_k,\emptyset)
        \qquad
        R;\Gamma \vdash M\ (\refrawsd{}{\multv{U},\multv{V}}{N}) : (\alpha,e)
      }
      { R;\Gamma \vdash  \refrawsl{}{\multv{U},\multv{V}}{M\ (\refssd{}{V}{N})
        } : (\alpha,e) }
      \\
      \inferrule* [Right=(subst-r)] {
        R;\Gamma \vdash r_k : \text{Reg}_{r_k} C_k
        \qquad
        \forall W \in (\multv{U} + \multv{V})(r_k):\ R;\Gamma \vdash W : (C_k,\emptyset)
        \qquad
        R;\Gamma \vdash \refrawsl{}{\multv{U},\multv{V}}{M\ (\refssd{}{V}{N})} :
        (\alpha,e)
      }
      { R;\Gamma \vdash \refssu{}{\multv{V}}{\refrawsl{}{\multv{U},\multv{V}}{M\ (\refssd{}{V}{N})
        }}  : (\alpha,e) }
    \end{mathpar}
  \item \rrulet{subst-r'}{app-right} : same as \rrulet{subst-r'}{app-left}
  \item \rrule{subst-r'}{\top}
    Assume that $\mathbf{S} = M_1 + \ldots + M_n + []$, with $n \geq 0$, then we
    have
      \begin{mathpar}
        \inferrule* [Right=(subst-r)] {
          R;\Gamma \vdash r_j : \text{Reg}_{r_j} A_j
          \qquad
          \forall V \in \multv{V}(r_j):\ R;\Gamma \vdash V : (A_j,\emptyset)
          \qquad
          R;\Gamma \vdash M : (\alpha,e)
        }
        { R;\Gamma \vdash \refssu{}{V}{M} : (\alpha,e) }
        \\
        \inferrule* [Right=(sum)] {
          \ptentre{i}{1}{n}\ R;\Gamma \vdash M_i : (\alpha,e)
          \qquad
          R;\Gamma \vdash \refssu{}{V}{M} : (\alpha,e)
        }
        { R;\Gamma \vdash S[\refssu{}{V}{M}] : (\alpha,e) }
      \end{mathpar}
      We juste have to remove the \rrulet{subst-r}{} rule to get the result :
      \begin{mathpar}
        \inferrule* [Right=(sum)] {
          \ptentre{i}{1}{n}\ R;\Gamma \vdash M_i : (\alpha,e)
          \qquad
          R;\Gamma \vdash M : (\alpha,e)
        }
        { R;\Gamma \vdash S[M] : (\alpha,e) }
      \end{mathpar}
\end{itemize}
\end{proof}

\begin{mlem*}{Progress}\label{mlem-progress}\\
  Let $R \vdash \mathbf{M} : (A,e)$ be a typable program that does not reduce
  further. Then $\mathbf{M} =
  \sum_{i=1}^n (M^i_1 \parallel \ldots \parallel M^i_{l_i})$ where $M^i_1$ is
  either a value or of the form
  $$ M_{\text{norm}} ::= \get{r} \mid
  \refssl{r}{V}{M_{\text{norm}}\ V} \mid \refssl{r}{V}{V\
    M_{\text{norm}}} \mid \refssl{r}{V}{M_{\text{norm}}\
    M_{\text{norm}}} $$
\end{mlem*}

\begin{proof}
  By recurrence on $\mathbf{M}$. First assume that $\mathbf{M} = M$ :
  \begin{itemize}
    \item If $M$ is a value or $M = \get{r}$, there is nothing to do
    \item If $M = \varss{\sigma}{M'}$, then there is always a \rrulet{subst}{}
      rule that can be applied whatever $M'$ is.
    \item If $M = \refssd{r}{V}{M'}$, we can use a \rrulet{subst-r}{} rule
      unless $M' = \varss{\sigma}{M''}$. But then, by the previous case, $M'$
      reduces hence so does $M = F[M']$.
    \item If $M = \refssl{r}{V}{P\ Q}$, we have the type derivation
      \begin{mathpar}
        \inferrule* [Right=(subst-r)] {
          \inferrule* [Right=(app)] {
            R; \vdash P : (A \sur{\to}{e_1} \alpha,e_2)
            \qquad
            R; \vdash Q : (A,e_3)
          }
          { R; \vdash P\ Q : (\alpha,e) }
        }
        { R; \vdash \refssl{r}{V}{P\ Q} : (\alpha,e) }
      \end{mathpar}
      If $P \to P'$ by any rule
      excepted \rrule{subst-r'}{\top}, $M = E[P]$ with $E =
      \refssl{r}{V}{[.]\ Q}$ and thus $M$ also reduces. The same
      applies to $Q$. \\
      Assume now that $P \to P'$ by \rrule{subst-r'}{\top}, meaning that $P =
      \refssu{r}{V}{P'}$. Then we can apply
      \rrulet{subst-r'}{app-left} to $M$. Similarly, we can apply
      \rrulet{subst-r'}{app-right} if $Q = \substup{r}{\mathcal{V}}{Q'}$.
      Thus by induction $P$ and $Q$ are themselves either values, of the form $M_\text{norm}$, or a
      parallel of values and $M_\text{norm}$ forms. It is immediate that neither
      $P$ or $Q$ can be of the form $M_1 \parallel M_2$ (they would have to be
      typed by $\mathbf{B}$ and coudn't be applied or applied to), thus $P$ and
      $Q$ are either values or $M_\text{norm}$.
      \\
      Now, if both are values (note that $P$ and $Q$ must be closed terms), the only way for $P$ to have
      type $A \sur{\to}{e_1} \alpha$ is to be an abstraction, but then $M$ would
      reduce by $(\beta_v)$. Thus one of them is of the form $M_\text{norm}$ and
      so is $M$.
    % \item If $M = \text{set}(r,V)$ then it reduces by \rrule{set}{}.
    \item if $M = \refssu{r}{V}{M'}$ then it reduces by
      \rrule{subst-r'}{\top}.
    \item if $M = P \parallel Q$, assume that $P \to P'$ by any
      rule excepted \rrule{subst-r'}{\top}, then so would $M$, taking $E =[.]$
      and $C = [.] \parallel Q$. Same for $Q$.
      \\
      Now if $P = \refssu{r}{V}{P'}$ (or $Q$), then $M$ reduces by
      \rrule{subst-r'}{\parallel}. Thus $P$ and $Q$ does not reduce, and by
      induction, are of
      the form $\parallel_i M_i$ with $M_i$ a value or of the form $M_\text{norm}$, hence so
      is $M$.
  \end{itemize}
  Finally, if $\mathcal{M} = \sum M_i$, then $\mathcal{M}$ is normal if and
  only if each $M_i$ is and the induction hypothesis immediatly gives the result.
\end{proof}


==> parts/simulation-languages.tex <==
\section{Simulation}

\subsection{Definitions and lemmas}

\newcommand{\vstore}{\multv{V}_S}
\newcommand{\strans}{$\overline{\phantom{M}}^S$}
\newcommand{\sleq}{\rightsquigarrow_s}

\begin{mdef}{Translation of \lamadio in \lthis}\\
    Let $M$ be a term and $S$ be a store of \lamadio.
    S can be written as
    \[
      S = r_1 \Leftarrow V^1_1 \parallel \ldots \parallel r_1
      \Leftarrow V^1_{k_1} \parallel \ldots \parallel r_n \Leftarrow
      V^n_1 \parallel \ldots \parallel r_n \Leftarrow
      V^n_{k_n}
    \]
    Let $\multv{V}_S : r_i \mapsto [V^i_1, \ldots, V^i_{k_i}]$.
  We define the translation of $M$ under $S$ by
    \begin{itemize}
      \item If $M = V$ or $M = \text{set}(s,V)$ then $\overline{M}^S = M$
      \item If $M = N\ N'$ then $\overline{M}^S = \refsrawsl{r}{\vstore}(\overline{N}^S)\
        (\overline{N'}^S)$
      \item If $M = \get{s}$ then $\overline{M}^S =
        \refsrawsd{r}{\vstore}{\get{s}}$
      \item If $M = N \parallel N'$ then $\overline{M}^S = \overline{N}^S
        \parallel \overline{N'}^S$
    \end{itemize}

    In fact, one can see that $\overline{M}^S$ is the normal form of
    $\refsrawsd{r}{\vstore}{M}$ for the reduction defined by all
    \rrulet{subst-r}{} rules except \rrulet{subst-r}{get}.

    We extend it to contexts $E,F$ and $G$ by adding the rule $\overline{[.]}^S = [.]$.
    \\
    Finally, for any program $P = M \parallel S$, we define $\overline{P} =
    \overline{M}^S$.
    If $P = M$ then $\overline{P} = \overline{M} = M$.
  \end{mdef}

  % Originally put restrictions like $M$ and $N$ must not be parallel,
  % or that some reduction on parallel must not be used, but now I don't
  % see why this would be the case, so just removing
  \begin{mlem}{Context reduction}\label{mlem-ctxt-red}\\
    Let $M,N$ be terms of \lthis such that $M \to^\ast N$ without using
    \rrule{subst-r}{\top}, then for any
    context $C$ and $E$, $C[E[M]] \to^\ast C[E[N]]$ using the same reduction
    rules.
  \end{mlem}

  \begin{mlem}{Context decomposition}\label{mlem-ctxt-decomp}\\
    Let $P$ be a program of \lamadio,
    \begin{itemize}
      \item $P = C[E[M]] \text{ with } C = [.] \text{ or } C = [.] \parallel N \implies
        \overline{P} = P$
      \item $P = C[E[M]] \text{ with } C = [.] \parallel N \parallel S \implies
        \overline{P} = \overline{E}^S[\overline{M}^S] \parallel \overline{N}^S$
    \end{itemize}
  \end{mlem}

  \begin{proof}
    This is an easy induction following the definition of \strans.
  \end{proof}

  \begin{mlem}{Substitution for \strans}\label{mlem-subst}\\
    Let $M,M'$ be terms, $V$ a value and $S$ a
    store of \lamadio. Then
    \[
      \overline{M[x/V]}^S = \overline{M}^S[x/V]
    \]
  \end{mlem}
  \begin{proof}
    By induction
  \end{proof}

  \begin{mlem}{Absorption}\label{mlem-absorption}\\
    Let $M$ be a term and $S = S' \parallel r \Leftarrow V$ be a store of
    \lamadio, $C$ and $E$ be context of \lthis, and $\multv{V}
    : r \mapsto [V]$. Then
    $$C[E[\refssd{}{V}{\overline{M}^{S'}}]] \to_\texttt{aux}^\ast
    C[E[\overline{M}^{S}]]$$
  \end{mlem}

  \begin{proof} By induction on $M$, using the definition of
    \strans and the \texttt{subst-r} reductions.
  \end{proof}

  \begin{mlem}{Diffusion}\label{mlem-diffusion}\\
    Let $N$ be a term, $E$ a context, $S = S' \parallel r \Leftarrow V$ a store of
    \lamadio and $\multv{V} : r \mapsto [V]$. Let $M$ be a term of \lthis. Then
    \begin{equation}\label{mlem-diff-eq1}
      \overline{E}^{S'}[\refssu{}{V}{M}]
      \to_\texttt{aux}^\ast \refssu{}{V}{\overline{E}^S[M]}
    \end{equation}
    \begin{equation}\label{mlem-diff-eq2}
      \refssu{}{V}{M} \parallel \overline{N}^{S'}
      \to_\texttt{aux}^\ast \refssu{}{V}{(M \parallel
      \overline{N}^S)}
    \end{equation}
    \begin{equation}\label{mlem-diff-eq3}
      \overline{E}^{S'}[\refssu{}{V}{M}] \parallel \overline{N}^{S'}
      \to_\texttt{aux}^\ast \refssu{}{V}{\overline{E}^S[M] \parallel
      \overline{N}^S}
    \end{equation}
    using only rules \rrulet{subst-r}{} or \rrulet{subst-r'}{}.
  \end{mlem}

  \begin{proof}
    \begin{itemize}

      \item For (\ref{mlem-diff-eq1}), we work by induction on $E$. As we
        will need \ref{mlem-ctxt-red}, we add the induction hypothesis
        that the rule $(\texttt{subst-r'}_\top)$ is not used.
        \begin{itemize}
          \item $\overline{E}^{S'} = [.]$ nothing to do
          \item $\overline{E}^{S'} = \refssl{s}{U}{\overline{E'}^{S'}\
          \overline{M'}^{S'}}$\\
            By IH, $\overline{E'}^{S'}[\refssu{}{V}{M}] \to^\ast
            \refssu{}{V}{\overline{E'}^{S}[M]}$ using no
            \rrule{subst-r'}{\top} rules.
            We use \ref{mlem-ctxt-red} and get
            $$\overline{E}^{S'}[\refssu{}{V}{M}] \to^\ast
            \refssl{s}{U}{(\refssu{}{V}{\overline{E'}^{S}[M]})
            \ \overline{M'}^{S'}}$$
            We then apply \rrulet{subst-r'}{lapp} to get
            $$\overline{E}^{S'}[\refssu{}{V}{M}] \to^\ast \refssu{}{V}{\refssl{t}{W}{(\overline{E'}^{S}[M])
            \ (\refssd{}{V}{\overline{M'}^{S'}})}}$$
            Using \ref{mlem-absorption}, we get that the right part of the
            application reduces to $\overline{M'}^S$. Finally, by definition of
            \strans, the right hand side is $\refssu{}{V}{\overline{E}^S[M]}$.
          \item Other cases are treated alike
         \end{itemize}
    \item To prove (\ref{mlem-diff-eq2}), we apply
      \rrule{subst-r'}{\parallel}. We then use
      \ref{mlem-absorption} on $\refssd{}{V}{\overline{N}^{S'}}$ to get
      $\overline{N}^S$ and \ref{mlem-ctxt-red} with $C = M \parallel [.]$
      to get the desired result.
    \item Finally, we prove (\ref{mlem-diff-eq3}) by combining the two results. We
      first use the strenghtened version of $(\ref{mlem-diff-eq1})$, so we can
      apply \ref{mlem-ctxt-red} and get
      $$\overline{E}^{S'}[\refssu{}{V}{M}] \parallel \overline{N}^{S'}
      \to^\ast \refssu{}{V}{M}{\overline{E}^S[M]} \parallel \overline{N}^{S'}$$.
      We use (\ref{mlem-diff-eq2}) with $M' = E[M]$ to get the result.
    \end{itemize}
  \end{proof}

  Our reduction have the drawback of not reducing under abstractions, such that
  some of the variable substitution propagation will be delayed until the
  corresponding lambda will be applied (or forever). To cope with this subtelty,
  we introduce a relation on terms of \lthis that morally states that a
  term $M$ is related to $N$ if $M$ is the same as $N$ up to some pending
  substitutions hidden under lambdas, such that if we could reduce these
  subtitution under abstraction $M$ would actually reduce to $N$.

  \begin{mdef}{Substitution order}\label{mdef-substitution-equivalence}\\
    We define $\sleq$ as :
    \begin{itemize}
      \item $x \sleq x$, $\get r \sleq \get r$, $\set r V \sleq \set r V$
      \item $\refssl{}{V}{M\ N} \sleq \refssl{}{V}{M'\ N'}$
        or $M \parallel N \sleq M' \parallel N'$ iff $M \sleq M'$ and $N \sleq N'$
      \item $\lambda x.M \sleq \lambda x.M'$ if $M =
        \varss{\sigma_1}{\varss{\ldots}{\varss{\sigma_n}{N}}}$ such that
        $N\{\sigma_1,\ldots,\sigma_n\} = N$.
      \item $\refssd{}{V}{M} \sleq \refssd{}{V}{M'}$ or $\refssu{}{V}{M}
        \sleq \refssu{}{V}{M'}$ iff $M \sleq M'$
    \end{itemize}
  \end{mdef}

  \begin{mlem}{Properties of the substitution
    order}\label{mlem-substitution-equivalence-prop}\\
    $\sleq$ is a simulation order, meaning that if $M \sleq N$ and $M \to
    M'$, then $N \to^\ast N'$ with $M' \sleq N'$
  \end{mlem}

  We can now state the following result modulo this equivalence

  \begin{mlem}{Explicit substitution}\label{mlem-expl-subst}\\
    Let $P = C[E[\varss{\sigma}{M}]]$ with $M$ containing no explicit
    substitutions nor upward reference substitution.
    Then $$P \to_\texttt{aux}^\ast P' \sleq C[E[\varmetas{x}{V}{M}]]$$
  \end{mlem}

  \begin{proof}
    By induction on $M$.
    \begin{itemize}
      \item Neutral \\
        If $M=\ast$, $M=\get{r}$ or $M=y$ with $y \neq x$, then
        $\varmetas{x}{V}{M}=M$. If we apply \rrulet{subst}{unit} (resp.
        \rrulet{subst}{get},\rrulet{subst}{var}) we also get
        that $$C[E[\varss{\sigma}{M}]] \to_\text{aux} C[E[M]]$$
      \item $M=x$ \\
        $\varmetas{x}{V}{M}=V$. By \rrulet{subst}{var},
        $$C[E[\varss{\sigma}{x}]] \to_\text{aux} C[E[V]]$$
      \item $M=\lambda y. M'$ \\
        $\varmetas{x}{V}{M}=\lambda y.(\varmetas{x}{V}{M'})$. By
        \rrule{subst}{\lambda},
        $$C[E[\varss{\sigma}{\lambda y. M'}]] \to_\text{aux}
        C[E[\lambda y. (\varss{\sigma}{M'})]]
        \sleq C[E[\lambda y.(M'\{\sigma\})]]$$
      \item \ldots \\
        The remaining cases are treated similarly, the reduction rules being
        designed to make this lemma work.
        TODO : explain why we don't care about reference substitution, that
        cannot have free variables in the translation
        % There is a little subtelty, depending on how the substitution
        % $\varmetas{M}{x}{V}$ is defined with respect to references substitutions, ie when $M =
        % \refssd{r}{\mathcal{V}}{M'}$ for example. Actually, the
        % variables appearing in $\mathcal{V}$ should not be bound by any lambda because these
        % values have been emitted by sets, and sets can't be reduced under
        % lambdas. Thus all substitutions of bound variables in $\mathcal{V}$
        % already occured, and only globally free variables can remain. We define $M[x/V]$ to be
        % $\substvg{r}{\mathcal{V}}{(M'[x/V])}$, which matches the reduction rule
        % $\texttt{subst}_{\texttt{subst}_\texttt{r}}$, and this case is treated
        % as others.
    \end{itemize}
  \end{proof}

\subsection{One-step simulation}
  We prove now the technical result that will give the main theorem, which is
  contained in this lemma :

  \begin{mthe}{One-step simulation}\label{mthe-simulation}\\
    Let $P,Q$ be \lamadio programs such that $P
    \rightarrow_\texttt{orig} Q$. Then
    $$\overline{P} \rightarrow_\texttt{aux}^\ast M \sleq \overline{Q}$$
  \end{mthe}

  \begin{proof}\ref{mthe-simulation}\\
    By case analysis on the reduction rule applied :
    \begin{description}
      \item[$\beta_v$] We have $P = E[(\lambda x. M)\ V] \parallel N \parallel
        S$ and $Q = E[\varmetas{x}{V}M] \parallel N \parallel S$. Let
        By ~\ref{mlem-ctxt-decomp}, $\overline{P} =
        \overline{E}^S[\refrawsl{r}{\vstore}{\lambda x. M
        \ V}] \parallel \overline{N}^S$ and $\overline{Q} =
          \overline{E}^S[\overline{\varmetas{x}{V}{M}}^S] \parallel \overline{N}^S$. Then, by
        one application of $\beta_v$ in \lthis, we have $\overline{P}
        \rightarrow_\texttt{aux} Q_0 =
        \overline{E}^S[\varss{\sigma}{\refrawsd{}{\vstore}{M}}] \parallel
        \overline{N}^S$.
        We apply \ref{mlem-absorption} with to deduce
        $Q_0 \to^\ast Q_1 = \overline{E}^S[\varss{\sigma}{\overline{M}^S}]
        \parallel \overline{N}^S$. Using \ref{mlem-expl-subst} and
        \ref{mlem-subst}, we get $Q_1
        \to^\ast Q_2 \sleq \overline{E}^S[\overline{\varmetas{x}{V}{M}}^S] \parallel
        \overline{N}^S=\overline{Q}$.
      \item[get] We have $P = E[\get{r}] \parallel N \parallel S$ with
        $S=S' \parallel
        r \Leftarrow V$, and $Q = E[V] \parallel N \parallel S$.
        By \ref{mlem-ctxt-decomp},
        $\overline{P} = \overline{E}^S[\refssd{}{V}{\get{r}}]
        \parallel \overline{N}^S$ and $\overline{Q} = \overline{E}^S[V]
        \parallel \overline{N}^S$.
        The rule \rrulet{subst-r}{get} gives $\overline{P} \to_\text{aux}
        \overline{E}^S[V] \parallel \overline{N}^S = \overline{Q}$.
      \item[set] We have $P = E[\set r V] \parallel N \parallel S'$ and $Q = E[\ast]
        \parallel N \parallel S$ with $S = S' \parallel r \Leftarrow V$. By
        \ref{mlem-ctxt-decomp}, $\overline{P} =
        \overline{E}^{S'}[\refssu{}{V}{\ast}]
        \parallel \overline{N}^{S'}$ and $\overline{Q} = \overline{E}^S[\ast]
        \parallel \overline{N}^S = \overline{E[\ast] \parallel N}^S$.
        We apply \ref{mlem-diffusion} to get
        $P \to^\ast \refssu{}{V}{(\overline{E}^S[\ast] \parallel
        \overline{N}^S)}$ and then use the rule \rrule{subst-r}{\top} to get
        rid of the toplevel reference substitution.
    \end{description}
  \end{proof}


==> parts/simulation-nets.tex <==
\section{Simulation of $\lamlang{aux}$ in nets}

\subsection{Nets}

\subsection{Definition}
We consider MELL Interaction Nets with co-contraction and co-weakening. Formulas
are
\begin{equation*}
  A,B ::= \mathbf{1} \mid \bot \mid \oc{A} \mid
  \wn{A} \mid A \otimes B \mid A \parr B
\end{equation*}

Nets are build using the following cells

\begin{center}
  \includegraphics{translation/asy/pdf/components.pdf}
\end{center}

Using the following reductions rules :

\begin{center}
\begin{longtable}{|c|c|c|}
\hline
Rule & Redex & Reduced net \\
\hline
\multicolumn{3}{c|}{MLL reductions} \\
\hline
$\otimes / \parr$ & \includegraphics{translation/asy/pdf/reduction-partensor-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-partensor-right.pdf} \\
\hline
\multicolumn{3}{c|}{Exponential reductions} \\
\hline
$\oc / \wn{d}$ & \includegraphics{translation/asy/pdf/reduction-derprom-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-derprom-right.pdf} \\
\hline
$\oc / \wn{w}$ & \includegraphics{translation/asy/pdf/reduction-weakprom-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-weakprom-right.pdf} \\
\hline
$\oc / \wn{c}$ & \includegraphics{translation/asy/pdf/reduction-contprom-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-contprom-right.pdf} \\
\hline
\multicolumn{3}{|c|}{Non-determinstic reduction} \\
\hline
$\oc{c} / \wn{d}$ & \includegraphics{translation/asy/pdf/reduction-dercocontr-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-dercocontr-right.pdf}\\
\hline
\multicolumn{3}{|c|}{Co-reductions} \\
\hline
$\oc{c} / \wn{c}$ &
\includegraphics{translation/asy/pdf/reduction-contcocontr-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-contcocontr-right.pdf} \\
\hline
$\oc{c} / \wn{w}$ &
\includegraphics{translation/asy/pdf/reduction-coweakcont-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-coweakcont-right.pdf} \\
\hline
$\oc{w} / \wn{c}$ &
\includegraphics{translation/asy/pdf/reduction-weakcocontr-left.pdf} &
\includegraphics{translation/asy/pdf/reduction-weakcocontr-right.pdf} \\
\hline
$\oc{w} / \wn{w}$ &
\includegraphics{translation/asy/pdf/reduction-weakcoweak-left.pdf} &
$\epsilon$ \\
\hline
$\oc{w} / \wn{d}$ &
\includegraphics{translation/asy/pdf/reduction-dercoweak-left.pdf} &
$0$ \\

\end{longtable}
\end{center}

\subsection{Simulation}

  \begin{mlem}{Base case}\label{mlem-simu-base-case}\\
    Let $R \vdash M : (\alpha,e)$ be a typing derivation, such that $M \to M'$
    by a base reduction (without contexts). For any $e' \supset e$, $R \vdash M
    : (\alpha,e')$ by adding \trule{sub} to the typing derivation of $M$, and by subject reduction, $R \vdash M' :
    (\alpha,e')$. Then $$\mathcal{C}(M) \to^\ast \mathcal{C}(M')$$
  \end{mlem}

  \begin{mthe}{Simulation}\label{mthe-simu-aux-nets}\\
    Let $R \vdash M : (\alpha,e)$. If $M \to M'$, then $\mathcal{C}(M) \to
    \mathcal{C}{M'}$.
  \end{mthe}


==> parts/translation-nets.tex <==
\section{Translation of $\lamlang{aux}$ in nets}

We translate the full typing derivation of a term into a MELL+Cocon interaction
net.
\begin{center}
\begin{longtable}{|c|c|}
\hline
Typing derivation of & Translation \\
\hline
$\infer[(var)]{\Gamma,x : A \vdash x : (A,\emptyset)}{}$
& \includegraphics{translation/asy/pdf/var.pdf} \\
\hline

$\infer[(unit)]{\Gamma \vdash \ast : (\texttt{Unit},\emptyset)}{}$
 & \includegraphics{translation/asy/pdf/unit.pdf} \\
\hline

$\infer[(lam)]
{ R;\Gamma \vdash \lambda{x}.M : (A \sur{\to}{e} \alpha, \emptyset) }
{ R;x:A,\Gamma \vdash M : (\alpha,e) }$
& \includegraphics{translation/asy/pdf/abstraction.pdf} \\
\hline

$\infer[(app)]
{ R;\Gamma \vdash M\ N : (\alpha, e=e_1 \cup e_2 \cup e_3) }
{ R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha, e_2)
\qquad R;\Gamma \vdash N : (A,e_3)}$
  & \includegraphics{translation/asy/pdf/application.pdf} \\
\hline

$\infer[(get)]
{ R;\Gamma \vdash \get{r} : (A,\{ r \}) }
{ R \vdash \Gamma }$
 & \includegraphics{translation/asy/pdf/get.pdf} \\
\hline

$\infer[(set)]
{ R;\Gamma \vdash set(r,V) : (\text{Unit},\{ r \}) }
{ R \vdash r:\text{Reg}_r\ A \qquad R;\Gamma \vdash V : (A,\emptyset) }$
 & \includegraphics{translation/asy/pdf/set.pdf}\\
\hline

$\infer[(par)]
{ R; \Gamma \vdash P_1 \parallel P_2 : \mathbf{B} }
{i=1,2 \qquad R;\Gamma \vdash P_i : \alpha_i }$
  & \includegraphics{translation/asy/pdf/parallel.pdf} \\
\hline

\infer[(subst)]
{ R; \Gamma \vdash \varss{\sigma}{M} : (\alpha, e) }
{ R; \Gamma, x : A \vdash M : (\alpha,e) \qquad R; \Gamma \vdash V : (A,\emptyset) }
  & \includegraphics{translation/asy/pdf/substv.pdf} \\
\hline

\infer[(subst\text{-}r\downarrow)]
{ R; \Gamma \vdash \substg{(r_i)}{(\mathcal{V}_i)}{M} : (\alpha, e) \qquad }
{ R; \Gamma \vdash M : (\alpha,e) \qquad R; \Gamma \vdash \mathcal{V}_i : (A_i,\emptyset) }
  & \includegraphics{translation/asy/pdf/substr.pdf} \\

\infer[(subst\text{-}r\uparrow)]
{ R; \Gamma \vdash \substup{(r_i)}{(\mathcal{V}_i)}{M} : (\alpha, e) \qquad }
{ R; \Gamma \vdash M : (\alpha,e) \qquad R; \Gamma \vdash \mathcal{V}_i : (A_i,\emptyset) }
  & \includegraphics{translation/asy/pdf/substr-up.pdf} \\
\hline
\end{longtable}
\end{center}

\paragraph{}
  Where
\begin{center}
\begin{tabular}{ccc}
\hline
\includegraphics{translation/asy/pdf/mycombox.pdf} & $=$
& \includegraphics{translation/asy/pdf/mycombox-expanded.pdf} \\
\hline
\includegraphics{translation/asy/pdf/myappbox.pdf} & $=$
& \includegraphics{translation/asy/pdf/myappbox-expanded.pdf} \\
\hline
\end{tabular}
\end{center}

For a net $M^\bullet$, we define its closed form $\mathcal{C}(M^\bullet)$ by cutting the free
wires corresponding to effects with weakening and coweakening cells :
\begin{center}
  \includegraphics{translation/asy/pdf/closed.pdf}
\end{center}

By extension, we define the translation $M^\bullet$ (and thus
$\mathcal{C}(M^\bullet))$ of a term $M$
of $\lamlang{orig}$ by $M^\bullet = \overline{M}^\bullet$.


==> parts/typing.tex <==
\begin{section}{Type and effect system}

\subsection{Types and effects}

%%% TYPE SYSTEM WITH POLARITY
\begin{comment}
\begin{center}
\begin{tabular}{lrcl}
  -effects & $e,e'$ & $\subset$ & $\{r,r^-,r^+,s,s^-,s^+,\ldots\}$ \\
  -types & $\alpha$ & $::=$ & $\mathbf{B} \mid A$ \\
  -values types & $A$ & $::=$ & $\text{Unit} \mid A \sur{\to}{e} \alpha
  \mid \text{Reg}_r A$ \\
  -variable contexts & $\Gamma$ & $::=$ & $x_1 : A_1,\ldots,x_n : A_n$ \\
  -region contexts & $R$ & $::=$ & $r_1 : A_1,\ldots,r_n : U_n$ \\
\end{tabular}
\paragraph{}
\end{center}
\end{comment}
%%% END TYPE SYSTEM WITH POLARITY

\begin{center}
\begin{tabular}{lrcl}
  -effects & $e,e'$ & $\subset$ & $\{r_1,r_2,\ldots\}$ \\
  -types & $\alpha$ & $::=$ & $\mathbf{B} \mid A$ \\
  -values types & $A$ & $::=$ & $\text{Unit} \mid A \sur{\to}{e} \alpha
  \mid \text{Reg}_r A$ \\
  -variable contexts & $\Gamma$ & $::=$ & $x_1 : A_1,\ldots,x_n : A_n$ \\
  -region contexts & $R$ & $::=$ & $r_1 : A_1,\ldots,r_n : A_n$ \\
\end{tabular}
\paragraph{}
\end{center}

\subsection{Stratification and context formation}

\paragraph{Stratification Rules}

\begin{gather*}
\infer[]
{\emptyset \vdash}{}
\qquad
\infer[]
{ R,r:A \vdash }
{ R \vdash A \qquad r \notin \text{dom}(R) }
\\
\\
\infer[]
{ R \vdash Unit }
{ R \vdash }
\qquad
\infer[]
{ R \vdash \mathbf{B}}
{ R \vdash }
\\
\\
\infer[]
{ R \vdash A \sur{\rightarrow}{e} \alpha }
{ R \vdash A \qquad R \vdash \alpha \qquad e \subseteq \text{dom}(R)}
\qquad
\infer[]
{ R \vdash \text{Reg}_r A }
{ R \vdash \qquad r : A \in R }
\end{gather*}

\paragraph{Stratification conditions}
Note that these typing rules are equivalent to the following conditions :
\begin{mlem*}{Stratification conditions}\\
  A type and effect $\alpha$ (or $\emptyset$) are well-formed
  under a reference context $R = r_1:A_1,\ldots,r_n:A_n$, meaning
  that the judgement
  \begin{equation*}
    R \vdash \alpha
  \end{equation*}
  holds, if and only if :
  \begin{itemize}
    \item
      $\text{Eff}(A_1,\ldots,A_n,\alpha) \subseteq \text{dom}(R)$
    \item
      There exists a total ordering $\leq_R$ on dom$(R)$ such that\\
      $\ptentre{i}{1}{n},\ \text{Eff}(A_i) \subseteq \dcl{\{r_i\}}
        \setminus \{ r_i \}$
  \end{itemize}
\end{mlem*}

\paragraph{}
where

\begin{tabular}{rcl}
  $\text{dom}(R)$ & $=$ & $\{ r_1,\ldots,r_n \}$ \\
  $\text{Eff}(U)$ & $=$ & $\emptyset$ \\
  $\text{Eff}(\mathbf{B})$ & $=$ & $\emptyset$ \\
  $\text{Eff}(A \sur{\to}{e} \alpha)$ & $=$ &
  $\text{Eff}(A) \cup e \cup \text{Eff}(\alpha)$
\end{tabular}

\paragraph{Type equations}

Let $R = r_1 : A_1, \ldots, r_n : A_n$. To each reference $r_i$ we
associate a type variable $X_{r_i}$.
We define the type equations
\begin{itemize}
  \item $\text{unit}^\bullet=\oc{1}$
  \item $\mathbf{B}^\bullet=?$
  \item $(A \sur{\to}{\{s_1, \ldots, s_m\}} \alpha)^\bullet = \oc{((A^\bullet
      \otimes X_{s_1} \ldots \otimes X_{s_m}) \multimap (X_{s_1} \otimes \ldots
      \otimes X_{s_m} \otimes \alpha^\bullet))}$
  \item $X_{r_i} = {A_i}^\bullet$
\end{itemize}

These equations are solvable if and only if $R \vdash \ $.


\subsection{Typing rules for \lamadio}

\begin{gather*}
\infer[(var)]
{R;\Gamma,x : A \vdash x : (A,\emptyset)}
{R \vdash \Gamma,x : A}
\\
\\
\infer[(unit)]
{R;\Gamma \vdash \ast : (\texttt{Unit},\emptyset)} {R \vdash \Gamma}
\\
\\
\infer[(reg)]
{R;\Gamma \vdash r : Reg_r{A}}
{R \vdash \Gamma \qquad r : A \in R}
\\
\\
\infer[(lam)]
{ R;\Gamma \vdash \lambda{x}.M : (A \sur{\to}{e} \alpha,\emptyset) }
{ R;\Gamma,x : A \vdash M : (\alpha,e) }
\\
\\
\infer[(app)]
{ R; \Gamma\vdash M\ N : (\alpha, e_1 \cup e_2 \cup e_3) }
{ R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha, e_2) \qquad R;\Gamma \vdash N : (A,e_3) }
\\
\\
\infer[(get)]
{ R;\Gamma \vdash \get{r} : (A,\{ r \}) }
{ R;\Gamma \vdash \text{Reg}_r{A} }
\\
\\
\infer[(set)]
{ R;\Gamma \vdash set(r,V) : (\text{Unit},\{ r \}) }
{ R;\Gamma \vdash r : \text{Reg}_r{A} \qquad R;\Gamma \vdash V : (A,\emptyset) }
\\
\\
\infer[(store)]
{ R;\Gamma \vdash r \Leftarrow V : (\mathbf{B},\emptyset) }
{ r : A \in R \qquad R;\Gamma \vdash V : (A,\emptyset) }
\\
\\
\infer[(par1)]
{ R;\Gamma \vdash P \parallel S : (\alpha,\emptyset) }
{ R;\Gamma \vdash P : (\alpha,e) \qquad R;\Gamma \vdash S : (\mathbf{B},\emptyset) }
\\
\\
\infer[(par2)]
{ R;\Gamma \vdash P_1 \parallel P_2 : (\mathbf{B},e_1 \cup e_2) }
{i=1,2 \qquad R;\Gamma \vdash P_i : (\alpha_i,e_i) }
\end{gather*}

\subsection{Typing rules for \lthis}

\begin{gather*}
\infer[(var)]
{R;\Gamma,x : A \vdash x : (A,\emptyset)}
{R \vdash \Gamma,x : A}
\\
\\
\infer[(unit)]
{R;\Gamma \vdash \ast : (\texttt{Unit},\emptyset)} {R \vdash \Gamma}
% \\
% \\
% \infer[(mval)]
% {R;\Gamma \vdash [V^s_1,\ldots,V^s_n] : (A, \emptyset)}
% {R;\Gamma \vdash V^s_i : (A,\emptyset) }
\\
\\
\infer[(reg)]
{R;\Gamma \vdash r : Reg_r{A}}
{R \vdash \Gamma \qquad r : A \in R}
\\
\\
\infer[(lam)]
{ R;\Gamma \vdash \lambda{x}.M : (A \sur{\to}{e} \alpha,\emptyset) }
{ R;\Gamma,x : A \vdash M : (\alpha,e) }
\\
\\
\infer[(app)]
{ R; \Gamma\vdash M\ N : (\alpha, e_1 \cup e_2 \cup e_3) }
{ R;\Gamma \vdash M : (A \sur{\to}{e_1} \alpha, e_2) \qquad R;\Gamma \vdash N : (A,e_3) }
\\
\\
\infer[(get)]
{ R;\Gamma \vdash \get{r} : (A,\{ r \}) }
{ R;\Gamma \vdash \text{Reg}_r{A} }
\\
\\
% \infer[(set)]
% { R;\Gamma \vdash \text{set(r,V)} : (\text{Unit},\{ r \}) }
% { R;\Gamma \vdash r : \text{Reg}_r{A} \qquad R;\Gamma \vdash V : (A,\emptyset) }
% \\
% \\
\infer[(subst)]
{ R; \Gamma \vdash \vars{x_i}{V_i}{M} : (\alpha, e) }
{ i=(1,\ldots,n) \qquad
  R; \Gamma, x_1 : A_1, \ldots, x_n : A_n \vdash M : (\alpha,e) \qquad
  R; \Gamma \vdash V_i : (A,\emptyset) }
\\
\\
\infer[(subst\text{-}r)]
{ R; \Gamma \vdash \sind{r_i / \mathscr{E}_i}{M}{\uparrow \mid \downarrow \mid
\lambda} (\alpha, e) \qquad }
{ R; \Gamma \vdash r_i : \text{Reg}_{r_i} A_i \qquad
  R; \Gamma \vdash M : (\alpha,e) \qquad
  r_i \in e \qquad
  R; \Gamma \vdash V \in \mathscr{E}_i : (A_i,\emptyset) }
\\
\\
\infer[(par)]
{ R;\Gamma \vdash M_1 \parallel M_2 : (\mathbf{B},e_1 \cup e_2) }
{i=1,2 \qquad R;\Gamma \vdash M_i : (\alpha_i,e_i) }
\\
\\
\infer[(sum)]
{ R;\Gamma \vdash \mathbf{M}_1 + \mathbf{M}_2 : (\alpha,e) }
{i=1,2 \qquad R;\Gamma \vdash \mathbf{M_i} : (\alpha,e) }
\end{gather*}

\subsection{Subtyping induced by effect containment}

\begin{gather*}
\infer[(ref)]
{R \vdash \alpha \leq \alpha}{}
\\
\\
\infer[(arrow)]
{ R \vdash A \sur{\to}{e} \alpha \leq A' \sur{\to}{e'}
\alpha' }
{ \qquad R \vdash (\alpha,e) \leq (\alpha',e') }
\\
\\
\infer[(cont)]
{ R \vdash (\alpha,e) \leq (\alpha',e') }
{ e \subset e' \subset \text{dom}(R) \qquad R \vdash \alpha \leq \alpha' }
\\
\\
\infer[(sub)]
{ R;\Gamma \vdash M : (\alpha',e') }
{ R;\Gamma \vdash M : (\alpha,e) \qquad R \vdash (\alpha,e) \leq (\alpha',e') }
\end{gather*}

\end{section}

